Algorithms for Efficient, Compact Online Data Stream Curation

Data stream algorithms tackle operations on high-volume sequences of read-once data items. Data stream scenarios include inherently real-time systems like sensor networks and financial markets. They also arise in purely-computational scenarios like ordered traversal of big data or long-running iterative simulations. In this work, we develop methods to maintain running archives of stream data that are temporally representative, a task we call "stream curation." Our approach contributes to rich existing literature on data stream binning, which we extend by providing stateless (i.e., non-iterative) curation schemes that enable key optimizations to trim archive storage overhead and streamline processing of incoming observations. We also broaden support to cover new trade-offs between curated archive size and temporal coverage. We present a suite of five stream curation algorithms that span $\mathcal{O}(n)$, $\mathcal{O}(\log n)$, and $\mathcal{O}(1)$ orders of growth for retained data items. Within each order of growth, algorithms are provided to maintain even coverage across history or bias coverage toward more recent time points. More broadly, memory-efficient stream curation can boost the data stream mining capabilities of low-grade hardware in roles such as sensor nodes and data logging devices.

==> Dockerfile <==
FROM mmore500/docker-texlive-full:sha-ea45eb5

SHELL ["/bin/bash", "-c"]

# Prevent interactive time zone config.
# adapted from https://askubuntu.com/a/1013396
ENV DEBIAN_FRONTEND=noninteractive

RUN \
  echo 'Acquire::http::Timeout "60";' >> "/etc/apt/apt.conf.d/99timeout" \
    && \
  echo 'Acquire::ftp::Timeout "60";' >> "/etc/apt/apt.conf.d/99timeout" \
    && \
  echo 'Acquire::Retries "100";' >> "/etc/apt/apt.conf.d/99timeout" \
    && \
  echo "buffed apt-get resiliency"

RUN \
  find /etc/apt -type f -name '*.list' -exec sed -i 's/\(^deb.*-backports.*\)/#\1/; s/\(^deb.*-updates.*\)/#\1/; s/\(^deb.*-proposed.*\)/#\1/; s/\(^deb.*-security.*\)/#\1/' {} + \
    && \
  rm -rf /var/lib/apt/lists/* \
    && \
  echo "removed -backports, -updates, -proposed, -security repositories"

# magic to fix java installation conflict in subsequent apt install
# see https://github.com/geerlingguy/ansible-role-java/issues/64
RUN \
  apt-get update -q --allow-unauthenticated \
    && \
  apt-get install -qy --no-install-recommends \
    man \
    && \
  rm -rf /var/lib/apt/lists/* \
    && \
  mkdir /usr/share/man/man1/

RUN \
  apt-get update -q --allow-unauthenticated \
    && \
  apt-get install -qy --no-install-recommends \
    bibtool \
    git \
    make \
    moreutils \
    nodejs \
    pcregrep \
    pdftk \
    tree \
    && \
  rm -rf /var/lib/apt/lists/*

CMD ["bash"]


==> Makefile <==
SHELL=/bin/bash

# get the basename of the containing directory
# this will be used to name othe output document
BUILD_DIR := $(shell basename $(abspath $(dir $(lastword $(MAKEFILE_LIST)))/..))

DRAFT_SUPPLEMENT_PAGE = $(shell pdftk ${BUILD_DIR}-draft.pdf dump_data_utf8 | pcregrep -M -o1 '^BookmarkBegin\nBookmarkTitle: Supplemental Material\nBookmarkLevel: 1\nBookmarkPageNumber: ([0-9]+)$$')

RELEASE_SUPPLEMENT_PAGE = $(shell pdftk ${BUILD_DIR}.pdf dump_data_utf8 | pcregrep -M -o1 '^BookmarkBegin\nBookmarkTitle: Supplemental Material\nBookmarkLevel: 1\nBookmarkPageNumber: ([0-9]+)$$')

all: ${BUILD_DIR}-draft.pdf

draft: ${BUILD_DIR}-draft.pdf ${BUILD_DIR}-manuscript-draft.pdf ${BUILD_DIR}-supplement-draft.pdf ${BUILD_DIR}-draft.tex

release: ${BUILD_DIR}.pdf ${BUILD_DIR}-manuscript.pdf ${BUILD_DIR}-supplement.pdf ${BUILD_DIR}.tex

quick:
	pdflatex main.tex

${BUILD_DIR}.pdf: main.tex
	latexmk -pdf -silent \
    -jobname=${BUILD_DIR} \
    -pdflatex="pdflatex -interaction=nonstopmode" main.tex

${BUILD_DIR}.tex: main.tex
	./script/latexpand.pl main.tex > ${BUILD_DIR}.tex

${BUILD_DIR}-manuscript.pdf: ${BUILD_DIR}.pdf
	pdftk ${BUILD_DIR}.pdf cat 1-$$(( $(RELEASE_SUPPLEMENT_PAGE) - 1 )) output ${BUILD_DIR}-manuscript.pdf

${BUILD_DIR}-supplement.pdf: ${BUILD_DIR}.pdf
	pdftk ${BUILD_DIR}.pdf cat $(RELEASE_SUPPLEMENT_PAGE)-end output ${BUILD_DIR}-supplement.pdf

${BUILD_DIR}-draft.pdf: main.tex
	latexmk -pdf -silent \
    -jobname=${BUILD_DIR}-draft \
    -pdflatex="pdflatex -interaction=nonstopmode" draft.tex

${BUILD_DIR}-draft.tex: main.tex
	./script/latexpand.pl draft.tex > ${BUILD_DIR}-draft.tex

${BUILD_DIR}-manuscript-draft.pdf: ${BUILD_DIR}-draft.pdf
	pdftk ${BUILD_DIR}-draft.pdf cat 1-$$(( $(DRAFT_SUPPLEMENT_PAGE) - 1 )) output ${BUILD_DIR}-manuscript-draft.pdf

${BUILD_DIR}-supplement-draft.pdf: ${BUILD_DIR}-draft.pdf
	pdftk ${BUILD_DIR}-draft.pdf cat $(DRAFT_SUPPLEMENT_PAGE)-end output ${BUILD_DIR}-supplement-draft.pdf

fresh: cleaner all

clean:
	rm -f ${BUILD_DIR}.pdf
	rm -f ${BUILD_DIR}.tex
	rm -f ${BUILD_DIR}-draft.pdf
	rm -f ${BUILD_DIR}-draft.tex
	rm -f ${BUILD_DIR}-manuscript.pdf
	rm -f ${BUILD_DIR}-manuscript-draft.pdf
	rm -f ${BUILD_DIR}-supplement.pdf
	rm -f ${BUILD_DIR}-supplement-draft.pdf

sview:
	xdg-open ${BUILD_DIR}-draft.pdf 2>/dev/null

cleaner: clean
	latexmk -CA
	# remove auxillary files, excepting .tex and .bib files
	find . -type f -name ${BUILD_DIR}"*" ! -name '*.tex' ! -name '*.bib' -delete
	rm -rf *.bbl *.blg *.aux

.PHONY: draft release clean sview cleaner fresh quick


==> alg/curbed-recency-proportional-resolution-algo-enum-retained-ranks.tex <==
% TODO: missing pseudocode
\begin{algorithm}
\caption{Curbed Recency-proportional Resolution Stratum Enumeration}
\label{alg:curbed-recency-proportional-algo-enum-retained-ranks}
\begin{algorithmic}[1]
\State{Define $P:=T:=\{ \{1\},\ldots,\{d\}$\}}
\While{$\#P > 1$}
\State{Find an optimal partition tree $T_{C^\prime}$ }
\State{Update $P := (P{\setminus} C^\prime) \cup \{ \bigcup_{t\in C^\prime} t \}$}
\State{Update $T := T \cup \{ \bigcup_{t\in\tau} t : \tau\in T_{C^\prime}{\setminus}
\mathcal{L}(T_{C^\prime})\}$}
\EndWhile
\Return $T$
\end{algorithmic}
\end{algorithm}


==> alg/curbed-recency-proportional-resolution-algo-gen-drop-ranks.tex <==
% TODO: missing pseudocode
\begin{algorithm}
\caption{Curbed Recency-proportional Resolution Stratum Discard Generator}
\label{alg:curbed-recency-proportional-algo-gen-drop-ranks}
\begin{algorithmic}[1]
\State{Define $P:=T:=\{ \{1\},\ldots,\{d\}$\}}
\While{$\#P > 1$}
\State{Find an optimal partition tree $T_{C^\prime}$ }
\State{Update $P := (P{\setminus} C^\prime) \cup \{ \bigcup_{t\in C^\prime} t \}$}
\State{Update $T := T \cup \{ \bigcup_{t\in\tau} t : \tau\in T_{C^\prime}{\setminus}
\mathcal{L}(T_{C^\prime})\}$}
\EndWhile
\Return $T$
\end{algorithmic}
\end{algorithm}


==> alg/curbed-recency-proportional-resolution-algo-pred-keep-rank.tex <==
% TODO: missing pseudocode
\begin{algorithm}
\caption{Curbed Recency-proportional Resolution Stratum Retention Predicate}
\label{alg:curbed-recency-proportional-algo-pred-keep-rank}
\begin{algorithmic}[1]
\State{Define $P:=T:=\{ \{1\},\ldots,\{d\}$\}}
\While{$\#P > 1$}
\State{Find an optimal partition tree $T_{C^\prime}$ }
\State{Update $P := (P{\setminus} C^\prime) \cup \{ \bigcup_{t\in C^\prime} t \}$}
\State{Update $T := T \cup \{ \bigcup_{t\in\tau} t : \tau\in T_{C^\prime}{\setminus}
\mathcal{L}(T_{C^\prime})\}$}
\EndWhile
\Return $T$
\end{algorithmic}
\end{algorithm}


==> alg/depth-proportional-resolution-algo-pred-keep-rank.tex <==
\begin{algorithm}
\caption{Depth-proportional Resolution Stratum Retention Predicate}
\label{alg:depth-proportional-resolution-algo-pred-keep-rank}
% STUB ALGORITHM
\end{algorithm}


==> alg/fixed-resolution-algo-enum-retained-ranks.tex <==
\begin{algorithm}
\caption{Fixed Resolution Stratum Enumeration}
\label{alg:fixed-resolution-enum-retained-rans}
% STUB ALGORITHM
% \begin{algorithmic}[1]
%     \Require{$\texttt{n}$ -- the number of strata deposited}
%     \Require{$\texttt{r}$ -- the fixed resolution desired}
%     \For{$i = 0$ \textbf{to} $\texttt{n} - 1$ \textbf{step} $\texttt{r}$}
%         \State{ \textbf{yield} $i$ }
%     \EndFor
%     \State{ $\texttt{last\_rank} \gets \texttt{n} - 1$ }
%     \If{$\texttt{last\_rank} > 0$ \textbf{and} $(\texttt{last\_rank} \mod \texttt{r}) \neq 0$}
%         \State{ \textbf{yield} $\texttt{last\_rank}$ }
%     \EndIf
% \end{algorithmic}
\end{algorithm}


==> alg/fixed-resolution-algo-gen-drop-ranks.tex <==
\begin{algorithm}
\caption{Fixed Resolution Stratum Enumeration}
\label{alg:fixed-resolution-enum-retained-rans}
% STUB ALGORITHM
\end{algorithm}


==> alg/fixed-resolution-algo-pred-keep-rank.tex <==
\begin{algorithm}
\caption{Fixed Resolution Stratum Retention Predicate}
\label{alg:fixed-resolution-pred-keep-rank}
% STUB ALGORITHM
\end{algorithm}


==> alg/geom-seq-nth-root-algo-gen-drop-ranks.tex <==
\begin{algorithm}
\caption{Geometric Sequence $n$th Root Stratum Discard Generator}
\label{alg:geom-seq-nth-root-gen-drop-ranks}
% STUB ALGORITHM
\end{algorithm}


==> alg/geom-seq-nth-root-algo-pred-keep-rank.tex <==
% TODO: missing pseudocode
\begin{algorithm}
\caption{Geometric Sequence $n$th Root Stratum Retention Predicate}
\label{alg:geom-seq-nth-root-algo-pred-keep-rank}
% STUB ALGORITHM
\end{algorithm}


==> alg/perfect-tracking-pruning.tex <==
\begin{algorithm}
    \caption{Perfect phylogenetic tracking with pruning}
    \label{alg:perfect-tracking-pruning}
    \textbf{Part 1: Initialization} \\
    Same as algorithm \ref{alg:perfect-tracking} \\
    \textbf{Part 2: Handle birth event}
    \begin{algorithmic}[1]
        \Require{$P_i$ = newly created organism, $P_j$ = $P_i$'s parent}
        \State{Add node representing $P_i$ to $T$}
        \State{Add edge in $T$ from $P_i$ to $P_j$}
        \State{Record that $P_i$ is alive}
        \State{Increment $P_j$'s count of living offspring lineages}
    \end{algorithmic}
    \textbf{Part 3: Handle removal event}
    \begin{algorithmic}[1]
        \Require{$P_i$ = newly removed organism}
        \State{$P_j$ $\gets$ parent of $P_i$}
        \State{Record that $P_i$ is not alive}

        \While{$P_i$ is not alive \textbf{and} $P_i$'s count of living offspring lineages == 0}
            \State{Remove $P_i$ from $T$}
            \State{Decrement $P_j$'s count of living offspring lineages}
            \State{$P_i$ $\gets$ $P_j$}
            \State{$P_j$ $\gets$ parent of $P_j$}
        \EndWhile

    \end{algorithmic}
\end{algorithm}


==> alg/perfect-tracking.tex <==
\renewcommand{\algorithmiccomment}[1]{ \newline \textbf{comment:} \textit{#1}}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}

\begin{algorithm}
    \caption{Perfect phylogenetic tracking}
    \label{alg:perfect-tracking}
    \textbf{Part 1: Initialization}
    \begin{algorithmic}[1]
    \State{Define $T:=$ an empty forest}
    \end{algorithmic}
    \textbf{Part 2: Handle birth event}
    \begin{algorithmic}[1]
        \Require{$P_i$ = newly created organism, $P_j$ = $P_i$'s parent}
        \State{Add node representing $P_i$ to $T$}
        \State{Add edge in $T$ from $P_j$ to $P_i$}
    \end{algorithmic}
\end{algorithm}


==> alg/recency-proportional-resolution-algo-enum-retained-ranks.tex <==
\begin{algorithm}
\caption{Geometric Sequence $n$th Root Stratum Enumeration}
\label{alg:recency-proportional-resolution-algo-enum-retained-ranks}
% STUB ALGORITHM
\end{algorithm}


==> alg/recency-proportional-resolution-algo-pred-keep-rank.tex <==
\begin{algorithm}
\caption{Recency-proportional Resolution Stratum Retention Predicate}
\label{alg:recency-proportional-resolution-algo-pred-keep-rank}
% STUB ALGORITHM
\end{algorithm}


==> draft.tex <==
\def\mydraft{
\usepackage{draftwatermark}
\usepackage{lineno}
\linenumbers
\renewcommand{\linenumberfont}{\normalfont\small\color{red}}
}
\input{main.tex}


==> hereditary-stratigraph-concept/tex-extended-abstract/lib/dependencies.tex <==
\usepackage[export]{adjustbox}
\usepackage{algorithmic}
\usepackage{amsmath,amsfonts}
\usepackage{array}
\usepackage{bibunits}
\usepackage{booktabs}
\usepackage{caption}
\usepackage{cite}
\usepackage{colortbl}
\usepackage{csvsimple}
\usepackage{etoolbox}
\usepackage{graphicx}
\usepackage{hyperref,cleveref}
\usepackage{ifthen}
\usepackage{import}
\usepackage{listings}
\usepackage{makecell}
\usepackage{multirow}
\usepackage{natbib}
\usepackage{pythonhighlight}
\usepackage{rotating}
\usepackage{siunitx}
\usepackage{stringstrings}
\usepackage{subcaption}
\usepackage{tabularx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{xfp}
\usepackage{xparse}
\usepackage{xstring}


==> hereditary-stratigraph-concept/tex-extended-abstract/text/abstract.tex <==
\begin{abstract}
Phylogenetic analyses can also enable insight into evolutionary and ecological dynamics such as selection pressure and frequency dependent selection in digital evolution systems.
Traditionally, digital evolution systems have recorded data for phylogenetic analyses through perfect tracking where each birth event is recorded in a centralized data structures.
This approach, however, does not easily scale to distributed computing environments where evolutionary individuals may migrate between a large number of disjoint processing elements.
To provide for phylogenetic analyses in these environments, we propose an approach to infer phylogenies via heritable genetic annotations rather than directly track them.
We introduce a ``hereditary stratigraphy'' algorithm that enables efficient, accurate phylogenetic reconstruction with tunable, explicit trade-offs between annotation memory footprint and reconstruction accuracy.
This approach can estimate, for example, MRCA generation of two genomes within 10\% relative error with 95\% confidence up to a depth of a trillion generations with genome annotations smaller than a kilobyte.
We also simulate inference over known lineages, recovering up to 85.70\% of the information contained in the original tree using a 64-bit annotation.
\end{abstract}


==> hereditary-stratigraph-concept/tex-extended-abstract/text/acknowledgement.tex <==
\section*{Acknowledgment}

This research was supported in part by NSF grants DEB-1655715 and DBI-0939454 as well as by Michigan State University through the computational resources provided by the Institute for Cyber-Enabled Research.
This material is based upon work supported by the National Science Foundation Graduate Research Fellowship under Grant No. DGE-1424871.
Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the National Science Foundation.


==> hereditary-stratigraph-concept/tex-extended-abstract/text/body.tex <==
\input{text/body/introduction.tex}

\input{text/body/methods.tex}

\input{text/body/results-and-discussion.tex}

\input{text/body/conclusion.tex}


==> hereditary-stratigraph-concept/tex-extended-abstract/text/body/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}

This and other methodology to enable decentralized observation and analysis of evolving systems will be essential for digital evolution experiments that use distributed and best-effort computing approaches.
Such methods will be crucial to enabling experimental analyses while preserving those systems' efficiency and scalability.
As parallel and distributed computing becomes increasingly ubiquitous and begins to more widely pervade digital evolution systems, hereditary stratigraphy should serve as a useful technique in this toolbox.


==> hereditary-stratigraph-concept/tex-extended-abstract/text/body/introduction.tex <==
\section{Introduction} \label{sec:introduction}

In non-parallelized digital evolution experiments, phylogenetic trees can be tracked perfectly as they progress \citep{bohm2017mabe,wang2018vine,lalejini2019data} rather than reconstructed afterward, as must be done in most biological studies of evolution.
Such direct phylogenetic tracking enables a dizzying suite of experimental possibilities unique to digital evolution, such as perfect reconstruction of the sequence of phylogenetic states that led to a particular evolutionary outcome \citep{lenski2003evolutionary, dolson2020interpreting}.
% In a shared-memory context, it is not difficult to maintain a complete phylogeny where offspring simply track their parent (or vice versa).
% As simulations progress for longer durations, memory usage will typically grow at least linearly if population sizes are fixed, or worse if populations are growing or organisms are becoming more complex.
% These problems are easily ameliorated, however, by performing garbage collection on extinct lineages and saving older history to disk \citep{bohm2017mabe,dolson2019modes}.

Phylogenetic tracking in a distributed context, where linages may traverse many machines, introduces implementation complexity and more significant runtime overhead cost.
% However, if sufficient memory or disk space can be afforded to log all reproduction events, recording a perfect phylogeny in a distributed context is still not especially difficult.
% Processes could maintain records of each reproduction event, storing the parent organism (and its associated process) with all generated offspring (and their destination processes).
% As long as no data goes missing and organisms are uniquely identified globally, these ``dangling ends'' could be joined in postprocessing to weave a continuous global phylogeny.
% Of course, for the huge population sizes made possible by distirbuted systems, such stitching may become a demanding task in and of itself.
%
% However, if memory and disk space are limited, distributed phylogeny tracking becomes a more burdonsome challenge.
% A naive approach might employ a server model to maintain a central store of phylogenetic data.
% Processes would dispatch notifications of birth and death events to the server, which would curate (and gabage collect) phylogenetic history much the same as current serial phylogenetic tracking implementations.
% Unfortunately, this server model approach would present profound scalability challenges: communication and computation burden on the server process would worsen in direct proportion to processor count, and processes would frequently need to pause while waiting for confirmation that a reproduction event was successfully reported.
% ELD: This is making me wonder if there's a middle ground that could be explored in the future where we could use a sort of UDP phylogeny protocol, where no confirmation occurs
An ideally scalable approach would record birth and death events only on the process(es) where they unfold.
% Even this localized technique would lead to serious performance challenges, however.
% Lineages that went extinct locally could not be safely garbage collected until the extinction of thair offspring's lineages on other processors could be confirmed.
% Thus, garbage collection would require extinction notifications to wind back across processes each lineage had traversed.

% Under a best-effort model, no system of phylogeny tracking can guarantee proper garbage collection.
% For example, it would be possible for an offspring that was dispatched to a neighboring process to have failed to arrive, and both processes would need to keep going, despite the failure.
% So, extinction notifications for the lineage founded by that offspring would never be dispatched --- putting in motion a memory leak of un-garbage-collectible phylogenetic history.
% The situation becomes even more leaky when the possibility of extinction notifications themselves being lost.

In a distributed context --- especially, a distributed, best-effort context --- phylogenetic reconstruction (as opposed to tracking) could prove simpler and more efficient at runtime while providing sufficient power to address experimental questions of interest.
However, phylogenetic reconstruction from genomes with a traditional model of divergence under grandual accumulation of random mutations poses its own difficulties \citep{lack2010identifying,casci2008lining,hagstrom2004using,kapli2020phylogenetic,sarkar2010hardware}.

% The computational flexibility of digital evolution experiments provides a unique opportunity to overcome these challenges: designing heritable genome annotations specifically to simplify and strengthen phylogenetic reconstruction efforts.
% For maximum applicability of such a solution, these annotations should be phenotypically neutral heritable instrumentation \citep{stanley2002evolving} that do not affect any encodings for functional genome content.

This work introduces ``hereditary stratigraphy,'' a novel heritable genome annotation system to facilitate post-hoc phylogenetic inference on asexual populations.
This system allows explicit control over trade-offs between space complexity and accuracy of phylogenetic inference.
Instead of modeling genome components undergoing neutral variation through a mutational process, we keep a record of historical checkpoints that allow comparison of two lineages to identify the range of time in which they diverged.

% In Section \ref{sec:methods} we motivate and explain the hereditary stratigraphy approach.
% Then, in Section \ref{sec:results} we simulate post-hoc inference on known phylogenies to assess the quality of phylogenetic reconstruction enabled by the hereditary stratigraphy method.


==> hereditary-stratigraph-concept/tex-extended-abstract/text/body/methods.tex <==
\section{Methods} \label{sec:methods}

\input{fig/column-comparison.tex}

Our algorithm, particularly the vocabulary we developed to describe it, draws on the concept of geological stratigraphy, inference of natural history through analysis of successive layers of geological material \citep{steno1916prodromus}.
As an introductory intuition, suppose a body of rock being built up through regular, discrete events depositing of geological material.
Note that in such a scenario we could easily infer the age of the body of rock by counting up the number of layers present.
% Note that it is crucial to this scenario that each layer has some differentiating feature that allows it to be distinguished from layers above and below it, but also potentially from layers present in another body of rock in a distant and unrelated geographic position.
Next, imagine making a copy of the rock body in its partially-formed state and then moving it far away.
As time runs forward on these two rock bodies, independent layering processes will cause consistent disparity in the layers forming on each forwards from their point of separation.

To deduce the historical relationship of these rock bodies after the fact, we could simply align and compare their layers.
Layers from their base up through the first disparity would correspond to shared ancestry; further disparate layers would correspond to diverged ancestry.
% Interestingly, and powerfully for phylogenetic inference, we can readily distinguish a scenario where both rock bodies deposited ten layers after diverging from a scenario where one deposited eighteen layers and the other deposited two.
Figure \ref{fig:column-comparison} depicts the process of comparing columns for phylogenetic inference.

Shifting now from intuition to implementation, a fixed-length randomly-generated binary tag provides a convenient and efficient mechanism to differentiate between our metaphorical ``layers.''
% We call this ``fingerprint'' tag a \textit{differentia}.
% The width of this tag controls the probability of spurious collisions between independently generated instances.
% At 64 bits wide the tag essentially functions as a UID: collisions between randomly generated tags are so unlikely ($p < 5.42\times10^{-20}$) they can essentially be ignored.
% At the other end of the spectrum, collision probability would be $1/256$ for a single byte and $1/2$ for a single bit.
% In the case of narrow differentia, in order to set a lower bound for the MRCA generation, you would have to backtrack common strata from the last commonality until the probability of that many successive spurious collisions was enough to satisfy your desired confidence level (e.g., 95\% confidence).
% Even then, there would be a possibility of the the true MRCA falling before the lower bound.
% Note, however, that no matter the width of the differentia the generation of the first discrepancy provides a hard upper bound on the generation of the MRCA.
%
In accordance with our geological analogy, we refer to the packet of data accumulated each generation as a \textit{stratum}.
This packet contains the differentia and, although not employed in this work, could hold other arbitrary user-defined data (i.e., simulation timestamp, phenotype characteristics, etc.).
% Again in accordance with the geological analogy, we refer to the chronological stack of strata that accumulate over successive depositions as a \textit{hereditary stratigraphic column}.

% \subsection{Stratum Retention Policy}

% \input{fig/deposit-process.tex}

As currently stated, fingerprints will accumulate proportionally to the length of evolutionary history simulated.
In an evolutionary run with thousands or millions of generations, this approach would soon become intractable --- particularly when columns are serialized and transmitted between distributed computing elements.
To solve this problem, we can trade off precision for compactness by deleting strata from columns as time progresses.
% Figure \ref{fig:deposit-process} overviews how stratum deposit and stratum elimination progress over two generations under the hereditary stratigraphic column scheme.
%
% Different patterns of deletion will lead to different trade-offs, both in terms of the scaling relationship of column size to generations elapsed and in terms of the arrangement of precision over evolutionary history (i.e., focusing precision on more recent evolutionary history versus spreading it evenly over the entire history).
%
We refer to the rule set used to selectively eliminate strata over time as the ``stratum retention policy.''
We devised three stratum retention policies, which provide
\begin{itemize}
  \item linear space complexity and constant inference error,
  \item constant space complexity and linear inference error with respect to phylogenetic depth, or
  \item logarithmic space complexity and inference error as a constant proportion of time elapsed since MRCA.
\end{itemize}

% We explore several different retention policy designs here, and implement our software to allows for free, modular interchange of retention policies.
% It is possible to define a policy through either of two mechanisms.
% First, policy can be defined as a ``predicate'' where the generation of a stratum and the current number of strata deposited is passed into a function that returns whether that strata should be retained at that point in time.
% Second, policy can be defined as a ``condemner'' generator where, given the current number of strata deposited, the set of ranks that should be deleted at this point in time are yielded.
% Although the predicate form is useful for analyzing and proving properties of policies, the condemner form is generally more efficient in practice.
% We provide predicate and condemner implementations for each stratum retention policy discussed here.

% It should be noted that condemners and predicates are both defined in terms of stratum generation, not stratum index among retained strata in the column.
% Therefore, it may seem necessary to store the generation of deposit within the stratum data structure.
% However, if you know the total number of generations deposited you can map backwards from index to recover the generation deposited without storing it.
% We provide this formula for each stratum retention policy.
% Finally, for each policy we provide a formula to calculate the exact number of strata retained under any parameterization after $n$ generations.
%
% In the next subsections, we introduce several stratum retention policies, provide the intuition behind their implementation, and elaborate their space complexity and resolution properties.
% For each policy, patterns of stratum retention are illustrated in Figure \ref{fig:retention-policies}.
% The formulas for number of strata retained after $n$ generations, the formulas to calculate stratum deposit generation from column index, and the retention predicate specifications of each policy are available in Supplementary Listing \ref{lst:StratumRetentionPredicateDepthProportionalResolution} \citep{moreno2022hstratconceptsupplement}.
% The condemner generator specification of each policy is available in Supplementary Listing \ref{lst:StratumRetentionCondemnerDepthProportionalResolution} \citep{moreno2022hstratconceptsupplement}.
% For tapered depth-proportional resolution and recency-proportional resolution, the accuracy of MRCA estimation can also be explored via an interactive in-browser web applet at \url{https://hopth.ru/bi}.
%
% \input{fig/retention-policies.tex}
%
% \subsection{Fixed Resolution Stratum Retention Policy}
%
% The fixed resolution retention policy provides a fixed absolute upper bound $r$ on the spacing between retained strata.
% The strategy to obtain this property is simple: permanently retain a stratum every $r$th generation
% (although, for arbitrary reasons of implementation convenience we require each stratum to be retained during at least the generation it is deposited).
%
% However, this retention policy suffers from linear growth in a column's memory footprint with respect to number of generations elapsed: every $r$th generation generation a new stratum is permanently retained
% For this reason, it is likely not useful in practice except potentially in scenarios where the number of generations is fixed in advance.
% We include it here largely for illustrative purposes as a gentle introduction to retention policies.
%
% \subsection{Depth-Proportional Resolution Stratum Retention Policy}
%
% The depth-proportional resolution policy ensures spacing between retained strata will be less than or equal to a proportion $r$ of total number of strata deposited.
% Achieving this limit on uncertainty requires retaining sufficient strata so that no more than $r$ ranks elapsed between any two strata.
% This policy accumulates retained strata at a fixed interval until twice as many as $r$ are at hand.
% Then, every other retained stratum is purged and the cycle repeats with a new twice-as-wide interval between retained strata.
%
% When comparing stratigraphic columns from different generations, the resolution guarantee holds in terms of the number of generations experienced by the older of the two columns.
% Because this retention policy is deterministic, for two columns with the same policy, every stratum that is held by the older column is also guaranteed to be present in the younger column (unless it hasn't yet been deposited on the younger column).
% Therefore, the strata that would enable the desired resolution when comparing two columns of the same age are guaranteed to be available.
%
% Because the number of strata retained under this policy is bounded as $2n+1$, space complexity scales as $O(1)$ with respect to the number of strata deposited.
% It follows that the MRCA rank estimate uncertainty scales as $O(n)$ with respect to the number of strata deposited.
%
% \subsection{Tapered Depth-Proportional Resolution Stratum Retention Policy}
%
% This policy refines the depth-proportional resolution policy to provide a more stable column memory footprint over time.
% The naive depth-proportional resolution policy builds up strata until twice as many are present as needed then purges half of them all at once.
% The tapered depth-proportional resolution policy functions identically to the depth-proportional policy except that it removes unnecessary strata gradually from back to front as new strata are deposited, instead of eliminating them simultaneously.
% The column footprint stability of this variation makes it easier to parameterize our experiments to ensure comparable end-state column footprints for fair comparison between retention policies, in addition to making this policy likely better suited to most use cases.
% By design, this policy has the same space complexity and MRCA estimation uncertainty scaling relationships with number generations elapsed as the naive depth-proporitonal resolution policy.
%
% \subsection{MRCA-Recency-Proportional Resolution Stratum Retention Policy}
%
% \input{tab/recency-proportional-space-complexity.tex}
%
% The MRCA-recency-proportional resolution policy ensures distance between the retained strata surrounding any generation point will be less than or equal to a user-specified proportion $r$ of the number of generations elapsed since.
%
% This policy can be constructed recursively, so to begin, let's consider setting up just the \textit{first} generation $g$ of the stratum after the root ancestor we will retain when $n$ generations have elapsed.
% A simple geometric analysis reveals that providing the guaranteed resolution for the worst-case generation within the window between generation 0 and generation $g$ (i.e., generation $g-1$) requires
% \begin{align*}
%   g \leq \lfloor n / (r + 1) \rfloor.
% \end{align*}
%
% We now have an upper bound for the rank of the first stratum generation we must retain.
% However, we must guarantee that these ranks are actually available for us to retain (i.e., it hasn't been purged out of the column at a previous time point as the column was grown by successive deposition).
% We will do this by picking the rank that is the highest power of 2 less than or equal to our bound.
% If we repeat this procedure as we recurse, we are guaranteed that this rank will have been preserved across all previous timepoints.
%
% Why does this work?
% Consider a sequence where all elements are powers of 2 and elements in the sequence are strictly nonincreasing.
% Consider the first element of the list.
% Partial sums along the sequence will include all multiples this first element.
% So, when we ratchet up $g$ to $2g$ as $n$ increases, we are guaranteed that $2g$ has been retained.
% This principle generalizes recursively down the list.
% This is a similar principle to the approach of strictly-doubling interval sizes used in the Naive and Tapered Depth-Proportional Resolution stratum retention policies described above.
%
% This step of truncating to the nearest less than or equal to power of 2 affects our recursive step size at most only by a constant factor of 2.
% So, because step size is a constant fraction of remaining generations $n$ (at worst $\frac{1}{2(r+1)}$), the number of steps made (and number of strata retained) scales as $O(\log(n))$ with respect to the number of strata deposited.
% Table \ref{tab:recency-proportional-space-complexity} provides exact figures for the number of strata retained under different parameterizations of the recency-proportional retention policy between one thousand and one trillion generations.
%
% As for rank estimate uncertainty, in the worst case it scales as $O(n)$ with respect to the greater number of strata deposited.
% However, with respect to estimating the rank of the MRCA when lineages diverged any fixed number of generations ago, uncertainty scales as $O(1)$.
%
% How does space complexity scale with respect to the policy's specified resolution $r$?
% Through extrapolation from OEIS sequences A063787 and A056791 via guess and check \citep{sloane2021a063787,sloane2021a056791}, we posited the exact number of strata retained after $n$ generations as
%
% \begin{align*}
%   \mathrm{HammingWeight}(n)
%   + \sum_1^r \lfloor \log_2( \lfloor n / r \rfloor ) \rfloor
%   + 1.
% \end{align*}
%
% This expression has been unit tested extensively to ensure perfect reliability.
% Approximating and applying logarithmic properties, this policy's space complexity can be calculated within a constant factor as
%
% \begin{align*}
% \log(n) + \log\Big(\frac{n^r}{r!}\Big).
% \end{align*}
%
% To answer our question, we will examine the ratio of space complexities required when scaling resolution $r$ up by a constant factor $f > 1$.
% Evaluating this ratio as $r \to \infty$, we find that space complexity scales directly proportional with the desired resolution $r$ at the limit,
%
% \begin{align*}
% \lim_{r \to \infty}
% \frac{
%   \log(n) + \log\Big(\frac{n^{fr}}{(fr)!}\Big)
% }{
%   \log(n) + \log\Big(\frac{n^r}{r!}\Big)
% }
% = f.
% \end{align*}
%
% Evaluating this ratio as $n \to \infty$, we find that this scaling relationship is never worse than directly proportional for any $r$,
%
% \begin{align*}
% \lim_{n \to \infty}
% \frac{
%   \log(n) + \log\Big(\frac{n^{fr}}{(fr)!}\Big)
% }{
%   \log(n) + \log\Big(\frac{n^r}{r!}\Big)
% }
% &= \frac{fr+1}{r+1}\\
% &= f\frac{r + 1/f}{r + 1}\\
% &\leq f.
% \end{align*}
%
%
% \subsection{Computational Experiments}
%
% These simulations propagated populations of between 100 and 165 bitstrings between 500 and 5,000 synchronous generations under the NK fitness landscape model \citep{kauffman1989nk}.
% In order to ensure coverage of a variety of phylogenetic conditions, we sampled a variety of selection schemes that impose profoundly different ecological regimens \citep{dolson2018ecological},
% \begin{itemize}
%   \item EcoEA Selection \citep{goings2012ecology},
%   \item Lexicase Selection \citep{helmuth2014solving},
%   \item Random Selection,
%   \item Sharing Selection \citep{goldberg1987genetic}
%   % \item Tournament Selection \citep{miller1995genetic}.
% \end{itemize}
%
% Supplementary Table \ref{tab:ground-truth-phylogenies} provides full details on the conditions each ground truth phylogeny was drawn from.
% The phylogenies themselves are available in our data repository for this project.
%
% For each ground truth phylogeny, we tested combinations of three configuration parameters:
% \begin{itemize}
%   \item target end-state memory footprints for extant columns (64, 512, and 4096 bits),
%   \item differentia width (1, 8, and 64 bits), and
%   \item stratum retention policy (tapered depth-proportional resolution and recency-proportional resolution).
% \end{itemize}
%
% Stratum retention policies were parameterized so that the maximum number of strata possible were present at the end of the experiment without exceeding the target memory footprint.
% If the target memory footprint is exceeded by the sparsest possible parameterization of a retention policy, then that sparsest possible parameterization is used.
% Supplementary Tables \cref{tab:experiment-column-sizes-nk-ecoea-selection,tab:experiment-column-sizes-nk-lexicase-selection,tab:experiment-column-sizes-nk-random-selection,tab:experiment-column-sizes-nk-sharing-selection,tab:experiment-column-sizes-nk-tournament-selection} provide the calculated paramaterizations and memory footprints of extant columns \citep{moreno2022hstratconceptsupplement}.
%
% In order to assess the viability of phylogenetic inference using hereditary stratigraphic columns from extant organisms, we used the end-state stratigraphs to estimate a reconstruction of the actual ground truth phylogenetic histories.
% The first step to reconstructing a phylogenetic tree for the history of an extant population at the end of an experiment is to construct a distance matrix by calculating all pairwise phylogenetic distances between extant columns.
% We defined phylogenetic distance between two extant columns as the sum of each extant organism's generational distance back to the generation of their MRCA, estimated as the mean of the upper and lower 95\% confidence bounds.
% Supplementary Figure \ref{fig:phylogenetic-inference} provides a cartoon summary of the process of calculating phylogenetic distance between two extant columns \citep{moreno2022hstratconceptsupplement}.
%
% We then used the unweighted pair group method with arithmetic mean (UPGMA) reconstruction tool provided by the BioPython package to generate estimate phylogenetic trees \citep{cock2009biopython,sokal1958statistical}.
% After generating the reconstructed tree topology, we performed a second pass to adjust branch lengths so that each tree node sat at the mean of its estimated 95\% confidence generation bounds.
% %We found that the neighbor joining (NJ) approach occasionally yielded reconstructions with impossible ``negative generation'' branches \citep{saitou1987neighbor} after knowledge bounding the absolute generation of internal nodes (i.e., MRCA's between pairs of extant organisms) was applied, so we did not use it.
%
% \subsection{Software and Data}
%
% % A prototype of this approach has been implemented \url{https://github.com/mmore500/dishtiny/blob/incoming/include/dish2/genome/PhyloFingerprints.hpp} and preliminarily tested \url{https://github.com/mmore500/dishtiny/blob/incoming/tests/dish2/genome/PhyloFingerprints.cpp}.
%
% As part of this work, we published the \texttt{hstrat} Python library with a stable public-facing API intended to enable incorporation in other projects with extensive documentation and unit testing on GitHub at \url{https://anonymous.4open.science/r/hstrat-115D/} and on PyPI.% at \url{https://pypi.org/project/hstrat/}. https://github.com/mmore500/hstrat
% In the near future, we intend to complete and publish a corresponding C++ library.
%
% Supporting software materials can be found on GitHub at \url{https://anonymous.4open.science/r/hereditary-stratigraph-concept-6BEC/}.%\url{https://github.com/mmore500/hereditary-stratigraph-concept}
% Supporting computational notebooks are available for in-browser use via BinderHub at \url{ANONYMIZED FOR PEER REVIEW} \citep{ragan2018binder}. %https://mybinder.org/v2/gh/mmore500/hereditary-stratigraph-concept/HEAD?labpath=binder%2F
% Our work benefited from many pieces of open source scientific software, including \citep{sukumaran2010dendropy,virtanen2020scipy,hunter2007matplotlib,virtanen2020scipy,waskom2021seaborn,bostock2011d3,meurer2017sympy,smith2020treedistdata,paradis2004ape,ushey2022reticulate,wickham2022dplyr}.
% The ground truth phylogenies used in this work as well as supplementary figures, tables, and text are available via the Open Science Framework at
% \url{https://osf.io/4sm72/?view\_only=69f37c6d184143b7855299c3323749ea} \citep{foster2017open,moreno2022hstratconceptsupplement}.
% Phylogenetic data associated with this project is stored in the Alife Community Data Standards format \citep{lalejini2019data}.


==> hereditary-stratigraph-concept/tex-extended-abstract/text/body/results-and-discussion.tex <==
\section{Results} \label{sec:results}

In order to assess the practical performance of the hereditary stratigraph approach in an applied setting, we simulated the process of stratigraph propagation over known ``ground truth'' phylogenies extracted from pre-existing digital evolution simulations \citep{hernandez2022phylogenetic}.
Across ground truth phylogenies, we were able to reconstruct the phylogenetic topology with between 47.75\% and 85.70\% of the information contained in the original tree using a 64-bit column memory footprint, between 47.75\% and 80.36\% using a 512-bit column memory footprint, and between 51.13\% and 83.53\% using a 4096-bit column memory footprint.


==> hereditary-stratigraph-concept/tex-extended-abstract/text/frontmatter.tex <==
\title{ Hereditary Stratigraphy: Genome Annotations to Enable Phylogenetic Inference over Distributed Populations }

%%
%% The "author" command and its associated commands are used to define
%% the authors and their affiliations.
%% Of note is the shared affiliation of the first two authors, and the
%% "authornote" and "authornotemark" commands
%% used to denote shared contribution to the research.
\author{Matthew Andres Moreno}
\orcid{0000-0003-4726-4479}
\affiliation{%
  \institution{Michigan Statue University}
  \city{East Lansing}
  \state{Michigan}
  \country{USA}
  \postcode{48103}
}

\author{Emily Dolson}
% \email{dolsonem@msu.edu}
\orcid{0000-0001-8616-4898}
\affiliation{%
  \institution{Michigan Statue University}
  \city{East Lansing}
  \state{Michigan}
  \country{USA}
  \postcode{48103}
}

\author{Charles Ofria}
% \email{ofria@msu.edu}
\orcid{0000-0003-2924-1732}
\affiliation{%
  \institution{Michigan Statue University}
  \city{East Lansing}
  \state{Michigan}
  \country{USA}
  \postcode{48103}
}


%%
%% By default, the full list of authors will be used in the page
%% headers. Often, this list is too long, and will overlap
%% other information printed in the page headers. This command allows
%% the author to define a more concise list
%% of authors' names for this purpose.
\renewcommand{\shortauthors}{Moreno et al.}

\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10010147.10010341.10010366.10010369</concept_id>
       <concept_desc>Computing methodologies~Simulation tools</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10010147.10010257.10010293.10011809.10011812</concept_id>
       <concept_desc>Computing methodologies~Genetic algorithms</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Computing methodologies~Simulation tools}
\ccsdesc[500]{Computing methodologies~Genetic algorithms}

\keywords{phylogenetics, decentralized algorithms, digital evolution, genetic algorithms, genetic programming}

\input{text/abstract.tex}

\maketitle


==> hereditary-stratigraph-concept/tex-extended-abstract/text/references.tex <==
% \section*{References}

\putbib


==> hereditary-stratigraph-concept/tex/draft.tex <==
\def\mydraft{
\usepackage{draftwatermark}
\usepackage{lineno}
\linenumbers
\renewcommand{\linenumberfont}{\normalfont\small\color{red}}
}
\input{main.tex}


==> hereditary-stratigraph-concept/tex/fig/cid_plot.tex <==
\begin{figure}
    \includegraphics[width=\columnwidth]{img/cid_plot}
    \caption{
    Reconstruction error for phylogenetic inference with ground truth sharing selection phylogeny.
    Lower is better.
    RPR is recency-proportional resolution policy and TDPR is tapered depth-proportional resolution policy.
    }
  \label{fig:cid_plot}
\end{figure}


==> hereditary-stratigraph-concept/tex/fig/column-comparison.tex <==
\begin{figure}
    \includegraphics[width=\columnwidth]{img/column-comparison}
    \caption{
    Inferring the generation of the most-recent common ancestor (MRCA) of two hereditary stratigraphic columns ``$A$'' and ``$B$''.
    Columns are aligned at corresponding generations.
    Then the first generation with disparate ``fingerprints'' is determined.
    % (If a particular generation's strata have been eliminated from one or both columns or have not yet been deposited on one column, then no comparison is performed at that generation.)
    This provides a hard upper bound on the generation of the MRCA: these strata \textit{must} have been deposited along separate lines of descent.
    Searching backward for the first commonality preceding that disparity provides a soft lower bound on the generation of the MRCA: these strata evidence common ancestry but \textit{might} collide by chance.
    Some strata mmay have been eliminated from the columns, as shown, in order to save space at the cost of increasing uncertainty of MRCA generation estimates.
    % (If a narrow ``fingerprint'' differentia like a single bit is used with plausible collision probability, a lower bound can be established by continuing to search backward until the probability of $k$ successive spurious collisions is sufficiently unlikely.)
    % This process yields certainty about the phylogenetic relationship between $A$ and $B$ shown at right above (i.e., common) and below (i.e., diverged) the MRCA bounds.
    }
  \label{fig:column-comparison}
\end{figure}


==> hereditary-stratigraph-concept/tex/fig/deposit-process.tex <==
\input{lib/dissertationexclude.tex}
\begin{figure*}
  \dissertationexclude{\begin{minipage}{0.6\textwidth}}
    \includegraphics[width=\textwidth]{img/deposit-process}
  \dissertationexclude{\end{minipage}}%
  \dissertationexclude{\begin{minipage}{0.4\textwidth}}
    \caption{
    Cartoon illustration of stratum deposit process.
    This process marks the elapse of a generation when a hereditary stratigraphic column is inherited by an offspring.
    First, a new stratum is appended to the end of the column with a randomly-generated ``fingerprint.''
    This ``fingerprint'' distinguishes strata that were generated along disparate lines of descent (e.g., \texttt{0xd01a} for 3rd Generation A and \texttt{0xe74a} for 3rd generation B).
    Then, the column's configured stratum retention policy is applied to ``prune'' the column by eliminating strata from specific generations.
    Although this cartoon depicts an empty space for eliminated strata, the underlying data structure behind a column (i.e., the pink overlay) can condense to reduce space complexity.
    }\label{fig:deposit-process}
  \dissertationexclude{\end{minipage}}
\end{figure*}


==> hereditary-stratigraph-concept/tex/fig/diffbits-clustering-information-distance.tex <==
\begin{sidewaysfigure}
  \includegraphics[width=\linewidth]{submodules/hereditary-stratigraph-concept-binder/binder/reconstruction-quality/teeplots/col=condition+hue=num-differentia-bits+kind=bar+row=policy+tree-comparison-metric=clustering-information-distance+viz=catplot+x=num-column-bits+y=score+ext=}
  \caption{
  Comparison of phylogenetic reconstruction quality across differentia bit counts.
  Reconstruction quality measured as clustering information distance between reconstructed phylogeny and ground truth phylogeny \citep{smith2020information, smith2020treedist}.
  Lower is better.
  RPR is recency-proportional resolution stratum retention policy and TDPR is tapered depth-proportional resolution stratum retention policy.
  }
  \label{fig:diffbits-clustering-information-distance}
\end{sidewaysfigure}


==> hereditary-stratigraph-concept/tex/fig/diffbits-mutual-clustering-information.tex <==
\begin{sidewaysfigure}
  \includegraphics[width=\linewidth]{submodules/hereditary-stratigraph-concept-binder/binder/reconstruction-quality/teeplots/col=condition+hue=num-differentia-bits+kind=bar+row=policy+tree-comparison-metric=mutual-clustering-information+viz=catplot+x=num-column-bits+y=score+ext=}
  \caption{
  Comparison of phylogenetic reconstruction quality across differentia bit counts.
  Reconstruction quality measured as mutual clustering information between reconstructed phylogeny and ground truth phylogeny \citep{smith2020information, smith2020treedist}.
  Higher is better.
  RPR is recency-proportional resolution stratum retention policy and TDPR is tapered depth-proportional resolution stratum retention policy.
  }
  \label{fig:diffbits-mutual-clustering-information}
\end{sidewaysfigure}


==> hereditary-stratigraph-concept/tex/fig/diffbits-robinson-foulds-similarity.tex <==
\begin{sidewaysfigure}
  \includegraphics[width=\linewidth]{submodules/hereditary-stratigraph-concept-binder/binder/reconstruction-quality/teeplots/col=condition+hue=num-differentia-bits+kind=bar+row=policy+tree-comparison-metric=generalized-robinson-foulds-similarity+viz=catplot+x=num-column-bits+y=score+ext=}
  \caption{
  Comparison of phylogenetic reconstruction quality across differentia bit counts.
  Reconstruction quality measured as generalized Robinson-Foulds similarity between reconstructed phylogeny and ground truth phylogeny \citep{smith2020information, smith2020treedist}.
  Higher is better.
  RPR is recency-proportional resolution stratum retention policy and TDPR is tapered depth-proportional resolution stratum retention policy.
  }
  \label{fig:diffbits-robinson-foulds-similarity}
\end{sidewaysfigure}


==> hereditary-stratigraph-concept/tex/fig/info_plot.tex <==
\begin{figure}
    \includegraphics[width=\columnwidth]{img/info_plot}
    \caption{
    Proportion of information present in the ground-truth ftness sharing phylogeny that was captureed by our reconstruction, across various retention policies.
    High is better (1 is perfect).
    RPR is recency-proportional resolution policy and TDPR is tapered depth-proportional resolution policy.
    } \label{fig:info_plot}
\end{figure}


==> hereditary-stratigraph-concept/tex/fig/phylogenetic-inference.tex <==
\begin{figure*}
  \centering
    \includegraphics[width=\textwidth]{img/phylogenetic-inference}
    \caption{
    Cartoon illustration of column inheritance along a phylogenetic tree and the process to infer phylogenetic history along extant columns.
    This scenario supposes a stratum retention policy where only strata from even generations are retained.
    The common ancestor of the focal clade, which is at generation 2, is shown at top.
    Generation 3 columns inherit that ancestor's strata and each append a new stratum.
    Generation 4 columns append another new stratum then eliminate their generation 3 strata.
    Finally, another generation elapses to yield generation 5 strata.
    Suppose that only generation 5 strata are extant.
    So, greyed-out columns above are not directly observable.
    Phylogenetic history is deduced by pairwise comparison between extant columns.
    For each pair (like the example highlighted in red) a phylogenetic distance can be computed as the sum generations elapsed to each extant column after the estimated generation of their MRCA.
    These pairwise distances can then be fed into a phylogeny reconstruction algorithm.
    }
  \label{fig:phylogenetic-inference}
\end{figure*}


==> hereditary-stratigraph-concept/tex/fig/policy-clustering-information-distance.tex <==
\begin{figure*}
    \includegraphics[width=\linewidth]{submodules/hereditary-stratigraph-concept-binder/binder/reconstruction-quality/teeplots/col=num-differentia-bits+hue=policy+kind=bar+row=num-column-bits+tree-comparison-metric=clustering-information-distance+viz=catplot+x=condition+y=score+ext=}
    \caption{
    Comparison of phylogenetic reconstruction quality between stratum retention policies.
    Reconstruction quality measured as clustering information distance between reconstructed phylogeny and ground truth phylogeny \citep{smith2020information, smith2020treedist}.
    Lower is better.
    RPR is recency-proportional resolution stratum retention policy and TDPR is tapered depth-proportional resolution stratum retention policy.
    }
    \label{fig:policy-clustering-information-distance}
\end{figure*}


==> hereditary-stratigraph-concept/tex/fig/policy-mutual-clustering-information.tex <==
\begin{figure*}
    \includegraphics[width=\linewidth]{submodules/hereditary-stratigraph-concept-binder/binder/reconstruction-quality/teeplots/col=num-differentia-bits+hue=policy+kind=bar+row=num-column-bits+tree-comparison-metric=mutual-clustering-information+viz=catplot+x=condition+y=score+ext=}
    \caption{
    Comparison of phylogenetic reconstruction quality between stratum retention policies.
    Reconstruction quality measured as mutual clustering information between reconstructed phylogeny and ground truth phylogeny \citep{smith2020information, smith2020treedist}.
    Higher is better.
    RPR is recency-proportional resolution stratum retention policy and TDPR is tapered depth-proportional resolution stratum retention policy.
    }
    \label{fig:policy-mutual-clustering-information}
\end{figure*}


==> hereditary-stratigraph-concept/tex/fig/policy-robinson-foulds-similarity.tex <==
\begin{figure*}
    \includegraphics[width=\linewidth]{submodules/hereditary-stratigraph-concept-binder/binder/reconstruction-quality/teeplots/col=num-differentia-bits+hue=policy+kind=bar+row=num-column-bits+tree-comparison-metric=generalized-robinson-foulds-similarity+viz=catplot+x=condition+y=score+ext=}
    \caption{
    Comparison of phylogenetic reconstruction quality between stratum retention policies.
    Reconstruction quality measured as generalized Robinson-Foulds similarity between reconstructed phylogeny and ground truth phylogeny \citep{smith2020information, smith2020treedist}.
    Higher is better.
    RPR is recency-proportional resolution stratum retention policy and TDPR is tapered depth-proportional resolution stratum retention policy.    }
    \label{fig:policy-robinson-foulds-similarity}
\end{figure*}


==> hereditary-stratigraph-concept/tex/fig/reconstruction-example.tex <==
\input{lib/importpath.tex}

\begin{figure*}%
%-------------------------------------------------------------------------------
  \begin{subfigure}[t]{0.32\linewidth}
    \centering
    % pass an arbitrary filename, potentially with unsafe characters
    % adapted from https://tex.stackexchange.com/a/36178
    \catcode`\%=12
    \providecommand\filename{}
    \renewcommand\filename{\detokenize{submodules/hereditary-stratigraph-concept-binder/binder/phylogenetic-inference/teeplots/a=true_phylogeny+source=a%reconstructed_phylogenies~source%nk_lexicaseselection_seed110_pop165_mut.01_snapshot_500.csv.gz+viz=truncate-phylo+ext=}}
    \catcode`\%=14
    \includegraphics[width=\linewidth]{\importpath\filename}
    \caption{Ground truth phylogeny.}
    \label{fig:reconstruction-example-true-phylogeny}
  \end{subfigure}%
  \hfill%
%-------------------------------------------------------------------------------
  \begin{subfigure}[t]{0.32\linewidth}
    \centering
    % pass an arbitrary filename, potentially with unsafe characters
    % adapted from https://tex.stackexchange.com/a/36178
    \catcode`\%=12
    \providecommand\filename{}
    \renewcommand\filename{\detokenize{submodules/hereditary-stratigraph-concept-binder/binder/phylogenetic-inference/teeplots/source=a%reconstructed_phylogenies~source%nk_lexicaseselection_seed110_pop165_mut.01_snapshot_500.csv.gz+treatment=differentia%1~policy%TaperedDepthProportionalResolution~target%64+viz=truncate-phylo-bounds+ext=}}
    \catcode`\%=14
    \includegraphics[width=\linewidth]{\importpath\filename}
    \caption{1-bit Fingerprint Differentia, Tapered Depth-Proportional Resolution Stratum Retention Predicate, 64 bit target column footprint.}
    \label{fig:reconstruction-example-d1-rp-t64}
  \end{subfigure}%
  \hfill%
%-------------------------------------------------------------------------------
  \begin{subfigure}[t]{0.32\linewidth}
    \centering
    % pass an arbitrary filename, potentially with unsafe characters
    % adapted from https://tex.stackexchange.com/a/36178
    \catcode`\%=12
    \providecommand\filename{}
    \renewcommand\filename{\detokenize{submodules/hereditary-stratigraph-concept-binder/binder/phylogenetic-inference/teeplots/source=a%reconstructed_phylogenies~source%nk_lexicaseselection_seed110_pop165_mut.01_snapshot_500.csv.gz+treatment=differentia%1~policy%RecencyProportionalResolution~target%64+viz=truncate-phylo-bounds+ext=}}
    \catcode`\%=14
    \includegraphics[width=\textwidth]{\importpath\filename}
    \caption{1-bit Fingerprint Differentia, MRCA-Recency-Proportional Resolution Stratum Retention Predicate, 64 bit target column footprint.}
    \label{fig:reconstruction-example-d1-tdp-t64}
  \end{subfigure}
%-------------------------------------------------------------------------------
  \caption{
    Example phylogeny reconstructions of ground-truth lexicase selection phylogeny from inference on extant hereditary stratigraphic columns.
    Shaded error bars on reconstructions indicate 95\% confidence intervals for the true generation of tree nodes.
    Arbitrary color is added to enhance distinguishability.
  }
  \label{fig:reconstruction-example}
\end{figure*}


==> hereditary-stratigraph-concept/tex/fig/retention-policies.tex <==
\input{lib/dissertationelse.tex}
\input{lib/dissertationonly.tex}

\begin{figure*}
  \centering
  \dissertationonly{\footnotesize}
  \begin{tabular}{m{0.05\textwidth}@{}|c@{}|c@{\hskip 0.01\textwidth}|m{0.14\textwidth}}
%-------------------------------------------------------------------------------
\hspace{-1ex}Policy&Lower-Resolution Parameterization&Higher-Resolution Parameterization&\makecell[c]{Properties}\\\hline
%-------------------------------------------------------------------------------
    \rotatebox{90}{\textbf{Fixed Resolution}}
  &
    \makecell{
      \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept-binder/binder/retention-policies/teeplots/fixed_resolution=512+num_layers=1024+stratum_retention_predicate=fixed-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
    \makecell{
      \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept-binder/binder/retention-policies/teeplots/fixed_resolution=128+num_layers=1024+stratum_retention_predicate=fixed-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
  \makecell[{{p{0.14\textwidth}}}]{
  \centering
    \bf{Space Complexity}\\
    $O(n)$\\
    \bf{MRCA Uncertainty}\\
    $O(1)$
  }
  \makecell[{{p{0.14\textwidth}}}]{
  \raggedright
    where $n$ is gens elapsed.
  }\\\hline
%-------------------------------------------------------------------------------
    \adjustbox{
      minipage=10em,
      rotate=90,
    }{
      \centering
      \textbf{Depth-Proportional Resolution}
      \par
    }
  &
    \makecell{
      \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept-binder/binder/retention-policies/teeplots/guaranteed_depth_proportional_resolution=1+num_layers=1024+stratum_retention_predicate=depth-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
    \makecell{
      \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept-binder/binder/retention-policies/teeplots/guaranteed_depth_proportional_resolution=4+num_layers=1024+stratum_retention_predicate=depth-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
  \makecell[{{p{0.14\textwidth}}}]{
  \centering
    \bf{Space Complexity}\\
    $O(1)$\\
    \bf{MRCA Uncertainty}\\
    $O(n)$
  }
  \makecell[{{p{0.14\textwidth}}}]{
  \raggedright
    where $n$ is gens elapsed.
  }\\\hline
%-------------------------------------------------------------------------------
    \adjustbox{
      minipage=15em,
      rotate=90,
    }{
      \centering
      \textbf{Tapered Depth-Proportional Resolution}
      \par
    }
  &
    \makecell{
      \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept-binder/binder/retention-policies/teeplots/guaranteed_depth_proportional_resolution=1+num_layers=1024+stratum_retention_predicate=tapered-depth-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
    \makecell{
      \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept-binder/binder/retention-policies/teeplots/guaranteed_depth_proportional_resolution=4+num_layers=1024+stratum_retention_predicate=tapered-depth-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
  \makecell[{{p{0.14\textwidth}}}]{
  \centering
    \bf{Space Complexity}\\
    $O(1)$\\
    \bf{MRCA Uncertainty}\\
    $O(n)$
  }
  \makecell[{{p{0.14\textwidth}}}]{
  \raggedright
    where $n$ is gens elapsed.
  }\\\hline
%-------------------------------------------------------------------------------
  \adjustbox{
    minipage=15em,
    rotate=90,
  }{
    \centering
    \textbf{Recency-Proportional\\Resolution}
    \par
  }
  &
  \makecell{
    \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept-binder/binder/retention-policies/teeplots/guaranteed_mrca_recency_proportional_resolution=0+num_layers=1024+stratum_retention_predicate=recency-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
  }
  &
  \makecell{
    \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept-binder/binder/retention-policies/teeplots/guaranteed_mrca_recency_proportional_resolution=4+num_layers=1024+stratum_retention_predicate=recency-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
  }
  &
  \makecell[{{p{0.14\textwidth}}}]{
  \centering
  \bf{Space Complexity}\\
  $O(\log(n))$\\
  \bf{MRCA Uncertainty}\\
  $O(m)$
  }
  \makecell[{{p{0.14\textwidth}}}]{
  \raggedright
  where $m$ is gens since MRCA and $n$ is total gens elapsed.
  }\\


  \end{tabular}
  \caption{
  Comparison of stratum retention policies.
  Policy visualizations show retained strata in black.
  Time progresses along the $y$-axis from top to bottom.
  New strata are introduced along the diagonal and then ``drip'' downward as a vertical line until eliminated.
  The set of retained strata present within a column at a particular generation $g$ can be read as intersections of retained vertical lines with a horizontal line with intercept $g$.
  Policy visualizations are provided for two parameterizations for each policy: the first where the maximum uncertainty of MRCA generation estimates would be 512 generations and the second where the maximum uncertainty of MRCA generation estimates would be 128 generations.
  }
  \label{fig:retention-policies}
\end{figure*}


==> hereditary-stratigraph-concept/tex/lib/C.tex <==
\input{lib/preservebackslash.tex}

% adapted from https://tex.stackexchange.com/a/449117
\newcolumntype{C}[1]{>{\PreserveBackslash\centering}p{#1}}


==> hereditary-stratigraph-concept/tex/lib/L.tex <==
\input{lib/preservebackslash.tex}

% adapted from https://tex.stackexchange.com/a/449117
\newcolumntype{L}[1]{>{\PreserveBackslash\raggedright}p{#1}}


==> hereditary-stratigraph-concept/tex/lib/dependencies.tex <==
\usepackage{natbib,alifeconf}  %% The order is important

\usepackage[export]{adjustbox}
\usepackage{algorithmic}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{array}
\usepackage{bibunits}
\usepackage{booktabs}
\usepackage{caption}
\usepackage{cite}
\usepackage{colortbl}
\usepackage{csvsimple}
\usepackage{etoolbox}
\usepackage[T1]{fontenc} % adapted from https://tex.stackexchange.com/a/388208
\usepackage{graphicx}
\usepackage{hyperref,cleveref}
\usepackage{ifthen}
\usepackage{import}
\usepackage{listings}
\usepackage{longtable}
\usepackage{makecell}
\usepackage{makecmds}
\usepackage{multirow}
\usepackage{natbib}
\usepackage[section]{placeins}
\usepackage{pythonhighlight}
\usepackage{rotating}
\usepackage{setspace}
\usepackage{siunitx}
\usepackage{stringstrings}
\usepackage{subcaption}
\usepackage{tabularx}
\usepackage{textcomp}
\usepackage{vcell}
\usepackage{xcolor}
\usepackage{xfp}
\usepackage{xparse}
\usepackage{xstring}


==> hereditary-stratigraph-concept/tex/lib/dissertationelse.tex <==
% \pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\providecommand{\dissertationelse}[2]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION
#1
\else
#2
\fi
}


==> hereditary-stratigraph-concept/tex/lib/dissertationexclude.tex <==
% \pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\providecommand{\dissertationexclude}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION
\else
#1
\fi
}


==> hereditary-stratigraph-concept/tex/lib/dissertationonly.tex <==
% \pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\providecommand{\dissertationonly}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION%
#1%
\else%
\fi
}


==> hereditary-stratigraph-concept/tex/lib/importpath.tex <==
% \pragmaonce

% adapted from https://tex.stackexchange.com/a/17491
\makeatletter
  \providecommand\importpath{\import@path}
\makeatother


==> hereditary-stratigraph-concept/tex/lib/pragmaonce.tex <==
% pragma once, adapted from https://tex.stackexchange.com/a/195173
\makeatletter
\let\pragma@iinput=\@iinput
\def\@iinput#1{\xdef\@pragmafile{#1}\pragma@iinput{#1} }
\def\@pragmafile{default}
\def\pragmaonce{%
   \csname pragma@\@pragmafile\endcsname
   \global\expandafter\let \csname pragma@\@pragmafile\endcsname = \endinput
}
\makeatother


==> hereditary-stratigraph-concept/tex/lib/preservebackslash.tex <==
\providecommand{\PreserveBackslash}[1]{\let\temp=\\#1\let\\=\temp}


==> hereditary-stratigraph-concept/tex/lib/safepercent.tex <==
% \pragmaonce

% adapted from https://tex.stackexchange.com/a/351125
\catcode`\%=12
\providecommand\safepercent{%}
\catcode`\%=14


==> hereditary-stratigraph-concept/tex/lib/safetilde.tex <==
% \pragmaonce

% adapted from https://tex.stackexchange.com/a/425957
\providecommand\safetilde{\string~}


==> hereditary-stratigraph-concept/tex/lst/StratumRetentionCondemnerDepthProportionalResolution.tex <==
\input{lib/dissertationelse.tex}

\provideenvironment{lstinputlistinghandle}{}{}

{\makeatletter\if@twocolumn\onecolumn\fi\makeatother
\begin{lstinputlistinghandle}
\lstinputlisting[%
language=Python,
caption={
  Depth-proportional resolution policy condemner implementation.
},
label={lst:StratumRetentionCondemnerDepthProportionalResolution},
style=mypython,
basicstyle=\dissertationelse{\fontsize{9}{10}\selectfont}{\scriptsize},
]{submodules/hstrat/hstrat/hstrat/stratum_retention_condemners/StratumRetentionCondemnerDepthProportionalResolution.py}
\end{lstinputlistinghandle}
}


==> hereditary-stratigraph-concept/tex/lst/StratumRetentionCondemnerFixedResolution.tex <==
\provideenvironment{lstinputlistinghandle}{}{}

{\makeatletter\if@twocolumn\onecolumn\fi\makeatother
\begin{lstinputlistinghandle}
\lstinputlisting[%
language=Python,
caption={
  Fixed resolution policy condemner implementation.
},
label={lst:StratumRetentionCondemnerFixedResolution},
style=mypython,
basicstyle=\dissertationelse{\fontsize{9}{10}\selectfont}{\scriptsize},
]{submodules/hstrat/hstrat/hstrat/stratum_retention_condemners/StratumRetentionCondemnerFixedResolution.py}
\end{lstinputlistinghandle}
}


==> hereditary-stratigraph-concept/tex/lst/StratumRetentionCondemnerRecencyProportionalResolution.tex <==
\provideenvironment{lstinputlistinghandle}{}{}

{\makeatletter\if@twocolumn\onecolumn\fi\makeatother
\begin{lstinputlistinghandle}
\lstinputlisting[%
language=Python,
caption={
  MRCA-recency-proportional resolution policy condemner implementation.
},
label={lst:StratumRetentionCondemnerRecencyProportionalResolution},
style=mypython,
basicstyle=\dissertationelse{\fontsize{9}{10}\selectfont}{\scriptsize},
]{submodules/hstrat/hstrat/hstrat/stratum_retention_condemners/StratumRetentionCondemnerRecencyProportionalResolution.py}
\end{lstinputlistinghandle}
}


==> hereditary-stratigraph-concept/tex/lst/StratumRetentionCondemnerTaperedDepthProportionalResolution.tex <==
\provideenvironment{lstinputlistinghandle}{}{}

{\makeatletter\if@twocolumn\onecolumn\fi\makeatother
\begin{lstinputlistinghandle}
\lstinputlisting[%
language=Python,
caption={
  Tapered depth-proportional resolution policy condemner implementation.
},
label={lst:StratumRetentionCondemnerTaperedDepthProportionalResolution},
style=mypython,
basicstyle=\dissertationelse{\fontsize{9}{10}\selectfont}{\scriptsize},
]{submodules/hstrat/hstrat/hstrat/stratum_retention_condemners/StratumRetentionCondemnerTaperedDepthProportionalResolution.py}
\end{lstinputlistinghandle}
}


==> hereditary-stratigraph-concept/tex/lst/StratumRetentionPredicateDepthProportionalResolution.tex <==
\provideenvironment{lstinputlistinghandle}{}{}

{\makeatletter\if@twocolumn\onecolumn\fi\makeatother
\begin{lstinputlistinghandle}
\lstinputlisting[%
language=Python,
caption={
  Depth-proportional resolution policy predicate implementation, including method to calculate exact number of strata retained by generation and method to calculate stratum deposition rank from column index.
},
label={lst:StratumRetentionPredicateDepthProportionalResolution},
style=mypython,
basicstyle=\dissertationelse{\fontsize{9}{10}\selectfont}{\scriptsize},
]{submodules/hstrat/hstrat/hstrat/stratum_retention_predicates/StratumRetentionPredicateDepthProportionalResolution.py}
\end{lstinputlistinghandle}
}


==> hereditary-stratigraph-concept/tex/lst/StratumRetentionPredicateFixedResolution.tex <==
\provideenvironment{lstinputlistinghandle}{}{}

{\makeatletter\if@twocolumn\onecolumn\fi\makeatother
\begin{lstinputlistinghandle}
\lstinputlisting[%
language=Python,
caption={
  Fixed resolution policy predicate implementation, including method to calculate exact number of strata retained by generation and method to calculate stratum deposition rank from column index.
},
label={lst:StratumRetentionPredicateFixedResolution},
style=mypython,
basicstyle=\dissertationelse{\fontsize{9}{10}\selectfont}{\scriptsize},
]{submodules/hstrat/hstrat/hstrat/stratum_retention_predicates/StratumRetentionPredicateFixedResolution.py}
\end{lstinputlistinghandle}
}


==> hereditary-stratigraph-concept/tex/lst/StratumRetentionPredicateRecencyProportionalResolution.tex <==
\provideenvironment{lstinputlistinghandle}{}{}

{\makeatletter\if@twocolumn\onecolumn\fi\makeatother
\begin{lstinputlistinghandle}
\lstinputlisting[%
language=Python,
caption={
  MRCA-recency-proportional resolution policy predicate implementation, including method to calculate exact number of strata retained by generation and method to calculate stratum deposition rank from column index.
},
label={lst:StratumRetentionPredicateRecencyProportionalResolution},
style=mypython,
basicstyle=\dissertationelse{\fontsize{9}{10}\selectfont}{\scriptsize},
]{submodules/hstrat/hstrat/hstrat/stratum_retention_predicates/StratumRetentionPredicateRecencyProportionalResolution.py}
\end{lstinputlistinghandle}
}


==> hereditary-stratigraph-concept/tex/lst/StratumRetentionPredicateTaperedDepthProportionalResolution.tex <==
\provideenvironment{lstinputlistinghandle}{}{}

{\makeatletter\if@twocolumn\onecolumn\fi\makeatother
\begin{lstinputlistinghandle}
\lstinputlisting[%
language=Python,
caption={
  Tapered depth-proportional resolution policy predicate implementation, including method to calculate exact number of strata retained by generation and method to calculate stratum deposition rank from column index.
},
label={lst:StratumRetentionPredicateTaperedDepthProportionalResolution},
style=mypython,
basicstyle=\dissertationelse{\fontsize{9}{10}\selectfont}{\scriptsize},
]{submodules/hstrat/hstrat/hstrat/stratum_retention_predicates/StratumRetentionPredicateTaperedDepthProportionalResolution.py}
\end{lstinputlistinghandle}
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex-extended-abstract/lib/dependencies.tex <==
\usepackage[export]{adjustbox}
\usepackage{algorithmic}
\usepackage{amsmath,amsfonts}
\usepackage{array}
\usepackage{bibunits}
\usepackage{booktabs}
\usepackage{caption}
\usepackage{cite}
\usepackage{colortbl}
\usepackage{csvsimple}
\usepackage{etoolbox}
\usepackage{graphicx}
\usepackage{hyperref,cleveref}
\usepackage{ifthen}
\usepackage{import}
\usepackage{listings}
\usepackage{makecell}
\usepackage{multirow}
\usepackage{natbib}
\usepackage{pythonhighlight}
\usepackage{rotating}
\usepackage{siunitx}
\usepackage{stringstrings}
\usepackage{subcaption}
\usepackage{tabularx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{xfp}
\usepackage{xparse}
\usepackage{xstring}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex-extended-abstract/text/abstract.tex <==
\begin{abstract}
Phylogenetic analyses can also enable insight into evolutionary and ecological dynamics such as selection pressure and frequency dependent selection in digital evolution systems.
Traditionally, digital evolution systems have recorded data for phylogenetic analyses through perfect tracking where each birth event is recorded in a centralized data structures.
This approach, however, does not easily scale to distributed computing environments where evolutionary individuals may migrate between a large number of disjoint processing elements.
To provide for phylogenetic analyses in these environments, we propose an approach to infer phylogenies via heritable genetic annotations rather than directly track them.
We introduce a ``hereditary stratigraphy'' algorithm that enables efficient, accurate phylogenetic reconstruction with tunable, explicit trade-offs between annotation memory footprint and reconstruction accuracy.
This approach can estimate, for example, MRCA generation of two genomes within 10\% relative error with 95\% confidence up to a depth of a trillion generations with genome annotations smaller than a kilobyte.
We also simulate inference over known lineages, recovering up to 85.70\% of the information contained in the original tree using a 64-bit annotation.
\end{abstract}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex-extended-abstract/text/acknowledgement.tex <==
\section*{Acknowledgment}

This research was supported in part by NSF grants DEB-1655715 and DBI-0939454 as well as by Michigan State University through the computational resources provided by the Institute for Cyber-Enabled Research.
This material is based upon work supported by the National Science Foundation Graduate Research Fellowship under Grant No. DGE-1424871.
Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the National Science Foundation.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex-extended-abstract/text/body.tex <==
\input{text/body/introduction.tex}

\input{text/body/methods.tex}

\input{text/body/results-and-discussion.tex}

\input{text/body/conclusion.tex}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex-extended-abstract/text/body/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}

This and other methodology to enable decentralized observation and analysis of evolving systems will be essential for digital evolution experiments that use distributed and best-effort computing approaches.
Such methods will be crucial to enabling experimental analyses while preserving those systems' efficiency and scalability.
As parallel and distributed computing becomes increasingly ubiquitous and begins to more widely pervade digital evolution systems, hereditary stratigraphy should serve as a useful technique in this toolbox.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex-extended-abstract/text/body/introduction.tex <==
\section{Introduction} \label{sec:introduction}

In non-parallelized digital evolution experiments, phylogenetic trees can be tracked perfectly as they progress \citep{bohm2017mabe,wang2018vine,lalejini2019data} rather than reconstructed afterward, as must be done in most biological studies of evolution.
Such direct phylogenetic tracking enables a dizzying suite of experimental possibilities unique to digital evolution, such as perfect reconstruction of the sequence of phylogenetic states that led to a particular evolutionary outcome \citep{lenski2003evolutionary, dolson2020interpreting}.
% In a shared-memory context, it is not difficult to maintain a complete phylogeny where offspring simply track their parent (or vice versa).
% As simulations progress for longer durations, memory usage will typically grow at least linearly if population sizes are fixed, or worse if populations are growing or organisms are becoming more complex.
% These problems are easily ameliorated, however, by performing garbage collection on extinct lineages and saving older history to disk \citep{bohm2017mabe,dolson2019modes}.

Phylogenetic tracking in a distributed context, where linages may traverse many machines, introduces implementation complexity and more significant runtime overhead cost.
% However, if sufficient memory or disk space can be afforded to log all reproduction events, recording a perfect phylogeny in a distributed context is still not especially difficult.
% Processes could maintain records of each reproduction event, storing the parent organism (and its associated process) with all generated offspring (and their destination processes).
% As long as no data goes missing and organisms are uniquely identified globally, these ``dangling ends'' could be joined in postprocessing to weave a continuous global phylogeny.
% Of course, for the huge population sizes made possible by distirbuted systems, such stitching may become a demanding task in and of itself.
%
% However, if memory and disk space are limited, distributed phylogeny tracking becomes a more burdonsome challenge.
% A naive approach might employ a server model to maintain a central store of phylogenetic data.
% Processes would dispatch notifications of birth and death events to the server, which would curate (and gabage collect) phylogenetic history much the same as current serial phylogenetic tracking implementations.
% Unfortunately, this server model approach would present profound scalability challenges: communication and computation burden on the server process would worsen in direct proportion to processor count, and processes would frequently need to pause while waiting for confirmation that a reproduction event was successfully reported.
% ELD: This is making me wonder if there's a middle ground that could be explored in the future where we could use a sort of UDP phylogeny protocol, where no confirmation occurs
An ideally scalable approach would record birth and death events only on the process(es) where they unfold.
% Even this localized technique would lead to serious performance challenges, however.
% Lineages that went extinct locally could not be safely garbage collected until the extinction of thair offspring's lineages on other processors could be confirmed.
% Thus, garbage collection would require extinction notifications to wind back across processes each lineage had traversed.

% Under a best-effort model, no system of phylogeny tracking can guarantee proper garbage collection.
% For example, it would be possible for an offspring that was dispatched to a neighboring process to have failed to arrive, and both processes would need to keep going, despite the failure.
% So, extinction notifications for the lineage founded by that offspring would never be dispatched --- putting in motion a memory leak of un-garbage-collectible phylogenetic history.
% The situation becomes even more leaky when the possibility of extinction notifications themselves being lost.

In a distributed context --- especially, a distributed, best-effort context --- phylogenetic reconstruction (as opposed to tracking) could prove simpler and more efficient at runtime while providing sufficient power to address experimental questions of interest.
However, phylogenetic reconstruction from genomes with a traditional model of divergence under grandual accumulation of random mutations poses its own difficulties \citep{lack2010identifying,casci2008lining,hagstrom2004using,kapli2020phylogenetic,sarkar2010hardware}.

% The computational flexibility of digital evolution experiments provides a unique opportunity to overcome these challenges: designing heritable genome annotations specifically to simplify and strengthen phylogenetic reconstruction efforts.
% For maximum applicability of such a solution, these annotations should be phenotypically neutral heritable instrumentation \citep{stanley2002evolving} that do not affect any encodings for functional genome content.

This work introduces ``hereditary stratigraphy,'' a novel heritable genome annotation system to facilitate post-hoc phylogenetic inference on asexual populations.
This system allows explicit control over trade-offs between space complexity and accuracy of phylogenetic inference.
Instead of modeling genome components undergoing neutral variation through a mutational process, we keep a record of historical checkpoints that allow comparison of two lineages to identify the range of time in which they diverged.

% In Section \ref{sec:methods} we motivate and explain the hereditary stratigraphy approach.
% Then, in Section \ref{sec:results} we simulate post-hoc inference on known phylogenies to assess the quality of phylogenetic reconstruction enabled by the hereditary stratigraphy method.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex-extended-abstract/text/body/methods.tex <==
\section{Methods} \label{sec:methods}

\input{fig/column-comparison.tex}

Our algorithm, particularly the vocabulary we developed to describe it, draws on the concept of geological stratigraphy, inference of natural history through analysis of successive layers of geological material \citep{steno1916prodromus}.
As an introductory intuition, suppose a body of rock being built up through regular, discrete events depositing of geological material.
Note that in such a scenario we could easily infer the age of the body of rock by counting up the number of layers present.
% Note that it is crucial to this scenario that each layer has some differentiating feature that allows it to be distinguished from layers above and below it, but also potentially from layers present in another body of rock in a distant and unrelated geographic position.
Next, imagine making a copy of the rock body in its partially-formed state and then moving it far away.
As time runs forward on these two rock bodies, independent layering processes will cause consistent disparity in the layers forming on each forwards from their point of separation.

To deduce the historical relationship of these rock bodies after the fact, we could simply align and compare their layers.
Layers from their base up through the first disparity would correspond to shared ancestry; further disparate layers would correspond to diverged ancestry.
% Interestingly, and powerfully for phylogenetic inference, we can readily distinguish a scenario where both rock bodies deposited ten layers after diverging from a scenario where one deposited eighteen layers and the other deposited two.
Figure \ref{fig:column-comparison} depicts the process of comparing columns for phylogenetic inference.

Shifting now from intuition to implementation, a fixed-length randomly-generated binary tag provides a convenient and efficient mechanism to differentiate between our metaphorical ``layers.''
% We call this ``fingerprint'' tag a \textit{differentia}.
% The width of this tag controls the probability of spurious collisions between independently generated instances.
% At 64 bits wide the tag essentially functions as a UID: collisions between randomly generated tags are so unlikely ($p < 5.42\times10^{-20}$) they can essentially be ignored.
% At the other end of the spectrum, collision probability would be $1/256$ for a single byte and $1/2$ for a single bit.
% In the case of narrow differentia, in order to set a lower bound for the MRCA generation, you would have to backtrack common strata from the last commonality until the probability of that many successive spurious collisions was enough to satisfy your desired confidence level (e.g., 95\% confidence).
% Even then, there would be a possibility of the the true MRCA falling before the lower bound.
% Note, however, that no matter the width of the differentia the generation of the first discrepancy provides a hard upper bound on the generation of the MRCA.
%
In accordance with our geological analogy, we refer to the packet of data accumulated each generation as a \textit{stratum}.
This packet contains the differentia and, although not employed in this work, could hold other arbitrary user-defined data (i.e., simulation timestamp, phenotype characteristics, etc.).
% Again in accordance with the geological analogy, we refer to the chronological stack of strata that accumulate over successive depositions as a \textit{hereditary stratigraphic column}.

% \subsection{Stratum Retention Policy}

% \input{fig/deposit-process.tex}

As currently stated, fingerprints will accumulate proportionally to the length of evolutionary history simulated.
In an evolutionary run with thousands or millions of generations, this approach would soon become intractable --- particularly when columns are serialized and transmitted between distributed computing elements.
To solve this problem, we can trade off precision for compactness by deleting strata from columns as time progresses.
% Figure \ref{fig:deposit-process} overviews how stratum deposit and stratum elimination progress over two generations under the hereditary stratigraphic column scheme.
%
% Different patterns of deletion will lead to different trade-offs, both in terms of the scaling relationship of column size to generations elapsed and in terms of the arrangement of precision over evolutionary history (i.e., focusing precision on more recent evolutionary history versus spreading it evenly over the entire history).
%
We refer to the rule set used to selectively eliminate strata over time as the ``stratum retention policy.''
We devised three stratum retention policies, which provide
\begin{itemize}
  \item linear space complexity and constant inference error,
  \item constant space complexity and linear inference error with respect to phylogenetic depth, or
  \item logarithmic space complexity and inference error as a constant proportion of time elapsed since MRCA.
\end{itemize}

% We explore several different retention policy designs here, and implement our software to allows for free, modular interchange of retention policies.
% It is possible to define a policy through either of two mechanisms.
% First, policy can be defined as a ``predicate'' where the generation of a stratum and the current number of strata deposited is passed into a function that returns whether that strata should be retained at that point in time.
% Second, policy can be defined as a ``condemner'' generator where, given the current number of strata deposited, the set of ranks that should be deleted at this point in time are yielded.
% Although the predicate form is useful for analyzing and proving properties of policies, the condemner form is generally more efficient in practice.
% We provide predicate and condemner implementations for each stratum retention policy discussed here.

% It should be noted that condemners and predicates are both defined in terms of stratum generation, not stratum index among retained strata in the column.
% Therefore, it may seem necessary to store the generation of deposit within the stratum data structure.
% However, if you know the total number of generations deposited you can map backwards from index to recover the generation deposited without storing it.
% We provide this formula for each stratum retention policy.
% Finally, for each policy we provide a formula to calculate the exact number of strata retained under any parameterization after $n$ generations.
%
% In the next subsections, we introduce several stratum retention policies, provide the intuition behind their implementation, and elaborate their space complexity and resolution properties.
% For each policy, patterns of stratum retention are illustrated in Figure \ref{fig:retention-policies}.
% The formulas for number of strata retained after $n$ generations, the formulas to calculate stratum deposit generation from column index, and the retention predicate specifications of each policy are available in Supplementary Listing \ref{lst:StratumRetentionPredicateDepthProportionalResolution} \citep{moreno2022hstratconceptsupplement}.
% The condemner generator specification of each policy is available in Supplementary Listing \ref{lst:StratumRetentionCondemnerDepthProportionalResolution} \citep{moreno2022hstratconceptsupplement}.
% For tapered depth-proportional resolution and recency-proportional resolution, the accuracy of MRCA estimation can also be explored via an interactive in-browser web applet at \url{https://hopth.ru/bi}.
%
% \input{fig/retention-policies.tex}
%
% \subsection{Fixed Resolution Stratum Retention Policy}
%
% The fixed resolution retention policy provides a fixed absolute upper bound $r$ on the spacing between retained strata.
% The strategy to obtain this property is simple: permanently retain a stratum every $r$th generation
% (although, for arbitrary reasons of implementation convenience we require each stratum to be retained during at least the generation it is deposited).
%
% However, this retention policy suffers from linear growth in a column's memory footprint with respect to number of generations elapsed: every $r$th generation generation a new stratum is permanently retained
% For this reason, it is likely not useful in practice except potentially in scenarios where the number of generations is fixed in advance.
% We include it here largely for illustrative purposes as a gentle introduction to retention policies.
%
% \subsection{Depth-Proportional Resolution Stratum Retention Policy}
%
% The depth-proportional resolution policy ensures spacing between retained strata will be less than or equal to a proportion $r$ of total number of strata deposited.
% Achieving this limit on uncertainty requires retaining sufficient strata so that no more than $r$ ranks elapsed between any two strata.
% This policy accumulates retained strata at a fixed interval until twice as many as $r$ are at hand.
% Then, every other retained stratum is purged and the cycle repeats with a new twice-as-wide interval between retained strata.
%
% When comparing stratigraphic columns from different generations, the resolution guarantee holds in terms of the number of generations experienced by the older of the two columns.
% Because this retention policy is deterministic, for two columns with the same policy, every stratum that is held by the older column is also guaranteed to be present in the younger column (unless it hasn't yet been deposited on the younger column).
% Therefore, the strata that would enable the desired resolution when comparing two columns of the same age are guaranteed to be available.
%
% Because the number of strata retained under this policy is bounded as $2n+1$, space complexity scales as $O(1)$ with respect to the number of strata deposited.
% It follows that the MRCA rank estimate uncertainty scales as $O(n)$ with respect to the number of strata deposited.
%
% \subsection{Tapered Depth-Proportional Resolution Stratum Retention Policy}
%
% This policy refines the depth-proportional resolution policy to provide a more stable column memory footprint over time.
% The naive depth-proportional resolution policy builds up strata until twice as many are present as needed then purges half of them all at once.
% The tapered depth-proportional resolution policy functions identically to the depth-proportional policy except that it removes unnecessary strata gradually from back to front as new strata are deposited, instead of eliminating them simultaneously.
% The column footprint stability of this variation makes it easier to parameterize our experiments to ensure comparable end-state column footprints for fair comparison between retention policies, in addition to making this policy likely better suited to most use cases.
% By design, this policy has the same space complexity and MRCA estimation uncertainty scaling relationships with number generations elapsed as the naive depth-proporitonal resolution policy.
%
% \subsection{MRCA-Recency-Proportional Resolution Stratum Retention Policy}
%
% \input{tab/recency-proportional-space-complexity.tex}
%
% The MRCA-recency-proportional resolution policy ensures distance between the retained strata surrounding any generation point will be less than or equal to a user-specified proportion $r$ of the number of generations elapsed since.
%
% This policy can be constructed recursively, so to begin, let's consider setting up just the \textit{first} generation $g$ of the stratum after the root ancestor we will retain when $n$ generations have elapsed.
% A simple geometric analysis reveals that providing the guaranteed resolution for the worst-case generation within the window between generation 0 and generation $g$ (i.e., generation $g-1$) requires
% \begin{align*}
%   g \leq \lfloor n / (r + 1) \rfloor.
% \end{align*}
%
% We now have an upper bound for the rank of the first stratum generation we must retain.
% However, we must guarantee that these ranks are actually available for us to retain (i.e., it hasn't been purged out of the column at a previous time point as the column was grown by successive deposition).
% We will do this by picking the rank that is the highest power of 2 less than or equal to our bound.
% If we repeat this procedure as we recurse, we are guaranteed that this rank will have been preserved across all previous timepoints.
%
% Why does this work?
% Consider a sequence where all elements are powers of 2 and elements in the sequence are strictly nonincreasing.
% Consider the first element of the list.
% Partial sums along the sequence will include all multiples this first element.
% So, when we ratchet up $g$ to $2g$ as $n$ increases, we are guaranteed that $2g$ has been retained.
% This principle generalizes recursively down the list.
% This is a similar principle to the approach of strictly-doubling interval sizes used in the Naive and Tapered Depth-Proportional Resolution stratum retention policies described above.
%
% This step of truncating to the nearest less than or equal to power of 2 affects our recursive step size at most only by a constant factor of 2.
% So, because step size is a constant fraction of remaining generations $n$ (at worst $\frac{1}{2(r+1)}$), the number of steps made (and number of strata retained) scales as $O(\log(n))$ with respect to the number of strata deposited.
% Table \ref{tab:recency-proportional-space-complexity} provides exact figures for the number of strata retained under different parameterizations of the recency-proportional retention policy between one thousand and one trillion generations.
%
% As for rank estimate uncertainty, in the worst case it scales as $O(n)$ with respect to the greater number of strata deposited.
% However, with respect to estimating the rank of the MRCA when lineages diverged any fixed number of generations ago, uncertainty scales as $O(1)$.
%
% How does space complexity scale with respect to the policy's specified resolution $r$?
% Through extrapolation from OEIS sequences A063787 and A056791 via guess and check \citep{sloane2021a063787,sloane2021a056791}, we posited the exact number of strata retained after $n$ generations as
%
% \begin{align*}
%   \mathrm{HammingWeight}(n)
%   + \sum_1^r \lfloor \log_2( \lfloor n / r \rfloor ) \rfloor
%   + 1.
% \end{align*}
%
% This expression has been unit tested extensively to ensure perfect reliability.
% Approximating and applying logarithmic properties, this policy's space complexity can be calculated within a constant factor as
%
% \begin{align*}
% \log(n) + \log\Big(\frac{n^r}{r!}\Big).
% \end{align*}
%
% To answer our question, we will examine the ratio of space complexities required when scaling resolution $r$ up by a constant factor $f > 1$.
% Evaluating this ratio as $r \to \infty$, we find that space complexity scales directly proportional with the desired resolution $r$ at the limit,
%
% \begin{align*}
% \lim_{r \to \infty}
% \frac{
%   \log(n) + \log\Big(\frac{n^{fr}}{(fr)!}\Big)
% }{
%   \log(n) + \log\Big(\frac{n^r}{r!}\Big)
% }
% = f.
% \end{align*}
%
% Evaluating this ratio as $n \to \infty$, we find that this scaling relationship is never worse than directly proportional for any $r$,
%
% \begin{align*}
% \lim_{n \to \infty}
% \frac{
%   \log(n) + \log\Big(\frac{n^{fr}}{(fr)!}\Big)
% }{
%   \log(n) + \log\Big(\frac{n^r}{r!}\Big)
% }
% &= \frac{fr+1}{r+1}\\
% &= f\frac{r + 1/f}{r + 1}\\
% &\leq f.
% \end{align*}
%
%
% \subsection{Computational Experiments}
%
% These simulations propagated populations of between 100 and 165 bitstrings between 500 and 5,000 synchronous generations under the NK fitness landscape model \citep{kauffman1989nk}.
% In order to ensure coverage of a variety of phylogenetic conditions, we sampled a variety of selection schemes that impose profoundly different ecological regimens \citep{dolson2018ecological},
% \begin{itemize}
%   \item EcoEA Selection \citep{goings2012ecology},
%   \item Lexicase Selection \citep{helmuth2014solving},
%   \item Random Selection,
%   \item Sharing Selection \citep{goldberg1987genetic}
%   % \item Tournament Selection \citep{miller1995genetic}.
% \end{itemize}
%
% Supplementary Table \ref{tab:ground-truth-phylogenies} provides full details on the conditions each ground truth phylogeny was drawn from.
% The phylogenies themselves are available in our data repository for this project.
%
% For each ground truth phylogeny, we tested combinations of three configuration parameters:
% \begin{itemize}
%   \item target end-state memory footprints for extant columns (64, 512, and 4096 bits),
%   \item differentia width (1, 8, and 64 bits), and
%   \item stratum retention policy (tapered depth-proportional resolution and recency-proportional resolution).
% \end{itemize}
%
% Stratum retention policies were parameterized so that the maximum number of strata possible were present at the end of the experiment without exceeding the target memory footprint.
% If the target memory footprint is exceeded by the sparsest possible parameterization of a retention policy, then that sparsest possible parameterization is used.
% Supplementary Tables \cref{tab:experiment-column-sizes-nk-ecoea-selection,tab:experiment-column-sizes-nk-lexicase-selection,tab:experiment-column-sizes-nk-random-selection,tab:experiment-column-sizes-nk-sharing-selection,tab:experiment-column-sizes-nk-tournament-selection} provide the calculated paramaterizations and memory footprints of extant columns \citep{moreno2022hstratconceptsupplement}.
%
% In order to assess the viability of phylogenetic inference using hereditary stratigraphic columns from extant organisms, we used the end-state stratigraphs to estimate a reconstruction of the actual ground truth phylogenetic histories.
% The first step to reconstructing a phylogenetic tree for the history of an extant population at the end of an experiment is to construct a distance matrix by calculating all pairwise phylogenetic distances between extant columns.
% We defined phylogenetic distance between two extant columns as the sum of each extant organism's generational distance back to the generation of their MRCA, estimated as the mean of the upper and lower 95\% confidence bounds.
% Supplementary Figure \ref{fig:phylogenetic-inference} provides a cartoon summary of the process of calculating phylogenetic distance between two extant columns \citep{moreno2022hstratconceptsupplement}.
%
% We then used the unweighted pair group method with arithmetic mean (UPGMA) reconstruction tool provided by the BioPython package to generate estimate phylogenetic trees \citep{cock2009biopython,sokal1958statistical}.
% After generating the reconstructed tree topology, we performed a second pass to adjust branch lengths so that each tree node sat at the mean of its estimated 95\% confidence generation bounds.
% %We found that the neighbor joining (NJ) approach occasionally yielded reconstructions with impossible ``negative generation'' branches \citep{saitou1987neighbor} after knowledge bounding the absolute generation of internal nodes (i.e., MRCA's between pairs of extant organisms) was applied, so we did not use it.
%
% \subsection{Software and Data}
%
% % A prototype of this approach has been implemented \url{https://github.com/mmore500/dishtiny/blob/incoming/include/dish2/genome/PhyloFingerprints.hpp} and preliminarily tested \url{https://github.com/mmore500/dishtiny/blob/incoming/tests/dish2/genome/PhyloFingerprints.cpp}.
%
% As part of this work, we published the \texttt{hstrat} Python library with a stable public-facing API intended to enable incorporation in other projects with extensive documentation and unit testing on GitHub at \url{https://anonymous.4open.science/r/hstrat-115D/} and on PyPI.% at \url{https://pypi.org/project/hstrat/}. https://github.com/mmore500/hstrat
% In the near future, we intend to complete and publish a corresponding C++ library.
%
% Supporting software materials can be found on GitHub at \url{https://anonymous.4open.science/r/hereditary-stratigraph-concept-6BEC/}.%\url{https://github.com/mmore500/hereditary-stratigraph-concept}
% Supporting computational notebooks are available for in-browser use via BinderHub at \url{ANONYMIZED FOR PEER REVIEW} \citep{ragan2018binder}. %https://mybinder.org/v2/gh/mmore500/hereditary-stratigraph-concept/HEAD?labpath=binder%2F
% Our work benefited from many pieces of open source scientific software, including \citep{sukumaran2010dendropy,virtanen2020scipy,hunter2007matplotlib,virtanen2020scipy,waskom2021seaborn,bostock2011d3,meurer2017sympy,smith2020treedistdata,paradis2004ape,ushey2022reticulate,wickham2022dplyr}.
% The ground truth phylogenies used in this work as well as supplementary figures, tables, and text are available via the Open Science Framework at
% \url{https://osf.io/4sm72/?view\_only=69f37c6d184143b7855299c3323749ea} \citep{foster2017open,moreno2022hstratconceptsupplement}.
% Phylogenetic data associated with this project is stored in the Alife Community Data Standards format \citep{lalejini2019data}.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex-extended-abstract/text/body/results-and-discussion.tex <==
\section{Results} \label{sec:results}

In order to assess the practical performance of the hereditary stratigraph approach in an applied setting, we simulated the process of stratigraph propagation over known ``ground truth'' phylogenies extracted from pre-existing digital evolution simulations \citep{hernandez2022phylogenetic}.
Across ground truth phylogenies, we were able to reconstruct the phylogenetic topology with between 47.75\% and 85.70\% of the information contained in the original tree using a 64-bit column memory footprint, between 47.75\% and 80.36\% using a 512-bit column memory footprint, and between 51.13\% and 83.53\% using a 4096-bit column memory footprint.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex-extended-abstract/text/frontmatter.tex <==
\title{ Hereditary Stratigraphy: Genome Annotations to Enable Phylogenetic Inference over Distributed Populations }

%%
%% The "author" command and its associated commands are used to define
%% the authors and their affiliations.
%% Of note is the shared affiliation of the first two authors, and the
%% "authornote" and "authornotemark" commands
%% used to denote shared contribution to the research.
\author{Matthew Andres Moreno}
\orcid{0000-0003-4726-4479}
\affiliation{%
  \institution{Michigan Statue University}
  \city{East Lansing}
  \state{Michigan}
  \country{USA}
  \postcode{48103}
}

\author{Emily Dolson}
% \email{dolsonem@msu.edu}
\orcid{0000-0001-8616-4898}
\affiliation{%
  \institution{Michigan Statue University}
  \city{East Lansing}
  \state{Michigan}
  \country{USA}
  \postcode{48103}
}

\author{Charles Ofria}
% \email{ofria@msu.edu}
\orcid{0000-0003-2924-1732}
\affiliation{%
  \institution{Michigan Statue University}
  \city{East Lansing}
  \state{Michigan}
  \country{USA}
  \postcode{48103}
}


%%
%% By default, the full list of authors will be used in the page
%% headers. Often, this list is too long, and will overlap
%% other information printed in the page headers. This command allows
%% the author to define a more concise list
%% of authors' names for this purpose.
\renewcommand{\shortauthors}{Moreno et al.}

\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10010147.10010341.10010366.10010369</concept_id>
       <concept_desc>Computing methodologies~Simulation tools</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10010147.10010257.10010293.10011809.10011812</concept_id>
       <concept_desc>Computing methodologies~Genetic algorithms</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Computing methodologies~Simulation tools}
\ccsdesc[500]{Computing methodologies~Genetic algorithms}

\keywords{phylogenetics, decentralized algorithms, digital evolution, genetic algorithms, genetic programming}

\input{text/abstract.tex}

\maketitle


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex-extended-abstract/text/references.tex <==
% \section*{References}

\putbib


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/draft.tex <==
\def\mydraft{
\usepackage{draftwatermark}
\usepackage{lineno}
\linenumbers
\renewcommand{\linenumberfont}{\normalfont\small\color{red}}
}
\input{main.tex}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/fig/cid_plot.tex <==
\begin{figure}
    \includegraphics[width=\columnwidth]{img/cid_plot}
    \caption{
    Reconstruction error for phylogenetic inference with ground truth sharing selection phylogeny.
    Lower is better.
    RPR is recency-proportional resolution policy and TDPR is tapered depth-proportional resolution policy.
    }
  \label{fig:cid_plot}
\end{figure}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/fig/column-comparison.tex <==
\begin{figure}
    \includegraphics[width=\columnwidth]{img/column-comparison}
    \caption{
    Inferring the generation of the most-recent common ancestor (MRCA) of two hereditary stratigraphic columns ``$A$'' and ``$B$''.
    Columns are aligned at corresponding generations.
    Then the first generation with disparate ``fingerprints'' is determined.
    % (If a particular generation's strata have been eliminated from one or both columns or have not yet been deposited on one column, then no comparison is performed at that generation.)
    This provides a hard upper bound on the generation of the MRCA: these strata \textit{must} have been deposited along separate lines of descent.
    Searching backward for the first commonality preceding that disparity provides a soft lower bound on the generation of the MRCA: these strata evidence common ancestry but \textit{might} collide by chance.
    Some strata mmay have been eliminated from the columns, as shown, in order to save space at the cost of increasing uncertainty of MRCA generation estimates.
    % (If a narrow ``fingerprint'' differentia like a single bit is used with plausible collision probability, a lower bound can be established by continuing to search backward until the probability of $k$ successive spurious collisions is sufficiently unlikely.)
    % This process yields certainty about the phylogenetic relationship between $A$ and $B$ shown at right above (i.e., common) and below (i.e., diverged) the MRCA bounds.
    }
  \label{fig:column-comparison}
\end{figure}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/fig/deposit-process.tex <==
\input{lib/dissertationexclude.tex}
\begin{figure*}
  \dissertationexclude{\begin{minipage}{0.6\textwidth}}
    \includegraphics[width=\textwidth]{img/deposit-process}
  \dissertationexclude{\end{minipage}}%
  \dissertationexclude{\begin{minipage}{0.4\textwidth}}
    \caption{
    Cartoon illustration of stratum deposit process.
    This process marks the elapse of a generation when a hereditary stratigraphic column is inherited by an offspring.
    First, a new stratum is appended to the end of the column with a randomly-generated ``fingerprint.''
    This ``fingerprint'' distinguishes strata that were generated along disparate lines of descent (e.g., \texttt{0xd01a} for 3rd Generation A and \texttt{0xe74a} for 3rd generation B).
    Then, the column's configured stratum retention policy is applied to ``prune'' the column by eliminating strata from specific generations.
    Although this cartoon depicts an empty space for eliminated strata, the underlying data structure behind a column (i.e., the pink overlay) can condense to reduce space complexity.
    }\label{fig:deposit-process}
  \dissertationexclude{\end{minipage}}
\end{figure*}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/fig/diffbits-clustering-information-distance.tex <==
\begin{sidewaysfigure}
  \includegraphics[width=\linewidth]{submodules/hereditary-stratigraph-concept-binder/binder/reconstruction-quality/teeplots/col=condition+hue=num-differentia-bits+kind=bar+row=policy+tree-comparison-metric=clustering-information-distance+viz=catplot+x=num-column-bits+y=score+ext=}
  \caption{
  Comparison of phylogenetic reconstruction quality across differentia bit counts.
  Reconstruction quality measured as clustering information distance between reconstructed phylogeny and ground truth phylogeny \citep{smith2020information, smith2020treedist}.
  Lower is better.
  RPR is recency-proportional resolution stratum retention policy and TDPR is tapered depth-proportional resolution stratum retention policy.
  }
  \label{fig:diffbits-clustering-information-distance}
\end{sidewaysfigure}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/fig/diffbits-mutual-clustering-information.tex <==
\begin{sidewaysfigure}
  \includegraphics[width=\linewidth]{submodules/hereditary-stratigraph-concept-binder/binder/reconstruction-quality/teeplots/col=condition+hue=num-differentia-bits+kind=bar+row=policy+tree-comparison-metric=mutual-clustering-information+viz=catplot+x=num-column-bits+y=score+ext=}
  \caption{
  Comparison of phylogenetic reconstruction quality across differentia bit counts.
  Reconstruction quality measured as mutual clustering information between reconstructed phylogeny and ground truth phylogeny \citep{smith2020information, smith2020treedist}.
  Higher is better.
  RPR is recency-proportional resolution stratum retention policy and TDPR is tapered depth-proportional resolution stratum retention policy.
  }
  \label{fig:diffbits-mutual-clustering-information}
\end{sidewaysfigure}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/fig/diffbits-robinson-foulds-similarity.tex <==
\begin{sidewaysfigure}
  \includegraphics[width=\linewidth]{submodules/hereditary-stratigraph-concept-binder/binder/reconstruction-quality/teeplots/col=condition+hue=num-differentia-bits+kind=bar+row=policy+tree-comparison-metric=generalized-robinson-foulds-similarity+viz=catplot+x=num-column-bits+y=score+ext=}
  \caption{
  Comparison of phylogenetic reconstruction quality across differentia bit counts.
  Reconstruction quality measured as generalized Robinson-Foulds similarity between reconstructed phylogeny and ground truth phylogeny \citep{smith2020information, smith2020treedist}.
  Higher is better.
  RPR is recency-proportional resolution stratum retention policy and TDPR is tapered depth-proportional resolution stratum retention policy.
  }
  \label{fig:diffbits-robinson-foulds-similarity}
\end{sidewaysfigure}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/fig/info_plot.tex <==
\begin{figure}
    \includegraphics[width=\columnwidth]{img/info_plot}
    \caption{
    Proportion of information present in the ground-truth ftness sharing phylogeny that was captureed by our reconstruction, across various retention policies.
    High is better (1 is perfect).
    RPR is recency-proportional resolution policy and TDPR is tapered depth-proportional resolution policy.
    } \label{fig:info_plot}
\end{figure}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/fig/phylogenetic-inference.tex <==
\begin{figure*}
  \centering
    \includegraphics[width=\textwidth]{img/phylogenetic-inference}
    \caption{
    Cartoon illustration of column inheritance along a phylogenetic tree and the process to infer phylogenetic history along extant columns.
    This scenario supposes a stratum retention policy where only strata from even generations are retained.
    The common ancestor of the focal clade, which is at generation 2, is shown at top.
    Generation 3 columns inherit that ancestor's strata and each append a new stratum.
    Generation 4 columns append another new stratum then eliminate their generation 3 strata.
    Finally, another generation elapses to yield generation 5 strata.
    Suppose that only generation 5 strata are extant.
    So, greyed-out columns above are not directly observable.
    Phylogenetic history is deduced by pairwise comparison between extant columns.
    For each pair (like the example highlighted in red) a phylogenetic distance can be computed as the sum generations elapsed to each extant column after the estimated generation of their MRCA.
    These pairwise distances can then be fed into a phylogeny reconstruction algorithm.
    }
  \label{fig:phylogenetic-inference}
\end{figure*}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/fig/policy-clustering-information-distance.tex <==
\begin{figure*}
    \includegraphics[width=\linewidth]{submodules/hereditary-stratigraph-concept-binder/binder/reconstruction-quality/teeplots/col=num-differentia-bits+hue=policy+kind=bar+row=num-column-bits+tree-comparison-metric=clustering-information-distance+viz=catplot+x=condition+y=score+ext=}
    \caption{
    Comparison of phylogenetic reconstruction quality between stratum retention policies.
    Reconstruction quality measured as clustering information distance between reconstructed phylogeny and ground truth phylogeny \citep{smith2020information, smith2020treedist}.
    Lower is better.
    RPR is recency-proportional resolution stratum retention policy and TDPR is tapered depth-proportional resolution stratum retention policy.
    }
    \label{fig:policy-clustering-information-distance}
\end{figure*}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/fig/policy-mutual-clustering-information.tex <==
\begin{figure*}
    \includegraphics[width=\linewidth]{submodules/hereditary-stratigraph-concept-binder/binder/reconstruction-quality/teeplots/col=num-differentia-bits+hue=policy+kind=bar+row=num-column-bits+tree-comparison-metric=mutual-clustering-information+viz=catplot+x=condition+y=score+ext=}
    \caption{
    Comparison of phylogenetic reconstruction quality between stratum retention policies.
    Reconstruction quality measured as mutual clustering information between reconstructed phylogeny and ground truth phylogeny \citep{smith2020information, smith2020treedist}.
    Higher is better.
    RPR is recency-proportional resolution stratum retention policy and TDPR is tapered depth-proportional resolution stratum retention policy.
    }
    \label{fig:policy-mutual-clustering-information}
\end{figure*}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/fig/policy-robinson-foulds-similarity.tex <==
\begin{figure*}
    \includegraphics[width=\linewidth]{submodules/hereditary-stratigraph-concept-binder/binder/reconstruction-quality/teeplots/col=num-differentia-bits+hue=policy+kind=bar+row=num-column-bits+tree-comparison-metric=generalized-robinson-foulds-similarity+viz=catplot+x=condition+y=score+ext=}
    \caption{
    Comparison of phylogenetic reconstruction quality between stratum retention policies.
    Reconstruction quality measured as generalized Robinson-Foulds similarity between reconstructed phylogeny and ground truth phylogeny \citep{smith2020information, smith2020treedist}.
    Higher is better.
    RPR is recency-proportional resolution stratum retention policy and TDPR is tapered depth-proportional resolution stratum retention policy.    }
    \label{fig:policy-robinson-foulds-similarity}
\end{figure*}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/fig/reconstruction-example.tex <==
\input{lib/importpath.tex}

\begin{figure*}%
%-------------------------------------------------------------------------------
  \begin{subfigure}[t]{0.32\linewidth}
    \centering
    % pass an arbitrary filename, potentially with unsafe characters
    % adapted from https://tex.stackexchange.com/a/36178
    \catcode`\%=12
    \providecommand\filename{}
    \renewcommand\filename{\detokenize{submodules/hereditary-stratigraph-concept-binder/binder/phylogenetic-inference/teeplots/a=true_phylogeny+source=a%reconstructed_phylogenies~source%nk_lexicaseselection_seed110_pop165_mut.01_snapshot_500.csv.gz+viz=truncate-phylo+ext=}}
    \catcode`\%=14
    \includegraphics[width=\linewidth]{\importpath\filename}
    \caption{Ground truth phylogeny.}
    \label{fig:reconstruction-example-true-phylogeny}
  \end{subfigure}%
  \hfill%
%-------------------------------------------------------------------------------
  \begin{subfigure}[t]{0.32\linewidth}
    \centering
    % pass an arbitrary filename, potentially with unsafe characters
    % adapted from https://tex.stackexchange.com/a/36178
    \catcode`\%=12
    \providecommand\filename{}
    \renewcommand\filename{\detokenize{submodules/hereditary-stratigraph-concept-binder/binder/phylogenetic-inference/teeplots/source=a%reconstructed_phylogenies~source%nk_lexicaseselection_seed110_pop165_mut.01_snapshot_500.csv.gz+treatment=differentia%1~policy%TaperedDepthProportionalResolution~target%64+viz=truncate-phylo-bounds+ext=}}
    \catcode`\%=14
    \includegraphics[width=\linewidth]{\importpath\filename}
    \caption{1-bit Fingerprint Differentia, Tapered Depth-Proportional Resolution Stratum Retention Predicate, 64 bit target column footprint.}
    \label{fig:reconstruction-example-d1-rp-t64}
  \end{subfigure}%
  \hfill%
%-------------------------------------------------------------------------------
  \begin{subfigure}[t]{0.32\linewidth}
    \centering
    % pass an arbitrary filename, potentially with unsafe characters
    % adapted from https://tex.stackexchange.com/a/36178
    \catcode`\%=12
    \providecommand\filename{}
    \renewcommand\filename{\detokenize{submodules/hereditary-stratigraph-concept-binder/binder/phylogenetic-inference/teeplots/source=a%reconstructed_phylogenies~source%nk_lexicaseselection_seed110_pop165_mut.01_snapshot_500.csv.gz+treatment=differentia%1~policy%RecencyProportionalResolution~target%64+viz=truncate-phylo-bounds+ext=}}
    \catcode`\%=14
    \includegraphics[width=\textwidth]{\importpath\filename}
    \caption{1-bit Fingerprint Differentia, MRCA-Recency-Proportional Resolution Stratum Retention Predicate, 64 bit target column footprint.}
    \label{fig:reconstruction-example-d1-tdp-t64}
  \end{subfigure}
%-------------------------------------------------------------------------------
  \caption{
    Example phylogeny reconstructions of ground-truth lexicase selection phylogeny from inference on extant hereditary stratigraphic columns.
    Shaded error bars on reconstructions indicate 95\% confidence intervals for the true generation of tree nodes.
    Arbitrary color is added to enhance distinguishability.
  }
  \label{fig:reconstruction-example}
\end{figure*}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/fig/retention-policies.tex <==
\input{lib/dissertationelse.tex}
\input{lib/dissertationonly.tex}

\begin{figure*}
  \centering
  \dissertationonly{\footnotesize}
  \begin{tabular}{m{0.05\textwidth}@{}|c@{}|c@{\hskip 0.01\textwidth}|m{0.14\textwidth}}
%-------------------------------------------------------------------------------
\hspace{-1ex}Policy&Lower-Resolution Parameterization&Higher-Resolution Parameterization&\makecell[c]{Properties}\\\hline
%-------------------------------------------------------------------------------
    \rotatebox{90}{\textbf{Fixed Resolution}}
  &
    \makecell{
      \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept-binder/binder/retention-policies/teeplots/fixed_resolution=512+num_layers=1024+stratum_retention_predicate=fixed-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
    \makecell{
      \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept-binder/binder/retention-policies/teeplots/fixed_resolution=128+num_layers=1024+stratum_retention_predicate=fixed-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
  \makecell[{{p{0.14\textwidth}}}]{
  \centering
    \bf{Space Complexity}\\
    $O(n)$\\
    \bf{MRCA Uncertainty}\\
    $O(1)$
  }
  \makecell[{{p{0.14\textwidth}}}]{
  \raggedright
    where $n$ is gens elapsed.
  }\\\hline
%-------------------------------------------------------------------------------
    \adjustbox{
      minipage=10em,
      rotate=90,
    }{
      \centering
      \textbf{Depth-Proportional Resolution}
      \par
    }
  &
    \makecell{
      \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept-binder/binder/retention-policies/teeplots/guaranteed_depth_proportional_resolution=1+num_layers=1024+stratum_retention_predicate=depth-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
    \makecell{
      \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept-binder/binder/retention-policies/teeplots/guaranteed_depth_proportional_resolution=4+num_layers=1024+stratum_retention_predicate=depth-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
  \makecell[{{p{0.14\textwidth}}}]{
  \centering
    \bf{Space Complexity}\\
    $O(1)$\\
    \bf{MRCA Uncertainty}\\
    $O(n)$
  }
  \makecell[{{p{0.14\textwidth}}}]{
  \raggedright
    where $n$ is gens elapsed.
  }\\\hline
%-------------------------------------------------------------------------------
    \adjustbox{
      minipage=15em,
      rotate=90,
    }{
      \centering
      \textbf{Tapered Depth-Proportional Resolution}
      \par
    }
  &
    \makecell{
      \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept-binder/binder/retention-policies/teeplots/guaranteed_depth_proportional_resolution=1+num_layers=1024+stratum_retention_predicate=tapered-depth-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
    \makecell{
      \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept-binder/binder/retention-policies/teeplots/guaranteed_depth_proportional_resolution=4+num_layers=1024+stratum_retention_predicate=tapered-depth-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
  \makecell[{{p{0.14\textwidth}}}]{
  \centering
    \bf{Space Complexity}\\
    $O(1)$\\
    \bf{MRCA Uncertainty}\\
    $O(n)$
  }
  \makecell[{{p{0.14\textwidth}}}]{
  \raggedright
    where $n$ is gens elapsed.
  }\\\hline
%-------------------------------------------------------------------------------
  \adjustbox{
    minipage=15em,
    rotate=90,
  }{
    \centering
    \textbf{Recency-Proportional\\Resolution}
    \par
  }
  &
  \makecell{
    \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept-binder/binder/retention-policies/teeplots/guaranteed_mrca_recency_proportional_resolution=0+num_layers=1024+stratum_retention_predicate=recency-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
  }
  &
  \makecell{
    \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept-binder/binder/retention-policies/teeplots/guaranteed_mrca_recency_proportional_resolution=4+num_layers=1024+stratum_retention_predicate=recency-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
  }
  &
  \makecell[{{p{0.14\textwidth}}}]{
  \centering
  \bf{Space Complexity}\\
  $O(\log(n))$\\
  \bf{MRCA Uncertainty}\\
  $O(m)$
  }
  \makecell[{{p{0.14\textwidth}}}]{
  \raggedright
  where $m$ is gens since MRCA and $n$ is total gens elapsed.
  }\\


  \end{tabular}
  \caption{
  Comparison of stratum retention policies.
  Policy visualizations show retained strata in black.
  Time progresses along the $y$-axis from top to bottom.
  New strata are introduced along the diagonal and then ``drip'' downward as a vertical line until eliminated.
  The set of retained strata present within a column at a particular generation $g$ can be read as intersections of retained vertical lines with a horizontal line with intercept $g$.
  Policy visualizations are provided for two parameterizations for each policy: the first where the maximum uncertainty of MRCA generation estimates would be 512 generations and the second where the maximum uncertainty of MRCA generation estimates would be 128 generations.
  }
  \label{fig:retention-policies}
\end{figure*}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/lib/C.tex <==
\input{lib/preservebackslash.tex}

% adapted from https://tex.stackexchange.com/a/449117
\newcolumntype{C}[1]{>{\PreserveBackslash\centering}p{#1}}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/lib/L.tex <==
\input{lib/preservebackslash.tex}

% adapted from https://tex.stackexchange.com/a/449117
\newcolumntype{L}[1]{>{\PreserveBackslash\raggedright}p{#1}}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/lib/dependencies.tex <==
\usepackage{natbib,alifeconf}  %% The order is important

\usepackage[export]{adjustbox}
\usepackage{algorithmic}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{array}
\usepackage{bibunits}
\usepackage{booktabs}
\usepackage{caption}
\usepackage{cite}
\usepackage{colortbl}
\usepackage{csvsimple}
\usepackage{etoolbox}
\usepackage[T1]{fontenc} % adapted from https://tex.stackexchange.com/a/388208
\usepackage{graphicx}
\usepackage{hyperref,cleveref}
\usepackage{ifthen}
\usepackage{import}
\usepackage{listings}
\usepackage{longtable}
\usepackage{makecell}
\usepackage{makecmds}
\usepackage{multirow}
\usepackage{natbib}
\usepackage[section]{placeins}
\usepackage{pythonhighlight}
\usepackage{rotating}
\usepackage{setspace}
\usepackage{siunitx}
\usepackage{stringstrings}
\usepackage{subcaption}
\usepackage{tabularx}
\usepackage{textcomp}
\usepackage{vcell}
\usepackage{xcolor}
\usepackage{xfp}
\usepackage{xparse}
\usepackage{xstring}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/lib/dissertationelse.tex <==
% \pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\providecommand{\dissertationelse}[2]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION
#1
\else
#2
\fi
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/lib/dissertationexclude.tex <==
% \pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\providecommand{\dissertationexclude}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION
\else
#1
\fi
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/lib/dissertationonly.tex <==
% \pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\providecommand{\dissertationonly}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION%
#1%
\else%
\fi
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/lib/importpath.tex <==
% \pragmaonce

% adapted from https://tex.stackexchange.com/a/17491
\makeatletter
  \providecommand\importpath{\import@path}
\makeatother


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/lib/pragmaonce.tex <==
% pragma once, adapted from https://tex.stackexchange.com/a/195173
\makeatletter
\let\pragma@iinput=\@iinput
\def\@iinput#1{\xdef\@pragmafile{#1}\pragma@iinput{#1} }
\def\@pragmafile{default}
\def\pragmaonce{%
   \csname pragma@\@pragmafile\endcsname
   \global\expandafter\let \csname pragma@\@pragmafile\endcsname = \endinput
}
\makeatother


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/lib/preservebackslash.tex <==
\providecommand{\PreserveBackslash}[1]{\let\temp=\\#1\let\\=\temp}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/lib/safepercent.tex <==
% \pragmaonce

% adapted from https://tex.stackexchange.com/a/351125
\catcode`\%=12
\providecommand\safepercent{%}
\catcode`\%=14


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/lib/safetilde.tex <==
% \pragmaonce

% adapted from https://tex.stackexchange.com/a/425957
\providecommand\safetilde{\string~}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/lst/StratumRetentionCondemnerDepthProportionalResolution.tex <==
\input{lib/dissertationelse.tex}

\provideenvironment{lstinputlistinghandle}{}{}

{\makeatletter\if@twocolumn\onecolumn\fi\makeatother
\begin{lstinputlistinghandle}
\lstinputlisting[%
language=Python,
caption={
  Depth-proportional resolution policy condemner implementation.
},
label={lst:StratumRetentionCondemnerDepthProportionalResolution},
style=mypython,
basicstyle=\dissertationelse{\fontsize{9}{10}\selectfont}{\scriptsize},
]{submodules/hstrat/hstrat/hstrat/stratum_retention_condemners/StratumRetentionCondemnerDepthProportionalResolution.py}
\end{lstinputlistinghandle}
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/lst/StratumRetentionCondemnerFixedResolution.tex <==
\provideenvironment{lstinputlistinghandle}{}{}

{\makeatletter\if@twocolumn\onecolumn\fi\makeatother
\begin{lstinputlistinghandle}
\lstinputlisting[%
language=Python,
caption={
  Fixed resolution policy condemner implementation.
},
label={lst:StratumRetentionCondemnerFixedResolution},
style=mypython,
basicstyle=\dissertationelse{\fontsize{9}{10}\selectfont}{\scriptsize},
]{submodules/hstrat/hstrat/hstrat/stratum_retention_condemners/StratumRetentionCondemnerFixedResolution.py}
\end{lstinputlistinghandle}
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/lst/StratumRetentionCondemnerRecencyProportionalResolution.tex <==
\provideenvironment{lstinputlistinghandle}{}{}

{\makeatletter\if@twocolumn\onecolumn\fi\makeatother
\begin{lstinputlistinghandle}
\lstinputlisting[%
language=Python,
caption={
  MRCA-recency-proportional resolution policy condemner implementation.
},
label={lst:StratumRetentionCondemnerRecencyProportionalResolution},
style=mypython,
basicstyle=\dissertationelse{\fontsize{9}{10}\selectfont}{\scriptsize},
]{submodules/hstrat/hstrat/hstrat/stratum_retention_condemners/StratumRetentionCondemnerRecencyProportionalResolution.py}
\end{lstinputlistinghandle}
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/lst/StratumRetentionCondemnerTaperedDepthProportionalResolution.tex <==
\provideenvironment{lstinputlistinghandle}{}{}

{\makeatletter\if@twocolumn\onecolumn\fi\makeatother
\begin{lstinputlistinghandle}
\lstinputlisting[%
language=Python,
caption={
  Tapered depth-proportional resolution policy condemner implementation.
},
label={lst:StratumRetentionCondemnerTaperedDepthProportionalResolution},
style=mypython,
basicstyle=\dissertationelse{\fontsize{9}{10}\selectfont}{\scriptsize},
]{submodules/hstrat/hstrat/hstrat/stratum_retention_condemners/StratumRetentionCondemnerTaperedDepthProportionalResolution.py}
\end{lstinputlistinghandle}
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/lst/StratumRetentionPredicateDepthProportionalResolution.tex <==
\provideenvironment{lstinputlistinghandle}{}{}

{\makeatletter\if@twocolumn\onecolumn\fi\makeatother
\begin{lstinputlistinghandle}
\lstinputlisting[%
language=Python,
caption={
  Depth-proportional resolution policy predicate implementation, including method to calculate exact number of strata retained by generation and method to calculate stratum deposition rank from column index.
},
label={lst:StratumRetentionPredicateDepthProportionalResolution},
style=mypython,
basicstyle=\dissertationelse{\fontsize{9}{10}\selectfont}{\scriptsize},
]{submodules/hstrat/hstrat/hstrat/stratum_retention_predicates/StratumRetentionPredicateDepthProportionalResolution.py}
\end{lstinputlistinghandle}
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/lst/StratumRetentionPredicateFixedResolution.tex <==
\provideenvironment{lstinputlistinghandle}{}{}

{\makeatletter\if@twocolumn\onecolumn\fi\makeatother
\begin{lstinputlistinghandle}
\lstinputlisting[%
language=Python,
caption={
  Fixed resolution policy predicate implementation, including method to calculate exact number of strata retained by generation and method to calculate stratum deposition rank from column index.
},
label={lst:StratumRetentionPredicateFixedResolution},
style=mypython,
basicstyle=\dissertationelse{\fontsize{9}{10}\selectfont}{\scriptsize},
]{submodules/hstrat/hstrat/hstrat/stratum_retention_predicates/StratumRetentionPredicateFixedResolution.py}
\end{lstinputlistinghandle}
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/lst/StratumRetentionPredicateRecencyProportionalResolution.tex <==
\provideenvironment{lstinputlistinghandle}{}{}

{\makeatletter\if@twocolumn\onecolumn\fi\makeatother
\begin{lstinputlistinghandle}
\lstinputlisting[%
language=Python,
caption={
  MRCA-recency-proportional resolution policy predicate implementation, including method to calculate exact number of strata retained by generation and method to calculate stratum deposition rank from column index.
},
label={lst:StratumRetentionPredicateRecencyProportionalResolution},
style=mypython,
basicstyle=\dissertationelse{\fontsize{9}{10}\selectfont}{\scriptsize},
]{submodules/hstrat/hstrat/hstrat/stratum_retention_predicates/StratumRetentionPredicateRecencyProportionalResolution.py}
\end{lstinputlistinghandle}
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/lst/StratumRetentionPredicateTaperedDepthProportionalResolution.tex <==
\provideenvironment{lstinputlistinghandle}{}{}

{\makeatletter\if@twocolumn\onecolumn\fi\makeatother
\begin{lstinputlistinghandle}
\lstinputlisting[%
language=Python,
caption={
  Tapered depth-proportional resolution policy predicate implementation, including method to calculate exact number of strata retained by generation and method to calculate stratum deposition rank from column index.
},
label={lst:StratumRetentionPredicateTaperedDepthProportionalResolution},
style=mypython,
basicstyle=\dissertationelse{\fontsize{9}{10}\selectfont}{\scriptsize},
]{submodules/hstrat/hstrat/hstrat/stratum_retention_predicates/StratumRetentionPredicateTaperedDepthProportionalResolution.py}
\end{lstinputlistinghandle}
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex-extended-abstract/lib/dependencies.tex <==
\usepackage[export]{adjustbox}
\usepackage{algorithmic}
\usepackage{amsmath,amsfonts}
\usepackage{array}
\usepackage{bibunits}
\usepackage{booktabs}
\usepackage{caption}
\usepackage{cite}
\usepackage{colortbl}
\usepackage{csvsimple}
\usepackage{etoolbox}
\usepackage{graphicx}
\usepackage{hyperref,cleveref}
\usepackage{ifthen}
\usepackage{import}
\usepackage{listings}
\usepackage{makecell}
\usepackage{multirow}
\usepackage{natbib}
\usepackage{pythonhighlight}
\usepackage{rotating}
\usepackage{siunitx}
\usepackage{stringstrings}
\usepackage{subcaption}
\usepackage{tabularx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{xfp}
\usepackage{xparse}
\usepackage{xstring}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex-extended-abstract/text/abstract.tex <==
\begin{abstract}
Phylogenetic analyses can also enable insight into evolutionary and ecological dynamics such as selection pressure and frequency dependent selection in digital evolution systems.
Traditionally, digital evolution systems have recorded data for phylogenetic analyses through perfect tracking where each birth event is recorded in a centralized data structures.
This approach, however, does not easily scale to distributed computing environments where evolutionary individuals may migrate between a large number of disjoint processing elements.
To provide for phylogenetic analyses in these environments, we propose an approach to infer phylogenies via heritable genetic annotations rather than directly track them.
We introduce a ``hereditary stratigraphy'' algorithm that enables efficient, accurate phylogenetic reconstruction with tunable, explicit trade-offs between annotation memory footprint and reconstruction accuracy.
This approach can estimate, for example, MRCA generation of two genomes within 10\% relative error with 95\% confidence up to a depth of a trillion generations with genome annotations smaller than a kilobyte.
We also simulate inference over known lineages, recovering up to 85.70\% of the information contained in the original tree using a 64-bit annotation.
\end{abstract}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex-extended-abstract/text/acknowledgement.tex <==
\section*{Acknowledgment}

This research was supported in part by NSF grants DEB-1655715 and DBI-0939454 as well as by Michigan State University through the computational resources provided by the Institute for Cyber-Enabled Research.
This material is based upon work supported by the National Science Foundation Graduate Research Fellowship under Grant No. DGE-1424871.
Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the National Science Foundation.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex-extended-abstract/text/body.tex <==
\input{text/body/introduction.tex}

\input{text/body/methods.tex}

\input{text/body/results-and-discussion.tex}

\input{text/body/conclusion.tex}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex-extended-abstract/text/body/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}

This and other methodology to enable decentralized observation and analysis of evolving systems will be essential for digital evolution experiments that use distributed and best-effort computing approaches.
Such methods will be crucial to enabling experimental analyses while preserving those systems' efficiency and scalability.
As parallel and distributed computing becomes increasingly ubiquitous and begins to more widely pervade digital evolution systems, hereditary stratigraphy should serve as a useful technique in this toolbox.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex-extended-abstract/text/body/introduction.tex <==
\section{Introduction} \label{sec:introduction}

In non-parallelized digital evolution experiments, phylogenetic trees can be tracked perfectly as they progress \citep{bohm2017mabe,wang2018vine,lalejini2019data} rather than reconstructed afterward, as must be done in most biological studies of evolution.
Such direct phylogenetic tracking enables a dizzying suite of experimental possibilities unique to digital evolution, such as perfect reconstruction of the sequence of phylogenetic states that led to a particular evolutionary outcome \citep{lenski2003evolutionary, dolson2020interpreting}.
% In a shared-memory context, it is not difficult to maintain a complete phylogeny where offspring simply track their parent (or vice versa).
% As simulations progress for longer durations, memory usage will typically grow at least linearly if population sizes are fixed, or worse if populations are growing or organisms are becoming more complex.
% These problems are easily ameliorated, however, by performing garbage collection on extinct lineages and saving older history to disk \citep{bohm2017mabe,dolson2019modes}.

Phylogenetic tracking in a distributed context, where linages may traverse many machines, introduces implementation complexity and more significant runtime overhead cost.
% However, if sufficient memory or disk space can be afforded to log all reproduction events, recording a perfect phylogeny in a distributed context is still not especially difficult.
% Processes could maintain records of each reproduction event, storing the parent organism (and its associated process) with all generated offspring (and their destination processes).
% As long as no data goes missing and organisms are uniquely identified globally, these ``dangling ends'' could be joined in postprocessing to weave a continuous global phylogeny.
% Of course, for the huge population sizes made possible by distirbuted systems, such stitching may become a demanding task in and of itself.
%
% However, if memory and disk space are limited, distributed phylogeny tracking becomes a more burdonsome challenge.
% A naive approach might employ a server model to maintain a central store of phylogenetic data.
% Processes would dispatch notifications of birth and death events to the server, which would curate (and gabage collect) phylogenetic history much the same as current serial phylogenetic tracking implementations.
% Unfortunately, this server model approach would present profound scalability challenges: communication and computation burden on the server process would worsen in direct proportion to processor count, and processes would frequently need to pause while waiting for confirmation that a reproduction event was successfully reported.
% ELD: This is making me wonder if there's a middle ground that could be explored in the future where we could use a sort of UDP phylogeny protocol, where no confirmation occurs
An ideally scalable approach would record birth and death events only on the process(es) where they unfold.
% Even this localized technique would lead to serious performance challenges, however.
% Lineages that went extinct locally could not be safely garbage collected until the extinction of thair offspring's lineages on other processors could be confirmed.
% Thus, garbage collection would require extinction notifications to wind back across processes each lineage had traversed.

% Under a best-effort model, no system of phylogeny tracking can guarantee proper garbage collection.
% For example, it would be possible for an offspring that was dispatched to a neighboring process to have failed to arrive, and both processes would need to keep going, despite the failure.
% So, extinction notifications for the lineage founded by that offspring would never be dispatched --- putting in motion a memory leak of un-garbage-collectible phylogenetic history.
% The situation becomes even more leaky when the possibility of extinction notifications themselves being lost.

In a distributed context --- especially, a distributed, best-effort context --- phylogenetic reconstruction (as opposed to tracking) could prove simpler and more efficient at runtime while providing sufficient power to address experimental questions of interest.
However, phylogenetic reconstruction from genomes with a traditional model of divergence under grandual accumulation of random mutations poses its own difficulties \citep{lack2010identifying,casci2008lining,hagstrom2004using,kapli2020phylogenetic,sarkar2010hardware}.

% The computational flexibility of digital evolution experiments provides a unique opportunity to overcome these challenges: designing heritable genome annotations specifically to simplify and strengthen phylogenetic reconstruction efforts.
% For maximum applicability of such a solution, these annotations should be phenotypically neutral heritable instrumentation \citep{stanley2002evolving} that do not affect any encodings for functional genome content.

This work introduces ``hereditary stratigraphy,'' a novel heritable genome annotation system to facilitate post-hoc phylogenetic inference on asexual populations.
This system allows explicit control over trade-offs between space complexity and accuracy of phylogenetic inference.
Instead of modeling genome components undergoing neutral variation through a mutational process, we keep a record of historical checkpoints that allow comparison of two lineages to identify the range of time in which they diverged.

% In Section \ref{sec:methods} we motivate and explain the hereditary stratigraphy approach.
% Then, in Section \ref{sec:results} we simulate post-hoc inference on known phylogenies to assess the quality of phylogenetic reconstruction enabled by the hereditary stratigraphy method.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex-extended-abstract/text/body/methods.tex <==
\section{Methods} \label{sec:methods}

\input{fig/column-comparison.tex}

Our algorithm, particularly the vocabulary we developed to describe it, draws on the concept of geological stratigraphy, inference of natural history through analysis of successive layers of geological material \citep{steno1916prodromus}.
As an introductory intuition, suppose a body of rock being built up through regular, discrete events depositing of geological material.
Note that in such a scenario we could easily infer the age of the body of rock by counting up the number of layers present.
% Note that it is crucial to this scenario that each layer has some differentiating feature that allows it to be distinguished from layers above and below it, but also potentially from layers present in another body of rock in a distant and unrelated geographic position.
Next, imagine making a copy of the rock body in its partially-formed state and then moving it far away.
As time runs forward on these two rock bodies, independent layering processes will cause consistent disparity in the layers forming on each forwards from their point of separation.

To deduce the historical relationship of these rock bodies after the fact, we could simply align and compare their layers.
Layers from their base up through the first disparity would correspond to shared ancestry; further disparate layers would correspond to diverged ancestry.
% Interestingly, and powerfully for phylogenetic inference, we can readily distinguish a scenario where both rock bodies deposited ten layers after diverging from a scenario where one deposited eighteen layers and the other deposited two.
Figure \ref{fig:column-comparison} depicts the process of comparing columns for phylogenetic inference.

Shifting now from intuition to implementation, a fixed-length randomly-generated binary tag provides a convenient and efficient mechanism to differentiate between our metaphorical ``layers.''
% We call this ``fingerprint'' tag a \textit{differentia}.
% The width of this tag controls the probability of spurious collisions between independently generated instances.
% At 64 bits wide the tag essentially functions as a UID: collisions between randomly generated tags are so unlikely ($p < 5.42\times10^{-20}$) they can essentially be ignored.
% At the other end of the spectrum, collision probability would be $1/256$ for a single byte and $1/2$ for a single bit.
% In the case of narrow differentia, in order to set a lower bound for the MRCA generation, you would have to backtrack common strata from the last commonality until the probability of that many successive spurious collisions was enough to satisfy your desired confidence level (e.g., 95\% confidence).
% Even then, there would be a possibility of the the true MRCA falling before the lower bound.
% Note, however, that no matter the width of the differentia the generation of the first discrepancy provides a hard upper bound on the generation of the MRCA.
%
In accordance with our geological analogy, we refer to the packet of data accumulated each generation as a \textit{stratum}.
This packet contains the differentia and, although not employed in this work, could hold other arbitrary user-defined data (i.e., simulation timestamp, phenotype characteristics, etc.).
% Again in accordance with the geological analogy, we refer to the chronological stack of strata that accumulate over successive depositions as a \textit{hereditary stratigraphic column}.

% \subsection{Stratum Retention Policy}

% \input{fig/deposit-process.tex}

As currently stated, fingerprints will accumulate proportionally to the length of evolutionary history simulated.
In an evolutionary run with thousands or millions of generations, this approach would soon become intractable --- particularly when columns are serialized and transmitted between distributed computing elements.
To solve this problem, we can trade off precision for compactness by deleting strata from columns as time progresses.
% Figure \ref{fig:deposit-process} overviews how stratum deposit and stratum elimination progress over two generations under the hereditary stratigraphic column scheme.
%
% Different patterns of deletion will lead to different trade-offs, both in terms of the scaling relationship of column size to generations elapsed and in terms of the arrangement of precision over evolutionary history (i.e., focusing precision on more recent evolutionary history versus spreading it evenly over the entire history).
%
We refer to the rule set used to selectively eliminate strata over time as the ``stratum retention policy.''
We devised three stratum retention policies, which provide
\begin{itemize}
  \item linear space complexity and constant inference error,
  \item constant space complexity and linear inference error with respect to phylogenetic depth, or
  \item logarithmic space complexity and inference error as a constant proportion of time elapsed since MRCA.
\end{itemize}

% We explore several different retention policy designs here, and implement our software to allows for free, modular interchange of retention policies.
% It is possible to define a policy through either of two mechanisms.
% First, policy can be defined as a ``predicate'' where the generation of a stratum and the current number of strata deposited is passed into a function that returns whether that strata should be retained at that point in time.
% Second, policy can be defined as a ``condemner'' generator where, given the current number of strata deposited, the set of ranks that should be deleted at this point in time are yielded.
% Although the predicate form is useful for analyzing and proving properties of policies, the condemner form is generally more efficient in practice.
% We provide predicate and condemner implementations for each stratum retention policy discussed here.

% It should be noted that condemners and predicates are both defined in terms of stratum generation, not stratum index among retained strata in the column.
% Therefore, it may seem necessary to store the generation of deposit within the stratum data structure.
% However, if you know the total number of generations deposited you can map backwards from index to recover the generation deposited without storing it.
% We provide this formula for each stratum retention policy.
% Finally, for each policy we provide a formula to calculate the exact number of strata retained under any parameterization after $n$ generations.
%
% In the next subsections, we introduce several stratum retention policies, provide the intuition behind their implementation, and elaborate their space complexity and resolution properties.
% For each policy, patterns of stratum retention are illustrated in Figure \ref{fig:retention-policies}.
% The formulas for number of strata retained after $n$ generations, the formulas to calculate stratum deposit generation from column index, and the retention predicate specifications of each policy are available in Supplementary Listing \ref{lst:StratumRetentionPredicateDepthProportionalResolution} \citep{moreno2022hstratconceptsupplement}.
% The condemner generator specification of each policy is available in Supplementary Listing \ref{lst:StratumRetentionCondemnerDepthProportionalResolution} \citep{moreno2022hstratconceptsupplement}.
% For tapered depth-proportional resolution and recency-proportional resolution, the accuracy of MRCA estimation can also be explored via an interactive in-browser web applet at \url{https://hopth.ru/bi}.
%
% \input{fig/retention-policies.tex}
%
% \subsection{Fixed Resolution Stratum Retention Policy}
%
% The fixed resolution retention policy provides a fixed absolute upper bound $r$ on the spacing between retained strata.
% The strategy to obtain this property is simple: permanently retain a stratum every $r$th generation
% (although, for arbitrary reasons of implementation convenience we require each stratum to be retained during at least the generation it is deposited).
%
% However, this retention policy suffers from linear growth in a column's memory footprint with respect to number of generations elapsed: every $r$th generation generation a new stratum is permanently retained
% For this reason, it is likely not useful in practice except potentially in scenarios where the number of generations is fixed in advance.
% We include it here largely for illustrative purposes as a gentle introduction to retention policies.
%
% \subsection{Depth-Proportional Resolution Stratum Retention Policy}
%
% The depth-proportional resolution policy ensures spacing between retained strata will be less than or equal to a proportion $r$ of total number of strata deposited.
% Achieving this limit on uncertainty requires retaining sufficient strata so that no more than $r$ ranks elapsed between any two strata.
% This policy accumulates retained strata at a fixed interval until twice as many as $r$ are at hand.
% Then, every other retained stratum is purged and the cycle repeats with a new twice-as-wide interval between retained strata.
%
% When comparing stratigraphic columns from different generations, the resolution guarantee holds in terms of the number of generations experienced by the older of the two columns.
% Because this retention policy is deterministic, for two columns with the same policy, every stratum that is held by the older column is also guaranteed to be present in the younger column (unless it hasn't yet been deposited on the younger column).
% Therefore, the strata that would enable the desired resolution when comparing two columns of the same age are guaranteed to be available.
%
% Because the number of strata retained under this policy is bounded as $2n+1$, space complexity scales as $O(1)$ with respect to the number of strata deposited.
% It follows that the MRCA rank estimate uncertainty scales as $O(n)$ with respect to the number of strata deposited.
%
% \subsection{Tapered Depth-Proportional Resolution Stratum Retention Policy}
%
% This policy refines the depth-proportional resolution policy to provide a more stable column memory footprint over time.
% The naive depth-proportional resolution policy builds up strata until twice as many are present as needed then purges half of them all at once.
% The tapered depth-proportional resolution policy functions identically to the depth-proportional policy except that it removes unnecessary strata gradually from back to front as new strata are deposited, instead of eliminating them simultaneously.
% The column footprint stability of this variation makes it easier to parameterize our experiments to ensure comparable end-state column footprints for fair comparison between retention policies, in addition to making this policy likely better suited to most use cases.
% By design, this policy has the same space complexity and MRCA estimation uncertainty scaling relationships with number generations elapsed as the naive depth-proporitonal resolution policy.
%
% \subsection{MRCA-Recency-Proportional Resolution Stratum Retention Policy}
%
% \input{tab/recency-proportional-space-complexity.tex}
%
% The MRCA-recency-proportional resolution policy ensures distance between the retained strata surrounding any generation point will be less than or equal to a user-specified proportion $r$ of the number of generations elapsed since.
%
% This policy can be constructed recursively, so to begin, let's consider setting up just the \textit{first} generation $g$ of the stratum after the root ancestor we will retain when $n$ generations have elapsed.
% A simple geometric analysis reveals that providing the guaranteed resolution for the worst-case generation within the window between generation 0 and generation $g$ (i.e., generation $g-1$) requires
% \begin{align*}
%   g \leq \lfloor n / (r + 1) \rfloor.
% \end{align*}
%
% We now have an upper bound for the rank of the first stratum generation we must retain.
% However, we must guarantee that these ranks are actually available for us to retain (i.e., it hasn't been purged out of the column at a previous time point as the column was grown by successive deposition).
% We will do this by picking the rank that is the highest power of 2 less than or equal to our bound.
% If we repeat this procedure as we recurse, we are guaranteed that this rank will have been preserved across all previous timepoints.
%
% Why does this work?
% Consider a sequence where all elements are powers of 2 and elements in the sequence are strictly nonincreasing.
% Consider the first element of the list.
% Partial sums along the sequence will include all multiples this first element.
% So, when we ratchet up $g$ to $2g$ as $n$ increases, we are guaranteed that $2g$ has been retained.
% This principle generalizes recursively down the list.
% This is a similar principle to the approach of strictly-doubling interval sizes used in the Naive and Tapered Depth-Proportional Resolution stratum retention policies described above.
%
% This step of truncating to the nearest less than or equal to power of 2 affects our recursive step size at most only by a constant factor of 2.
% So, because step size is a constant fraction of remaining generations $n$ (at worst $\frac{1}{2(r+1)}$), the number of steps made (and number of strata retained) scales as $O(\log(n))$ with respect to the number of strata deposited.
% Table \ref{tab:recency-proportional-space-complexity} provides exact figures for the number of strata retained under different parameterizations of the recency-proportional retention policy between one thousand and one trillion generations.
%
% As for rank estimate uncertainty, in the worst case it scales as $O(n)$ with respect to the greater number of strata deposited.
% However, with respect to estimating the rank of the MRCA when lineages diverged any fixed number of generations ago, uncertainty scales as $O(1)$.
%
% How does space complexity scale with respect to the policy's specified resolution $r$?
% Through extrapolation from OEIS sequences A063787 and A056791 via guess and check \citep{sloane2021a063787,sloane2021a056791}, we posited the exact number of strata retained after $n$ generations as
%
% \begin{align*}
%   \mathrm{HammingWeight}(n)
%   + \sum_1^r \lfloor \log_2( \lfloor n / r \rfloor ) \rfloor
%   + 1.
% \end{align*}
%
% This expression has been unit tested extensively to ensure perfect reliability.
% Approximating and applying logarithmic properties, this policy's space complexity can be calculated within a constant factor as
%
% \begin{align*}
% \log(n) + \log\Big(\frac{n^r}{r!}\Big).
% \end{align*}
%
% To answer our question, we will examine the ratio of space complexities required when scaling resolution $r$ up by a constant factor $f > 1$.
% Evaluating this ratio as $r \to \infty$, we find that space complexity scales directly proportional with the desired resolution $r$ at the limit,
%
% \begin{align*}
% \lim_{r \to \infty}
% \frac{
%   \log(n) + \log\Big(\frac{n^{fr}}{(fr)!}\Big)
% }{
%   \log(n) + \log\Big(\frac{n^r}{r!}\Big)
% }
% = f.
% \end{align*}
%
% Evaluating this ratio as $n \to \infty$, we find that this scaling relationship is never worse than directly proportional for any $r$,
%
% \begin{align*}
% \lim_{n \to \infty}
% \frac{
%   \log(n) + \log\Big(\frac{n^{fr}}{(fr)!}\Big)
% }{
%   \log(n) + \log\Big(\frac{n^r}{r!}\Big)
% }
% &= \frac{fr+1}{r+1}\\
% &= f\frac{r + 1/f}{r + 1}\\
% &\leq f.
% \end{align*}
%
%
% \subsection{Computational Experiments}
%
% These simulations propagated populations of between 100 and 165 bitstrings between 500 and 5,000 synchronous generations under the NK fitness landscape model \citep{kauffman1989nk}.
% In order to ensure coverage of a variety of phylogenetic conditions, we sampled a variety of selection schemes that impose profoundly different ecological regimens \citep{dolson2018ecological},
% \begin{itemize}
%   \item EcoEA Selection \citep{goings2012ecology},
%   \item Lexicase Selection \citep{helmuth2014solving},
%   \item Random Selection,
%   \item Sharing Selection \citep{goldberg1987genetic}
%   % \item Tournament Selection \citep{miller1995genetic}.
% \end{itemize}
%
% Supplementary Table \ref{tab:ground-truth-phylogenies} provides full details on the conditions each ground truth phylogeny was drawn from.
% The phylogenies themselves are available in our data repository for this project.
%
% For each ground truth phylogeny, we tested combinations of three configuration parameters:
% \begin{itemize}
%   \item target end-state memory footprints for extant columns (64, 512, and 4096 bits),
%   \item differentia width (1, 8, and 64 bits), and
%   \item stratum retention policy (tapered depth-proportional resolution and recency-proportional resolution).
% \end{itemize}
%
% Stratum retention policies were parameterized so that the maximum number of strata possible were present at the end of the experiment without exceeding the target memory footprint.
% If the target memory footprint is exceeded by the sparsest possible parameterization of a retention policy, then that sparsest possible parameterization is used.
% Supplementary Tables \cref{tab:experiment-column-sizes-nk-ecoea-selection,tab:experiment-column-sizes-nk-lexicase-selection,tab:experiment-column-sizes-nk-random-selection,tab:experiment-column-sizes-nk-sharing-selection,tab:experiment-column-sizes-nk-tournament-selection} provide the calculated paramaterizations and memory footprints of extant columns \citep{moreno2022hstratconceptsupplement}.
%
% In order to assess the viability of phylogenetic inference using hereditary stratigraphic columns from extant organisms, we used the end-state stratigraphs to estimate a reconstruction of the actual ground truth phylogenetic histories.
% The first step to reconstructing a phylogenetic tree for the history of an extant population at the end of an experiment is to construct a distance matrix by calculating all pairwise phylogenetic distances between extant columns.
% We defined phylogenetic distance between two extant columns as the sum of each extant organism's generational distance back to the generation of their MRCA, estimated as the mean of the upper and lower 95\% confidence bounds.
% Supplementary Figure \ref{fig:phylogenetic-inference} provides a cartoon summary of the process of calculating phylogenetic distance between two extant columns \citep{moreno2022hstratconceptsupplement}.
%
% We then used the unweighted pair group method with arithmetic mean (UPGMA) reconstruction tool provided by the BioPython package to generate estimate phylogenetic trees \citep{cock2009biopython,sokal1958statistical}.
% After generating the reconstructed tree topology, we performed a second pass to adjust branch lengths so that each tree node sat at the mean of its estimated 95\% confidence generation bounds.
% %We found that the neighbor joining (NJ) approach occasionally yielded reconstructions with impossible ``negative generation'' branches \citep{saitou1987neighbor} after knowledge bounding the absolute generation of internal nodes (i.e., MRCA's between pairs of extant organisms) was applied, so we did not use it.
%
% \subsection{Software and Data}
%
% % A prototype of this approach has been implemented \url{https://github.com/mmore500/dishtiny/blob/incoming/include/dish2/genome/PhyloFingerprints.hpp} and preliminarily tested \url{https://github.com/mmore500/dishtiny/blob/incoming/tests/dish2/genome/PhyloFingerprints.cpp}.
%
% As part of this work, we published the \texttt{hstrat} Python library with a stable public-facing API intended to enable incorporation in other projects with extensive documentation and unit testing on GitHub at \url{https://anonymous.4open.science/r/hstrat-115D/} and on PyPI.% at \url{https://pypi.org/project/hstrat/}. https://github.com/mmore500/hstrat
% In the near future, we intend to complete and publish a corresponding C++ library.
%
% Supporting software materials can be found on GitHub at \url{https://anonymous.4open.science/r/hereditary-stratigraph-concept-6BEC/}.%\url{https://github.com/mmore500/hereditary-stratigraph-concept}
% Supporting computational notebooks are available for in-browser use via BinderHub at \url{ANONYMIZED FOR PEER REVIEW} \citep{ragan2018binder}. %https://mybinder.org/v2/gh/mmore500/hereditary-stratigraph-concept/HEAD?labpath=binder%2F
% Our work benefited from many pieces of open source scientific software, including \citep{sukumaran2010dendropy,virtanen2020scipy,hunter2007matplotlib,virtanen2020scipy,waskom2021seaborn,bostock2011d3,meurer2017sympy,smith2020treedistdata,paradis2004ape,ushey2022reticulate,wickham2022dplyr}.
% The ground truth phylogenies used in this work as well as supplementary figures, tables, and text are available via the Open Science Framework at
% \url{https://osf.io/4sm72/?view\_only=69f37c6d184143b7855299c3323749ea} \citep{foster2017open,moreno2022hstratconceptsupplement}.
% Phylogenetic data associated with this project is stored in the Alife Community Data Standards format \citep{lalejini2019data}.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex-extended-abstract/text/body/results-and-discussion.tex <==
\section{Results} \label{sec:results}

In order to assess the practical performance of the hereditary stratigraph approach in an applied setting, we simulated the process of stratigraph propagation over known ``ground truth'' phylogenies extracted from pre-existing digital evolution simulations \citep{hernandez2022phylogenetic}.
Across ground truth phylogenies, we were able to reconstruct the phylogenetic topology with between 47.75\% and 85.70\% of the information contained in the original tree using a 64-bit column memory footprint, between 47.75\% and 80.36\% using a 512-bit column memory footprint, and between 51.13\% and 83.53\% using a 4096-bit column memory footprint.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex-extended-abstract/text/frontmatter.tex <==
\title{ Hereditary Stratigraphy: Genome Annotations to Enable Phylogenetic Inference over Distributed Populations }

%%
%% The "author" command and its associated commands are used to define
%% the authors and their affiliations.
%% Of note is the shared affiliation of the first two authors, and the
%% "authornote" and "authornotemark" commands
%% used to denote shared contribution to the research.
\author{Matthew Andres Moreno}
\orcid{0000-0003-4726-4479}
\affiliation{%
  \institution{Michigan Statue University}
  \city{East Lansing}
  \state{Michigan}
  \country{USA}
  \postcode{48103}
}

\author{Emily Dolson}
% \email{dolsonem@msu.edu}
\orcid{0000-0001-8616-4898}
\affiliation{%
  \institution{Michigan Statue University}
  \city{East Lansing}
  \state{Michigan}
  \country{USA}
  \postcode{48103}
}

\author{Charles Ofria}
% \email{ofria@msu.edu}
\orcid{0000-0003-2924-1732}
\affiliation{%
  \institution{Michigan Statue University}
  \city{East Lansing}
  \state{Michigan}
  \country{USA}
  \postcode{48103}
}


%%
%% By default, the full list of authors will be used in the page
%% headers. Often, this list is too long, and will overlap
%% other information printed in the page headers. This command allows
%% the author to define a more concise list
%% of authors' names for this purpose.
\renewcommand{\shortauthors}{Moreno et al.}

\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10010147.10010341.10010366.10010369</concept_id>
       <concept_desc>Computing methodologies~Simulation tools</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10010147.10010257.10010293.10011809.10011812</concept_id>
       <concept_desc>Computing methodologies~Genetic algorithms</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Computing methodologies~Simulation tools}
\ccsdesc[500]{Computing methodologies~Genetic algorithms}

\keywords{phylogenetics, decentralized algorithms, digital evolution, genetic algorithms, genetic programming}

\input{text/abstract.tex}

\maketitle


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex-extended-abstract/text/references.tex <==
% \section*{References}

\putbib


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/draft.tex <==
\def\mydraft{
\usepackage{draftwatermark}
\usepackage{lineno}
\linenumbers
\renewcommand{\linenumberfont}{\normalfont\small\color{red}}
}
\input{main.tex}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/fig/cid_plot.tex <==
\begin{figure}
    \includegraphics[width=\columnwidth]{img/cid_plot}
    \caption{
    Reconstruction error for phylogenetic inference with ground truth sharing selection phylogeny.
    Lower is better.
    RPR is recency-proportional resolution policy and TDPR is tapered depth-proportional resolution policy.
    }
  \label{fig:cid_plot}
\end{figure}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/fig/column-comparison.tex <==
\begin{figure}
    \includegraphics[width=\columnwidth]{img/column-comparison}
    \caption{
    Inferring the generation of the most-recent common ancestor (MRCA) of two hereditary stratigraphic columns ``$A$'' and ``$B$''.
    Columns are aligned at corresponding generations.
    Then the first generation with disparate ``fingerprints'' is determined.
    % (If a particular generation's strata have been eliminated from one or both columns or have not yet been deposited on one column, then no comparison is performed at that generation.)
    This provides a hard upper bound on the generation of the MRCA: these strata \textit{must} have been deposited along separate lines of descent.
    Searching backward for the first commonality preceding that disparity provides a soft lower bound on the generation of the MRCA: these strata evidence common ancestry but \textit{might} collide by chance.
    Some strata mmay have been eliminated from the columns, as shown, in order to save space at the cost of increasing uncertainty of MRCA generation estimates.
    % (If a narrow ``fingerprint'' differentia like a single bit is used with plausible collision probability, a lower bound can be established by continuing to search backward until the probability of $k$ successive spurious collisions is sufficiently unlikely.)
    % This process yields certainty about the phylogenetic relationship between $A$ and $B$ shown at right above (i.e., common) and below (i.e., diverged) the MRCA bounds.
    }
  \label{fig:column-comparison}
\end{figure}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/fig/deposit-process.tex <==
\begin{figure*}
  \begin{minipage}{0.6\textwidth}
    \includegraphics[width=\textwidth]{img/deposit-process}
  \end{minipage}%
  \begin{minipage}{0.4\textwidth}
    \caption{
    Cartoon illustration of stratum deposit process.
    This process marks the elapse of a generation when a hereditary stratigraphic column is inherited by an offspring.
    First, a new stratum is appended to the end of the column with a randomly-generated ``fingerprint.''
    This ``fingerprint'' distinguishes strata that were generated along disparate lines of descent (e.g., \texttt{0xd01a} for 3rd Generation A and \texttt{0xe74a} for 3rd generation B).
    Then, the column's configured stratum retention policy is applied to ``prune'' the column by eliminating strata from specific generations.
    Although this cartoon depicts an empty space for eliminated strata, the underlying data structure behind a column (i.e., the pink overlay) can condense to reduce space complexity.
    }\label{fig:deposit-process}
  \end{minipage}
\end{figure*}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/fig/diffbits-clustering-information-distance.tex <==
\begin{sidewaysfigure}
  \includegraphics[width=\linewidth]{submodules/hereditary-stratigraph-concept/binder/reconstruction-quality/teeplots/col=condition+hue=num-differentia-bits+kind=bar+row=policy+tree-comparison-metric=clustering-information-distance+viz=catplot+x=num-column-bits+y=score+ext=}
  \caption{
  Comparison of phylogenetic reconstruction quality across differentia bit counts.
  Reconstruction quality measured as clustering information distance between reconstructed phylogeny and ground truth phylogeny \citep{smith2020information, smith2020treedist}.
  Lower is better.
  RPR is recency-proportional resolution stratum retention policy and TDPR is tapered depth-proportional resolution stratum retention policy.
  }
  \label{fig:diffbits-clustering-information-distance}
\end{sidewaysfigure}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/fig/diffbits-mutual-clustering-information.tex <==
\begin{sidewaysfigure}
  \includegraphics[width=\linewidth]{submodules/hereditary-stratigraph-concept/binder/reconstruction-quality/teeplots/col=condition+hue=num-differentia-bits+kind=bar+row=policy+tree-comparison-metric=mutual-clustering-information+viz=catplot+x=num-column-bits+y=score+ext=}
  \caption{
  Comparison of phylogenetic reconstruction quality across differentia bit counts.
  Reconstruction quality measured as mutual clustering information between reconstructed phylogeny and ground truth phylogeny \citep{smith2020information, smith2020treedist}.
  Higher is better.
  RPR is recency-proportional resolution stratum retention policy and TDPR is tapered depth-proportional resolution stratum retention policy.
  }
  \label{fig:diffbits-mutual-clustering-information}
\end{sidewaysfigure}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/fig/diffbits-robinson-foulds-similarity.tex <==
\begin{sidewaysfigure}
  \includegraphics[width=\linewidth]{submodules/hereditary-stratigraph-concept/binder/reconstruction-quality/teeplots/col=condition+hue=num-differentia-bits+kind=bar+row=policy+tree-comparison-metric=generalized-robinson-foulds-similarity+viz=catplot+x=num-column-bits+y=score+ext=}
  \caption{
  Comparison of phylogenetic reconstruction quality across differentia bit counts.
  Reconstruction quality measured as generalized Robinson-Foulds similarity between reconstructed phylogeny and ground truth phylogeny \citep{smith2020information, smith2020treedist}.
  Higher is better.
  RPR is recency-proportional resolution stratum retention policy and TDPR is tapered depth-proportional resolution stratum retention policy.
  }
  \label{fig:diffbits-robinson-foulds-similarity}
\end{sidewaysfigure}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/fig/info_plot.tex <==
\begin{figure}
    \includegraphics[width=\columnwidth]{img/info_plot}
    \caption{
    Proportion of information present in the ground-truth ftness sharing phylogeny that was captureed by our reconstruction, across various retention policies.
    High is better (1 is perfect).
    RPR is recency-proportional resolution policy and TDPR is tapered depth-proportional resolution policy.
    } \label{fig:info_plot}
\end{figure}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/fig/phylogenetic-inference.tex <==
\begin{figure*}
  \centering
    \includegraphics[width=\textwidth]{img/phylogenetic-inference}
    \caption{
    Cartoon illustration of column inheritance along a phylogenetic tree and the process to infer phylogenetic history along extant columns.
    This scenario supposes a stratum retention policy where only strata from even generations are retained.
    The common ancestor of the focal clade, which is at generation 2, is shown at top.
    Generation 3 columns inherit that ancestor's strata and each append a new stratum.
    Generation 4 columns append another new stratum then eliminate their generation 3 strata.
    Finally, another generation elapses to yield generation 5 strata.
    Suppose that only generation 5 strata are extant.
    So, greyed-out columns above are not directly observable.
    Phylogenetic history is deduced by pairwise comparison between extant columns.
    For each pair (like the example highlighted in red) a phylogenetic distance can be computed as the sum generations elapsed to each extant column after the estimated generation of their MRCA.
    These pairwise distances can then be fed into a phylogeny reconstruction algorithm.
    }
  \label{fig:phylogenetic-inference}
\end{figure*}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/fig/policy-clustering-information-distance.tex <==
\begin{sidewaysfigure}
  \begin{minipage}{0.7\linewidth}
    \includegraphics[width=\linewidth]{submodules/hereditary-stratigraph-concept/binder/reconstruction-quality/teeplots/col=num-differentia-bits+hue=policy+kind=bar+row=num-column-bits+tree-comparison-metric=clustering-information-distance+viz=catplot+x=condition+y=score+ext=}
  \end{minipage}%
  \begin{minipage}{0.3\linewidth}
    \caption{
    Comparison of phylogenetic reconstruction quality between stratum retention policies.
    Reconstruction quality measured as clustering information distance between reconstructed phylogeny and ground truth phylogeny \citep{smith2020information, smith2020treedist}.
    Lower is better.
    RPR is recency-proportional resolution stratum retention policy and TDPR is tapered depth-proportional resolution stratum retention policy.
    }
    \label{fig:diffbits-clustering-information-distance}
  \end{minipage}
\end{sidewaysfigure}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/fig/policy-mutual-clustering-information.tex <==
\begin{sidewaysfigure}
  \begin{minipage}{0.7\linewidth}
    \includegraphics[width=\linewidth]{submodules/hereditary-stratigraph-concept/binder/reconstruction-quality/teeplots/col=num-differentia-bits+hue=policy+kind=bar+row=num-column-bits+tree-comparison-metric=mutual-clustering-information+viz=catplot+x=condition+y=score+ext=}
  \end{minipage}%
  \begin{minipage}{0.3\linewidth}
    \caption{
    Comparison of phylogenetic reconstruction quality between stratum retention policies.
    Reconstruction quality measured as mutual clustering information between reconstructed phylogeny and ground truth phylogeny \citep{smith2020information, smith2020treedist}.
    Higher is better.
    RPR is recency-proportional resolution stratum retention policy and TDPR is tapered depth-proportional resolution stratum retention policy.
    }
    \label{fig:diffbits-mutual-clustering-information}
  \end{minipage}
\end{sidewaysfigure}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/fig/policy-robinson-foulds-similarity.tex <==
\begin{sidewaysfigure}
  \begin{minipage}{0.7\linewidth}
    \includegraphics[width=\linewidth]{submodules/hereditary-stratigraph-concept/binder/reconstruction-quality/teeplots/col=num-differentia-bits+hue=policy+kind=bar+row=num-column-bits+tree-comparison-metric=generalized-robinson-foulds-similarity+viz=catplot+x=condition+y=score+ext=}
  \end{minipage}%
  \begin{minipage}{0.3\linewidth}
    \caption{
    Comparison of phylogenetic reconstruction quality between stratum retention policies.
    Reconstruction quality measured as generalized Robinson-Foulds similarity between reconstructed phylogeny and ground truth phylogeny \citep{smith2020information, smith2020treedist}.
    Higher is better.
    RPR is recency-proportional resolution stratum retention policy and TDPR is tapered depth-proportional resolution stratum retention policy.    }
    \label{fig:diffbits-robinson-foulds-similarity}
  \end{minipage}
\end{sidewaysfigure}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/fig/reconstruction-example.tex <==
\input{lib/importpath.tex}

\begin{figure*}%
%-------------------------------------------------------------------------------
  \begin{subfigure}[b]{0.33\linewidth}
    \centering
    % pass an arbitrary filename, potentially with unsafe characters
    % adapted from https://tex.stackexchange.com/a/36178
    \catcode`\%=12
    \providecommand\filename{}
    \renewcommand\filename{\detokenize{submodules/hereditary-stratigraph-concept/binder/phylogenetic-inference/teeplots/a=true_phylogeny+source=a%reconstructed_phylogenies~source%nk_lexicaseselection_seed110_pop165_mut.01_snapshot_500.csv.gz+viz=truncate-phylo+ext=}}
    \catcode`\%=14
    \includegraphics[width=\linewidth]{\importpath\filename}
    \caption{Ground truth phylogeny.}
    \label{fig:reconstruction-example-true-phylogeny}
  \end{subfigure}%
%-------------------------------------------------------------------------------
  \begin{subfigure}[b]{0.33\linewidth}
    \centering
    % pass an arbitrary filename, potentially with unsafe characters
    % adapted from https://tex.stackexchange.com/a/36178
    \catcode`\%=12
    \providecommand\filename{}
    \renewcommand\filename{\detokenize{submodules/hereditary-stratigraph-concept/binder/phylogenetic-inference/teeplots/source=a%reconstructed_phylogenies~source%nk_lexicaseselection_seed110_pop165_mut.01_snapshot_500.csv.gz+treatment=differentia%1~policy%TaperedDepthProportionalResolution~target%64+viz=truncate-phylo-bounds+ext=}}
    \catcode`\%=14
    \includegraphics[width=\linewidth]{\importpath\filename}
    \caption{1-bit Fingerprint Differentia, Tapered Depth-Proportional Resolution Stratum Retention Predicate, 64 bit target column footprint.}
    \label{fig:reconstruction-example-d1-rp-t64}
  \end{subfigure}%
%-------------------------------------------------------------------------------
  \begin{subfigure}[b]{0.33\linewidth}
    \centering
    % pass an arbitrary filename, potentially with unsafe characters
    % adapted from https://tex.stackexchange.com/a/36178
    \catcode`\%=12
    \providecommand\filename{}
    \renewcommand\filename{\detokenize{submodules/hereditary-stratigraph-concept/binder/phylogenetic-inference/teeplots/source=a%reconstructed_phylogenies~source%nk_lexicaseselection_seed110_pop165_mut.01_snapshot_500.csv.gz+treatment=differentia%1~policy%RecencyProportionalResolution~target%64+viz=truncate-phylo-bounds+ext=}}
    \catcode`\%=14
    \includegraphics[width=\textwidth]{\importpath\filename}
    \caption{1-bit Fingerprint Differentia, MRCA-Recency-Proportional Resolution Stratum Retention Predicate, 64 bit target column footprint.}
    \label{fig:reconstruction-example-d1-tdp-t64}
  \end{subfigure}
%-------------------------------------------------------------------------------
  \caption{
    Example phylogeny reconstructions of ground-truth lexicase selection phylogeny from inference on extant hereditary stratigraphic columns.
    Shaded error bars on reconstructions indicate 95\% confidence intervals for the true generation of tree nodes.
    Arbitrary color is added to enhance distinguishability.
  }
  \label{fig:reconstruction-example}
\end{figure*}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/fig/retention-policies.tex <==
\input{lib/dissertationelse.tex}
\input{lib/dissertationonly.tex}

\begin{figure*}
  \centering
  \dissertationonly{\footnotesize}
  \begin{tabular}{m{0.05\textwidth}@{}|c@{}|c@{\hskip 0.01\textwidth}|m{0.14\textwidth}}
%-------------------------------------------------------------------------------
\hspace{-1ex}Policy&Lower-Resolution Parameterization&Higher-Resolution Parameterization&\makecell[c]{Properties}\\\hline
%-------------------------------------------------------------------------------
    \rotatebox{90}{\textbf{Fixed Resolution}}
  &
    \makecell{
      \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept/binder/retention-policies/teeplots/fixed_resolution=512+num_layers=1024+stratum_retention_predicate=fixed-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
    \makecell{
      \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept/binder/retention-policies/teeplots/fixed_resolution=128+num_layers=1024+stratum_retention_predicate=fixed-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
  \makecell[{{p{0.14\textwidth}}}]{
  \centering
    \bf{Space Complexity}\\
    $O(n)$\\
    \bf{MRCA Uncertainty}\\
    $O(1)$
  }
  \makecell[{{p{0.14\textwidth}}}]{
  \raggedright
    where $n$ is gens elapsed.
  }\\\hline
%-------------------------------------------------------------------------------
    \adjustbox{
      minipage=10em,
      rotate=90,
    }{
      \centering
      \textbf{Depth-Proportional Resolution}
      \par
    }
  &
    \makecell{
      \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept/binder/retention-policies/teeplots/guaranteed_depth_proportional_resolution=1+num_layers=1024+stratum_retention_predicate=depth-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
    \makecell{
      \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept/binder/retention-policies/teeplots/guaranteed_depth_proportional_resolution=4+num_layers=1024+stratum_retention_predicate=depth-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
  \makecell[{{p{0.14\textwidth}}}]{
  \centering
    \bf{Space Complexity}\\
    $O(1)$\\
    \bf{MRCA Uncertainty}\\
    $O(n)$
  }
  \makecell[{{p{0.14\textwidth}}}]{
  \raggedright
    where $n$ is gens elapsed.
  }\\\hline
%-------------------------------------------------------------------------------
    \adjustbox{
      minipage=15em,
      rotate=90,
    }{
      \centering
      \textbf{Tapered Depth-Proportional Resolution}
      \par
    }
  &
    \makecell{
      \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept/binder/retention-policies/teeplots/guaranteed_depth_proportional_resolution=1+num_layers=1024+stratum_retention_predicate=tapered-depth-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
    \makecell{
      \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept/binder/retention-policies/teeplots/guaranteed_depth_proportional_resolution=4+num_layers=1024+stratum_retention_predicate=tapered-depth-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
  \makecell[{{p{0.14\textwidth}}}]{
  \centering
    \bf{Space Complexity}\\
    $O(1)$\\
    \bf{MRCA Uncertainty}\\
    $O(n)$
  }
  \makecell[{{p{0.14\textwidth}}}]{
  \raggedright
    where $n$ is gens elapsed.
  }\\\hline
%-------------------------------------------------------------------------------
  \adjustbox{
    minipage=15em,
    rotate=90,
  }{
    \centering
    \textbf{Recency-Proportional\\Resolution}
    \par
  }
  &
  \makecell{
    \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept/binder/retention-policies/teeplots/guaranteed_mrca_recency_proportional_resolution=0+num_layers=1024+stratum_retention_predicate=recency-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
  }
  &
  \makecell{
    \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept/binder/retention-policies/teeplots/guaranteed_mrca_recency_proportional_resolution=4+num_layers=1024+stratum_retention_predicate=recency-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
  }
  &
  \makecell[{{p{0.14\textwidth}}}]{
  \centering
  \bf{Space Complexity}\\
  $O(\log(n))$\\
  \bf{MRCA Uncertainty}\\
  $O(m)$
  }
  \makecell[{{p{0.14\textwidth}}}]{
  \raggedright
  where $m$ is gens since MRCA and $n$ is total gens elapsed.
  }\\


  \end{tabular}
  \caption{
  Comparison of stratum retention policies.
  Policy visualizations show retained strata in black.
  Time progresses along the $y$-axis from top to bottom.
  New strata are introduced along the diagonal and then ``drip'' downward as a vertical line until eliminated.
  The set of retained strata present within a column at a particular generation $g$ can be read as intersections of retained vertical lines with a horizontal line with intercept $g$.
  Policy visualizations are provided for two parameterizations for each policy: the first where the maximum uncertainty of MRCA generation estimates would be 512 generations and the second where the maximum uncertainty of MRCA generation estimates would be 128 generations.
  }
  \label{fig:retention-policies}
\end{figure*}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/lib/C.tex <==
\input{lib/preservebackslash.tex}

% adapted from https://tex.stackexchange.com/a/449117
\newcolumntype{C}[1]{>{\PreserveBackslash\centering}p{#1}}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/lib/L.tex <==
\input{lib/preservebackslash.tex}

% adapted from https://tex.stackexchange.com/a/449117
\newcolumntype{L}[1]{>{\PreserveBackslash\raggedright}p{#1}}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/lib/dependencies.tex <==
\usepackage{natbib,alifeconf}  %% The order is important

\usepackage[export]{adjustbox}
\usepackage{algorithmic}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{array}
\usepackage{bibunits}
\usepackage{booktabs}
\usepackage{caption}
\usepackage{cite}
\usepackage{colortbl}
\usepackage{csvsimple}
\usepackage{etoolbox}
\usepackage[T1]{fontenc} % adapted from https://tex.stackexchange.com/a/388208
\usepackage{graphicx}
\usepackage{hyperref,cleveref}
\usepackage{ifthen}
\usepackage{import}
\usepackage{listings}
\usepackage{longtable}
\usepackage{makecell}
\usepackage{multirow}
\usepackage{natbib}
\usepackage[section]{placeins}
\usepackage{pythonhighlight}
\usepackage{rotating}
\usepackage{siunitx}
\usepackage{stringstrings}
\usepackage{subcaption}
\usepackage{tabularx}
\usepackage{textcomp}
\usepackage{vcell}
\usepackage{xcolor}
\usepackage{xfp}
\usepackage{xparse}
\usepackage{xstring}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/lib/dissertationelse.tex <==
% \pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\providecommand{\dissertationelse}[2]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION
#1
\else
#2
\fi
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/lib/dissertationexclude.tex <==
% \pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\providecommand{\dissertationexclude}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION
\else
#1
\fi
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/lib/dissertationonly.tex <==
% \pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\providecommand{\dissertationonly}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION%
#1%
\else%
\fi
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/lib/importpath.tex <==
% \pragmaonce

% adapted from https://tex.stackexchange.com/a/17491
\makeatletter
  \providecommand\importpath{\import@path}
\makeatother


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/lib/pragmaonce.tex <==
% pragma once, adapted from https://tex.stackexchange.com/a/195173
\makeatletter
\let\pragma@iinput=\@iinput
\def\@iinput#1{\xdef\@pragmafile{#1}\pragma@iinput{#1} }
\def\@pragmafile{default}
\def\pragmaonce{%
   \csname pragma@\@pragmafile\endcsname
   \global\expandafter\let \csname pragma@\@pragmafile\endcsname = \endinput
}
\makeatother


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/lib/preservebackslash.tex <==
\providecommand{\PreserveBackslash}[1]{\let\temp=\\#1\let\\=\temp}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/lib/safepercent.tex <==
% \pragmaonce

% adapted from https://tex.stackexchange.com/a/351125
\catcode`\%=12
\providecommand\safepercent{%}
\catcode`\%=14


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/lib/safetilde.tex <==
% \pragmaonce

% adapted from https://tex.stackexchange.com/a/425957
\providecommand\safetilde{\string~}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/lst/StratumRetentionCondemnerDepthProportionalResolution.tex <==
{\onecolumn
\lstinputlisting[%
language=Python,
caption={
  Depth-proportional resolution policy condemner implementation.
},
label={lst:StratumRetentionCondemnerDepthProportionalResolution},
style=mypython,
basicstyle=\scriptsize,
]{submodules/hstrat/hstrat/hstrat/stratum_retention_condemners/StratumRetentionCondemnerDepthProportionalResolution.py}
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/lst/StratumRetentionCondemnerFixedResolution.tex <==
{\onecolumn
\lstinputlisting[%
language=Python,
caption={
  Fixed resolution policy condemner implementation.
},
label={lst:StratumRetentionCondemnerFixedResolution},
style=mypython,
basicstyle=\scriptsize,
]{submodules/hstrat/hstrat/hstrat/stratum_retention_condemners/StratumRetentionCondemnerFixedResolution.py}
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/lst/StratumRetentionCondemnerRecencyProportionalResolution.tex <==
{\onecolumn
\lstinputlisting[%
language=Python,
caption={
  MRCA-recency-proportional resolution policy condemner implementation.
},
label={lst:StratumRetentionCondemnerRecencyProportionalResolution},
style=mypython,
basicstyle=\scriptsize,
]{submodules/hstrat/hstrat/hstrat/stratum_retention_condemners/StratumRetentionCondemnerRecencyProportionalResolution.py}
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/lst/StratumRetentionCondemnerTaperedDepthProportionalResolution.tex <==
{\onecolumn
\lstinputlisting[%
language=Python,
caption={
  Tapered depth-proportional resolution policy condemner implementation.
},
label={lst:StratumRetentionCondemnerTaperedDepthProportionalResolution},
style=mypython,
basicstyle=\scriptsize,
]{submodules/hstrat/hstrat/hstrat/stratum_retention_condemners/StratumRetentionCondemnerTaperedDepthProportionalResolution.py}
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/lst/StratumRetentionPredicateDepthProportionalResolution.tex <==
{\onecolumn
\lstinputlisting[%
language=Python,
caption={
  Depth-proportional resolution policy predicate implementation, including method to calculate exact number of strata retained by generation and method to calculate stratum deposition rank from column index.
},
label={lst:StratumRetentionPredicateDepthProportionalResolution},
style=mypython,
basicstyle=\scriptsize,
]{submodules/hstrat/hstrat/hstrat/stratum_retention_predicates/StratumRetentionPredicateDepthProportionalResolution.py}
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/lst/StratumRetentionPredicateFixedResolution.tex <==
{\onecolumn
\lstinputlisting[%
language=Python,
caption={
  Fixed resolution policy predicate implementation, including method to calculate exact number of strata retained by generation and method to calculate stratum deposition rank from column index.
},
label={lst:StratumRetentionPredicateFixedResolution},
style=mypython,
basicstyle=\scriptsize,
]{submodules/hstrat/hstrat/hstrat/stratum_retention_predicates/StratumRetentionPredicateFixedResolution.py}
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/lst/StratumRetentionPredicateRecencyProportionalResolution.tex <==
{\onecolumn
\lstinputlisting[%
language=Python,
caption={
  MRCA-recency-proportional resolution policy predicate implementation, including method to calculate exact number of strata retained by generation and method to calculate stratum deposition rank from column index.
},
label={lst:StratumRetentionPredicateRecencyProportionalResolution},
style=mypython,
basicstyle=\scriptsize,
]{submodules/hstrat/hstrat/hstrat/stratum_retention_predicates/StratumRetentionPredicateRecencyProportionalResolution.py}
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/lst/StratumRetentionPredicateTaperedDepthProportionalResolution.tex <==
{\onecolumn
\lstinputlisting[%
language=Python,
caption={
  Tapered depth-proportional resolution policy predicate implementation, including method to calculate exact number of strata retained by generation and method to calculate stratum deposition rank from column index.
},
label={lst:StratumRetentionPredicateTaperedDepthProportionalResolution},
style=mypython,
basicstyle=\scriptsize,
]{submodules/hstrat/hstrat/hstrat/stratum_retention_predicates/StratumRetentionPredicateTaperedDepthProportionalResolution.py}
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex-extended-abstract/lib/dependencies.tex <==
\usepackage[export]{adjustbox}
\usepackage{algorithmic}
\usepackage{amsmath,amsfonts}
\usepackage{array}
\usepackage{bibunits}
\usepackage{booktabs}
\usepackage{caption}
\usepackage{cite}
\usepackage{colortbl}
\usepackage{csvsimple}
\usepackage{etoolbox}
\usepackage{graphicx}
\usepackage{hyperref,cleveref}
\usepackage{ifthen}
\usepackage{import}
\usepackage{listings}
\usepackage{makecell}
\usepackage{multirow}
\usepackage{natbib}
\usepackage{pythonhighlight}
\usepackage{rotating}
\usepackage{siunitx}
\usepackage{stringstrings}
\usepackage{subcaption}
\usepackage{tabularx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{xfp}
\usepackage{xparse}
\usepackage{xstring}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex-extended-abstract/text/abstract.tex <==
\begin{abstract}
Phylogenetic analyses can also enable insight into evolutionary and ecological dynamics such as selection pressure and frequency dependent selection in digital evolution systems.
Traditionally, digital evolution systems have recorded data for phylogenetic analyses through perfect tracking where each birth event is recorded in a centralized data structures.
This approach, however, does not easily scale to distributed computing environments where evolutionary individuals may migrate between a large number of disjoint processing elements.
To provide for phylogenetic analyses in these environments, we propose an approach to infer phylogenies via heritable genetic annotations rather than directly track them.
We introduce a ``hereditary stratigraphy'' algorithm that enables efficient, accurate phylogenetic reconstruction with tunable, explicit trade-offs between annotation memory footprint and reconstruction accuracy.
This approach can estimate, for example, MRCA generation of two genomes within 10\% relative error with 95\% confidence up to a depth of a trillion generations with genome annotations smaller than a kilobyte.
We also simulate inference over known lineages, recovering up to 85.70\% of the information contained in the original tree using a 64-bit annotation.
\end{abstract}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex-extended-abstract/text/acknowledgement.tex <==
\section*{Acknowledgment}

This research was supported in part by NSF grants DEB-1655715 and DBI-0939454 as well as by Michigan State University through the computational resources provided by the Institute for Cyber-Enabled Research.
This material is based upon work supported by the National Science Foundation Graduate Research Fellowship under Grant No. DGE-1424871.
Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the National Science Foundation.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex-extended-abstract/text/body.tex <==
\input{text/body/introduction.tex}

\input{text/body/methods.tex}

\input{text/body/results-and-discussion.tex}

\input{text/body/conclusion.tex}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex-extended-abstract/text/body/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}

This and other methodology to enable decentralized observation and analysis of evolving systems will be essential for digital evolution experiments that use distributed and best-effort computing approaches.
Such methods will be crucial to enabling experimental analyses while preserving those systems' efficiency and scalability.
As parallel and distributed computing becomes increasingly ubiquitous and begins to more widely pervade digital evolution systems, hereditary stratigraphy should serve as a useful technique in this toolbox.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex-extended-abstract/text/body/introduction.tex <==
\section{Introduction} \label{sec:introduction}

In non-parallelized digital evolution experiments, phylogenetic trees can be tracked perfectly as they progress \citep{bohm2017mabe,wang2018vine,lalejini2019data} rather than reconstructed afterward, as must be done in most biological studies of evolution.
Such direct phylogenetic tracking enables a dizzying suite of experimental possibilities unique to digital evolution, such as perfect reconstruction of the sequence of phylogenetic states that led to a particular evolutionary outcome \citep{lenski2003evolutionary, dolson2020interpreting}.
% In a shared-memory context, it is not difficult to maintain a complete phylogeny where offspring simply track their parent (or vice versa).
% As simulations progress for longer durations, memory usage will typically grow at least linearly if population sizes are fixed, or worse if populations are growing or organisms are becoming more complex.
% These problems are easily ameliorated, however, by performing garbage collection on extinct lineages and saving older history to disk \citep{bohm2017mabe,dolson2019modes}.

Phylogenetic tracking in a distributed context, where linages may traverse many machines, introduces implementation complexity and more significant runtime overhead cost.
% However, if sufficient memory or disk space can be afforded to log all reproduction events, recording a perfect phylogeny in a distributed context is still not especially difficult.
% Processes could maintain records of each reproduction event, storing the parent organism (and its associated process) with all generated offspring (and their destination processes).
% As long as no data goes missing and organisms are uniquely identified globally, these ``dangling ends'' could be joined in postprocessing to weave a continuous global phylogeny.
% Of course, for the huge population sizes made possible by distirbuted systems, such stitching may become a demanding task in and of itself.
%
% However, if memory and disk space are limited, distributed phylogeny tracking becomes a more burdonsome challenge.
% A naive approach might employ a server model to maintain a central store of phylogenetic data.
% Processes would dispatch notifications of birth and death events to the server, which would curate (and gabage collect) phylogenetic history much the same as current serial phylogenetic tracking implementations.
% Unfortunately, this server model approach would present profound scalability challenges: communication and computation burden on the server process would worsen in direct proportion to processor count, and processes would frequently need to pause while waiting for confirmation that a reproduction event was successfully reported.
% ELD: This is making me wonder if there's a middle ground that could be explored in the future where we could use a sort of UDP phylogeny protocol, where no confirmation occurs
An ideally scalable approach would record birth and death events only on the process(es) where they unfold.
% Even this localized technique would lead to serious performance challenges, however.
% Lineages that went extinct locally could not be safely garbage collected until the extinction of thair offspring's lineages on other processors could be confirmed.
% Thus, garbage collection would require extinction notifications to wind back across processes each lineage had traversed.

% Under a best-effort model, no system of phylogeny tracking can guarantee proper garbage collection.
% For example, it would be possible for an offspring that was dispatched to a neighboring process to have failed to arrive, and both processes would need to keep going, despite the failure.
% So, extinction notifications for the lineage founded by that offspring would never be dispatched --- putting in motion a memory leak of un-garbage-collectible phylogenetic history.
% The situation becomes even more leaky when the possibility of extinction notifications themselves being lost.

In a distributed context --- especially, a distributed, best-effort context --- phylogenetic reconstruction (as opposed to tracking) could prove simpler and more efficient at runtime while providing sufficient power to address experimental questions of interest.
However, phylogenetic reconstruction from genomes with a traditional model of divergence under grandual accumulation of random mutations poses its own difficulties \citep{lack2010identifying,casci2008lining,hagstrom2004using,kapli2020phylogenetic,sarkar2010hardware}.

% The computational flexibility of digital evolution experiments provides a unique opportunity to overcome these challenges: designing heritable genome annotations specifically to simplify and strengthen phylogenetic reconstruction efforts.
% For maximum applicability of such a solution, these annotations should be phenotypically neutral heritable instrumentation \citep{stanley2002evolving} that do not affect any encodings for functional genome content.

This work introduces ``hereditary stratigraphy,'' a novel heritable genome annotation system to facilitate post-hoc phylogenetic inference on asexual populations.
This system allows explicit control over trade-offs between space complexity and accuracy of phylogenetic inference.
Instead of modeling genome components undergoing neutral variation through a mutational process, we keep a record of historical checkpoints that allow comparison of two lineages to identify the range of time in which they diverged.

% In Section \ref{sec:methods} we motivate and explain the hereditary stratigraphy approach.
% Then, in Section \ref{sec:results} we simulate post-hoc inference on known phylogenies to assess the quality of phylogenetic reconstruction enabled by the hereditary stratigraphy method.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex-extended-abstract/text/body/methods.tex <==
\section{Methods} \label{sec:methods}

\input{fig/column-comparison.tex}

Our algorithm, particularly the vocabulary we developed to describe it, draws on the concept of geological stratigraphy, inference of natural history through analysis of successive layers of geological material \citep{steno1916prodromus}.
As an introductory intuition, suppose a body of rock being built up through regular, discrete events depositing of geological material.
Note that in such a scenario we could easily infer the age of the body of rock by counting up the number of layers present.
% Note that it is crucial to this scenario that each layer has some differentiating feature that allows it to be distinguished from layers above and below it, but also potentially from layers present in another body of rock in a distant and unrelated geographic position.
Next, imagine making a copy of the rock body in its partially-formed state and then moving it far away.
As time runs forward on these two rock bodies, independent layering processes will cause consistent disparity in the layers forming on each forwards from their point of separation.

To deduce the historical relationship of these rock bodies after the fact, we could simply align and compare their layers.
Layers from their base up through the first disparity would correspond to shared ancestry; further disparate layers would correspond to diverged ancestry.
% Interestingly, and powerfully for phylogenetic inference, we can readily distinguish a scenario where both rock bodies deposited ten layers after diverging from a scenario where one deposited eighteen layers and the other deposited two.
Figure \ref{fig:column-comparison} depicts the process of comparing columns for phylogenetic inference.

Shifting now from intuition to implementation, a fixed-length randomly-generated binary tag provides a convenient and efficient mechanism to differentiate between our metaphorical ``layers.''
% We call this ``fingerprint'' tag a \textit{differentia}.
% The width of this tag controls the probability of spurious collisions between independently generated instances.
% At 64 bits wide the tag essentially functions as a UID: collisions between randomly generated tags are so unlikely ($p < 5.42\times10^{-20}$) they can essentially be ignored.
% At the other end of the spectrum, collision probability would be $1/256$ for a single byte and $1/2$ for a single bit.
% In the case of narrow differentia, in order to set a lower bound for the MRCA generation, you would have to backtrack common strata from the last commonality until the probability of that many successive spurious collisions was enough to satisfy your desired confidence level (e.g., 95\% confidence).
% Even then, there would be a possibility of the the true MRCA falling before the lower bound.
% Note, however, that no matter the width of the differentia the generation of the first discrepancy provides a hard upper bound on the generation of the MRCA.
%
In accordance with our geological analogy, we refer to the packet of data accumulated each generation as a \textit{stratum}.
This packet contains the differentia and, although not employed in this work, could hold other arbitrary user-defined data (i.e., simulation timestamp, phenotype characteristics, etc.).
% Again in accordance with the geological analogy, we refer to the chronological stack of strata that accumulate over successive depositions as a \textit{hereditary stratigraphic column}.

% \subsection{Stratum Retention Policy}

% \input{fig/deposit-process.tex}

As currently stated, fingerprints will accumulate proportionally to the length of evolutionary history simulated.
In an evolutionary run with thousands or millions of generations, this approach would soon become intractable --- particularly when columns are serialized and transmitted between distributed computing elements.
To solve this problem, we can trade off precision for compactness by deleting strata from columns as time progresses.
% Figure \ref{fig:deposit-process} overviews how stratum deposit and stratum elimination progress over two generations under the hereditary stratigraphic column scheme.
%
% Different patterns of deletion will lead to different trade-offs, both in terms of the scaling relationship of column size to generations elapsed and in terms of the arrangement of precision over evolutionary history (i.e., focusing precision on more recent evolutionary history versus spreading it evenly over the entire history).
%
We refer to the rule set used to selectively eliminate strata over time as the ``stratum retention policy.''
We devised three stratum retention policies, which provide
\begin{itemize}
  \item linear space complexity and constant inference error,
  \item constant space complexity and linear inference error with respect to phylogenetic depth, or
  \item logarithmic space complexity and inference error as a constant proportion of time elapsed since MRCA.
\end{itemize}

% We explore several different retention policy designs here, and implement our software to allows for free, modular interchange of retention policies.
% It is possible to define a policy through either of two mechanisms.
% First, policy can be defined as a ``predicate'' where the generation of a stratum and the current number of strata deposited is passed into a function that returns whether that strata should be retained at that point in time.
% Second, policy can be defined as a ``condemner'' generator where, given the current number of strata deposited, the set of ranks that should be deleted at this point in time are yielded.
% Although the predicate form is useful for analyzing and proving properties of policies, the condemner form is generally more efficient in practice.
% We provide predicate and condemner implementations for each stratum retention policy discussed here.

% It should be noted that condemners and predicates are both defined in terms of stratum generation, not stratum index among retained strata in the column.
% Therefore, it may seem necessary to store the generation of deposit within the stratum data structure.
% However, if you know the total number of generations deposited you can map backwards from index to recover the generation deposited without storing it.
% We provide this formula for each stratum retention policy.
% Finally, for each policy we provide a formula to calculate the exact number of strata retained under any parameterization after $n$ generations.
%
% In the next subsections, we introduce several stratum retention policies, provide the intuition behind their implementation, and elaborate their space complexity and resolution properties.
% For each policy, patterns of stratum retention are illustrated in Figure \ref{fig:retention-policies}.
% The formulas for number of strata retained after $n$ generations, the formulas to calculate stratum deposit generation from column index, and the retention predicate specifications of each policy are available in Supplementary Listing \ref{lst:StratumRetentionPredicateDepthProportionalResolution} \citep{moreno2022hstratconceptsupplement}.
% The condemner generator specification of each policy is available in Supplementary Listing \ref{lst:StratumRetentionCondemnerDepthProportionalResolution} \citep{moreno2022hstratconceptsupplement}.
% For tapered depth-proportional resolution and recency-proportional resolution, the accuracy of MRCA estimation can also be explored via an interactive in-browser web applet at \url{https://hopth.ru/bi}.
%
% \input{fig/retention-policies.tex}
%
% \subsection{Fixed Resolution Stratum Retention Policy}
%
% The fixed resolution retention policy provides a fixed absolute upper bound $r$ on the spacing between retained strata.
% The strategy to obtain this property is simple: permanently retain a stratum every $r$th generation
% (although, for arbitrary reasons of implementation convenience we require each stratum to be retained during at least the generation it is deposited).
%
% However, this retention policy suffers from linear growth in a column's memory footprint with respect to number of generations elapsed: every $r$th generation generation a new stratum is permanently retained
% For this reason, it is likely not useful in practice except potentially in scenarios where the number of generations is fixed in advance.
% We include it here largely for illustrative purposes as a gentle introduction to retention policies.
%
% \subsection{Depth-Proportional Resolution Stratum Retention Policy}
%
% The depth-proportional resolution policy ensures spacing between retained strata will be less than or equal to a proportion $r$ of total number of strata deposited.
% Achieving this limit on uncertainty requires retaining sufficient strata so that no more than $r$ ranks elapsed between any two strata.
% This policy accumulates retained strata at a fixed interval until twice as many as $r$ are at hand.
% Then, every other retained stratum is purged and the cycle repeats with a new twice-as-wide interval between retained strata.
%
% When comparing stratigraphic columns from different generations, the resolution guarantee holds in terms of the number of generations experienced by the older of the two columns.
% Because this retention policy is deterministic, for two columns with the same policy, every stratum that is held by the older column is also guaranteed to be present in the younger column (unless it hasn't yet been deposited on the younger column).
% Therefore, the strata that would enable the desired resolution when comparing two columns of the same age are guaranteed to be available.
%
% Because the number of strata retained under this policy is bounded as $2n+1$, space complexity scales as $O(1)$ with respect to the number of strata deposited.
% It follows that the MRCA rank estimate uncertainty scales as $O(n)$ with respect to the number of strata deposited.
%
% \subsection{Tapered Depth-Proportional Resolution Stratum Retention Policy}
%
% This policy refines the depth-proportional resolution policy to provide a more stable column memory footprint over time.
% The naive depth-proportional resolution policy builds up strata until twice as many are present as needed then purges half of them all at once.
% The tapered depth-proportional resolution policy functions identically to the depth-proportional policy except that it removes unnecessary strata gradually from back to front as new strata are deposited, instead of eliminating them simultaneously.
% The column footprint stability of this variation makes it easier to parameterize our experiments to ensure comparable end-state column footprints for fair comparison between retention policies, in addition to making this policy likely better suited to most use cases.
% By design, this policy has the same space complexity and MRCA estimation uncertainty scaling relationships with number generations elapsed as the naive depth-proporitonal resolution policy.
%
% \subsection{MRCA-Recency-Proportional Resolution Stratum Retention Policy}
%
% \input{tab/recency-proportional-space-complexity.tex}
%
% The MRCA-recency-proportional resolution policy ensures distance between the retained strata surrounding any generation point will be less than or equal to a user-specified proportion $r$ of the number of generations elapsed since.
%
% This policy can be constructed recursively, so to begin, let's consider setting up just the \textit{first} generation $g$ of the stratum after the root ancestor we will retain when $n$ generations have elapsed.
% A simple geometric analysis reveals that providing the guaranteed resolution for the worst-case generation within the window between generation 0 and generation $g$ (i.e., generation $g-1$) requires
% \begin{align*}
%   g \leq \lfloor n / (r + 1) \rfloor.
% \end{align*}
%
% We now have an upper bound for the rank of the first stratum generation we must retain.
% However, we must guarantee that these ranks are actually available for us to retain (i.e., it hasn't been purged out of the column at a previous time point as the column was grown by successive deposition).
% We will do this by picking the rank that is the highest power of 2 less than or equal to our bound.
% If we repeat this procedure as we recurse, we are guaranteed that this rank will have been preserved across all previous timepoints.
%
% Why does this work?
% Consider a sequence where all elements are powers of 2 and elements in the sequence are strictly nonincreasing.
% Consider the first element of the list.
% Partial sums along the sequence will include all multiples this first element.
% So, when we ratchet up $g$ to $2g$ as $n$ increases, we are guaranteed that $2g$ has been retained.
% This principle generalizes recursively down the list.
% This is a similar principle to the approach of strictly-doubling interval sizes used in the Naive and Tapered Depth-Proportional Resolution stratum retention policies described above.
%
% This step of truncating to the nearest less than or equal to power of 2 affects our recursive step size at most only by a constant factor of 2.
% So, because step size is a constant fraction of remaining generations $n$ (at worst $\frac{1}{2(r+1)}$), the number of steps made (and number of strata retained) scales as $O(\log(n))$ with respect to the number of strata deposited.
% Table \ref{tab:recency-proportional-space-complexity} provides exact figures for the number of strata retained under different parameterizations of the recency-proportional retention policy between one thousand and one trillion generations.
%
% As for rank estimate uncertainty, in the worst case it scales as $O(n)$ with respect to the greater number of strata deposited.
% However, with respect to estimating the rank of the MRCA when lineages diverged any fixed number of generations ago, uncertainty scales as $O(1)$.
%
% How does space complexity scale with respect to the policy's specified resolution $r$?
% Through extrapolation from OEIS sequences A063787 and A056791 via guess and check \citep{sloane2021a063787,sloane2021a056791}, we posited the exact number of strata retained after $n$ generations as
%
% \begin{align*}
%   \mathrm{HammingWeight}(n)
%   + \sum_1^r \lfloor \log_2( \lfloor n / r \rfloor ) \rfloor
%   + 1.
% \end{align*}
%
% This expression has been unit tested extensively to ensure perfect reliability.
% Approximating and applying logarithmic properties, this policy's space complexity can be calculated within a constant factor as
%
% \begin{align*}
% \log(n) + \log\Big(\frac{n^r}{r!}\Big).
% \end{align*}
%
% To answer our question, we will examine the ratio of space complexities required when scaling resolution $r$ up by a constant factor $f > 1$.
% Evaluating this ratio as $r \to \infty$, we find that space complexity scales directly proportional with the desired resolution $r$ at the limit,
%
% \begin{align*}
% \lim_{r \to \infty}
% \frac{
%   \log(n) + \log\Big(\frac{n^{fr}}{(fr)!}\Big)
% }{
%   \log(n) + \log\Big(\frac{n^r}{r!}\Big)
% }
% = f.
% \end{align*}
%
% Evaluating this ratio as $n \to \infty$, we find that this scaling relationship is never worse than directly proportional for any $r$,
%
% \begin{align*}
% \lim_{n \to \infty}
% \frac{
%   \log(n) + \log\Big(\frac{n^{fr}}{(fr)!}\Big)
% }{
%   \log(n) + \log\Big(\frac{n^r}{r!}\Big)
% }
% &= \frac{fr+1}{r+1}\\
% &= f\frac{r + 1/f}{r + 1}\\
% &\leq f.
% \end{align*}
%
%
% \subsection{Computational Experiments}
%
% These simulations propagated populations of between 100 and 165 bitstrings between 500 and 5,000 synchronous generations under the NK fitness landscape model \citep{kauffman1989nk}.
% In order to ensure coverage of a variety of phylogenetic conditions, we sampled a variety of selection schemes that impose profoundly different ecological regimens \citep{dolson2018ecological},
% \begin{itemize}
%   \item EcoEA Selection \citep{goings2012ecology},
%   \item Lexicase Selection \citep{helmuth2014solving},
%   \item Random Selection,
%   \item Sharing Selection \citep{goldberg1987genetic}
%   % \item Tournament Selection \citep{miller1995genetic}.
% \end{itemize}
%
% Supplementary Table \ref{tab:ground-truth-phylogenies} provides full details on the conditions each ground truth phylogeny was drawn from.
% The phylogenies themselves are available in our data repository for this project.
%
% For each ground truth phylogeny, we tested combinations of three configuration parameters:
% \begin{itemize}
%   \item target end-state memory footprints for extant columns (64, 512, and 4096 bits),
%   \item differentia width (1, 8, and 64 bits), and
%   \item stratum retention policy (tapered depth-proportional resolution and recency-proportional resolution).
% \end{itemize}
%
% Stratum retention policies were parameterized so that the maximum number of strata possible were present at the end of the experiment without exceeding the target memory footprint.
% If the target memory footprint is exceeded by the sparsest possible parameterization of a retention policy, then that sparsest possible parameterization is used.
% Supplementary Tables \cref{tab:experiment-column-sizes-nk-ecoea-selection,tab:experiment-column-sizes-nk-lexicase-selection,tab:experiment-column-sizes-nk-random-selection,tab:experiment-column-sizes-nk-sharing-selection,tab:experiment-column-sizes-nk-tournament-selection} provide the calculated paramaterizations and memory footprints of extant columns \citep{moreno2022hstratconceptsupplement}.
%
% In order to assess the viability of phylogenetic inference using hereditary stratigraphic columns from extant organisms, we used the end-state stratigraphs to estimate a reconstruction of the actual ground truth phylogenetic histories.
% The first step to reconstructing a phylogenetic tree for the history of an extant population at the end of an experiment is to construct a distance matrix by calculating all pairwise phylogenetic distances between extant columns.
% We defined phylogenetic distance between two extant columns as the sum of each extant organism's generational distance back to the generation of their MRCA, estimated as the mean of the upper and lower 95\% confidence bounds.
% Supplementary Figure \ref{fig:phylogenetic-inference} provides a cartoon summary of the process of calculating phylogenetic distance between two extant columns \citep{moreno2022hstratconceptsupplement}.
%
% We then used the unweighted pair group method with arithmetic mean (UPGMA) reconstruction tool provided by the BioPython package to generate estimate phylogenetic trees \citep{cock2009biopython,sokal1958statistical}.
% After generating the reconstructed tree topology, we performed a second pass to adjust branch lengths so that each tree node sat at the mean of its estimated 95\% confidence generation bounds.
% %We found that the neighbor joining (NJ) approach occasionally yielded reconstructions with impossible ``negative generation'' branches \citep{saitou1987neighbor} after knowledge bounding the absolute generation of internal nodes (i.e., MRCA's between pairs of extant organisms) was applied, so we did not use it.
%
% \subsection{Software and Data}
%
% % A prototype of this approach has been implemented \url{https://github.com/mmore500/dishtiny/blob/incoming/include/dish2/genome/PhyloFingerprints.hpp} and preliminarily tested \url{https://github.com/mmore500/dishtiny/blob/incoming/tests/dish2/genome/PhyloFingerprints.cpp}.
%
% As part of this work, we published the \texttt{hstrat} Python library with a stable public-facing API intended to enable incorporation in other projects with extensive documentation and unit testing on GitHub at \url{https://anonymous.4open.science/r/hstrat-115D/} and on PyPI.% at \url{https://pypi.org/project/hstrat/}. https://github.com/mmore500/hstrat
% In the near future, we intend to complete and publish a corresponding C++ library.
%
% Supporting software materials can be found on GitHub at \url{https://anonymous.4open.science/r/hereditary-stratigraph-concept-6BEC/}.%\url{https://github.com/mmore500/hereditary-stratigraph-concept}
% Supporting computational notebooks are available for in-browser use via BinderHub at \url{ANONYMIZED FOR PEER REVIEW} \citep{ragan2018binder}. %https://mybinder.org/v2/gh/mmore500/hereditary-stratigraph-concept/HEAD?labpath=binder%2F
% Our work benefited from many pieces of open source scientific software, including \citep{sukumaran2010dendropy,virtanen2020scipy,hunter2007matplotlib,virtanen2020scipy,waskom2021seaborn,bostock2011d3,meurer2017sympy,smith2020treedistdata,paradis2004ape,ushey2022reticulate,wickham2022dplyr}.
% The ground truth phylogenies used in this work as well as supplementary figures, tables, and text are available via the Open Science Framework at
% \url{https://osf.io/4sm72/?view\_only=69f37c6d184143b7855299c3323749ea} \citep{foster2017open,moreno2022hstratconceptsupplement}.
% Phylogenetic data associated with this project is stored in the Alife Community Data Standards format \citep{lalejini2019data}.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex-extended-abstract/text/body/results-and-discussion.tex <==
\section{Results} \label{sec:results}

In order to assess the practical performance of the hereditary stratigraph approach in an applied setting, we simulated the process of stratigraph propagation over known ``ground truth'' phylogenies extracted from pre-existing digital evolution simulations \citep{hernandez2022phylogenetic}.
Across ground truth phylogenies, we were able to reconstruct the phylogenetic topology with between 47.75\% and 85.70\% of the information contained in the original tree using a 64-bit column memory footprint, between 47.75\% and 80.36\% using a 512-bit column memory footprint, and between 51.13\% and 83.53\% using a 4096-bit column memory footprint.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex-extended-abstract/text/frontmatter.tex <==
\title{ Hereditary Stratigraphy: Genome Annotations to Enable Phylogenetic Inference over Distributed Populations }

%%
%% The "author" command and its associated commands are used to define
%% the authors and their affiliations.
%% Of note is the shared affiliation of the first two authors, and the
%% "authornote" and "authornotemark" commands
%% used to denote shared contribution to the research.
\author{Matthew Andres Moreno}
\orcid{0000-0003-4726-4479}
\affiliation{%
  \institution{Michigan Statue University}
  \city{East Lansing}
  \state{Michigan}
  \country{USA}
  \postcode{48103}
}

\author{Emily Dolson}
% \email{dolsonem@msu.edu}
\orcid{0000-0001-8616-4898}
\affiliation{%
  \institution{Michigan Statue University}
  \city{East Lansing}
  \state{Michigan}
  \country{USA}
  \postcode{48103}
}

\author{Charles Ofria}
% \email{ofria@msu.edu}
\orcid{0000-0003-2924-1732}
\affiliation{%
  \institution{Michigan Statue University}
  \city{East Lansing}
  \state{Michigan}
  \country{USA}
  \postcode{48103}
}


%%
%% By default, the full list of authors will be used in the page
%% headers. Often, this list is too long, and will overlap
%% other information printed in the page headers. This command allows
%% the author to define a more concise list
%% of authors' names for this purpose.
\renewcommand{\shortauthors}{Moreno et al.}

\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10010147.10010341.10010366.10010369</concept_id>
       <concept_desc>Computing methodologies~Simulation tools</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10010147.10010257.10010293.10011809.10011812</concept_id>
       <concept_desc>Computing methodologies~Genetic algorithms</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Computing methodologies~Simulation tools}
\ccsdesc[500]{Computing methodologies~Genetic algorithms}

\keywords{phylogenetics, decentralized algorithms, digital evolution, genetic algorithms, genetic programming}

\input{text/abstract.tex}

\maketitle


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex-extended-abstract/text/references.tex <==
% \section*{References}

\putbib


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/draft.tex <==
\def\mydraft{
\usepackage{draftwatermark}
\usepackage{lineno}
\linenumbers
\renewcommand{\linenumberfont}{\normalfont\small\color{red}}
}
\input{main.tex}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/fig/cid_plot.tex <==
\begin{figure}
    \includegraphics[width=\columnwidth]{img/cid_plot}
    \caption{
    Reconstruction error for phylogenetic inference with ground truth sharing selection phylogeny.
    Lower is better.
    RPR is recency-proportional resolution policy and TDPR is tapered depth-proportional resolution policy.
    }
  \label{fig:cid_plot}
\end{figure}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/fig/column-comparison.tex <==
\begin{figure}
    \includegraphics[width=\columnwidth]{img/column-comparison}
    \caption{
    Inferring the generation of the most-recent common ancestor (MRCA) of two hereditary stratigraphic columns ``$A$'' and ``$B$''.
    Columns are aligned at corresponding generations.
    Then the first generation with disparate ``fingerprints'' is determined.
    % (If a particular generation's strata have been eliminated from one or both columns or have not yet been deposited on one column, then no comparison is performed at that generation.)
    This provides a hard upper bound on the generation of the MRCA: these strata \textit{must} have been deposited along separate lines of descent.
    Searching backward for the first commonality preceding that disparity provides a soft lower bound on the generation of the MRCA: these strata evidence common ancestry but \textit{might} collide by chance.
    Some strata mmay have been eliminated from the columns, as shown, in order to save space at the cost of increasing uncertainty of MRCA generation estimates.
    % (If a narrow ``fingerprint'' differentia like a single bit is used with plausible collision probability, a lower bound can be established by continuing to search backward until the probability of $k$ successive spurious collisions is sufficiently unlikely.)
    % This process yields certainty about the phylogenetic relationship between $A$ and $B$ shown at right above (i.e., common) and below (i.e., diverged) the MRCA bounds.
    }
  \label{fig:column-comparison}
\end{figure}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/fig/deposit-process.tex <==
\begin{figure*}
  \begin{minipage}{0.6\textwidth}
    \includegraphics[width=\textwidth]{img/deposit-process}
  \end{minipage}%
  \begin{minipage}{0.4\textwidth}
    \caption{
    Cartoon illustration of stratum deposit process.
    This process marks the elapse of a generation when a hereditary stratigraphic column is inherited by an offspring.
    First, a new stratum is appended to the end of the column with a randomly-generated ``fingerprint.''
    This ``fingerprint'' distinguishes strata that were generated along disparate lines of descent (e.g., \texttt{0xd01a} for 3rd Generation A and \texttt{0xe74a} for 3rd generation B).
    Then, the column's configured stratum retention policy is applied to ``prune'' the column by eliminating strata from specific generations.
    Although this cartoon depicts an empty space for eliminated strata, the underlying data structure behind a column (i.e., the pink overlay) can condense to reduce space complexity.
    }\label{fig:deposit-process}
  \end{minipage}
\end{figure*}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/fig/info_plot.tex <==
\begin{figure}
    \includegraphics[width=\columnwidth]{img/info_plot}
    \caption{
    Proportion of information present in the ground-truth ftness sharing phylogeny that was captureed by our reconstruction, across various retention policies.
    High is better (1 is perfect).
    RPR is recency-proportional resolution policy and TDPR is tapered depth-proportional resolution policy.
    } \label{fig:info_plot}
\end{figure}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/fig/phylogenetic-inference.tex <==
\begin{figure*}
  \centering
    \includegraphics[width=\textwidth]{img/phylogenetic-inference}
    \caption{
    Cartoon illustration of column inheritance along a phylogenetic tree and the process to infer phylogenetic history along extant columns.
    This scenario supposes a stratum retention policy where only strata from even generations are retained.
    The common ancestor of the focal clade, which is at generation 2, is shown at top.
    Generation 3 columns inherit that ancestor's strata and each append a new stratum.
    Generation 4 columns append another new stratum then eliminate their generation 3 strata.
    Finally, another generation elapses to yield generation 5 strata.
    Suppose that only generation 5 strata are extant.
    So, greyed-out columns above are not directly observable.
    Phylogenetic history is deduced by pairwise comparison between extant columns.
    For each pair (like the example highlighted in red) a phylogenetic distance can be computed as the sum generations elapsed to each extant column after the estimated generation of their MRCA.
    These pairwise distances can then be fed into a phylogeny reconstruction algorithm.
    }
  \label{fig:phylogenetic-inference}
\end{figure*}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/fig/reconstruction-example.tex <==
\input{lib/importpath.tex}

\begin{figure*}%
%-------------------------------------------------------------------------------
  \begin{subfigure}[b]{0.33\linewidth}
    \centering
    % pass an arbitrary filename, potentially with unsafe characters
    % adapted from https://tex.stackexchange.com/a/36178
    \catcode`\%=12
    \providecommand\filename{}
    \renewcommand\filename{\detokenize{submodules/hereditary-stratigraph-concept/binder/phylogenetic-inference/teeplots/a=true_phylogeny+source=a%reconstructed_phylogenies~source%nk_lexicaseselection_seed110_pop165_mut.01_snapshot_500.csv.gz+viz=draw+ext=}}
    \catcode`\%=14
    \includegraphics[width=\linewidth]{\importpath\filename}
    \caption{Ground truth phylogeny.}
    \label{fig:reconstruction-example-true-phylogeny}
  \end{subfigure}%
%-------------------------------------------------------------------------------
  \begin{subfigure}[b]{0.33\linewidth}
    \centering
    % pass an arbitrary filename, potentially with unsafe characters
    % adapted from https://tex.stackexchange.com/a/36178
    \catcode`\%=12
    \providecommand\filename{}
    \renewcommand\filename{\detokenize{submodules/hereditary-stratigraph-concept/binder/phylogenetic-inference/teeplots/source=a%reconstructed_phylogenies~source%nk_lexicaseselection_seed110_pop165_mut.01_snapshot_500.csv.gz+treatment=differentia%1~policy%TaperedDepthProportionalResolution~target%64+viz=draw-biopython-tree-with-origin-time-bounds+ext=}}
    \catcode`\%=14
    \includegraphics[width=\linewidth]{\importpath\filename}
    \caption{1-bit Fingerprint Differentia, Tapered Depth-Proportional Resolution Stratum Retention Predicate, 64 bit target column footprint.}
    \label{fig:reconstruction-example-d1-rp-t64}
  \end{subfigure}%
%-------------------------------------------------------------------------------
  \begin{subfigure}[b]{0.33\linewidth}
    \centering
    % pass an arbitrary filename, potentially with unsafe characters
    % adapted from https://tex.stackexchange.com/a/36178
    \catcode`\%=12
    \providecommand\filename{}
    \renewcommand\filename{\detokenize{submodules/hereditary-stratigraph-concept/binder/phylogenetic-inference/teeplots/source=a%reconstructed_phylogenies~source%nk_lexicaseselection_seed110_pop165_mut.01_snapshot_500.csv.gz+treatment=differentia%1~policy%RecencyProportionalResolution~target%64+viz=draw-biopython-tree-with-origin-time-bounds+ext=}}
    \catcode`\%=14
    \includegraphics[width=\textwidth]{\importpath\filename}
    \caption{1-bit Fingerprint Differentia, MRCA-Recency-Proportional Resolution Stratum Retention Predicate, 64 bit target column footprint.}
    \label{fig:reconstruction-example-d1-tdp-t64}
  \end{subfigure}
%-------------------------------------------------------------------------------
  \caption{
    Example phylogeny reconstructions of ground-truth lexicase selection phylogeny from inference on extant hereditary stratigraphic columns.
    Shaded error bars on reconstructions indicate 95\% confidence intervals for the true generation of tree nodes.
    Arbitrary color is added to enhance distinguishability.
  }
  \label{fig:reconstruction-example}
\end{figure*}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/fig/retention-policies.tex <==
\input{lib/dissertationelse.tex}
\input{lib/dissertationonly.tex}

\begin{figure*}
  \centering
  \dissertationonly{\footnotesize}
  \begin{tabular}{m{0.05\textwidth}@{}|c@{}|c@{\hskip 0.01\textwidth}|m{0.14\textwidth}}
%-------------------------------------------------------------------------------
\hspace{-1ex}Policy&Lower-Resolution Parameterization&Higher-Resolution Parameterization&\makecell[c]{Properties}\\\hline
%-------------------------------------------------------------------------------
    \rotatebox{90}{\textbf{Fixed Resolution}}
  &
    \makecell{
      \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept/binder/retention-policies/teeplots/fixed_resolution=512+num_layers=1024+stratum_retention_predicate=fixed-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
    \makecell{
      \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept/binder/retention-policies/teeplots/fixed_resolution=128+num_layers=1024+stratum_retention_predicate=fixed-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
  \makecell[{{p{0.14\textwidth}}}]{
  \centering
    \bf{Space Complexity}\\
    $O(n)$\\
    \bf{MRCA Uncertainty}\\
    $O(1)$
  }
  \makecell[{{p{0.14\textwidth}}}]{
  \raggedright
    where $n$ is gens elapsed.
  }\\\hline
%-------------------------------------------------------------------------------
    \adjustbox{
      minipage=10em,
      rotate=90,
    }{
      \centering
      \textbf{Depth-Proportional Resolution}
      \par
    }
  &
    \makecell{
      \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept/binder/retention-policies/teeplots/guaranteed_depth_proportional_resolution=1+num_layers=1024+stratum_retention_predicate=depth-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
    \makecell{
      \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept/binder/retention-policies/teeplots/guaranteed_depth_proportional_resolution=4+num_layers=1024+stratum_retention_predicate=depth-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
  \makecell[{{p{0.14\textwidth}}}]{
  \centering
    \bf{Space Complexity}\\
    $O(1)$\\
    \bf{MRCA Uncertainty}\\
    $O(n)$
  }
  \makecell[{{p{0.14\textwidth}}}]{
  \raggedright
    where $n$ is gens elapsed.
  }\\\hline
%-------------------------------------------------------------------------------
    \adjustbox{
      minipage=15em,
      rotate=90,
    }{
      \centering
      \textbf{Tapered Depth-Proportional Resolution}
      \par
    }
  &
    \makecell{
      \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept/binder/retention-policies/teeplots/guaranteed_depth_proportional_resolution=1+num_layers=1024+stratum_retention_predicate=tapered-depth-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
    \makecell{
      \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept/binder/retention-policies/teeplots/guaranteed_depth_proportional_resolution=4+num_layers=1024+stratum_retention_predicate=tapered-depth-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
  \makecell[{{p{0.14\textwidth}}}]{
  \centering
    \bf{Space Complexity}\\
    $O(1)$\\
    \bf{MRCA Uncertainty}\\
    $O(n)$
  }
  \makecell[{{p{0.14\textwidth}}}]{
  \raggedright
    where $n$ is gens elapsed.
  }\\\hline
%-------------------------------------------------------------------------------
  \adjustbox{
    minipage=15em,
    rotate=90,
  }{
    \centering
    \textbf{Recency-Proportional\\Resolution}
    \par
  }
  &
  \makecell{
    \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept/binder/retention-policies/teeplots/guaranteed_mrca_recency_proportional_resolution=0+num_layers=1024+stratum_retention_predicate=recency-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
  }
  &
  \makecell{
    \includegraphics[valign=t,width=\dissertationelse{0.3}{0.4}\textwidth]{submodules/hereditary-stratigraph-concept/binder/retention-policies/teeplots/guaranteed_mrca_recency_proportional_resolution=4+num_layers=1024+stratum_retention_predicate=recency-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
  }
  &
  \makecell[{{p{0.14\textwidth}}}]{
  \centering
  \bf{Space Complexity}\\
  $O(\log(n))$\\
  \bf{MRCA Uncertainty}\\
  $O(m)$
  }
  \makecell[{{p{0.14\textwidth}}}]{
  \raggedright
  where $m$ is gens since MRCA and $n$ is total gens elapsed.
  }\\


  \end{tabular}
  \caption{
  Comparison of stratum retention policies.
  Policy visualizations show retained strata in black.
  Time progresses along the $y$-axis from top to bottom.
  New strata are introduced along the diagonal and then ``drip'' downward as a vertical line until eliminated.
  The set of retained strata present within a column at a particular generation $g$ can be read as intersections of retained vertical lines with a horizontal line with intercept $g$.
  Policy visualizations are provided for two parameterizations for each policy: the first where the maximum uncertainty of MRCA generation estimates would be 512 generations and the second where the maximum uncertainty of MRCA generation estimates would be 128 generations.
  }
  \label{fig:retention-policies}
\end{figure*}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/lib/dependencies.tex <==
\usepackage{natbib,alifeconf}  %% The order is important

\usepackage[export]{adjustbox}
\usepackage{algorithmic}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{array}
\usepackage{bibunits}
\usepackage{booktabs}
\usepackage{caption}
\usepackage{cite}
\usepackage{colortbl}
\usepackage{csvsimple}
\usepackage{etoolbox}
\usepackage[T1]{fontenc} % adapted from https://tex.stackexchange.com/a/388208
\usepackage{graphicx}
\usepackage{hyperref,cleveref}
\usepackage{ifthen}
\usepackage{import}
\usepackage{listings}
\usepackage{makecell}
\usepackage{multirow}
\usepackage{natbib}
\usepackage[section]{placeins}
\usepackage{pythonhighlight}
\usepackage{rotating}
\usepackage{siunitx}
\usepackage{stringstrings}
\usepackage{subcaption}
\usepackage{tabularx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{xfp}
\usepackage{xparse}
\usepackage{xstring}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/lib/dissertationelse.tex <==
% \pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\providecommand{\dissertationelse}[2]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION
#1
\else
#2
\fi
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/lib/dissertationexclude.tex <==
% \pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\providecommand{\dissertationexclude}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION
\else
#1
\fi
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/lib/dissertationonly.tex <==
% \pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\providecommand{\dissertationonly}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION%
#1%
\else%
\fi
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/lib/importpath.tex <==
% \pragmaonce

% adapted from https://tex.stackexchange.com/a/17491
\makeatletter
  \providecommand\importpath{\import@path}
\makeatother


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/lib/pragmaonce.tex <==
% pragma once, adapted from https://tex.stackexchange.com/a/195173
\makeatletter
\let\pragma@iinput=\@iinput
\def\@iinput#1{\xdef\@pragmafile{#1}\pragma@iinput{#1} }
\def\@pragmafile{default}
\def\pragmaonce{%
   \csname pragma@\@pragmafile\endcsname
   \global\expandafter\let \csname pragma@\@pragmafile\endcsname = \endinput
}
\makeatother


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/lib/safepercent.tex <==
% \pragmaonce

% adapted from https://tex.stackexchange.com/a/351125
\catcode`\%=12
\providecommand\safepercent{%}
\catcode`\%=14


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/lib/safetilde.tex <==
% \pragmaonce

% adapted from https://tex.stackexchange.com/a/425957
\providecommand\safetilde{\string~}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/lst/StratumRetentionCondemnerDepthProportionalResolution.tex <==
{\onecolumn
\lstinputlisting[%
language=Python,
caption={
  Depth-proportional resolution policy condemner implementation.
},
label={lst:StratumRetentionCondemnerDepthProportionalResolution},
style=mypython,
basicstyle=\scriptsize,
]{submodules/hstrat/hstrat/hstrat/stratum_retention_condemners/StratumRetentionCondemnerDepthProportionalResolution.py}
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/lst/StratumRetentionCondemnerFixedResolution.tex <==
{\onecolumn
\lstinputlisting[%
language=Python,
caption={
  Fixed resolution policy condemner implementation.
},
label={lst:StratumRetentionCondemnerFixedResolution},
style=mypython,
basicstyle=\scriptsize,
]{submodules/hstrat/hstrat/hstrat/stratum_retention_condemners/StratumRetentionCondemnerFixedResolution.py}
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/lst/StratumRetentionCondemnerRecencyProportionalResolution.tex <==
{\onecolumn
\lstinputlisting[%
language=Python,
caption={
  MRCA-recency-proportional resolution policy condemner implementation.
},
label={lst:StratumRetentionCondemnerRecencyProportionalResolution},
style=mypython,
basicstyle=\scriptsize,
]{submodules/hstrat/hstrat/hstrat/stratum_retention_condemners/StratumRetentionCondemnerRecencyProportionalResolution.py}
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/lst/StratumRetentionCondemnerTaperedDepthProportionalResolution.tex <==
{\onecolumn
\lstinputlisting[%
language=Python,
caption={
  Tapered depth-proportional resolution policy condemner implementation.
},
label={lst:StratumRetentionCondemnerTaperedDepthProportionalResolution},
style=mypython,
basicstyle=\scriptsize,
]{submodules/hstrat/hstrat/hstrat/stratum_retention_condemners/StratumRetentionCondemnerTaperedDepthProportionalResolution.py}
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/lst/StratumRetentionPredicateDepthProportionalResolution.tex <==
{\onecolumn
\lstinputlisting[%
language=Python,
caption={
  Depth-proportional resolution policy predicate implementation, including method to calculate exact number of strata retained by generation and method to calculate stratum deposition rank from column index.
},
label={lst:StratumRetentionPredicateDepthProportionalResolution},
style=mypython,
basicstyle=\scriptsize,
]{submodules/hstrat/hstrat/hstrat/stratum_retention_predicates/StratumRetentionPredicateDepthProportionalResolution.py}
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/lst/StratumRetentionPredicateFixedResolution.tex <==
{\onecolumn
\lstinputlisting[%
language=Python,
caption={
  Fixed resolution policy predicate implementation, including method to calculate exact number of strata retained by generation and method to calculate stratum deposition rank from column index.
},
label={lst:StratumRetentionPredicateFixedResolution},
style=mypython,
basicstyle=\scriptsize,
]{submodules/hstrat/hstrat/hstrat/stratum_retention_predicates/StratumRetentionPredicateFixedResolution.py}
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/lst/StratumRetentionPredicateRecencyProportionalResolution.tex <==
{\onecolumn
\lstinputlisting[%
language=Python,
caption={
  MRCA-recency-proportional resolution policy predicate implementation, including method to calculate exact number of strata retained by generation and method to calculate stratum deposition rank from column index.
},
label={lst:StratumRetentionPredicateRecencyProportionalResolution},
style=mypython,
basicstyle=\scriptsize,
]{submodules/hstrat/hstrat/hstrat/stratum_retention_predicates/StratumRetentionPredicateRecencyProportionalResolution.py}
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/lst/StratumRetentionPredicateTaperedDepthProportionalResolution.tex <==
{\onecolumn
\lstinputlisting[%
language=Python,
caption={
  Tapered depth-proportional resolution policy predicate implementation, including method to calculate exact number of strata retained by generation and method to calculate stratum deposition rank from column index.
},
label={lst:StratumRetentionPredicateTaperedDepthProportionalResolution},
style=mypython,
basicstyle=\scriptsize,
]{submodules/hstrat/hstrat/hstrat/stratum_retention_predicates/StratumRetentionPredicateTaperedDepthProportionalResolution.py}
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/draft.tex <==
\def\mydraft{
\usepackage{draftwatermark}
\usepackage{lineno}
\linenumbers
\renewcommand{\linenumberfont}{\normalfont\small\color{red}}
}
\input{main.tex}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/fig/column-comparison.tex <==
\begin{figure}
    \includegraphics[width=\columnwidth]{img/column-comparison}
    \caption{
    Cartoon illustration of process to infer the generation of the most-recent common ancestor (MRCA) of two hereditary stratigraphic columns $A$ and $B$.
    Columns are aligned so that strata deposited at corresponding generations can be compared.
    Then, the first generation with disparate ``fingerprints'' is determined.
    (If a particular generation's strata have been eliminated from one or both columns or have not yet been deposited on one column, then no comparison is performed at that generation.)
    This provides a hard upper bound on the generation of the MRCA: these strata \textit{must} have been deposited along separate lines of descent.
    Then, searching backward for first commonality preceding that disparity provides a soft lower bound on the generation of the MRCA: these strata evidence common ancestry but \textit{might} collide by chance.
    (If a narrow ``fingerprint'' differentia like a single bit is used with plausible collision probability, a lower bound can be established by continuing to search backward until the probability of $k$ successive spurious collisions is sufficiently unlikely.)
    This process yields certainty about the phylogenetic relationship between $A$ and $B$ shown at right above (i.e., common) and below (i.e., diverged) the MRCA bounds.
    }
  \label{fig:column-comparison}
\end{figure}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/fig/deposit-process.tex <==
\begin{figure*}
  \begin{minipage}{0.6\textwidth}
    \includegraphics[width=\textwidth]{img/deposit-process}
  \end{minipage}%
  \begin{minipage}{0.4\textwidth}
    \caption{
    Cartoon illustration of stratum deposit process.
    This process marks the elapse of a generation when a hereditary stratigraphic column is inherited by an offspring.
    First, a new stratum is appended to the end of the column with a randomly-generated ``fingerprint.''
    This ``fingerprint'' distinguishes strata that were generated along disparate lines of descent (e.g., \texttt{0xd01a} for 3rd Generation A and \texttt{0xe74a} for 3rd generation B).
    Then, the column's configured stratum retention policy is applied to ``prune'' the column by eliminating strata from specific generations.
    Although this cartoon depicts an empty space for eliminated strata, the underlying data structure behind a column (i.e., the pink overlay) can condense to reduce space complexity.
    }
  \end{minipage}
  \label{fig:deposit-process}
\end{figure*}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/fig/phylogenetic-inference.tex <==
\begin{figure*}
  \centering
    \includegraphics[width=\textwidth]{img/phylogenetic-inference}
    \caption{
    Cartoon illustration of column inheritance along a phylogenetic tree and the process to infer phylogenetic history along extant columns.
    This scenario supposes a stratum retention policy where only strata from even generations are retained.
    The common ancestor of the focal clade, which is at generation 2, is shown at top.
    Generation 3 columns inherit that ancestor's strata and each append a new stratum.
    Generation 4 columns append another new stratum then eliminate their generation 3 strata.
    Finally, another generation elapses to yield generation 5 strata.
    Suppose that only generation 5 strata are extant.
    So, greyed-out columns above are not directly observable.
    Phylogenetic history is deduced by pairwise comparison between extant columns.
    For each pair (like the example highlighted in red) a phylogenetic distance can be computed as the sum generations elapsed to each extant column after the estimated generation of their MRCA.
    These pairwise distances can then be fed into a phylogeny reconstruction algorithm.
    }
  \label{fig:phylogenetic-inference}
\end{figure*}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/fig/retention-policies.tex <==
\begin{figure*}
  \centering
  \begin{tabular}{m{0.05\textwidth}@{}|c@{}|c@{\hskip 0.01\textwidth}|m{0.14\textwidth}}
%-------------------------------------------------------------------------------
\hspace{-1ex}Policy&Lower-Resolution Parameterization&Higher-Resolution Parameterization&\makecell[c]{Properties}\\\hline
%-------------------------------------------------------------------------------
    \rotatebox{90}{\textbf{Fixed Resolution}}
  &
    \makecell{
      \includegraphics[valign=t,width=0.4\textwidth]{submodules/hereditary-stratigraph-concept/binder/retention-policies/teeplots/fixed_resolution=512+num_layers=1024+stratum_retention_predicate=fixed-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
    \makecell{
      \includegraphics[valign=t,width=0.4\textwidth]{submodules/hereditary-stratigraph-concept/binder/retention-policies/teeplots/fixed_resolution=128+num_layers=1024+stratum_retention_predicate=fixed-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
  \makecell[{{p{0.14\textwidth}}}]{
  \centering
    \bf{Space Complexity}\\
    $O(n)$\\
    \bf{MRCA Uncertainty}\\
    $O(1)$
  }
  \makecell[{{p{0.14\textwidth}}}]{
  \raggedright
    where $n$ is gens elapsed.
  }\\\hline
%-------------------------------------------------------------------------------
    \adjustbox{
      minipage=10em,
      rotate=90,
    }{
      \centering
      \textbf{Depth-Proportional Resolution}
      \par
    }
  &
    \makecell{
      \includegraphics[valign=t,width=0.4\textwidth]{submodules/hereditary-stratigraph-concept/binder/retention-policies/teeplots/guaranteed_depth_proportional_resolution=1+num_layers=1024+stratum_retention_predicate=depth-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
    \makecell{
      \includegraphics[valign=t,width=0.4\textwidth]{submodules/hereditary-stratigraph-concept/binder/retention-policies/teeplots/guaranteed_depth_proportional_resolution=4+num_layers=1024+stratum_retention_predicate=depth-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
  \makecell[{{p{0.14\textwidth}}}]{
  \centering
    \bf{Space Complexity}\\
    $O(1)$\\
    \bf{MRCA Uncertainty}\\
    $O(n)$
  }
  \makecell[{{p{0.14\textwidth}}}]{
  \raggedright
    where $n$ is gens elapsed.
  }\\\hline
%-------------------------------------------------------------------------------
    \adjustbox{
      minipage=15em,
      rotate=90,
    }{
      \centering
      \textbf{Tapered Depth-Proportional Resolution}
      \par
    }
  &
    \makecell{
      \includegraphics[valign=t,width=0.4\textwidth]{submodules/hereditary-stratigraph-concept/binder/retention-policies/teeplots/guaranteed_depth_proportional_resolution=1+num_layers=1000+stratum_retention_predicate=tapered-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
    \makecell{
      \includegraphics[valign=t,width=0.4\textwidth]{submodules/hereditary-stratigraph-concept/binder/retention-policies/teeplots/guaranteed_depth_proportional_resolution=4+num_layers=1000+stratum_retention_predicate=tapered-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
  \makecell[{{p{0.14\textwidth}}}]{
  \centering
    \bf{Space Complexity}\\
    $O(1)$\\
    \bf{MRCA Uncertainty}\\
    $O(n)$
  }
  \makecell[{{p{0.14\textwidth}}}]{
  \raggedright
    where $n$ is gens elapsed.
  }\\\hline
%-------------------------------------------------------------------------------
  \adjustbox{
    minipage=15em,
    rotate=90,
  }{
    \centering
    \textbf{Recency-Proportional\\Resolution}
    \par
  }
  &
  \makecell{
    \includegraphics[valign=t,width=0.4\textwidth]{submodules/hereditary-stratigraph-concept/binder/retention-policies/teeplots/guaranteed_mrca_recency_proportional_resolution=0+num_layers=1024+stratum_retention_predicate=recency-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
  }
  &
  \makecell{
    \includegraphics[valign=t,width=0.4\textwidth]{submodules/hereditary-stratigraph-concept/binder/retention-policies/teeplots/guaranteed_mrca_recency_proportional_resolution=4+num_layers=1024+stratum_retention_predicate=recency-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
  }
  &
  \makecell[{{p{0.14\textwidth}}}]{
  \centering
  \bf{Space Complexity}\\
  $O(\log(n))$\\
  \bf{MRCA Uncertainty}\\
  $O(m)$
  }
  \makecell[{{p{0.14\textwidth}}}]{
  \raggedright
  where $m$ is gens since MRCA and $n$ is total gens elapsed.
  }\\


  \end{tabular}
  \caption{
  Comparison of stratum retention policies.
  Policy visualizations show retained strata in black.
  Time progresses along the $y$-axis from top to bottom.
  New strata are introduced along the diagonal and then ``drip'' downward as a vertical line until eliminated.
  The set of retained strata present within a column at a particular generation $g$ can be read as intersections of retained vertical lines with a horizontal line with intercept $g$.
  Policy visualizations are provided for two parameterizations for each policy: the first where the maximum uncertainty of MRCA generation estimates would be 512 generations and the second where the maximum uncertainty of MRCA generation estimates would be 128 generations.
  }
  \label{fig:retention-policies}
\end{figure*}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/lib/dependencies.tex <==
\usepackage{natbib,alifeconf}  %% The order is important

\usepackage[export]{adjustbox}
\usepackage{algorithmic}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{array}
\usepackage{bibunits}
\usepackage{booktabs}
\usepackage{caption}
\usepackage{cite}
\usepackage{csvsimple}
\usepackage{etoolbox}
\usepackage{graphicx}
\usepackage{hyperref}
\usepackage{import}
\usepackage{makecell}
\usepackage{multirow}
\usepackage{natbib}
\usepackage{rotating}
\usepackage{siunitx}
\usepackage{subcaption}
\usepackage{tabularx}
\usepackage{textcomp}
\usepackage{xcolor}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/lib/dissertationexclude.tex <==
\pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\newcommand{\dissertationexclude}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION
\else
#1
\fi
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/lib/dissertationonly.tex <==
\pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\newcommand{\dissertationonly}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION%
#1%
\else%
\fi
asdf
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/lib/importpath.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/17491
\makeatletter
  \def\importpath{\import@path}
\makeatother


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/lib/pragmaonce.tex <==
% pragma once, adapted from https://tex.stackexchange.com/a/195173
\makeatletter
\let\pragma@iinput=\@iinput
\def\@iinput#1{\xdef\@pragmafile{#1}\pragma@iinput{#1} }
\def\@pragmafile{default}
\def\pragmaonce{%
   \csname pragma@\@pragmafile\endcsname
   \global\expandafter\let \csname pragma@\@pragmafile\endcsname = \endinput
}
\makeatother


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/lib/safepercent.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/351125
\catcode`\%=12
\newcommand\safepercent{%}
\catcode`\%=14


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/lib/safetilde.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/425957
\newcommand\safetilde{\string~}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/draft.tex <==
\def\mydraft{
\usepackage{draftwatermark}
\usepackage{lineno}
\linenumbers
\renewcommand{\linenumberfont}{\normalfont\small\color{red}}
}
\input{main.tex}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/lib/dependencies.tex <==
\usepackage{adjustbox}
\usepackage{algorithmic}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{array}
\usepackage{bibunits}
\usepackage{booktabs}
\usepackage{caption}
\usepackage{cite}
\usepackage{csvsimple}
\usepackage{etoolbox}
\usepackage{graphicx}
\usepackage{hyperref}
\usepackage{import}
\usepackage{natbib}
\usepackage{siunitx}
\usepackage{subcaption}
\usepackage{textcomp}
\usepackage{xcolor}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/lib/dissertationexclude.tex <==
\pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\newcommand{\dissertationexclude}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION
\else
#1
\fi
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/lib/dissertationonly.tex <==
\pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\newcommand{\dissertationonly}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION%
#1%
\else%
\fi
asdf
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/lib/importpath.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/17491
\makeatletter
  \def\importpath{\import@path}
\makeatother


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/lib/pragmaonce.tex <==
% pragma once, adapted from https://tex.stackexchange.com/a/195173
\makeatletter
\let\pragma@iinput=\@iinput
\def\@iinput#1{\xdef\@pragmafile{#1}\pragma@iinput{#1} }
\def\@pragmafile{default}
\def\pragmaonce{%
   \csname pragma@\@pragmafile\endcsname
   \global\expandafter\let \csname pragma@\@pragmafile\endcsname = \endinput
}
\makeatother


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/lib/safepercent.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/351125
\catcode`\%=12
\newcommand\safepercent{%}
\catcode`\%=14


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/lib/safetilde.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/425957
\newcommand\safetilde{\string~}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/text/acknowledgement.tex <==
\section*{Acknowledgment}

This research was supported in part by NSF grants DEB-1655715 and DBI-0939454 as well as by Michigan State University through the computational resources provided by the Institute for Cyber-Enabled Research.
This material is based upon work supported by the National Science Foundation Graduate Research Fellowship under Grant No. DGE-1424871.
Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the National Science Foundation.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/text/body.tex <==
\input{text/body/abstract.tex}

\input{text/body/introduction.tex}

\input{text/body/methods.tex}

\input{text/body/results-and-discussion.tex}

\input{text/body/conclusion.tex}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/text/body/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/text/body/introduction.tex <==
\section{Introduction} \label{sec:introduction}

example \citep{gagliardi2019international}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/text/body/methods.tex <==
\section{Methods} \label{sec:methods}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/text/body/results-and-discussion.tex <==
\section{Results and Discussion} \label{sec:results}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/text/frontmatter.tex <==
\title{ Hereditary Stratigraph Proof of Concept }

\author{
Matthew Andres Moreno\\
Computer Science and Engineering \\
Michigan State University\\
East Lansing, United States \\
\url{https://orcid.org/0000-0003-4726-4479} \\
\and
Charles Ofria
Computer Science and Engineering \\
Michigan State University\\
East Lansing, United States \\
\url{https://orcid.org/0000-0003-2924-1732}
}

\maketitle


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/text/references.tex <==
\section*{References}

\putbib


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/tab/recency-proportional-space-complexity.tex <==
\begin{table}

\begin{tabularx}{\columnwidth}{c | X | X | X | X}%
  \multirow{2}{*}{\makecell{\bfseries Num\\ \bfseries Generations \\ \bfseries Elapsed}}& \multicolumn{4}{m{0.6\columnwidth}}{\bfseries \centering
  Guaranteed MRCA-Recency-Proportional Resolution}\\ % specify table head
  \bfseries  & 1 & 4 & 10 & 100\\\hline\hline  % specify table head
  \csvreader[
    filter expr={
          test{\ifnumgreater{\thecsvinputline}{2}}
    }
  ]{submodules/hereditary-stratigraph-concept/binder/retention-policies/a=space-complexity+policy=recency-proportional-resolution+ext=.csv}{}% use head of csv as column names
{\num[scientific-notation=true,round-precision=2,round-mode=figures]{\csvcolii} & \csvcoliii & \csvcoliv & \csvcolv & \csvcolvi\\}% specify your columns here
\end{tabularx}
\caption{
Number of strata retained after one thousand, one million, one billion, and one trillion generations under the recency-proportional resolution stratum retention policy.
Four different policy parameterizations are shown, the first where MRCA generation can be determined between two extant columns with a guaranteed relative error of 100\%, the second 25\%, the third 10\%, and the fourth 1\%.
A column's memory footprint will be a constant factor of these retained counts based on the fingerprint differentia width chosen.
For example, if single byte differentia were used, the column's memory footprint in bits would be $8\times$ the number of strata retained.
}
\end{table}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/text/acknowledgement.tex <==
\section*{Acknowledgment}

This research was supported in part by NSF grants DEB-1655715 and DBI-0939454 as well as by Michigan State University through the computational resources provided by the Institute for Cyber-Enabled Research.
This material is based upon work supported by the National Science Foundation Graduate Research Fellowship under Grant No. DGE-1424871.
Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the National Science Foundation.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/text/body.tex <==
\input{text/body/abstract.tex}

\input{text/body/introduction.tex}

\input{text/body/methods.tex}

\input{text/body/results-and-discussion.tex}

\input{text/body/conclusion.tex}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/text/body/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/text/body/introduction.tex <==
\section{Introduction} \label{sec:introduction}

example \citep{gagliardi2019international}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/text/body/methods.tex <==
\section{Methods} \label{sec:methods}

\input{fig/retention-policies.tex}

\input{fig/column-comparison.tex}

\input{fig/deposit-process.tex}

\input{fig/phylogenetic-inference.tex}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/text/body/results-and-discussion.tex <==
\section{Results and Discussion} \label{sec:results}

\input{tab/recency-proportional-space-complexity.tex}

\input{fig/reconstruction-example.tex}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/text/frontmatter.tex <==
\title{ Hereditary Stratigraph Proof of Concept }

\author{
Matthew Andres Moreno\\
Computer Science and Engineering \\
Michigan State University\\
East Lansing, United States \\
\url{https://orcid.org/0000-0003-4726-4479} \\
\and
Charles Ofria
Computer Science and Engineering \\
Michigan State University\\
East Lansing, United States \\
\url{https://orcid.org/0000-0003-2924-1732}
}

\maketitle


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept/tex/text/references.tex <==
\section*{References}

\putbib


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/tab/_experimentcolumnsizesmacro.tex <==
% \pragmaonce
% ^adapted from https://tex.stackexchange.com/a/195173

% adapted from https://tex.stackexchange.com/a/118450
\providecommand{\experimentcolumnsizesmacro}[2]{
\def\dataname{#1}\def\fulldataname{#2}\input{tab/_experimentcolumnsizestemplate.tex}
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/tab/_experimentcolumnsizestemplate.tex <==
% \input{lib/importpath.tex}
\makeatletter
  \def\importpathx{\import@path}
\makeatother

\begin{table}

\begin{tabularx}{\columnwidth}{X | X | X | X | X | X}%
  \adjustbox{
    minipage=12em,
    rotate=90,
  }{
    \raggedright
    \bfseries
    Target Per-Column Memory Footprint (bits)
    \par
  }
  & \adjustbox{
      minipage=12em,
      rotate=90,
    }{
      \raggedright
      \bfseries
      Actual Mean Per-Column Memory Footprint (bits)
      \par
  }
  & \adjustbox{
      minipage=12em,
      rotate=90,
    }{
      \raggedright
      \bfseries
      Memory Footprint Percent Error
      \par
  }
  & \adjustbox{
      minipage=12em,
      rotate=90,
    }{
      \raggedright
      \bfseries
      Fingerprint Differentia Width (bits)
      \par
  }
  & \adjustbox{
      minipage=12em,
      rotate=90,
    }{
      \raggedright
      \bfseries
      Stratum Retention Policy
      \par
  }
  & \adjustbox{
      minipage=12em,
      rotate=90,
    }{
      \raggedright
      \bfseries
      Retention Policy Resolution Parameter
      \par
  }
  \\\hline\hline  % specify table head
  \csvreader[
    filter expr={
          test{\ifnumgreater{\thecsvinputline}{2}}
    }
  ]{\importpathx submodules/hereditary-stratigraph-concept/binder/phylogenetic-inference/\fulldataname }{}% use head of csv as column names
{
  \csvcolix
  & \num[round-precision=1,round-mode=places]{\csvcolii}
  &
  \ifthenelse{
    \lengthtest{\csuse{csvcolii}pt > \csuse{csvcolix}pt}
    }{\cellcolor{red!25}}{}%

  \num[round-precision=1,round-mode=places]{
    \fpeval{ 100 * \csvcolii / \csvcolix - 100 }
  }
  & \csvcolvi
  &
  \StrDel{\csvcolvii}{a}[\temp]
  \StrDel{\temp}{b}[\temp]
  \StrDel{\temp}{c}[\temp]
  \StrDel{\temp}{d}[\temp]
  \StrDel{\temp}{e}[\temp]
  \StrDel{\temp}{f}[\temp]
  \StrDel{\temp}{g}[\temp]
  \StrDel{\temp}{h}[\temp]
  \StrDel{\temp}{i}[\temp]
  \StrDel{\temp}{j}[\temp]
  \StrDel{\temp}{k}[\temp]
  \StrDel{\temp}{l}[\temp]
  \StrDel{\temp}{m}[\temp]
  \StrDel{\temp}{n}[\temp]
  \StrDel{\temp}{o}[\temp]
  \StrDel{\temp}{p}[\temp]
  \StrDel{\temp}{q}[\temp]
  \StrDel{\temp}{r}[\temp]
  \StrDel{\temp}{s}[\temp]
  \StrDel{\temp}{t}[\temp]
  \StrDel{\temp}{u}[\temp]
  \StrDel{\temp}{v}[\temp]
  \StrDel{\temp}{w}[\temp]
  \StrDel{\temp}{x}[\temp]
  \StrDel{\temp}{y}[\temp]
  \StrDel{\temp}{z}
  & \csvcolviii
  \\
}% specify your columns here
\end{tabularx}
\caption{
Hereditary stratigraph column memory footprint outcomes for phylogenetic reconstruction experiments on the \dataname dataset.
All treatments' stratum retention policies were parameterized to use as much of the target per-column memory footprint as possible without exceeding it.
Treatments where the stratum retention policy could not be parameterized low enough to meet the target per-column memory footprint are highlighted in red.
TDPR denotes the ``Tapered Depth-Proportional Resolution'' policy and RPR denotes the ``Recency-Proportional Resolution'' policy.
}

% adapted from https://tex.stackexchange.com/a/15708
\StrSubstitute{\dataname}{ }{-}[\temp]
\StrSubstitute{\temp}{A}{a}[\temp]
\StrSubstitute{\temp}{B}{b}[\temp]
\StrSubstitute{\temp}{C}{c}[\temp]
\StrSubstitute{\temp}{D}{d}[\temp]
\StrSubstitute{\temp}{E}{e}[\temp]
\StrSubstitute{\temp}{F}{f}[\temp]
\StrSubstitute{\temp}{G}{g}[\temp]
\StrSubstitute{\temp}{H}{h}[\temp]
\StrSubstitute{\temp}{I}{i}[\temp]
\StrSubstitute{\temp}{J}{j}[\temp]
\StrSubstitute{\temp}{K}{k}[\temp]
\StrSubstitute{\temp}{L}{l}[\temp]
\StrSubstitute{\temp}{M}{m}[\temp]
\StrSubstitute{\temp}{N}{n}[\temp]
\StrSubstitute{\temp}{O}{o}[\temp]
\StrSubstitute{\temp}{P}{p}[\temp]
\StrSubstitute{\temp}{Q}{q}[\temp]
\StrSubstitute{\temp}{R}{r}[\temp]
\StrSubstitute{\temp}{S}{s}[\temp]
\StrSubstitute{\temp}{T}{t}[\temp]
\StrSubstitute{\temp}{U}{u}[\temp]
\StrSubstitute{\temp}{V}{v}[\temp]
\StrSubstitute{\temp}{w}{w}[\temp]
\StrSubstitute{\temp}{X}{x}[\temp]
\StrSubstitute{\temp}{Y}{y}[\temp]
\StrSubstitute{\temp}{Z}{z}[\temp]

\def\labeltext{%
  {tab:experiment-column-sizes-\temp}%
}
\expandafter\label\labeltext
\end{table}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/tab/experiment-column-sizes-nk-ecoeaselection.tex <==
\input{tab/_experimentcolumnsizesmacro.tex}

\experimentcolumnsizesmacro{NK EcoEA Selection}{a=actual_retained_bits+source=nk_ecoeaselection_seed110_pop100_mut.01_snapshot_3000.csv}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/tab/experiment-column-sizes-nk-lexicaseselection.tex <==
\input{tab/_experimentcolumnsizesmacro.tex}

\experimentcolumnsizesmacro{NK Lexicase Selection}{a=actual_retained_bits+source=nk_lexicaseselection_seed110_pop165_mut.01_snapshot_500.csv}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/tab/experiment-column-sizes-nk-randomselection.tex <==
\input{tab/_experimentcolumnsizesmacro.tex}

\experimentcolumnsizesmacro{NK Random Selection}{a=actual_retained_bits+source=nk_randomselection_seed7_pop100_mut.01_snapshot_5000.csv}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/tab/experiment-column-sizes-nk-sharingselection.tex <==
\input{tab/_experimentcolumnsizesmacro.tex}

\experimentcolumnsizesmacro{NK Sharing Selection}{a=actual_retained_bits+source=nk_sharingselection_seed10_pop100_mut.01_snapshot_5000.csv}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/tab/experiment-column-sizes-nk-tournamentselection.tex <==
\input{tab/_experimentcolumnsizesmacro.tex}

\experimentcolumnsizesmacro{NK Tournament Selection}{a=actual_retained_bits+source=nk_tournamentselection_seed140_pop100_mut.01_snapshot_5000.csv}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/tab/ground-truth-phylogenies.tex <==
\begin{sidewaystable}[]
\begin{tabular}{lllll}
Selection Scheme & Per-bit Mutation Rate & Number Generations & Population Size & Phylogeny Download URL \\
Eco-EA           & 0.01                  & 3000               & 100             & \url{https://osf.io/5d3be/} \\
Lexicase         & 0.01                  & 500                & 165             & \url{https://osf.io/8ycq7/} \\
Random           & 0.01                  & 5000               & 100             & \url{https://osf.io/ydxt7/} \\
Sharing          & 0.01                  & 5000               & 100             & \url{https://osf.io/cz9fk/} \\
Tournament       & 0.01                  & 5000               & 100             & \url{https://osf.io/5ubn8/}
\end{tabular}
\caption{
Evolutionary conditions of ground-truth phylogenies taken from \citep{dolson2018applying}.
} \label{tab:ground-truth-phylogenies}
\end{sidewaystable}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/tab/recency-proportional-space-complexity.tex <==
\input{lib/importpath.tex}

\begin{table}
{\footnotesize
\begin{tabularx}{\columnwidth}{c | X | X | X | X}%
  \multirow{2}{*}{\makecell{\bfseries Num Gens \\ \bfseries Elapsed}}& \multicolumn{4}{m{0.6\columnwidth}}{\bfseries \centering
  Guaranteed MRCA-Recency-Proportional Resolution}\\ % specify table head
  \bfseries  & 1 & 4 & 10 & 100\\\hline\hline  % specify table head
  \csvreader[
    filter expr={
          test{\ifnumgreater{\thecsvinputline}{2}}
    }
  ]{\importpath submodules/hereditary-stratigraph-concept/binder/retention-policies/a=space-complexity+policy=recency-proportional-resolution+ext=.csv}{}% use head of csv as column names
{\num[scientific-notation=true,round-precision=2,round-mode=figures]{\csvcolii} & \csvcoliii & \csvcoliv & \csvcolv & \csvcolvi\\}% specify your columns here
\end{tabularx}
}
\caption{
Number strata retained after one thousand, one million, one billion, and one trillion generations under the recency-proportional resolution stratum retention policy.
Four different policy parameterizations are shown, the first where MRCA generation can be determined between two extant columns with a guaranteed relative error of 100\%, the second 25\%, the third 10\%, and the fourth 1\%.
A column's memory footprint will be a constant factor of these retained counts based on the fingerprint differentia width chosen.
For example, if single byte differentia were used, the column's memory footprint in bits would be $8\times$ the number of strata retained.
} \label{tab:recency-proportional-space-complexity}
\end{table}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/text/abstract.tex <==
\begin{abstract}
Phylogenies provide direct accounts of the evolutionary trajectories behind evolved artifacts in genetic algorithm and artificial life systems.
Phylogenetic analyses can also enable insight into evolutionary and ecological dynamics such as selection pressure and frequency-dependent selection.
Traditionally, digital evolution systems have recorded data for phylogenetic analyses through perfect tracking where each birth event is recorded in a centralized data structure.
This approach, however, does not easily scale to distributed computing environments where evolutionary individuals may migrate between a large number of disjoint processing elements.
To provide for phylogenetic analyses in these environments, we propose an approach to enable phylogenies to be inferred via heritable genetic annotations rather than directly tracked.
We introduce a “hereditary stratigraphy” algorithm that enables efficient, accurate phylogenetic reconstruction with tunable, explicit trade-offs between annotation memory footprint and reconstruction accuracy.
In particular, we demonstrate an approach that enables estimation of the most recent common ancestor (MRCA) between two individuals with fixed relative accuracy irrespective of lineage depth while only requiring logarithmic annotation space complexity with respect to lineage depth.
This approach can estimate, for example, MRCA generation of two genomes within 10\% relative error with 95\% confidence up to a depth of a trillion generations with genome annotations smaller than a kilobyte.
We also simulate inference over known lineages, recovering up to 85.70\% of the information contained in the original tree using 64-bit annotations.
\end{abstract}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/text/acknowledgement.tex <==
\section*{Acknowledgment}


This research was supported in part by NSF grants DEB-1655715 and DBI-0939454 as well as by Michigan State University through the computational resources provided by the Institute for Cyber-Enabled Research.
This material is based upon work supported by the National Science Foundation Graduate Research Fellowship under Grant No. DGE-1424871.
Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the National Science Foundation.
Thank you to Santiago Rodriguez Papa for manuscript comments.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/text/body.tex <==
\input{text/body/introduction.tex}

\input{text/body/methods.tex}

\input{text/body/results-and-discussion.tex}

\input{text/body/conclusion.tex}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/text/body/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}

To our knowledge, this work provides a novel design for digital genome components that enable phylogenetic inference on asexual populations.
This provides a viable alternative to perfect phylogenetic tracking, which is complex and possibly cumbersome in distributed computing scenarios, especially with fallible nodes.
Our approach enables flexible, explicit trade-offs between space complexity and inference accuracy.
Hereditary stratigraphic columns are efficient: our approach can estimate, for example, the MRCA generation of two genomes within 10\% error with 95\% confidence up to a depth of a trillion generations with genome annotations smaller than a kilobyte.
However, they are also powerful: we were able to achieve tree reconstructions recovering up to 85.70\% of the information contained in the original tree with only a 64-bit memory footprint.

This and other methodology to enable decentralized observation and analysis of evolving systems will be essential for artificial life experiments that use distributed and best-effort computing approaches.
Such systems will be crucial to enabling advances in the field of artificial life, particularly with respect to the question of open-ended evolution \citep{ackley2011pursue,moreno2021conduit,moreno2021case}
Mork work is called for to further enable experimental analyses in distributed, best-effort systems while preserving those systems' efficiency and scalability.
As parallel and distributed computing becomes increasingly ubiquitous and begins to more widely pervade artificial life systems, hereditary stratigraphy should serve as a useful technique in this toolbox.

Important work extending and analyzing hereditary stratigraphy remains to be done.
Analyses should be performed to expound MRCA resolution guarantees of stratum retention policies when using narrow (i.e., single-bit) differentia.
Constant-size-complexity stratum retention policies that preferentially retain a denser sampling of more-recent strata should be developed and analyzed.
Extensions to sexual populations should be explored, including the possibility of annotating and tracking individual genome components instead of whole-genome individuals.
An alternate approach might be to define a preferential inheritance rule so that at each generation slot within a column, a single differentia sweeps over an entire interbreeding population.
Optimization of tree reconstruction from extant hereditary stratigraphs remains an open question, too, particularly with regard to properly handling multifurcations.
It would be particularly valuable to develop methodology to annotate inner nodes of trees reconstructed from hereditary stratigraphs with confidence levels.

The problem of designing genomes to maximize phylogenetic reconstructability raises unique questions about phylogenetic estimation.
Such a backward problem --- optimizing genomes to make analyses trivial as opposed to the usual process of optimizing analyses to genomes --- puts questions about the genetic information analyses operate on in a new light.
In particular, it would be interesting to derive upper bounds on phylogenetic inference accuracy given genome size and generations elapsed.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/text/body/introduction.tex <==
\section{Introduction} \label{sec:introduction}

In traditional serially-processed digital evolution experiments, phylogenetic trees can be tracked perfectly as they progress \citep{bohm2017mabe,wang2018vine,lalejini2019data} rather than reconstructed afterward, as must be done in most biological studies of evolution.
Such direct phylogenetic tracking enables experimental possibilities unique to digital evolution, such as perfect reconstruction of the sequence of phylogenetic states that led to a particular evolutionary outcome \citep{lenski2003evolutionary, dolson2020interpreting}.
In a shared-memory context, it is not difficult to maintain a complete phylogeny by ensuring that offspring retain a permanent reference to their parent (or vice versa).
As simulations progress, however, memory usage would balloon if all simulated organisms were stored permanently.
Garbage collecting extinct lineages and saving older history to disk greatly ameliorates this issue \citep{bohm2017mabe,dolson2019modes}.

If sufficient memory or disk space can be afforded to log all reproduction events, recording a perfect phylogeny in a distributed context is also not especially difficult.
Processes could maintain records of each reproduction event, storing the parent organism (and its associated process) with all generated offspring (and their destination processes).
As long organisms are uniquely identified globally, these ``dangling ends'' could be joined in postprocessing to weave a continuous global phylogeny.
Of course, for the huge population sizes made possible by distributed systems, such stitching may become a demanding task in and of itself.
Additionally, even small amounts of lost or corrupted data could fundamentaly degrade tracking by disjoining large tree subsections.

However, if memory and disk space are limited, distributed phylogeny tracking becomes a more burdonsome challenge.
A naive approach might employ a server model to maintain a central store of phylogenetic data.
Processes would dispatch notifications of birth and death events to the server, which would curate (and gabage collect) phylogenetic history much the same as current serial phylogenetic tracking implementations.
Unfortunately, this server model approach would present scalability challenges: burden on the server process would worsen in direct proportion to processor count.
% ELD: This is making me wonder if there's a middle ground that could be explored in the future where we could use a sort of UDP phylogeny protocol, where no confirmation occurs
This approach would also be similarly brittle to any lost or corrupted data.

A more scalable approach might record birth and death events only on the process(es) where they unfold.
However, lineages that went extinct locally could not be safely garbage collected until the extinction of their offspring's lineages on other processors could be confirmed.
Garbage collection would thus require extinction notifications to wind back across processes each lineage had traversed.
Again, this approach would also be brittle to loss or corruption of data.

% Under a best-effort model, no system of phylogeny tracking can guarantee proper garbage collection.
% For example, it would be possible for an offspring that was dispatched to a neighboring process to have failed to arrive, and both processes would need to keep going, despite the failure.
% So, extinction notifications for the lineage founded by that offspring would never be dispatched --- putting in motion a memory leak of un-garbage-collectible phylogenetic history.
% The situation becomes even more leaky when the possibility of extinction notifications themselves being lost.

In a distributed context --- especially, a distributed, best-effort context --- phylogenetic reconstruction (as opposed to tracking) could prove simpler to implement, more efficient at runtime, and more robust to data loss while providing sufficient information to address experimental questions of interest.
However, phylogenetic reconstruction from genomes with a traditional model of divergence under grandual accumulation of random mutations poses its own difficulties, including
\begin{itemize}
\item accounting for heterogeneity in evolutionary rates (i.e., the rate at which mutations accumulate due to divergent mutation rates or selection pressures) between lineages \citep{lack2010identifying},
\item performing sequence alignment \citep{casci2008lining},
\item mutational saturation \citep{hagstrom2004using},
\item appropriately selecting and applying complex reconstruction algorithms \citep{kapli2020phylogenetic}, and
\item computational intensity \citep{sarkar2010hardware}.
\end{itemize}

The computational flexibility of digital artificial life experiments provides a unique opportunity to ovecome these challenges: designing heritable genome annotations specifically to ensure simple, efficient, and effective phylogenetic reconstruction.
For maximum applicability of such a solution, these annotations should be phenotypically neutral heritable instrumentation \citep{stanley2002evolving} that can be applied to any digital genome.

In this paper, we present ``hereditary stratigraphy,'' a novel heritable genome annotation system to facilitate post-hoc phylogenetic inference on asexual populations.
This system allows explicit control over trade-offs between space complexity and accuracy of phylogenetic inference.
Instead of modeling genome components diverging through a neutral mutational process, we keep a record of historical checkpoints that allow comparison of two lineages to identify the range of time in which they diverged.
Careful management of these checkpoints allows for a variety of trade-off options, including:
\begin{itemize}
  \item linear space complexity and fixed-magnitude inference error,
  \item constant space complexity and inference error linearly proportional to phylogenetic depth, and
  \item logarithmic space complexity and inference error linearly proportional to time elapsed since MRCA (which we suspect will be the most broadly useful trade-off).
\end{itemize}

In Methods we motivate and explain the hereditary stratigraphy approach.
Then, in Results and Discussion we simulate post-hoc inference on known phylogenies to assess the quality of phylogenetic reconstruction enabled by the hereditary stratigraphy method.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/text/body/methods.tex <==
\section{Methods} \label{sec:methods}

This section will introduce intuition for the strategy of our hereditary stratigraph approach, define the vocabulary we developed to describe aspects of this approach, overview configurable aspects of the approach, present mathematical exposition of the properties of space complexity and inference quality under particular configurations, and then recap digital experiments that demonstrate this approach in an applied setting.

\subsection{Hereditary Strata and the Hereditary Stratigraphic Column}

\input{fig/column-comparison.tex}

Our algorithm, particularly the vocabulary we developed to describe it, draws loose inspiration from the concept of geological stratigraphy, inference of natural history through analysis of successive layers of geological material \citep{steno1916prodromus}.
As an introductory intuition, suppose a body of rock being built up through regular, discrete events depositing of geological material.
Note that in such a scenario we could easily infer the age of the body of rock by counting up the number of layers present.
% Note that it is crucial to this scenario that each layer has some differentiating feature that allows it to be distinguished from layers above and below it, but also potentially from layers present in another body of rock in a distant and unrelated geographic position.
Next, imagine making a copy of the rock body in its partially-formed state and then moving it far away.
As time runs forward on these two rock bodies, independent layering processes will cause consistent disparity in the layers forming on each forwards from their point of separation.

To deduce the historical relationship of these rock bodies, we could simply align and compare their layers.
Layers from their base up through the first disparity would correspond to shared ancestry; further disparate layers would correspond to diverged ancestry.
% Interestingly, and powerfully for phylogenetic inference, we can readily distinguish a scenario where both rock bodies deposited ten layers after diverging from a scenario where one deposited eighteen layers and the other deposited two.
Figure \ref{fig:column-comparison} depicts the process of comparing columns for phylogenetic inference.

Shifting now from intuition to implementation, a fixed-length randomly-generated binary tag provides a suitable ``fingerprint'' mechanism mirroring our metaphorical ``rock layers.''
We call this ``fingerprint'' tag a \textit{differentia}.
The width of this tag controls the probability of spurious collisions between independently generated instances.
At 64 bits wide the tag effectively functions as a UID: collisions between randomly generated tags are so unlikely ($p < 5.42\times10^{-20}$) they can essentially be ignored.
At the other end of the spectrum, collision probability would be $1/256$ for a single byte and $1/2$ for a single bit.
In the case of narrow differentia, in order to set a lower bound for the MRCA generation, you would have to backtrack common strata from the last commonality until the probability of that many successive spurious collisions was enough to satisfy your desired confidence level (e.g., 95\% confidence).
Even then, there would be a possibility of the the true MRCA falling before the estimated lower bound.
Note, however, that no matter the width of the differentia the generation of the first discrepancy provides a hard upper bound on the generation of the MRCA.

In accordance with our geological analogy, we refer to the packet of data accumulated each generation as a \textit{stratum}.
This packet contains the differentia and, although not employed in this work, could hold other arbitrary user-defined data (i.e., simulation timestamp, phenotype characteristics, etc.).
Again in accordance with the geological analogy, we refer to the chronological stack of strata that accumulate over successive generations as a \textit{hereditary stratigraphic column}.

\subsection{Stratum Retention Policy}

\input{fig/deposit-process.tex}

As currently stated, strata in each column will accumulate proportionally to the length of evolutionary history simulated.
In an evolutionary run with thousands or millions of generations, this approach would soon become intractable --- particularly when columns are serialized and transmitted between distributed computing elements.
To solve this problem, we can trade off precision for compactness by strategically deleting strata from columns as time progresses.
Figure \ref{fig:deposit-process} overviews how stratum deposit and stratum elimination might progress over two generations under the hereditary stratigraphic column scheme.

Different patterns of deletion will lead to different trade-offs, both in terms of the scaling relationship of column size to generations elapsed and in terms of the arrangement of inference precision over evolutionary history (i.e., focusing precision on more recent evolutionary history versus spreading it evenly over the entire history).

We refer to the rule set used to selectively eliminate strata over time as the ``stratum retention policy.''
We explore several different retention policy designs here, and implement our software to allows for free, modular interchange of retention policies.

Our software allows specification of a policy as either a ``predicate'' or a ``generator.''
The predicate method requires a function that takes the generation of a stratum and the current number of strata deposited and returns whether that stratum should be retained at that point in time.
The generator method requires a function that takes the current number of strata deposited and yields the set of generations that should be deleted at that point in time.
Although the predicate form of a policy is useful for analyzing and proving properties of policies, the generator form is generally more efficient in practice.
We provide equivalent predicate and generator implementations for each stratum retention policy discussed here.

Strata elimination causes a stratum's position within the column data structure to no longer correspond to the generation it was deposited.
Therefore, it may seem necessary to store the generation of deposit within the stratum data structure.
However, for all deterministic retention policies a perfect mapping exists backwards from column index to recover generation deposited without storing it.
We provide this formula for each stratum retention policy surveyed here.
Finally, for each policy we provide a formula to calculate the exact number of strata retained under any parameterization after $n$ generations.

The next subsections introduce several stratum retention policies, explain the intuition behind their implementation, and elaborate their space complexity and resolution properties.
For each policy, patterns of stratum retention are illustrated in Figure \ref{fig:retention-policies}.
The formulas for number of strata retained after $n$ generations, the formulas to calculate stratum deposit generation from column index, and the retention predicate specifications of each policy are available in Supplementary Section \ref{sec:condemner-implementations}.
The generator specification of each policy is available in Supplementary Section \ref{sec:predicate-implementations}.
For tapered depth-proportional resolution and recency-proportional resolution, the accuracy of MRCA estimation can also be explored via an interactive in-browser web applet at \url{https://hopth.ru/bi}.

\input{fig/retention-policies.tex}

\subsection{Fixed Resolution Stratum Retention Policy}

The fixed resolution retention policy imposes a fixed absolute upper bound $r$ on the spacing between retained strata.
The strategy is simple: permanently retain a stratum every $r$th generation.
(For arbitrary reasons of implementation convenience, we also require each stratum to be retained during at least the generation it is deposited).
See top panel of Figure \ref{fig:retention-policies}.

This retention policy suffers from linear growth in a column's memory footprint with respect to number of generations elapsed: every $r$th generation generation a new stratum is permanently retained.
For this reason, it is likely not useful in practice except potentially in scenarios where the number of generations is small and fixed in advance.
We include it here largely for illustrative purposes as a gentle introduction to retention policies.

\subsection{Depth-Proportional Resolution Stratum Retention Policy}

The depth-proportional resolution policy ensures spacing between retained strata will be less than or equal to a proportion $1/r$ of total number of strata deposited $n$.
Achieving this limit on uncertainty requires retaining sufficient strata so that no more than $n/r$ generations elapsed between any two strata.
This policy accumulates retained strata at a fixed interval until twice as many as $r$ are at hand.
Then, every other retained stratum is purged and the cycle repeats with a new twice-as-wide interval between retained strata.
See second from top panel of Figure \ref{fig:retention-policies}.

When comparing stratigraphic columns from different generations, the resolution guarantee holds in terms of the number of generations experienced by the older of the two columns.
Because this retention policy is deterministic, for two columns with the same policy, every stratum that is held by the older column is also guaranteed to be present in the younger column (unless it hasn't yet been deposited on the younger column).
Therefore, the strata that would enable the desired resolution when comparing two columns of the same age are guaranteed to be available, even when one colummn has elapsed more generations.

Because the number of strata retained under this policy is bounded as $2r+1$, space complexity scales as $O(1)$ with respect to the number of strata deposited.
It follows that the MRCA generation estimate uncertainty scales as $O(n)$ with respect to the number of strata deposited.

\subsection{Tapered Depth-Proportional Resolution Stratum Retention Policy}

This policy refines the depth-proportional resolution policy to provide a more stable column memory footprint over time.
The naive depth-proportional resolution policy builds up strata until twice as many are present as needed then purges half of them all at once.
The tapered depth-proportional resolution policy functions identically to the depth-proportional policy except that it removes unnecessary strata gradually from back to front as new strata are deposited, instead of eliminating them simultaneously.
See third from top panel of Figure \ref{fig:retention-policies}.

The column footprint stability of this variation makes it easier to parameterize our experiments to ensure comparable end-state column footprints for fair comparison between retention policies, in addition to making this policy likely better suited to most use cases.
By design, this policy has the same space complexity and MRCA estimation uncertainty scaling relationships with number generations elapsed as the naive depth-proporitonal resolution policy.

\subsection{MRCA-Recency-Proportional Resolution Stratum Retention Policy}

\input{tab/recency-proportional-space-complexity.tex}

The MRCA-recency-proportional resolution policy ensures distance between the retained strata surrounding any generation point will be less than or equal to a user-specified proportion $1/r$ of the number of generations elapsed since that generation.

This policy can be constructed recursively.
So, to begin, let's consider setting up just the \textit{first} generation $g$ of the stratum after the root ancestor we will retain when $n$ generations have elapsed.
A simple geometric analysis reveals that providing the guaranteed resolution for the worst-case generation within the window between generation 0 and generation $g$ (i.e., generation $g-1$) requires
\begin{align*}
  g \leq \lfloor n / (r + 1) \rfloor.
\end{align*}

We now have an upper bound for the generation of the first stratum generation we must retain.
However, we must guarantee that strata at these generations are actually available for us to retain (i.e., haven't been purged out of the column at a previous time point).
We will do this by picking the generation that is the highest power of 2 less than or equal to our bound.
If we repeat this procedure as we recurse, we are guaranteed that this generation's stratum will have been preserved across all previous timepoints.

Why does this work?
Consider a sequence where all elements are spaced out by strictly nonincreasing powers of 2.
Consider the first element of the list.
All multiples this first element will be included in the list.
So, when we ratchet up $g$ to $2g$ as $n$ increases, we are guaranteed that $2g$ has been retained.
This principle generalizes recursively down the list.
This is a similar principle to the approach of strictly-doubling interval sizes used in the Depth-Proportional Resolution stratum retention policies described above.

This step of truncating to the nearest less than or equal to power of 2 affects our recursive step size is at most halved.
So, because step size is a constant fraction of remaining generations $n$ (at worst $\frac{n}{2(r+1)}$), the number of steps made (and number of strata retained) scales as $O(\log(n))$ with respect to the number of strata deposited.
Table \ref{tab:recency-proportional-space-complexity} provides exact figures for the number of strata retained under different parameterizations of the recency-proportional retention policy between one thousand and one trillion generations.

As for MRCA generation estimate uncertainty, in the worst case it scales as $O(n)$ with respect to the greater number of strata deposited.
However, with respect to estimating the generation of the MRCA for lineages diverged any fixed number of generations ago, uncertainty scales as $O(1)$.

How does space complexity scale with respect to the policy's specified resolution $r$?
Through extrapolation from OEIS sequences A063787 and A056791 via guess and check \citep{sloane2021a063787,sloane2021a056791}, we posited the exact number of strata retained after $n$ generations as

\begin{align*}
  \mathrm{HammingWeight}(n)
  + \sum_1^r \lfloor \log_2( \lfloor n / r \rfloor ) \rfloor
  + 1.
\end{align*}

This expression has been unit tested extensively to ensure perfect reliability.
Approximating and applying logarithmic properties, this policy's space complexity can be calculated within a constant factor as

\begin{align*}
\log(n) + \log\Big(\frac{n^r}{r!}\Big).
\end{align*}

To analyze the relationship between space complexity and resolution $r$, we will examine the ratio of space complexities induced when scaling resolution $r$ up by a constant factor $f > 1$.
Evaluating this ratio as $r \to \infty$, we find that space complexity scales directly proportional to $f$,

\begin{align*}
\lim_{r \to \infty}
\frac{
  \log(n) + \log\Big(\frac{n^{fr}}{(fr)!}\Big)
}{
  \log(n) + \log\Big(\frac{n^r}{r!}\Big)
}
= f.
\end{align*}

Evaluating this ratio as $n \to \infty$, we find that this scaling relationship is never worse than directly proportional for any $r$,

\begin{align*}
\lim_{n \to \infty}
\frac{
  \log(n) + \log\Big(\frac{n^{fr}}{(fr)!}\Big)
}{
  \log(n) + \log\Big(\frac{n^r}{r!}\Big)
}
&= \frac{fr+1}{r+1}\\
&= f\frac{r + 1/f}{r + 1}\\
&\leq f.
\end{align*}


\subsection{Computational Experiments}

In order to assess the practical performance of the hereditary stratigraph approach in an applied setting, we simulated the process of stratigraph propagation over known ``ground truth'' phylogenies extracted from pre-existing digital evolution simulations \citep{hernandez2022phylogenetic}.
These simulations propagated populations of between 100 and 165 bitstrings between 500 and 5,000 synchronous generations under the NK fitness landscape model \citep{kauffman1989nk}.
In order to ensure coverage of a variety of phylogenetic conditions, we sampled a variety of selection schemes that impose profoundly different ecological regimens \citep{dolson2018ecological},
\begin{itemize}
  \item EcoEA Selection \citep{goings2012ecology},
  \item Lexicase Selection \citep{helmuth2014solving},
  \item Random Selection, and
  \item Sharing Selection \citep{goldberg1987genetic}.
  % \item Tournament Selection \citep{miller1995genetic}.
\end{itemize}

Supplementary Table \ref{tab:ground-truth-phylogenies} provides full details on the conditions each ground truth phylogeny was drawn from.
The phylogenies themselves are available with our supplementary material.

For each ground truth phylogeny, we tested combinations of three configuration parameters:
\begin{itemize}
  \item target end-state memory footprints for extant columns (64, 512, and 4096 bits),
  \item differentia width (1, 8, and 64 bits), and
  \item stratum retention policy (tapered depth-proportional resolution and recency-proportional resolution).
\end{itemize}

Stratum retention policies were parameterized so that the maximum number of strata possible were present at the end of the experiment without exceeding the target memory footprint.
If the target memory footprint is exceeded by the sparsest possible parameterization of a retention policy, then that sparsest possible parameterization was used.
Supplementary Tables \cref{tab:experiment-column-sizes-nk-ecoea-selection,tab:experiment-column-sizes-nk-lexicase-selection,tab:experiment-column-sizes-nk-random-selection,tab:experiment-column-sizes-nk-sharing-selection,tab:experiment-column-sizes-nk-tournament-selection} provide the calculated paramaterizations and memory footprints of extant columns.

\input{fig/phylogenetic-inference.tex}

In order to assess the viability of phylogenetic inference using hereditary stratigraphic columns from extant organisms, we used the end-state stratigraphs to reconstruct an estimate of the actual ground truth phylogenetic histories.
The first step to reconstructing a phylogenetic tree for the history of an extant population at the end of an experiment is to construct a distance matrix by calculating all pairwise phylogenetic distances between extant columns.
We defined phylogenetic distance between two extant columns as the sum of each extant organism's generational distance back to the generation of their MRCA, estimated as the mean of the upper and lower 95\% confidence bounds.
Figure \ref{fig:phylogenetic-inference} provides a cartoon summary of the process of calculating phylogenetic distance between two extant columns.

We then used the unweighted pair group method with arithmetic mean (UPGMA) reconstruction tool provided by the BioPython package to generate estimate phylogenetic trees \citep{cock2009biopython,sokal1958statistical}.
After generating the reconstructed tree topology, we performed a second pass to adjust branch lengths so that each internal tree node sat at the mean of its estimated 95\% confidence generation bounds.
%We found that the neighbor joining (NJ) approach occasionally yielded reconstructions with impossible ``negative generation'' branches \citep{saitou1987neighbor} after knowledge bounding the absolute generation of internal nodes (i.e., MRCA's between pairs of extant organisms) was applied, so we did not use it.

\subsection{Software and Data}

% A prototype of this approach has been implemented \url{https://github.com/mmore500/dishtiny/blob/incoming/include/dish2/genome/PhyloFingerprints.hpp} and preliminarily tested \url{https://github.com/mmore500/dishtiny/blob/incoming/tests/dish2/genome/PhyloFingerprints.cpp}.

As part of this work, we published the \texttt{hstrat} Python library with a stable public-facing API intended to enable incorporation in other projects with extensive documentation and unit testing on GitHub at \url{https://github.com/mmore500/hstrat} and on PyPI.% at \url{https://pypi.org/project/hstrat/}.
In the near future, we intend to complete and publish a corresponding C++ library.

Supporting software materials can be found on GitHub at \url{https://github.com/mmore500/hereditary-stratigraph-concept}
Supporting computational notebooks are available for in-browser use via BinderHub at \url{https://hopth.ru/bk} \citep{ragan2018binder}.
Our work benefited from many pieces of open source scientific software \citep{sukumaran2010dendropy,virtanen2020scipy,hunter2007matplotlib,virtanen2020scipy,waskom2021seaborn,bostock2011d3,meurer2017sympy,smith2020treedistdata,paradis2004ape,ushey2022reticulate,wickham2022dplyr}.
The ground truth phylogenies used in this work as well as supplementary figures, tables, and text are available via the Open Science Framework at
\url{https://osf.io/4sm72/} \citep{foster2017open,moreno2022hstratconceptsupplement}.
Phylogenetic data associated with this project is stored in the Alife Community Data Standards format \citep{lalejini2019data}.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/text/body/results-and-discussion.tex <==
\section{Results and Discussion} \label{sec:results}

\input{fig/reconstruction-example.tex}

In this section, we analyze the quality of reconstructions of known phylogenetic trees using hereditary stratigraphy.
Figure \ref{fig:reconstruction-example} compares an example reconstruction from columns using tapered depth-proportional stratum retention, an example reconstruction using recency-proportional stratum retention,  and the underlying ground truth phylogeny.
Interactive in-browser visualizations comparing all reconstructed phylogenies to their corresponding ground truth are available at \url{https://hopth.ru/bi}. %TODO: replace this with anonymous link

\subsection{Reconstruction Accuracy}

Measuring tree similarity is a challenging problem, with many conflicting approaches that all provide different information \citep{smith2020treedist}.
Ideally, we would use a metric of reconstruction accuracy that 1) is commonly used so that there exists sufficient context to understand what constitutes a good value, 2) behaves consistently across different types of trees, and 3) behaves reasonably for the types of trees common in artificial life data.
Unfortunately, these objectives are somewhat in conflict.
The primary source of this problem is multifurcations, nodes from which more than two lineages branch at once.
In reconstructed phylogenies in biology, multifurcations are generally assumed to be the result of insufficient information.
It is thought that the real phylogeny had multiple bifurcations that occurred so close together that the reconstruction algorithm is unable to separate them.
In artificial life phylogenies, however, we have the opposite problem.
When we perfectly track a phylogeny, it is common for us to know that a multifurcation did in fact occur.
However, it is challenging for our reconstructions to properly identify multifurcations, because it requires perfectly lining up multiple divergence times.
Many of the most popular tree distance metrics interpret the difference between a multifurcation and a set of bifurcations as a dramatic change in topology.
For some use cases, this change in topology may indeed be meaningful, although research on the extent of this problem is limited.
Nevertheless, we suspect that for the majority of use cases, the tiny branch lengths between the internal nodes will make this source of error relatively minor.

To overcome this obstacle, we have measured our reconstruction accuracy using multiple metrics.
We will primarily focus on Mutual Clustering Information (as implemented in the R TreeDist package) \citep{smith2020treedist}, which is a direct measure of the quantity of information in the ground truth phylogeny that was successfully captured in the reconstruction.
It is relatively unaffected by the failure to perfectly reproduce multifurcations.
For the purposes of easy comparison to the literature, we also measured the Clustering Information Distance \citep{smith2020treedist}.

\input{fig/info_plot.tex}

Across ground truth phylogenies, we were able to reconstruct the phylogenetic topology with between 47.75\% and 85.70\% of the information contained in the original tree using a 64-bit column memory footprint, between 47.75\% and 80.36\% using a 512-bit column memory footprint, and between 51.13\% and 83.53\% using a 4096-bit column memory footprint.
While the Clustering Information Distance reached its maximum possible score (1.0) for the heavily-multifurcated EcoEA phylogeny, it agreed with the Mutual Clustering Information score for less multifurcated phylogenies, such as fitness sharing.
Using the Recency Proportional Resolution retention policy and a 4096-bit column memory footprint, we were able to reconstruct a fitness sharing phylogeny with a Clustering Information Distance of only 0.2923471 from the ground truth.
For context, that result is comparable to the distance between phylogenies reconstructed from two closely-related proteins in H3N2 flu (0.25) \citep{jones2021parallel}.
To build further intution, we strongly encourage readers to refer to our interactive web reconstruction.
Figure \ref{fig:info_plot} summarizes error reconstructing the fitness sharing selection phylogeny in terms of the mutual clustering information metric \citep{smith2022robust}.
The phylogenies reconstructed from the EcoEA condition performed comparably, with lexicase and random selection faring somewhat worse \citep{moreno2022hstratconceptsupplement}.
In the case of random selection, we suspect that this reduced performance is the result of having many nodes that originated very close together at the end of the experiment.
As expected, we did observe overall more accurate reconstructions from columns that were allowed to occupy larger memory footprints.

\subsection{Differentia Size}

Among the surveyed ground truth phylogenies and target column footprints, we consistently found that smaller differentia were able to yield more or as accurate phylogenetic reconstructions.
The stronger performance of narrow differentia was particularly apparent in low-memory-footprint scenarios where overall phylogenetic inference power was weaker.
Overall, single-bit differentia outperformed 64-bit differentia under 20 condtions, and were indistinguishable under 7 conditions, and were worse under 3 conditions.
Full results are available in Supplementary Section \ref{sec:differentia-size-full}.
Although narrower differentia have less distinguishing power on their own, their smaller size allows more to be packed into the memory footprint to cover more generations, which seems to help reconstruction power.
We must note that narrower differentia can pack more thoroughly into the footprint caps we imposed on column size, so their extant columns tended to have slightly more overall bits.
However, this was a small enough imbalance (in most cases $<10\%$) that we believe it is unlikely to fully account for the stronger performance of narrow-differentia configurations.

\subsection{Retention Policy}

Across the surveyed ground truth phylogenies and target column memory footprints, we found that the recency-proportional resolution stratum retention policy generally yielded better phylogenetic reconstructions.
Phylogenetic reconstruction quality was better in 28 conditions, equivalent in 14 conditions, and worse in 3 conditions.
Again, this effect was most apparent in the small-stratum-count scenarios where overal inference power was weaker.
Full results are available in Supplementary Section \ref{sec:retention-policy-full}.
The stronger performance of recency-proportional resolution is likely due to the denser retention of recent strata under the recency-proportional metric, which help to resolve the more numerous (and therefore typically more tightly spaced) phylogenetic events in the near past \citep{zhaxybayeva2004cladogenesis}.
Recency-proportional resolution tended to be able to fit fewer strata within the prescribed memory footprints (except in cases where it could not fit within the footprint) so its stronger performance cannot be attributed to more retained bits in the end-state extant columns.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/text/frontmatter.tex <==
\title{ Hereditary Stratigraphy: Genome Annotations to Enable Phylogenetic Inference over Distributed Populations }

\author{Matthew Andres Moreno, Emily Dolson, \and Charles Ofria \\
\mbox{}\\
Michigan State University, East Lansing, MI 48103 \\
mmore500@msu.edu}

\maketitle


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept/tex/text/references.tex <==
% \section*{References}

\putbib


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/tab/_experimentcolumnsizesmacro.tex <==
% \pragmaonce
% ^adapted from https://tex.stackexchange.com/a/195173

% adapted from https://tex.stackexchange.com/a/118450
\providecommand{\experimentcolumnsizesmacro}[2]{
\def\dataname{#1}\def\fulldataname{#2}\input{tab/_experimentcolumnsizestemplate.tex}
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/tab/_experimentcolumnsizestemplate.tex <==
% \input{lib/importpath.tex}
\makeatletter
  \def\importpathx{\import@path}
\makeatother

\begin{table}

\begin{tabularx}{\columnwidth}{X | X | X | X | X | X}%
  \adjustbox{
    minipage=12em,
    rotate=90,
  }{
    \raggedright
    \bfseries
    Target Per-Column Memory Footprint (bits)
    \par
  }
  & \adjustbox{
      minipage=12em,
      rotate=90,
    }{
      \raggedright
      \bfseries
      Actual Mean Per-Column Memory Footprint (bits)
      \par
  }
  & \adjustbox{
      minipage=12em,
      rotate=90,
    }{
      \raggedright
      \bfseries
      Memory Footprint Percent Error
      \par
  }
  & \adjustbox{
      minipage=12em,
      rotate=90,
    }{
      \raggedright
      \bfseries
      Fingerprint Differentia Width (bits)
      \par
  }
  & \adjustbox{
      minipage=12em,
      rotate=90,
    }{
      \raggedright
      \bfseries
      Stratum Retention Policy
      \par
  }
  & \adjustbox{
      minipage=12em,
      rotate=90,
    }{
      \raggedright
      \bfseries
      Retention Policy Resolution Parameter
      \par
  }
  \\\hline\hline  % specify table head
  \csvreader[
    filter expr={
          test{\ifnumgreater{\thecsvinputline}{2}}
    }
  ]{\importpathx submodules/hereditary-stratigraph-concept/binder/phylogenetic-inference/\fulldataname }{}% use head of csv as column names
{
  \csvcolix
  & \num[round-precision=1,round-mode=places]{\csvcolii}
  &
  \ifthenelse{
    \lengthtest{\csuse{csvcolii}pt > \csuse{csvcolix}pt}
    }{\cellcolor{red!25}}{}%

  \num[round-precision=1,round-mode=places]{
    \fpeval{ 100 * \csvcolii / \csvcolix - 100 }
  }
  & \csvcolvi
  &
  \StrDel{\csvcolvii}{a}[\temp]
  \StrDel{\temp}{b}[\temp]
  \StrDel{\temp}{c}[\temp]
  \StrDel{\temp}{d}[\temp]
  \StrDel{\temp}{e}[\temp]
  \StrDel{\temp}{f}[\temp]
  \StrDel{\temp}{g}[\temp]
  \StrDel{\temp}{h}[\temp]
  \StrDel{\temp}{i}[\temp]
  \StrDel{\temp}{j}[\temp]
  \StrDel{\temp}{k}[\temp]
  \StrDel{\temp}{l}[\temp]
  \StrDel{\temp}{m}[\temp]
  \StrDel{\temp}{n}[\temp]
  \StrDel{\temp}{o}[\temp]
  \StrDel{\temp}{p}[\temp]
  \StrDel{\temp}{q}[\temp]
  \StrDel{\temp}{r}[\temp]
  \StrDel{\temp}{s}[\temp]
  \StrDel{\temp}{t}[\temp]
  \StrDel{\temp}{u}[\temp]
  \StrDel{\temp}{v}[\temp]
  \StrDel{\temp}{w}[\temp]
  \StrDel{\temp}{x}[\temp]
  \StrDel{\temp}{y}[\temp]
  \StrDel{\temp}{z}
  & \csvcolviii
  \\
}% specify your columns here
\end{tabularx}
\caption{
Hereditary stratigraph column memory footprint outcomes for phylogenetic reconstruction experiments on the \dataname dataset.
All treatments' stratum retention policies were parameterized to use as much of the target per-column memory footprint as possible without exceeding it.
Treatments where the stratum retention policy could not be parameterized low enough to meet the target per-column memory footprint are highlighted in red.
TDPR denotes the ``Tapered Depth-Proportional Resolution'' policy and RPR denotes the ``Recency-Proportional Resolution'' policy.
}

% adapted from https://tex.stackexchange.com/a/15708
\StrSubstitute{\dataname}{ }{-}[\temp]
\StrSubstitute{\temp}{A}{a}[\temp]
\StrSubstitute{\temp}{B}{b}[\temp]
\StrSubstitute{\temp}{C}{c}[\temp]
\StrSubstitute{\temp}{D}{d}[\temp]
\StrSubstitute{\temp}{E}{e}[\temp]
\StrSubstitute{\temp}{F}{f}[\temp]
\StrSubstitute{\temp}{G}{g}[\temp]
\StrSubstitute{\temp}{H}{h}[\temp]
\StrSubstitute{\temp}{I}{i}[\temp]
\StrSubstitute{\temp}{J}{j}[\temp]
\StrSubstitute{\temp}{K}{k}[\temp]
\StrSubstitute{\temp}{L}{l}[\temp]
\StrSubstitute{\temp}{M}{m}[\temp]
\StrSubstitute{\temp}{N}{n}[\temp]
\StrSubstitute{\temp}{O}{o}[\temp]
\StrSubstitute{\temp}{P}{p}[\temp]
\StrSubstitute{\temp}{Q}{q}[\temp]
\StrSubstitute{\temp}{R}{r}[\temp]
\StrSubstitute{\temp}{S}{s}[\temp]
\StrSubstitute{\temp}{T}{t}[\temp]
\StrSubstitute{\temp}{U}{u}[\temp]
\StrSubstitute{\temp}{V}{v}[\temp]
\StrSubstitute{\temp}{w}{w}[\temp]
\StrSubstitute{\temp}{X}{x}[\temp]
\StrSubstitute{\temp}{Y}{y}[\temp]
\StrSubstitute{\temp}{Z}{z}[\temp]

\def\labeltext{%
  {tab:experiment-column-sizes-\temp}%
}
\expandafter\label\labeltext
\end{table}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/tab/experiment-column-sizes-nk-ecoeaselection.tex <==
\input{tab/_experimentcolumnsizesmacro.tex}

\experimentcolumnsizesmacro{NK EcoEA Selection}{a=actual_retained_bits+source=nk_ecoeaselection_seed110_pop100_mut.01_snapshot_3000.csv}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/tab/experiment-column-sizes-nk-lexicaseselection.tex <==
\input{tab/_experimentcolumnsizesmacro.tex}

\experimentcolumnsizesmacro{NK Lexicase Selection}{a=actual_retained_bits+source=nk_lexicaseselection_seed110_pop165_mut.01_snapshot_500.csv}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/tab/experiment-column-sizes-nk-randomselection.tex <==
\input{tab/_experimentcolumnsizesmacro.tex}

\experimentcolumnsizesmacro{NK Random Selection}{a=actual_retained_bits+source=nk_randomselection_seed7_pop100_mut.01_snapshot_5000.csv}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/tab/experiment-column-sizes-nk-sharingselection.tex <==
\input{tab/_experimentcolumnsizesmacro.tex}

\experimentcolumnsizesmacro{NK Sharing Selection}{a=actual_retained_bits+source=nk_sharingselection_seed10_pop100_mut.01_snapshot_5000.csv}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/tab/experiment-column-sizes-nk-tournamentselection.tex <==
\input{tab/_experimentcolumnsizesmacro.tex}

\experimentcolumnsizesmacro{NK Tournament Selection}{a=actual_retained_bits+source=nk_tournamentselection_seed140_pop100_mut.01_snapshot_5000.csv}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/tab/ground-truth-phylogenies.tex <==
\begin{sidewaystable}[]
\begin{tabular}{lllll}
Selection Scheme & Per-bit Mutation Rate & Number Generations & Population Size & Phylogeny Download URL \\
Eco-EA           & 0.01                  & 3000               & 100             & \url{https://osf.io/5d3be/} \\
Lexicase         & 0.01                  & 500                & 165             & \url{https://osf.io/8ycq7/} \\
Random           & 0.01                  & 5000               & 100             & \url{https://osf.io/ydxt7/} \\
Sharing          & 0.01                  & 5000               & 100             & \url{https://osf.io/cz9fk/} \\
Tournament       & 0.01                  & 5000               & 100             & \url{https://osf.io/5ubn8/}
\end{tabular}
\caption{
Evolutionary conditions of ground-truth phylogenies taken from \citep{dolson2018applying}.
} \label{tab:ground-truth-phylogenies}
\end{sidewaystable}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/tab/recency-proportional-space-complexity.tex <==
\input{lib/importpath.tex}

\begin{table}
{\footnotesize
\begin{tabularx}{\columnwidth}{c | X | X | X | X}%
  \multirow{2}{*}{\makecell{\bfseries Num Gens \\ \bfseries Elapsed}}& \multicolumn{4}{m{0.6\columnwidth}}{\bfseries \centering
  Guaranteed MRCA-Recency-Proportional Resolution}\\ % specify table head
  \bfseries  & 1 & 4 & 10 & 100\\\hline\hline  % specify table head
  \csvreader[
    filter expr={
          test{\ifnumgreater{\thecsvinputline}{2}}
    }
  ]{\importpath submodules/hereditary-stratigraph-concept/binder/retention-policies/a=space-complexity+policy=recency-proportional-resolution+ext=.csv}{}% use head of csv as column names
{\num[scientific-notation=true,round-precision=2,round-mode=figures]{\csvcolii} & \csvcoliii & \csvcoliv & \csvcolv & \csvcolvi\\}% specify your columns here
\end{tabularx}
}
\caption{
Number strata retained after one thousand, one million, one billion, and one trillion generations under the recency-proportional resolution stratum retention policy.
Four different policy parameterizations are shown, the first where MRCA generation can be determined between two extant columns with a guaranteed relative error of 100\%, the second 25\%, the third 10\%, and the fourth 1\%.
A column's memory footprint will be a constant factor of these retained counts based on the fingerprint differentia width chosen.
For example, if single byte differentia were used, the column's memory footprint in bits would be $8\times$ the number of strata retained.
} \label{tab:recency-proportional-space-complexity}
\end{table}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/tab/reconstruction-quality-results-by-differentia-bits.tex <==
\input{lib/C.tex}

\csvreader[
  longtable=C{3cm}cccccc,
  table head=\caption{
    Comparison of phylogenetic reconstruction quality across differentia bit counts.
    Reconstruction quality measured as clustering information distance (lower is better), mutual clustering information (higher is better), and generalized Robinson-Foulds similarity (higher is better) between reconstructed phylogeny and ground truth phylogeny \citep{smith2020information, smith2020treedist}.
    RPR is recency-proportional resolution stratum retention policy and TDPR is tapered depth-proportional resolution stratum retention policy.
  }\label{tab:reconstruction-quality-results-by-differentia-bits} \\
    \toprule \thead{Tree Comparison Metric} & \thead{Selection\\ Scheme} & \thead{Stratum\\ Retention\\ Policy} & \thead{Target\\ Num\\ Column\\ Bits} & \thead{1 \\Differentia \\ Bit\\ Score} & \thead{8 \\Differentia \\ Bits\\ Score} & \thead{64 \\Differentia \\ Bits\\ Score} \\ \midrule\endhead
    \bottomrule\endfoot,
  late after line=\\,
]{%
submodules/hereditary-stratigraph-concept/binder/reconstruction-quality/outplots/reconstruction_quality_results_by_differentia_bits.csv%
}{}{%
\vcell{\csvcoli} & \vcell{\csvcolii} & \vcell{\csvcoliii} & \vcell{\csvcoliv} & \vcell{\csvcolv} & \vcell{\csvcolvi} & \vcell{\csvcolvii} \\[-\rowheight]
\printcellmiddle & \printcellmiddle & \printcellmiddle & \printcellmiddle & \printcellmiddle & \printcellmiddle & \printcellmiddle \\
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/tab/reconstruction-quality-results-by-policy.tex <==
\csvreader[
  longtable=cccccc,
  table head=\caption{
    Comparison of phylogenetic reconstruction quality between stratum retention policies.
    Reconstruction quality measured as clustering information distance (lower is better), mutual clustering information (higher is better), and generalized Robinson-Foulds similarity (higher is better) between reconstructed phylogeny and ground truth phylogeny \citep{smith2020information, smith2020treedist}.  }\label{tab:reconstruction-quality-results-by-policy} \\
    \toprule \thead{Tree Comparison Metric} & \thead{Selection\\ Scheme} & \thead{Num\\ Differentia\\ Bits} & \thead{Target\\ Num\\ Column\\ Bits} & \thead{Recency- \\Proportional \\ Resolution\\ Score} & \thead{Tapered\\ Depth-\\ Proportional\\ Resolution\\ Score} \\ \midrule\endhead
    \bottomrule\endfoot,
  late after line=\\,
]{%
submodules/hereditary-stratigraph-concept/binder/reconstruction-quality/outplots/reconstruction_quality_results_by_policy.csv%
}{}{%
\csvcoli & \csvcolii & \csvcoliii & \csvcoliv & \csvcolv & \csvcolvi
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/text/abstract.tex <==
\begin{abstract}
Phylogenies provide direct accounts of the evolutionary trajectories behind evolved artifacts in genetic algorithm and artificial life systems.
Phylogenetic analyses can also enable insight into evolutionary and ecological dynamics such as selection pressure and frequency-dependent selection.
Traditionally, digital evolution systems have recorded data for phylogenetic analyses through perfect tracking where each birth event is recorded in a centralized data structure.
This approach, however, does not easily scale to distributed computing environments where evolutionary individuals may migrate between a large number of disjoint processing elements.
To provide for phylogenetic analyses in these environments, we propose an approach to enable phylogenies to be inferred via heritable genetic annotations rather than directly tracked.
We introduce a “hereditary stratigraphy” algorithm that enables efficient, accurate phylogenetic reconstruction with tunable, explicit trade-offs between annotation memory footprint and reconstruction accuracy.
In particular, we demonstrate an approach that enables estimation of the most recent common ancestor (MRCA) between two individuals with fixed relative accuracy irrespective of lineage depth while only requiring logarithmic annotation space complexity with respect to lineage depth.
This approach can estimate, for example, MRCA generation of two genomes within 10\% relative error with 95\% confidence up to a depth of a trillion generations with genome annotations smaller than a kilobyte.
We also simulate inference over known lineages, recovering up to 85.70\% of the information contained in the original tree using 64-bit annotations.
\end{abstract}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/text/acknowledgement.tex <==
\section*{Acknowledgment}


This research was supported in part by NSF grants DEB-1655715 and DBI-0939454 as well as by Michigan State University through the computational resources provided by the Institute for Cyber-Enabled Research.
This material is based upon work supported by the National Science Foundation Graduate Research Fellowship under Grant No. DGE-1424871.
Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the National Science Foundation.
Thank you to Santiago Rodriguez Papa for manuscript comments.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/text/body.tex <==
\input{text/body/introduction.tex}

\input{text/body/methods.tex}

\input{text/body/results-and-discussion.tex}

\input{text/body/conclusion.tex}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/text/body/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}

To our knowledge, this work provides a novel design for digital genome components that enable phylogenetic inference on asexual populations.
This provides a viable alternative to perfect phylogenetic tracking, which is complex and possibly cumbersome in distributed computing scenarios, especially with fallible nodes.
Our approach enables flexible, explicit trade-offs between space complexity and inference accuracy.
Hereditary stratigraphic columns are efficient: our approach can estimate, for example, the MRCA generation of two genomes within 10\% error with 95\% confidence up to a depth of a trillion generations with genome annotations smaller than a kilobyte.
However, they are also powerful: we were able to achieve tree reconstructions recovering up to 85.70\% of the information contained in the original tree with only a 64-bit memory footprint.

This and other methodology to enable decentralized observation and analysis of evolving systems will be essential for artificial life experiments that use distributed and best-effort computing approaches.
Such systems will be crucial to enabling advances in the field of artificial life, particularly with respect to the question of open-ended evolution \citep{ackley2011pursue,moreno2021conduit,moreno2021case}
Mork work is called for to further enable experimental analyses in distributed, best-effort systems while preserving those systems' efficiency and scalability.
As parallel and distributed computing becomes increasingly ubiquitous and begins to more widely pervade artificial life systems, hereditary stratigraphy should serve as a useful technique in this toolbox.

Important work extending and analyzing hereditary stratigraphy remains to be done.
Analyses should be performed to expound MRCA resolution guarantees of stratum retention policies when using narrow (i.e., single-bit) differentia.
Constant-size-complexity stratum retention policies that preferentially retain a denser sampling of more-recent strata should be developed and analyzed.
Extensions to sexual populations should be explored, including the possibility of annotating and tracking individual genome components instead of whole-genome individuals.
An alternate approach might be to define a preferential inheritance rule so that at each generation slot within a column, a single differentia sweeps over an entire interbreeding population.
Optimization of tree reconstruction from extant hereditary stratigraphs remains an open question, too, particularly with regard to properly handling multifurcations.
It would be particularly valuable to develop methodology to annotate inner nodes of trees reconstructed from hereditary stratigraphs with confidence levels.

The problem of designing genomes to maximize phylogenetic reconstructability raises unique questions about phylogenetic estimation.
Such a backward problem --- optimizing genomes to make analyses trivial as opposed to the usual process of optimizing analyses to genomes --- puts questions about the genetic information analyses operate on in a new light.
In particular, it would be interesting to derive upper bounds on phylogenetic inference accuracy given genome size and generations elapsed.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/text/body/introduction.tex <==
\section{Introduction} \label{sec:introduction}

In traditional serially-processed digital evolution experiments, phylogenetic trees can be tracked perfectly as they progress \citep{bohm2017mabe,wang2018vine,lalejini2019data} rather than reconstructed afterward, as must be done in most biological studies of evolution.
Such direct phylogenetic tracking enables experimental possibilities unique to digital evolution, such as perfect reconstruction of the sequence of phylogenetic states that led to a particular evolutionary outcome \citep{lenski2003evolutionary, dolson2020interpreting}.
In a shared-memory context, it is not difficult to maintain a complete phylogeny by ensuring that offspring retain a permanent reference to their parent (or vice versa).
As simulations progress, however, memory usage would balloon if all simulated organisms were stored permanently.
Garbage collecting extinct lineages and saving older history to disk greatly ameliorates this issue \citep{bohm2017mabe,dolson2019modes}.

If sufficient memory or disk space can be afforded to log all reproduction events, recording a perfect phylogeny in a distributed context is also not especially difficult.
Processes could maintain records of each reproduction event, storing the parent organism (and its associated process) with all generated offspring (and their destination processes).
As long organisms are uniquely identified globally, these ``dangling ends'' could be joined in postprocessing to weave a continuous global phylogeny.
Of course, for the huge population sizes made possible by distributed systems, such stitching may become a demanding task in and of itself.
Additionally, even small amounts of lost or corrupted data could fundamentally degrade tracking by disjoining large tree subsections.

However, if memory and disk space are limited, distributed phylogeny tracking becomes a more burdensome challenge.
A naive approach might employ a server model to maintain a central store of phylogenetic data.
Processes would dispatch notifications of birth and death events to the server, which would curate (and garbage collect) phylogenetic history much the same as current serial phylogenetic tracking implementations.
Unfortunately, this server model approach would present scalability challenges: burden on the server process would worsen in direct proportion to processor count.
% ELD: This is making me wonder if there's a middle ground that could be explored in the future where we could use a sort of UDP phylogeny protocol, where no confirmation occurs
This approach would also be similarly brittle to any lost or corrupted data.

A more scalable approach might record birth and death events only on the process(es) where they unfold.
However, lineages that went extinct locally could not be safely garbage collected until the extinction of their offspring's lineages on other processors could be confirmed.
Garbage collection would thus require extinction notifications to wind back across processes each lineage had traversed.
Again, this approach would also be brittle to loss or corruption of data.

% Under a best-effort model, no system of phylogeny tracking can guarantee proper garbage collection.
% For example, it would be possible for an offspring that was dispatched to a neighboring process to have failed to arrive, and both processes would need to keep going, despite the failure.
% So, extinction notifications for the lineage founded by that offspring would never be dispatched --- putting in motion a memory leak of un-garbage-collectible phylogenetic history.
% The situation becomes even more leaky when the possibility of extinction notifications themselves being lost.

In a distributed context --- especially, a distributed, best-effort context --- phylogenetic reconstruction (as opposed to tracking) could prove simpler to implement, more efficient at runtime, and more robust to data loss while providing sufficient information to address experimental questions of interest.
However, phylogenetic reconstruction from genomes with a traditional model of divergence under gradual accumulation of random mutations poses its own difficulties, including
\begin{itemize}
\item accounting for heterogeneity in evolutionary rates (i.e., the rate at which mutations accumulate due to divergent mutation rates or selection pressures) between lineages \citep{lack2010identifying},
\item performing sequence alignment \citep{casci2008lining},
\item mutational saturation \citep{hagstrom2004using},
\item appropriately selecting and applying complex reconstruction algorithms \citep{kapli2020phylogenetic}, and
\item computational intensity \citep{sarkar2010hardware}.
\end{itemize}

The computational flexibility of digital artificial life experiments provides a unique opportunity to overcome these challenges: designing heritable genome annotations specifically to ensure simple, efficient, and effective phylogenetic reconstruction.
For maximum applicability of such a solution, these annotations should be phenotypically neutral heritable instrumentation \citep{stanley2002evolving} that can be applied to any digital genome.

In this paper, we present ``hereditary stratigraphy,'' a novel heritable genome annotation system to facilitate post-hoc phylogenetic inference on asexual populations.
This system allows explicit control over trade-offs between space complexity and accuracy of phylogenetic inference.
Instead of modeling genome components diverging through a neutral mutational process, we keep a record of historical checkpoints that allow comparison of two lineages to identify the range of time in which they diverged.
Careful management of these checkpoints allows for a variety of trade-off options, including:
\begin{itemize}
  \item linear space complexity and fixed-magnitude inference error,
  \item constant space complexity and inference error linearly proportional to phylogenetic depth, and
  \item logarithmic space complexity and inference error linearly proportional to time elapsed since MRCA (which we suspect will be the most broadly useful trade-off).
\end{itemize}

In Methods we motivate and explain the hereditary stratigraphy approach.
Then, in Results and Discussion we simulate post-hoc inference on known phylogenies to assess the quality of phylogenetic reconstruction enabled by the hereditary stratigraphy method.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/text/body/methods.tex <==
\section{Methods} \label{sec:methods}

This section will introduce intuition for the strategy of our hereditary stratigraph approach, define the vocabulary we developed to describe aspects of this approach, overview configurable aspects of the approach, present mathematical exposition of the properties of space complexity and inference quality under particular configurations, and then recap digital experiments that demonstrate this approach in an applied setting.

\subsection{Hereditary Strata and the Hereditary Stratigraphic Column}

\input{fig/column-comparison.tex}

Our algorithm, particularly the vocabulary we developed to describe it, draws loose inspiration from the concept of geological stratigraphy, inference of natural history through analysis of successive layers of geological material \citep{steno1916prodromus}.
As an introductory intuition, suppose a body of rock being built up through regular, discrete events depositing of geological material.
Note that in such a scenario we could easily infer the age of the body of rock by counting up the number of layers present.
% Note that it is crucial to this scenario that each layer has some differentiating feature that allows it to be distinguished from layers above and below it, but also potentially from layers present in another body of rock in a distant and unrelated geographic position.
Next, imagine making a copy of the rock body in its partially-formed state and then moving it far away.
As time runs forward on these two rock bodies, independent layering processes will cause consistent disparity in the layers forming on each forwards from their point of separation.

To deduce the historical relationship of these rock bodies, we could simply align and compare their layers.
Layers from their base up through the first disparity would correspond to shared ancestry; further disparate layers would correspond to diverged ancestry.
% Interestingly, and powerfully for phylogenetic inference, we can readily distinguish a scenario where both rock bodies deposited ten layers after diverging from a scenario where one deposited eighteen layers and the other deposited two.
Figure \ref{fig:column-comparison} depicts the process of comparing columns for phylogenetic inference.

Shifting now from intuition to implementation, a fixed-length randomly-generated binary tag provides a suitable ``fingerprint'' mechanism mirroring our metaphorical ``rock layers.''
We call this ``fingerprint'' tag a \textit{differentia}.
The width of this tag controls the probability of spurious collisions between independently generated instances.
At 64 bits wide the tag effectively functions as a UID: collisions between randomly generated tags are so unlikely ($p < 5.42\times10^{-20}$) they can essentially be ignored.
At the other end of the spectrum, collision probability would be $1/256$ for a single byte and $1/2$ for a single bit.
In the case of narrow differentia, in order to set a lower bound for the MRCA generation, you would have to backtrack common strata from the last commonality until the probability of that many successive spurious collisions was enough to satisfy your desired confidence level (e.g., 95\% confidence).
Even then, there would be a possibility of the the true MRCA falling before the estimated lower bound.
Note, however, that no matter the width of the differentia the generation of the first discrepancy provides a hard upper bound on the generation of the MRCA.

In accordance with our geological analogy, we refer to the packet of data accumulated each generation as a \textit{stratum}.
This packet contains the differentia and, although not employed in this work, could hold other arbitrary user-defined data (i.e., simulation timestamp, phenotype characteristics, etc.).
Again in accordance with the geological analogy, we refer to the chronological stack of strata that accumulate over successive generations as a \textit{hereditary stratigraphic column}.

\subsection{Stratum Retention Policy}

\input{fig/deposit-process.tex}

As currently stated, strata in each column will accumulate proportionally to the length of evolutionary history simulated.
In an evolutionary run with thousands or millions of generations, this approach would soon become intractable --- particularly when columns are serialized and transmitted between distributed computing elements.
To solve this problem, we can trade off precision for compactness by strategically deleting strata from columns as time progresses.
Figure \ref{fig:deposit-process} overviews how stratum deposit and stratum elimination might progress over two generations under the hereditary stratigraphic column scheme.

Different patterns of deletion will lead to different trade-offs, both in terms of the scaling relationship of column size to generations elapsed and in terms of the arrangement of inference precision over evolutionary history (i.e., focusing precision on more recent evolutionary history versus spreading it evenly over the entire history).

We refer to the rule set used to selectively eliminate strata over time as the ``stratum retention policy.''
We explore several different retention policy designs here, and implement our software to allows for free, modular interchange of retention policies.

Our software allows specification of a policy as either a ``predicate'' or a ``generator.''
The predicate method requires a function that takes the generation of a stratum and the current number of strata deposited and returns whether that stratum should be retained at that point in time.
The generator method requires a function that takes the current number of strata deposited and yields the set of generations that should be deleted at that point in time.
Although the predicate form of a policy is useful for analyzing and proving properties of policies, the generator form is generally more efficient in practice.
We provide equivalent predicate and generator implementations for each stratum retention policy discussed here.

Strata elimination causes a stratum's position within the column data structure to no longer correspond to the generation it was deposited.
Therefore, it may seem necessary to store the generation of deposit within the stratum data structure.
However, for all deterministic retention policies a perfect mapping exists backwards from column index to recover generation deposited without storing it.
We provide this formula for each stratum retention policy surveyed here.
Finally, for each policy we provide a formula to calculate the exact number of strata retained under any parameterization after $n$ generations.

The next subsections introduce several stratum retention policies, explain the intuition behind their implementation, and elaborate their space complexity and resolution properties.
For each policy, patterns of stratum retention are illustrated in Figure \ref{fig:retention-policies}.
The formulas for number of strata retained after $n$ generations, the formulas to calculate stratum deposit generation from column index, and the retention predicate specifications of each policy are available in Supplementary Section \ref{sec:condemner-implementations}.
The generator specification of each policy is available in Supplementary Section \ref{sec:predicate-implementations}.
For tapered depth-proportional resolution and recency-proportional resolution, the accuracy of MRCA estimation can also be explored via an interactive in-browser web applet at \url{https://hopth.ru/bi}.

\input{fig/retention-policies.tex}

\subsection{Fixed Resolution Stratum Retention Policy}

The fixed resolution retention policy imposes a fixed absolute upper bound $r$ on the spacing between retained strata.
The strategy is simple: permanently retain a stratum every $r$th generation.
(For arbitrary reasons of implementation convenience, we also require each stratum to be retained during at least the generation it is deposited).
See top panel of Figure \ref{fig:retention-policies}.

This retention policy suffers from linear growth in a column's memory footprint with respect to number of generations elapsed: every $r$th generation generation a new stratum is permanently retained.
For this reason, it is likely not useful in practice except potentially in scenarios where the number of generations is small and fixed in advance.
We include it here largely for illustrative purposes as a gentle introduction to retention policies.

\subsection{Depth-Proportional Resolution Stratum Retention Policy}

The depth-proportional resolution policy ensures spacing between retained strata will be less than or equal to a proportion $1/r$ of total number of strata deposited $n$.
Achieving this limit on uncertainty requires retaining sufficient strata so that no more than $n/r$ generations elapsed between any two strata.
This policy accumulates retained strata at a fixed interval until twice as many as $r$ are at hand.
Then, every other retained stratum is purged and the cycle repeats with a new twice-as-wide interval between retained strata.
See second from top panel of Figure \ref{fig:retention-policies}.

When comparing stratigraphic columns from different generations, the resolution guarantee holds in terms of the number of generations experienced by the older of the two columns.
Because this retention policy is deterministic, for two columns with the same policy, every stratum that is held by the older column is also guaranteed to be present in the younger column (unless it hasn't yet been deposited on the younger column).
Therefore, the strata that would enable the desired resolution when comparing two columns of the same age are guaranteed to be available, even when one column has elapsed more generations.

Because the number of strata retained under this policy is bounded as $2r+1$, space complexity scales as $O(1)$ with respect to the number of strata deposited.
It follows that the MRCA generation estimate uncertainty scales as $O(n)$ with respect to the number of strata deposited.

\subsection{Tapered Depth-Proportional Resolution Stratum Retention Policy}

This policy refines the depth-proportional resolution policy to provide a more stable column memory footprint over time.
The naive depth-proportional resolution policy builds up strata until twice as many are present as needed then purges half of them all at once.
The tapered depth-proportional resolution policy functions identically to the depth-proportional policy except that it removes unnecessary strata gradually from back to front as new strata are deposited, instead of eliminating them simultaneously.
See third from top panel of Figure \ref{fig:retention-policies}.

The column footprint stability of this variation makes it easier to parameterize our experiments to ensure comparable end-state column footprints for fair comparison between retention policies, in addition to making this policy likely better suited to most use cases.
By design, this policy has the same space complexity and MRCA estimation uncertainty scaling relationships with number generations elapsed as the naive depth-proportional resolution policy.

\subsection{MRCA-Recency-Proportional Resolution Stratum Retention Policy}

\input{tab/recency-proportional-space-complexity.tex}

The MRCA-recency-proportional resolution policy ensures distance between the retained strata surrounding any generation point will be less than or equal to a user-specified proportion $1/r$ of the number of generations elapsed since that generation.

This policy can be constructed recursively.
So, to begin, let's consider setting up just the \textit{first} generation $g$ of the stratum after the root ancestor we will retain when $n$ generations have elapsed.
A simple geometric analysis reveals that providing the guaranteed resolution for the worst-case generation within the window between generation 0 and generation $g$ (i.e., generation $g-1$) requires
\begin{align*}
  g \leq \lfloor n / (r + 1) \rfloor.
\end{align*}

We now have an upper bound for the generation of the first stratum generation we must retain.
However, we must guarantee that strata at these generations are actually available for us to retain (i.e., haven't been purged out of the column at a previous time point).
We will do this by picking the generation that is the highest power of 2 less than or equal to our bound.
If we repeat this procedure as we recurse, we are guaranteed that this generation's stratum will have been preserved across all previous timepoints.

Why does this work?
Consider a sequence where all elements are spaced out by strictly nonincreasing powers of 2.
Consider the first element of the list.
All multiples this first element will be included in the list.
So, when we ratchet up $g$ to $2g$ as $n$ increases, we are guaranteed that $2g$ has been retained.
This principle generalizes recursively down the list.
This is a similar principle to the approach of strictly-doubling interval sizes used in the Depth-Proportional Resolution stratum retention policies described above.

This step of truncating to the nearest less than or equal to power of 2 affects our recursive step size is at most halved.
So, because step size is a constant fraction of remaining generations $n$ (at worst $\frac{n}{2(r+1)}$), the number of steps made (and number of strata retained) scales as $O(\log(n))$ with respect to the number of strata deposited.
Table \ref{tab:recency-proportional-space-complexity} provides exact figures for the number of strata retained under different parameterizations of the recency-proportional retention policy between one thousand and one trillion generations.

As for MRCA generation estimate uncertainty, in the worst case it scales as $O(n)$ with respect to the greater number of strata deposited.
However, with respect to estimating the generation of the MRCA for lineages diverged any fixed number of generations ago, uncertainty scales as $O(1)$.

How does space complexity scale with respect to the policy's specified resolution $r$?
Through extrapolation from OEIS sequences A063787 and A056791 via guess and check \citep{sloane2021a063787,sloane2021a056791}, we posited the exact number of strata retained after $n$ generations as

\begin{align*}
  \mathrm{HammingWeight}(n)
  + \sum_1^r \lfloor \log_2( \lfloor n / r \rfloor ) \rfloor
  + 1.
\end{align*}

This expression has been unit tested extensively to ensure perfect reliability.
Approximating and applying logarithmic properties, this policy's space complexity can be calculated within a constant factor as

\begin{align*}
\log(n) + \log\Big(\frac{n^r}{r!}\Big).
\end{align*}

To analyze the relationship between space complexity and resolution $r$, we will examine the ratio of space complexities induced when scaling resolution $r$ up by a constant factor $f > 1$.
Evaluating this ratio as $r \to \infty$, we find that space complexity scales directly proportional to $f$,

\begin{align*}
\lim_{r \to \infty}
\frac{
  \log(n) + \log\Big(\frac{n^{fr}}{(fr)!}\Big)
}{
  \log(n) + \log\Big(\frac{n^r}{r!}\Big)
}
= f.
\end{align*}

Evaluating this ratio as $n \to \infty$, we find that this scaling relationship is never worse than directly proportional for any $r$,

\begin{align*}
\lim_{n \to \infty}
\frac{
  \log(n) + \log\Big(\frac{n^{fr}}{(fr)!}\Big)
}{
  \log(n) + \log\Big(\frac{n^r}{r!}\Big)
}
&= \frac{fr+1}{r+1}\\
&= f\frac{r + 1/f}{r + 1}\\
&\leq f.
\end{align*}


\subsection{Computational Experiments}

In order to assess the practical performance of the hereditary stratigraph approach in an applied setting, we simulated the process of stratigraph propagation over known ``ground truth'' phylogenies extracted from pre-existing digital evolution simulations \citep{hernandez2022phylogenetic}.
These simulations propagated populations of between 100 and 165 bitstrings between 500 and 5,000 synchronous generations under the NK fitness landscape model \citep{kauffman1989nk}.
In order to ensure coverage of a variety of phylogenetic conditions, we sampled a variety of selection schemes that impose profoundly different ecological regimens \citep{dolson2018ecological},
\begin{itemize}
  \item EcoEA Selection \citep{goings2012ecology},
  \item Lexicase Selection \citep{helmuth2014solving},
  \item Random Selection, and
  \item Sharing Selection \citep{goldberg1987genetic}.
  % \item Tournament Selection \citep{miller1995genetic}.
\end{itemize}

Supplementary Table \ref{tab:ground-truth-phylogenies} provides full details on the conditions each ground truth phylogeny was drawn from.
The phylogenies themselves are available with our supplementary material.

For each ground truth phylogeny, we tested combinations of three configuration parameters:
\begin{itemize}
  \item target end-state memory footprints for extant columns (64, 512, and 4096 bits),
  \item differentia width (1, 8, and 64 bits), and
  \item stratum retention policy (tapered depth-proportional resolution and recency-proportional resolution).
\end{itemize}

Stratum retention policies were parameterized so that the maximum number of strata possible were present at the end of the experiment without exceeding the target memory footprint.
If the target memory footprint is exceeded by the sparsest possible parameterization of a retention policy, then that sparsest possible parameterization was used.
Supplementary Tables \cref{tab:experiment-column-sizes-nk-ecoea-selection,tab:experiment-column-sizes-nk-lexicase-selection,tab:experiment-column-sizes-nk-random-selection,tab:experiment-column-sizes-nk-sharing-selection,tab:experiment-column-sizes-nk-tournament-selection} provide the calculated paramaterizations and memory footprints of extant columns.

\input{fig/phylogenetic-inference.tex}

In order to assess the viability of phylogenetic inference using hereditary stratigraphic columns from extant organisms, we used the end-state stratigraphs to reconstruct an estimate of the actual ground truth phylogenetic histories.
The first step to reconstructing a phylogenetic tree for the history of an extant population at the end of an experiment is to construct a distance matrix by calculating all pairwise phylogenetic distances between extant columns.
We defined phylogenetic distance between two extant columns as the sum of each extant organism's generational distance back to the generation of their MRCA, estimated as the mean of the upper and lower 95\% confidence bounds.
Figure \ref{fig:phylogenetic-inference} provides a cartoon summary of the process of calculating phylogenetic distance between two extant columns.

We then used the unweighted pair group method with arithmetic mean (UPGMA) reconstruction tool provided by the BioPython package to generate estimate phylogenetic trees \citep{cock2009biopython,sokal1958statistical}.
After generating the reconstructed tree topology, we performed a second pass to adjust branch lengths so that each internal tree node sat at the mean of its estimated 95\% confidence generation bounds.
%We found that the neighbor joining (NJ) approach occasionally yielded reconstructions with impossible ``negative generation'' branches \citep{saitou1987neighbor} after knowledge bounding the absolute generation of internal nodes (i.e., MRCA's between pairs of extant organisms) was applied, so we did not use it.

\subsection{Software and Data}

% A prototype of this approach has been implemented \url{https://github.com/mmore500/dishtiny/blob/incoming/include/dish2/genome/PhyloFingerprints.hpp} and preliminarily tested \url{https://github.com/mmore500/dishtiny/blob/incoming/tests/dish2/genome/PhyloFingerprints.cpp}.

As part of this work, we published the \texttt{hstrat} Python library with a stable public-facing API intended to enable incorporation in other projects with extensive documentation and unit testing on GitHub at \url{https://github.com/mmore500/hstrat} and on PyPI.% at \url{https://pypi.org/project/hstrat/}.
In the near future, we intend to complete and publish a corresponding C++ library.

Supporting software materials can be found on GitHub at \url{https://github.com/mmore500/hereditary-stratigraph-concept}
Supporting computational notebooks are available for in-browser use via BinderHub at \url{https://hopth.ru/bk} \citep{ragan2018binder}.
Our work benefited from many pieces of open source scientific software \citep{sukumaran2010dendropy,virtanen2020scipy,hunter2007matplotlib,virtanen2020scipy,waskom2021seaborn,bostock2011d3,meurer2017sympy,smith2020treedistdata,paradis2004ape,ushey2022reticulate,wickham2022dplyr}.
The ground truth phylogenies used in this work as well as supplementary figures, tables, and text are available via the Open Science Framework at
\url{https://osf.io/4sm72/} \citep{foster2017open,moreno2022hstratconceptsupplement}.
Phylogenetic data associated with this project is stored in the Alife Community Data Standards format \citep{lalejini2019data}.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/text/body/results-and-discussion.tex <==
\section{Results and Discussion} \label{sec:results}

\input{fig/reconstruction-example.tex}

In this section, we analyze the quality of reconstructions of known phylogenetic trees using hereditary stratigraphy.
Figure \ref{fig:reconstruction-example} compares an example reconstruction from columns using tapered depth-proportional stratum retention, an example reconstruction using recency-proportional stratum retention,  and the underlying ground truth phylogeny.
Interactive in-browser visualizations comparing all reconstructed phylogenies to their corresponding ground truth are available at \url{https://hopth.ru/bi}. %TODO: replace this with anonymous link

\subsection{Reconstruction Accuracy}

Measuring tree similarity is a challenging problem, with many conflicting approaches that all provide different information \citep{smith2020information}.
Ideally, we would use a metric of reconstruction accuracy that 1) is commonly used so that there exists sufficient context to understand what constitutes a good value, 2) behaves consistently across different types of trees, and 3) behaves reasonably for the types of trees common in artificial life data.
Unfortunately, these objectives are somewhat in conflict.
The primary source of this problem is multifurcations, nodes from which more than two lineages branch at once.
In reconstructed phylogenies in biology, multifurcations are generally assumed to be the result of insufficient information.
It is thought that the real phylogeny had multiple bifurcations that occurred so close together that the reconstruction algorithm is unable to separate them.
In artificial life phylogenies, however, we have the opposite problem.
When we perfectly track a phylogeny, it is common for us to know that a multifurcation did in fact occur.
However, it is challenging for our reconstructions to properly identify multifurcations, because it requires perfectly lining up multiple divergence times.
Many of the most popular tree distance metrics interpret the difference between a multifurcation and a set of bifurcations as a dramatic change in topology.
For some use cases, this change in topology may indeed be meaningful, although research on the extent of this problem is limited.
Nevertheless, we suspect that for the majority of use cases, the tiny branch lengths between the internal nodes will make this source of error relatively minor.

To overcome this obstacle, we have measured our reconstruction accuracy using multiple metrics.
We will primarily focus on Mutual Clustering Information (as implemented in the R TreeDist package) \citep{smith2020treedist}, which is a direct measure of the quantity of information in the ground truth phylogeny that was successfully captured in the reconstruction.
It is relatively unaffected by the failure to perfectly reproduce multifurcations.
For the purposes of easy comparison to the literature, we also measured the Clustering Information Distance \citep{smith2020treedist}.

\input{fig/info_plot.tex}

Across ground truth phylogenies, we were able to reconstruct the phylogenetic topology with between 47.75\% and 85.70\% of the information contained in the original tree using a 64-bit column memory footprint, between 47.75\% and 80.36\% using a 512-bit column memory footprint, and between 51.13\% and 83.53\% using a 4096-bit column memory footprint.
While the Clustering Information Distance reached its maximum possible score (1.0) for the heavily-multifurcated EcoEA phylogeny, it agreed with the Mutual Clustering Information score for less multifurcated phylogenies, such as fitness sharing.
Using the Recency Proportional Resolution retention policy and a 4096-bit column memory footprint, we were able to reconstruct a fitness sharing phylogeny with a Clustering Information Distance of only 0.2923471 from the ground truth.
For context, that result is comparable to the distance between phylogenies reconstructed from two closely-related proteins in H3N2 flu (0.25) \citep{jones2021parallel}.
To build further intuition, we strongly encourage readers to refer to our interactive web reconstruction.
Figure \ref{fig:info_plot} summarizes error reconstructing the fitness sharing selection phylogeny in terms of the mutual clustering information metric \citep{smith2022robust}.
The phylogenies reconstructed from the EcoEA condition performed comparably, with lexicase and random selection faring somewhat worse \citep{moreno2022hstratconceptsupplement}.
In the case of random selection, we suspect that this reduced performance is the result of having many nodes that originated very close together at the end of the experiment.
As expected, we did observe overall more accurate reconstructions from columns that were allowed to occupy larger memory footprints.

\subsection{Differentia Size}

Among the surveyed ground truth phylogenies and target column footprints, we consistently found that smaller differentia were able to yield more or as accurate phylogenetic reconstructions.
The stronger performance of narrow differentia was particularly apparent in low-memory-footprint scenarios where overall phylogenetic inference power was weaker.
Overall, single-bit differentia outperformed 64-bit differentia under 20 conditions, and were indistinguishable under 6 conditions, and were worse under 4 conditions.
We used Cluster Information Distance to perform these comparisons.
Full results are available in Supplementary Section \ref{sec:differentia-size-full}.
Although narrower differentia have less distinguishing power on their own, their smaller size allows more to be packed into the memory footprint to cover more generations, which seems to help reconstruction power.
We must note that narrower differentia can pack more thoroughly into the footprint caps we imposed on column size, so their extant columns tended to have slightly more overall bits.
However, this was a small enough imbalance (in most cases $<10\%$) that we believe it is unlikely to fully account for the stronger performance of narrow-differentia configurations.

\subsection{Retention Policy}

Across the surveyed ground truth phylogenies and target column memory footprints, we found that the recency-proportional resolution stratum retention policy generally yielded better phylogenetic reconstructions.
Phylogenetic reconstruction quality was better in 28 conditions, equivalent in 13 conditions, and worse in 4 conditions.
Again, this effect was most apparent in the small-stratum-count scenarios where overall inference power was weaker.
We used Cluster Information Distance to perform these comparisons.
Full results are available in Supplementary Section \ref{sec:retention-policy-full}.
The stronger performance of recency-proportional resolution is likely due to the denser retention of recent strata under the recency-proportional metric, which help to resolve the more numerous (and therefore typically more tightly spaced) phylogenetic events in the near past \citep{zhaxybayeva2004cladogenesis}.
Recency-proportional resolution tended to be able to fit fewer strata within the prescribed memory footprints (except in cases where it could not fit within the footprint) so its stronger performance cannot be attributed to more retained bits in the end-state extant columns.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/text/frontmatter.tex <==
\title{ Hereditary Stratigraphy: Genome Annotations to Enable Phylogenetic Inference over Distributed Populations }

\author{Matthew Andres Moreno, Emily Dolson, \and Charles Ofria \\
\mbox{}\\
Michigan State University, East Lansing, MI 48103 \\
mmore500@msu.edu}

\maketitle


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/submodules/hereditary-stratigraph-concept-binder/tex/text/references.tex <==
% \section*{References}

\putbib


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/tab/_experimentcolumnsizesmacro.tex <==
% \pragmaonce
% ^adapted from https://tex.stackexchange.com/a/195173

% adapted from https://tex.stackexchange.com/a/118450
\providecommand{\experimentcolumnsizesmacro}[2]{
\def\dataname{#1}\def\fulldataname{#2}\input{tab/_experimentcolumnsizestemplate.tex}
}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/tab/_experimentcolumnsizestemplate.tex <==
\input{lib/dissertationonly.tex}
% \input{lib/importpath.tex}
\makeatletter
  \def\importpathx{\import@path}
\makeatother

\begin{table}[h!]

  \caption{
  Hereditary stratigraph column memory footprint outcomes for phylogenetic reconstruction experiments on the \dataname dataset.
  All treatments' stratum retention policies were parameterized to use as much of the target per-column memory footprint as possible without exceeding it.
  Treatments where the stratum retention policy could not be parameterized low enough to meet the target per-column memory footprint are highlighted in red.
  TDPR denotes the ``Tapered Depth-Proportional Resolution'' policy and RPR denotes the ``Recency-Proportional Resolution'' policy.
  }

  % adapted from https://tex.stackexchange.com/a/15708
  \StrSubstitute{\dataname}{ }{-}[\temp]
  \StrSubstitute{\temp}{A}{a}[\temp]
  \StrSubstitute{\temp}{B}{b}[\temp]
  \StrSubstitute{\temp}{C}{c}[\temp]
  \StrSubstitute{\temp}{D}{d}[\temp]
  \StrSubstitute{\temp}{E}{e}[\temp]
  \StrSubstitute{\temp}{F}{f}[\temp]
  \StrSubstitute{\temp}{G}{g}[\temp]
  \StrSubstitute{\temp}{H}{h}[\temp]
  \StrSubstitute{\temp}{I}{i}[\temp]
  \StrSubstitute{\temp}{J}{j}[\temp]
  \StrSubstitute{\temp}{K}{k}[\temp]
  \StrSubstitute{\temp}{L}{l}[\temp]
  \StrSubstitute{\temp}{M}{m}[\temp]
  \StrSubstitute{\temp}{N}{n}[\temp]
  \StrSubstitute{\temp}{O}{o}[\temp]
  \StrSubstitute{\temp}{P}{p}[\temp]
  \StrSubstitute{\temp}{Q}{q}[\temp]
  \StrSubstitute{\temp}{R}{r}[\temp]
  \StrSubstitute{\temp}{S}{s}[\temp]
  \StrSubstitute{\temp}{T}{t}[\temp]
  \StrSubstitute{\temp}{U}{u}[\temp]
  \StrSubstitute{\temp}{V}{v}[\temp]
  \StrSubstitute{\temp}{w}{w}[\temp]
  \StrSubstitute{\temp}{X}{x}[\temp]
  \StrSubstitute{\temp}{Y}{y}[\temp]
  \StrSubstitute{\temp}{Z}{z}[\temp]

  \def\labeltext{%
    {tab:experiment-column-sizes-\temp}%
  }
  \expandafter\label\labeltext

\begin{tabularx}{\columnwidth}{X | X | X | X | X | X}%
  \adjustbox{
    minipage=12em,
    rotate=90,
  }{
    \raggedright
    \bfseries
    Target Per-Column Memory Footprint (bits)
    \par
  }
  & \adjustbox{
      minipage=12em,
      rotate=90,
    }{
      \raggedright
      \bfseries
      Actual Mean Per-Column Memory Footprint (bits)
      \par
  }
  & \adjustbox{
      minipage=12em,
      rotate=90,
    }{
      \raggedright
      \bfseries
      Memory Footprint Percent Error
      \par
  }
  & \adjustbox{
      minipage=12em,
      rotate=90,
    }{
      \raggedright
      \bfseries
      Fingerprint Differentia Width (bits)
      \par
  }
  & \adjustbox{
      minipage=12em,
      rotate=90,
    }{
      \raggedright
      \bfseries
      Stratum Retention Policy
      \par
  }
  & \adjustbox{
      minipage=12em,
      rotate=90,
    }{
      \raggedright
      \bfseries
      Retention Policy Resolution Parameter
      \par
  }
  \\\hline\hline  % specify table head
  \csvreader[
    filter expr={
          test{\ifnumgreater{\thecsvinputline}{2}}
    }
  ]{\importpathx submodules/hereditary-stratigraph-concept-binder/binder/phylogenetic-inference/\fulldataname }{}% use head of csv as column names
{
  \csvcolix
  & \num[round-precision=1,round-mode=places]{\csvcolii}
  &
  \ifthenelse{
    \lengthtest{\csuse{csvcolii}pt > \csuse{csvcolix}pt}
    }{\cellcolor{red!25}}{}%

  \num[round-precision=1,round-mode=places]{
    \fpeval{ 100 * \csvcolii / \csvcolix - 100 }
  }
  & \csvcolvi
  &
  \StrDel{\csvcolvii}{a}[\temp]
  \StrDel{\temp}{b}[\temp]
  \StrDel{\temp}{c}[\temp]
  \StrDel{\temp}{d}[\temp]
  \StrDel{\temp}{e}[\temp]
  \StrDel{\temp}{f}[\temp]
  \StrDel{\temp}{g}[\temp]
  \StrDel{\temp}{h}[\temp]
  \StrDel{\temp}{i}[\temp]
  \StrDel{\temp}{j}[\temp]
  \StrDel{\temp}{k}[\temp]
  \StrDel{\temp}{l}[\temp]
  \StrDel{\temp}{m}[\temp]
  \StrDel{\temp}{n}[\temp]
  \StrDel{\temp}{o}[\temp]
  \StrDel{\temp}{p}[\temp]
  \StrDel{\temp}{q}[\temp]
  \StrDel{\temp}{r}[\temp]
  \StrDel{\temp}{s}[\temp]
  \StrDel{\temp}{t}[\temp]
  \StrDel{\temp}{u}[\temp]
  \StrDel{\temp}{v}[\temp]
  \StrDel{\temp}{w}[\temp]
  \StrDel{\temp}{x}[\temp]
  \StrDel{\temp}{y}[\temp]
  \StrDel{\temp}{z}
  & \csvcolviii
  \\
}% specify your columns here
\end{tabularx}
\end{table}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/tab/experiment-column-sizes-nk-ecoeaselection.tex <==
\input{tab/_experimentcolumnsizesmacro.tex}

\experimentcolumnsizesmacro{NK EcoEA Selection}{a=actual_retained_bits+source=nk_ecoeaselection_seed110_pop100_mut.01_snapshot_3000.csv}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/tab/experiment-column-sizes-nk-lexicaseselection.tex <==
\input{tab/_experimentcolumnsizesmacro.tex}

\experimentcolumnsizesmacro{NK Lexicase Selection}{a=actual_retained_bits+source=nk_lexicaseselection_seed110_pop165_mut.01_snapshot_500.csv}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/tab/experiment-column-sizes-nk-randomselection.tex <==
\input{tab/_experimentcolumnsizesmacro.tex}

\experimentcolumnsizesmacro{NK Random Selection}{a=actual_retained_bits+source=nk_randomselection_seed7_pop100_mut.01_snapshot_5000.csv}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/tab/experiment-column-sizes-nk-sharingselection.tex <==
\input{tab/_experimentcolumnsizesmacro.tex}

\experimentcolumnsizesmacro{NK Sharing Selection}{a=actual_retained_bits+source=nk_sharingselection_seed10_pop100_mut.01_snapshot_5000.csv}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/tab/experiment-column-sizes-nk-tournamentselection.tex <==
\input{tab/_experimentcolumnsizesmacro.tex}

\experimentcolumnsizesmacro{NK Tournament Selection}{a=actual_retained_bits+source=nk_tournamentselection_seed140_pop100_mut.01_snapshot_5000.csv}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/tab/ground-truth-phylogenies.tex <==
\begin{table}[ht]
\centering
\caption{
Evolutionary conditions of ground-truth phylogenies taken from \citep{dolson2018applying}.
} \label{tab:ground-truth-phylogenies}
\begin{tabular}{p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}}
Selection Scheme & Per-bit Mutation Rate & Number Generations & Population Size & Phylogeny Download URL \\\toprule
Eco-EA           & 0.01                  & 3000               & 100             & \url{https://osf.io/5d3be/} \\
Lexicase         & 0.01                  & 500                & 165             & \url{https://osf.io/8ycq7/} \\
Random           & 0.01                  & 5000               & 100             & \url{https://osf.io/ydxt7/} \\
Sharing          & 0.01                  & 5000               & 100             & \url{https://osf.io/cz9fk/} \\
Tournament       & 0.01                  & 5000               & 100             & \url{https://osf.io/5ubn8/}
\end{tabular}
\end{table}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/tab/recency-proportional-space-complexity.tex <==
\input{lib/dissertationelse.tex}
\input{lib/importpath.tex}

\begin{table}
{\dissertationelse{\fontsize{9}{10}\selectfont}{\footnotesize}
\begin{tabularx}{\columnwidth}{c | X | X | X | X}%
  \multirow{2}{*}{\makecell{\bfseries Num Gens \\ \bfseries Elapsed}}& \multicolumn{4}{m{0.6\columnwidth}}{\bfseries \centering
  Guaranteed MRCA-Recency-Proportional Resolution}\\ % specify table head
  \bfseries  & 1 & 4 & 10 & 100\\\hline\hline  % specify table head
  \csvreader[
    filter expr={
          test{\ifnumgreater{\thecsvinputline}{2}}
    }
  ]{\importpath submodules/hereditary-stratigraph-concept-binder/binder/retention-policies/a=space-complexity+policy=recency-proportional-resolution+ext=.csv}{}% use head of csv as column names
{\num[scientific-notation=true,round-precision=2,round-mode=figures]{\csvcolii} & \csvcoliii & \csvcoliv & \csvcolv & \csvcolvi\\}% specify your columns here
\end{tabularx}
}
\caption{
Number strata retained after one thousand, one million, one billion, and one trillion generations under the recency-proportional resolution stratum retention policy.
Four different policy parameterizations are shown, the first where MRCA generation can be determined between two extant columns with a guaranteed relative error of 100\%, the second 25\%, the third 10\%, and the fourth 1\%.
A column's memory footprint will be a constant factor of these retained counts based on the fingerprint differentia width chosen.
For example, if single byte differentia were used, the column's memory footprint in bits would be $8\times$ the number of strata retained.
} \label{tab:recency-proportional-space-complexity}
\end{table}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/tab/reconstruction-quality-results-by-differentia-bits.tex <==
\input{lib/C.tex}
\input{lib/dissertationonly.tex}
% \input{lib/importpath.tex}
\makeatletter
  \def\importpathx{\import@path}
\makeatother

\begin{singlespacing}
\dissertationonly{\fontsize{9}{10}\selectfont}
\csvreader[
  longtable=C{3cm}cccccc,
  table head=\caption{
    Comparison of phylogenetic reconstruction quality across differentia bit counts.
    Reconstruction quality measured as clustering information distance (lower is better), mutual clustering information (higher is better), and generalized Robinson-Foulds similarity (higher is better) between reconstructed phylogeny and ground truth phylogeny \citep{smith2020information, smith2020treedist}.
    RPR is recency-proportional resolution stratum retention policy and TDPR is tapered depth-proportional resolution stratum retention policy.
  }\label{tab:reconstruction-quality-results-by-differentia-bits} \\
    \toprule \thead{Tree Comparison Metric} & \thead{Selection\\ Scheme} & \thead{Stratum\\ Retention\\ Policy} & \thead{Target\\ Num\\ Column\\ Bits} & \thead{1 \\Differentia \\ Bit\\ Score} & \thead{8 \\Differentia \\ Bits\\ Score} & \thead{64 \\Differentia \\ Bits\\ Score} \\ \midrule\endfirsthead
    \caption*{\tablename{} \thetable{} (cont'd)} \\
    \toprule \thead{Tree Comparison Metric} & \thead{Selection\\ Scheme} & \thead{Stratum\\ Retention\\ Policy} & \thead{Target\\ Num\\ Column\\ Bits} & \thead{1 \\Differentia \\ Bit\\ Score} & \thead{8 \\Differentia \\ Bits\\ Score} & \thead{64 \\Differentia \\ Bits\\ Score} \\ \midrule\endhead
    \bottomrule\endfoot,
  late after line=\\,
]{\importpathx submodules/hereditary-stratigraph-concept-binder/binder/reconstruction-quality/outplots/reconstruction_quality_results_by_differentia_bits.csv}{}
{\vcell{\csvcoli} & \vcell{\csvcolii} & \vcell{\csvcoliii} & \vcell{\csvcoliv} & \vcell{\csvcolv} & \vcell{\csvcolvi} & \vcell{\csvcolvii} \\[-\rowheight]
\printcellmiddle & \printcellmiddle & \printcellmiddle & \printcellmiddle & \printcellmiddle & \printcellmiddle & \printcellmiddle \\}
\end{singlespacing}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/tab/reconstruction-quality-results-by-policy.tex <==
\input{lib/dissertationonly.tex}

% \input{lib/importpath.tex}
\makeatletter
  \def\importpathx{\import@path}
\makeatother

\begin{singlespacing}
\dissertationonly{\fontsize{9}{10}\selectfont}
\csvreader[
  longtable=cccccc,
  table head=\caption{
    Comparison of phylogenetic reconstruction quality between stratum retention policies.
    Reconstruction quality measured as clustering information distance (lower is better), mutual clustering information (higher is better), and generalized Robinson-Foulds similarity (higher is better) between reconstructed phylogeny and ground truth phylogeny \citep{smith2020information, smith2020treedist}.  }\label{tab:reconstruction-quality-results-by-policy} \\
    \toprule \thead{Tree Comparison Metric} & \thead{Selection\\ Scheme} & \thead{Num\\ Differentia\\ Bits} & \thead{Target\\ Num\\ Column\\ Bits} & \thead{Recency- \\Proportional \\ Resolution\\ Score} & \thead{Tapered\\ Depth-\\ Proportional\\ Resolution\\ Score} \\ \midrule\endfirsthead
    \caption*{\tablename{} \thetable{} (cont'd)} \\
    \toprule \thead{Tree Comparison Metric} & \thead{Selection\\ Scheme} & \thead{Num\\ Differentia\\ Bits} & \thead{Target\\ Num\\ Column\\ Bits} & \thead{Recency- \\Proportional \\ Resolution\\ Score} & \thead{Tapered\\ Depth-\\ Proportional\\ Resolution\\ Score} \\ \midrule\endhead
    \bottomrule\endfoot,
  late after line=\\,
]{\importpathx submodules/hereditary-stratigraph-concept-binder/binder/reconstruction-quality/outplots/reconstruction_quality_results_by_policy.csv}{}
{\csvcoli & \csvcolii & \csvcoliii & \csvcoliv & \csvcolv & \csvcolvi}
\end{singlespacing}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/text/abstract.tex <==
\begin{abstract}
Phylogenies provide direct accounts of the evolutionary trajectories behind evolved artifacts in genetic algorithm and artificial life systems.
Phylogenetic analyses can also enable insight into evolutionary and ecological dynamics such as selection pressure and frequency-dependent selection.
Traditionally, digital evolution systems have recorded data for phylogenetic analyses through perfect tracking where each birth event is recorded in a centralized data structure.
This approach, however, does not easily scale to distributed computing environments where evolutionary individuals may migrate between a large number of disjoint processing elements.
To provide for phylogenetic analyses in these environments, we propose an approach to enable phylogenies to be inferred via heritable genetic annotations rather than directly tracked.
We introduce a “hereditary stratigraphy” algorithm that enables efficient, accurate phylogenetic reconstruction with tunable, explicit trade-offs between annotation memory footprint and reconstruction accuracy.
In particular, we demonstrate an approach that enables estimation of the most recent common ancestor (MRCA) between two individuals with fixed relative accuracy irrespective of lineage depth while only requiring logarithmic annotation space complexity with respect to lineage depth.
This approach can estimate, for example, MRCA generation of two genomes within 10\% relative error with 95\% confidence up to a depth of a trillion generations with genome annotations smaller than a kilobyte.
We also simulate inference over known lineages, recovering up to 85.70\% of the information contained in the original tree using 64-bit annotations.
\end{abstract}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/text/acknowledgement.tex <==
\section*{Acknowledgment}


This research was supported in part by NSF grants DEB-1655715 and DBI-0939454 as well as by Michigan State University through the computational resources provided by the Institute for Cyber-Enabled Research.
This material is based upon work supported by the National Science Foundation Graduate Research Fellowship under Grant No. DGE-1424871.
Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the National Science Foundation.
Thank you to Santiago Rodriguez Papa for manuscript comments.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/text/body.tex <==
\input{text/body/introduction.tex}

\input{text/body/methods.tex}

\input{text/body/results-and-discussion.tex}

\input{text/body/conclusion.tex}


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/text/body/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}

To our knowledge, this work provides a novel design for digital genome components that enable phylogenetic inference on asexual populations.
This provides a viable alternative to perfect phylogenetic tracking, which is complex and possibly cumbersome in distributed computing scenarios, especially with fallible nodes.
Our approach enables flexible, explicit trade-offs between space complexity and inference accuracy.
Hereditary stratigraphic columns are efficient: our approach can estimate, for example, the MRCA generation of two genomes within 10\% error with 95\% confidence up to a depth of a trillion generations with genome annotations smaller than a kilobyte.
However, they are also powerful: we were able to achieve tree reconstructions recovering up to 85.70\% of the information contained in the original tree with only a 64-bit memory footprint.

This and other methodology to enable decentralized observation and analysis of evolving systems will be essential for artificial life experiments that use distributed and best-effort computing approaches.
Such systems will be crucial to enabling advances in the field of artificial life, particularly with respect to the question of open-ended evolution \citep{ackley2011pursue,moreno2021conduit,moreno2021case}
Mork work is called for to further enable experimental analyses in distributed, best-effort systems while preserving those systems' efficiency and scalability.
As parallel and distributed computing becomes increasingly ubiquitous and begins to more widely pervade artificial life systems, hereditary stratigraphy should serve as a useful technique in this toolbox.

Important work extending and analyzing hereditary stratigraphy remains to be done.
Analyses should be performed to expound MRCA resolution guarantees of stratum retention policies when using narrow (i.e., single-bit) differentia.
Constant-size-complexity stratum retention policies that preferentially retain a denser sampling of more-recent strata should be developed and analyzed.
Extensions to sexual populations should be explored, including the possibility of annotating and tracking individual genome components instead of whole-genome individuals.
An alternate approach might be to define a preferential inheritance rule so that at each generation slot within a column, a single differentia sweeps over an entire interbreeding population.
Optimization of tree reconstruction from extant hereditary stratigraphs remains an open question, too, particularly with regard to properly handling multifurcations.
It would be particularly valuable to develop methodology to annotate inner nodes of trees reconstructed from hereditary stratigraphs with confidence levels.

The problem of designing genomes to maximize phylogenetic reconstructability raises unique questions about phylogenetic estimation.
Such a backward problem --- optimizing genomes to make analyses trivial as opposed to the usual process of optimizing analyses to genomes --- puts questions about the genetic information analyses operate on in a new light.
In particular, it would be interesting to derive upper bounds on phylogenetic inference accuracy given genome size and generations elapsed.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/text/body/introduction.tex <==
\section{Introduction} \label{sec:introduction}

In traditional serially-processed digital evolution experiments, phylogenetic trees can be tracked perfectly as they progress \citep{bohm2017mabe,wang2018vine,lalejini2019data} rather than reconstructed afterward, as must be done in most biological studies of evolution.
Such direct phylogenetic tracking enables experimental possibilities unique to digital evolution, such as perfect reconstruction of the sequence of phylogenetic states that led to a particular evolutionary outcome \citep{lenski2003evolutionary, dolson2020interpreting}.
In a shared-memory context, it is not difficult to maintain a complete phylogeny by ensuring that offspring retain a permanent reference to their parent (or vice versa).
As simulations progress, however, memory usage would balloon if all simulated organisms were stored permanently.
Garbage collecting extinct lineages and saving older history to disk greatly ameliorates this issue \citep{bohm2017mabe,dolson2019modes}.

If sufficient memory or disk space can be afforded to log all reproduction events, recording a perfect phylogeny in a distributed context is also not especially difficult.
Processes could maintain records of each reproduction event, storing the parent organism (and its associated process) with all generated offspring (and their destination processes).
As long organisms are uniquely identified globally, these ``dangling ends'' could be joined in postprocessing to weave a continuous global phylogeny.
Of course, for the huge population sizes made possible by distributed systems, such stitching may become a demanding task in and of itself.
Additionally, even small amounts of lost or corrupted data could fundamentally degrade tracking by disjoining large tree subsections.

However, if memory and disk space are limited, distributed phylogeny tracking becomes a more burdensome challenge.
A naive approach might employ a server model to maintain a central store of phylogenetic data.
Processes would dispatch notifications of birth and death events to the server, which would curate (and garbage collect) phylogenetic history much the same as current serial phylogenetic tracking implementations.
Unfortunately, this server model approach would present scalability challenges: burden on the server process would worsen in direct proportion to processor count.
% ELD: This is making me wonder if there's a middle ground that could be explored in the future where we could use a sort of UDP phylogeny protocol, where no confirmation occurs
This approach would also be similarly brittle to any lost or corrupted data.

A more scalable approach might record birth and death events only on the process(es) where they unfold.
However, lineages that went extinct locally could not be safely garbage collected until the extinction of their offspring's lineages on other processors could be confirmed.
Garbage collection would thus require extinction notifications to wind back across processes each lineage had traversed.
Again, this approach would also be brittle to loss or corruption of data.

% Under a best-effort model, no system of phylogeny tracking can guarantee proper garbage collection.
% For example, it would be possible for an offspring that was dispatched to a neighboring process to have failed to arrive, and both processes would need to keep going, despite the failure.
% So, extinction notifications for the lineage founded by that offspring would never be dispatched --- putting in motion a memory leak of un-garbage-collectible phylogenetic history.
% The situation becomes even more leaky when the possibility of extinction notifications themselves being lost.

In a distributed context --- especially, a distributed, best-effort context --- phylogenetic reconstruction (as opposed to tracking) could prove simpler to implement, more efficient at runtime, and more robust to data loss while providing sufficient information to address experimental questions of interest.
However, phylogenetic reconstruction from genomes with a traditional model of divergence under gradual accumulation of random mutations poses its own difficulties, including
\begin{itemize}
\item accounting for heterogeneity in evolutionary rates (i.e., the rate at which mutations accumulate due to divergent mutation rates or selection pressures) between lineages \citep{lack2010identifying},
\item performing sequence alignment \citep{casci2008lining},
\item mutational saturation \citep{hagstrom2004using},
\item appropriately selecting and applying complex reconstruction algorithms \citep{kapli2020phylogenetic}, and
\item computational intensity \citep{sarkar2010hardware}.
\end{itemize}

The computational flexibility of digital artificial life experiments provides a unique opportunity to overcome these challenges: designing heritable genome annotations specifically to ensure simple, efficient, and effective phylogenetic reconstruction.
For maximum applicability of such a solution, these annotations should be phenotypically neutral heritable instrumentation \citep{stanley2002evolving} that can be applied to any digital genome.

In this paper, we present ``hereditary stratigraphy,'' a novel heritable genome annotation system to facilitate post-hoc phylogenetic inference on asexual populations.
This system allows explicit control over trade-offs between space complexity and accuracy of phylogenetic inference.
Instead of modeling genome components diverging through a neutral mutational process, we keep a record of historical checkpoints that allow comparison of two lineages to identify the range of time in which they diverged.
Careful management of these checkpoints allows for a variety of trade-off options, including:
\begin{itemize}
  \item linear space complexity and fixed-magnitude inference error,
  \item constant space complexity and inference error linearly proportional to phylogenetic depth, and
  \item logarithmic space complexity and inference error linearly proportional to time elapsed since MRCA (which we suspect will be the most broadly useful trade-off).
\end{itemize}

In Methods we motivate and explain the hereditary stratigraphy approach.
Then, in Results and Discussion we simulate post-hoc inference on known phylogenies to assess the quality of phylogenetic reconstruction enabled by the hereditary stratigraphy method.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/text/body/methods.tex <==
\section{Methods} \label{sec:methods}

This section will introduce intuition for the strategy of our hereditary stratigraph approach, define the vocabulary we developed to describe aspects of this approach, overview configurable aspects of the approach, present mathematical exposition of the properties of space complexity and inference quality under particular configurations, and then recap digital experiments that demonstrate this approach in an applied setting.

\subsection{Hereditary Strata and the Hereditary Stratigraphic Column}

\input{fig/column-comparison.tex}

Our algorithm, particularly the vocabulary we developed to describe it, draws loose inspiration from the concept of geological stratigraphy, inference of natural history through analysis of successive layers of geological material \citep{steno1916prodromus}.
As an introductory intuition, suppose a body of rock being built up through regular, discrete events depositing of geological material.
Note that in such a scenario we could easily infer the age of the body of rock by counting up the number of layers present.
% Note that it is crucial to this scenario that each layer has some differentiating feature that allows it to be distinguished from layers above and below it, but also potentially from layers present in another body of rock in a distant and unrelated geographic position.
Next, imagine making a copy of the rock body in its partially-formed state and then moving it far away.
As time runs forward on these two rock bodies, independent layering processes will cause consistent disparity in the layers forming on each forwards from their point of separation.

To deduce the historical relationship of these rock bodies, we could simply align and compare their layers.
Layers from their base up through the first disparity would correspond to shared ancestry; further disparate layers would correspond to diverged ancestry.
% Interestingly, and powerfully for phylogenetic inference, we can readily distinguish a scenario where both rock bodies deposited ten layers after diverging from a scenario where one deposited eighteen layers and the other deposited two.
Figure \ref{fig:column-comparison} depicts the process of comparing columns for phylogenetic inference.

Shifting now from intuition to implementation, a fixed-length randomly-generated binary tag provides a suitable ``fingerprint'' mechanism mirroring our metaphorical ``rock layers.''
We call this ``fingerprint'' tag a \textit{differentia}.
The width of this tag controls the probability of spurious collisions between independently generated instances.
At 64 bits wide the tag effectively functions as a UID: collisions between randomly generated tags are so unlikely ($p < 5.42\times10^{-20}$) they can essentially be ignored.
At the other end of the spectrum, collision probability would be $1/256$ for a single byte and $1/2$ for a single bit.
In the case of narrow differentia, in order to set a lower bound for the MRCA generation, you would have to backtrack common strata from the last commonality until the probability of that many successive spurious collisions was enough to satisfy your desired confidence level (e.g., 95\% confidence).
Even then, there would be a possibility of the the true MRCA falling before the estimated lower bound.
Note, however, that no matter the width of the differentia the generation of the first discrepancy provides a hard upper bound on the generation of the MRCA.

In accordance with our geological analogy, we refer to the packet of data accumulated each generation as a \textit{stratum}.
This packet contains the differentia and, although not employed in this work, could hold other arbitrary user-defined data (i.e., simulation timestamp, phenotype characteristics, etc.).
Again in accordance with the geological analogy, we refer to the chronological stack of strata that accumulate over successive generations as a \textit{hereditary stratigraphic column}.

\subsection{Stratum Retention Policy}

\input{fig/deposit-process.tex}

As currently stated, strata in each column will accumulate proportionally to the length of evolutionary history simulated.
In an evolutionary run with thousands or millions of generations, this approach would soon become intractable --- particularly when columns are serialized and transmitted between distributed computing elements.
To solve this problem, we can trade off precision for compactness by strategically deleting strata from columns as time progresses.
Figure \ref{fig:deposit-process} overviews how stratum deposit and stratum elimination might progress over two generations under the hereditary stratigraphic column scheme.

Different patterns of deletion will lead to different trade-offs, both in terms of the scaling relationship of column size to generations elapsed and in terms of the arrangement of inference precision over evolutionary history (i.e., focusing precision on more recent evolutionary history versus spreading it evenly over the entire history).

We refer to the rule set used to selectively eliminate strata over time as the ``stratum retention policy.''
We explore several different retention policy designs here, and implement our software to allows for free, modular interchange of retention policies.

Our software allows specification of a policy as either a ``predicate'' or a ``generator.''
The predicate method requires a function that takes the generation of a stratum and the current number of strata deposited and returns whether that stratum should be retained at that point in time.
The generator method requires a function that takes the current number of strata deposited and yields the set of generations that should be deleted at that point in time.
Although the predicate form of a policy is useful for analyzing and proving properties of policies, the generator form is generally more efficient in practice.
We provide equivalent predicate and generator implementations for each stratum retention policy discussed here.

Strata elimination causes a stratum's position within the column data structure to no longer correspond to the generation it was deposited.
Therefore, it may seem necessary to store the generation of deposit within the stratum data structure.
However, for all deterministic retention policies a perfect mapping exists backwards from column index to recover generation deposited without storing it.
We provide this formula for each stratum retention policy surveyed here.
Finally, for each policy we provide a formula to calculate the exact number of strata retained under any parameterization after $n$ generations.

The next subsections introduce several stratum retention policies, explain the intuition behind their implementation, and elaborate their space complexity and resolution properties.
For each policy, patterns of stratum retention are illustrated in Figure \ref{fig:retention-policies}.
The formulas for number of strata retained after $n$ generations, the formulas to calculate stratum deposit generation from column index, and the retention predicate specifications of each policy are available in Supplementary Section \ref{sec:condemner-implementations}.
The generator specification of each policy is available in Supplementary Section \ref{sec:predicate-implementations}.
For tapered depth-proportional resolution and recency-proportional resolution, the accuracy of MRCA estimation can also be explored via an interactive in-browser web applet at \url{https://hopth.ru/bi}.

\input{fig/retention-policies.tex}

\subsection{Fixed Resolution Stratum Retention Policy}

The fixed resolution retention policy imposes a fixed absolute upper bound $r$ on the spacing between retained strata.
The strategy is simple: permanently retain a stratum every $r$th generation.
(For arbitrary reasons of implementation convenience, we also require each stratum to be retained during at least the generation it is deposited).
See top panel of Figure \ref{fig:retention-policies}.

This retention policy suffers from linear growth in a column's memory footprint with respect to number of generations elapsed: every $r$th generation generation a new stratum is permanently retained.
For this reason, it is likely not useful in practice except potentially in scenarios where the number of generations is small and fixed in advance.
We include it here largely for illustrative purposes as a gentle introduction to retention policies.

\subsection{Depth-Proportional Resolution Stratum Retention Policy}

The depth-proportional resolution policy ensures spacing between retained strata will be less than or equal to a proportion $1/r$ of total number of strata deposited $n$.
Achieving this limit on uncertainty requires retaining sufficient strata so that no more than $n/r$ generations elapsed between any two strata.
This policy accumulates retained strata at a fixed interval until twice as many as $r$ are at hand.
Then, every other retained stratum is purged and the cycle repeats with a new twice-as-wide interval between retained strata.
See second from top panel of Figure \ref{fig:retention-policies}.

When comparing stratigraphic columns from different generations, the resolution guarantee holds in terms of the number of generations experienced by the older of the two columns.
Because this retention policy is deterministic, for two columns with the same policy, every stratum that is held by the older column is also guaranteed to be present in the younger column (unless it hasn't yet been deposited on the younger column).
Therefore, the strata that would enable the desired resolution when comparing two columns of the same age are guaranteed to be available, even when one column has elapsed more generations.

Because the number of strata retained under this policy is bounded as $2r+1$, space complexity scales as $O(1)$ with respect to the number of strata deposited.
It follows that the MRCA generation estimate uncertainty scales as $O(n)$ with respect to the number of strata deposited.

\subsection{Tapered Depth-Proportional Resolution Stratum Retention Policy}

This policy refines the depth-proportional resolution policy to provide a more stable column memory footprint over time.
The naive depth-proportional resolution policy builds up strata until twice as many are present as needed then purges half of them all at once.
The tapered depth-proportional resolution policy functions identically to the depth-proportional policy except that it removes unnecessary strata gradually from back to front as new strata are deposited, instead of eliminating them simultaneously.
See third from top panel of Figure \ref{fig:retention-policies}.

The column footprint stability of this variation makes it easier to parameterize our experiments to ensure comparable end-state column footprints for fair comparison between retention policies, in addition to making this policy likely better suited to most use cases.
By design, this policy has the same space complexity and MRCA estimation uncertainty scaling relationships with number generations elapsed as the naive depth-proportional resolution policy.

\subsection{MRCA-Recency-Proportional Resolution Stratum Retention Policy}

\input{tab/recency-proportional-space-complexity.tex}

The MRCA-recency-proportional resolution policy ensures distance between the retained strata surrounding any generation point will be less than or equal to a user-specified proportion $1/r$ of the number of generations elapsed since that generation.

This policy can be constructed recursively.
So, to begin, let's consider setting up just the \textit{first} generation $g$ of the stratum after the root ancestor we will retain when $n$ generations have elapsed.
A simple geometric analysis reveals that providing the guaranteed resolution for the worst-case generation within the window between generation 0 and generation $g$ (i.e., generation $g-1$) requires
\begin{align*}
  g \leq \lfloor n / (r + 1) \rfloor.
\end{align*}

We now have an upper bound for the generation of the first stratum generation we must retain.
However, we must guarantee that strata at these generations are actually available for us to retain (i.e., haven't been purged out of the column at a previous time point).
We will do this by picking the generation that is the highest power of 2 less than or equal to our bound.
If we repeat this procedure as we recurse, we are guaranteed that this generation's stratum will have been preserved across all previous timepoints.

Why does this work?
Consider a sequence where all elements are spaced out by strictly nonincreasing powers of 2.
Consider the first element of the list.
All multiples this first element will be included in the list.
So, when we ratchet up $g$ to $2g$ as $n$ increases, we are guaranteed that $2g$ has been retained.
This principle generalizes recursively down the list.
This is a similar principle to the approach of strictly-doubling interval sizes used in the Depth-Proportional Resolution stratum retention policies described above.

This step of truncating to the nearest less than or equal to power of 2 affects our recursive step size is at most halved.
So, because step size is a constant fraction of remaining generations $n$ (at worst $\frac{n}{2(r+1)}$), the number of steps made (and number of strata retained) scales as $O(\log(n))$ with respect to the number of strata deposited.
Table \ref{tab:recency-proportional-space-complexity} provides exact figures for the number of strata retained under different parameterizations of the recency-proportional retention policy between one thousand and one trillion generations.

As for MRCA generation estimate uncertainty, in the worst case it scales as $O(n)$ with respect to the greater number of strata deposited.
However, with respect to estimating the generation of the MRCA for lineages diverged any fixed number of generations ago, uncertainty scales as $O(1)$.

How does space complexity scale with respect to the policy's specified resolution $r$?
Through extrapolation from OEIS sequences A063787 and A056791 via guess and check \citep{sloane2021a063787,sloane2021a056791}, we posited the exact number of strata retained after $n$ generations as

\begin{align*}
  \mathrm{HammingWeight}(n)
  + \sum_1^r \lfloor \log_2( \lfloor n / r \rfloor ) \rfloor
  + 1.
\end{align*}

This expression has been unit tested extensively to ensure perfect reliability.
Approximating and applying logarithmic properties, this policy's space complexity can be calculated within a constant factor as

\begin{align*}
\log(n) + \log\Big(\frac{n^r}{r!}\Big).
\end{align*}

To analyze the relationship between space complexity and resolution $r$, we will examine the ratio of space complexities induced when scaling resolution $r$ up by a constant factor $f > 1$.
Evaluating this ratio as $r \to \infty$, we find that space complexity scales directly proportional to $f$,

\begin{align*}
\lim_{r \to \infty}
\frac{
  \log(n) + \log\Big(\frac{n^{fr}}{(fr)!}\Big)
}{
  \log(n) + \log\Big(\frac{n^r}{r!}\Big)
}
= f.
\end{align*}

Evaluating this ratio as $n \to \infty$, we find that this scaling relationship is never worse than directly proportional for any $r$,

\begin{align*}
\lim_{n \to \infty}
\frac{
  \log(n) + \log\Big(\frac{n^{fr}}{(fr)!}\Big)
}{
  \log(n) + \log\Big(\frac{n^r}{r!}\Big)
}
&= \frac{fr+1}{r+1}\\
&= f\frac{r + 1/f}{r + 1}\\
&\leq f.
\end{align*}


\subsection{Computational Experiments}

In order to assess the practical performance of the hereditary stratigraph approach in an applied setting, we simulated the process of stratigraph propagation over known ``ground truth'' phylogenies extracted from pre-existing digital evolution simulations \citep{hernandez2022phylogenetic}.
These simulations propagated populations of between 100 and 165 bitstrings between 500 and 5,000 synchronous generations under the NK fitness landscape model \citep{kauffman1989nk}.
In order to ensure coverage of a variety of phylogenetic conditions, we sampled a variety of selection schemes that impose profoundly different ecological regimens \citep{dolson2018ecological},
\begin{itemize}
  \item EcoEA Selection \citep{goings2012ecology},
  \item Lexicase Selection \citep{helmuth2014solving},
  \item Random Selection, and
  \item Sharing Selection \citep{goldberg1987genetic}.
  % \item Tournament Selection \citep{miller1995genetic}.
\end{itemize}

Supplementary Table \ref{tab:ground-truth-phylogenies} provides full details on the conditions each ground truth phylogeny was drawn from.
The phylogenies themselves are available with our supplementary material.

For each ground truth phylogeny, we tested combinations of three configuration parameters:
\begin{itemize}
  \item target end-state memory footprints for extant columns (64, 512, and 4096 bits),
  \item differentia width (1, 8, and 64 bits), and
  \item stratum retention policy (tapered depth-proportional resolution and recency-proportional resolution).
\end{itemize}

Stratum retention policies were parameterized so that the maximum number of strata possible were present at the end of the experiment without exceeding the target memory footprint.
If the target memory footprint is exceeded by the sparsest possible parameterization of a retention policy, then that sparsest possible parameterization was used.
Supplementary Tables \cref{tab:experiment-column-sizes-nk-ecoea-selection,tab:experiment-column-sizes-nk-lexicase-selection,tab:experiment-column-sizes-nk-random-selection,tab:experiment-column-sizes-nk-sharing-selection,tab:experiment-column-sizes-nk-tournament-selection} provide the calculated paramaterizations and memory footprints of extant columns.

\input{fig/phylogenetic-inference.tex}

In order to assess the viability of phylogenetic inference using hereditary stratigraphic columns from extant organisms, we used the end-state stratigraphs to reconstruct an estimate of the actual ground truth phylogenetic histories.
The first step to reconstructing a phylogenetic tree for the history of an extant population at the end of an experiment is to construct a distance matrix by calculating all pairwise phylogenetic distances between extant columns.
We defined phylogenetic distance between two extant columns as the sum of each extant organism's generational distance back to the generation of their MRCA, estimated as the mean of the upper and lower 95\% confidence bounds.
Figure \ref{fig:phylogenetic-inference} provides a cartoon summary of the process of calculating phylogenetic distance between two extant columns.

We then used the unweighted pair group method with arithmetic mean (UPGMA) reconstruction tool provided by the BioPython package to generate estimate phylogenetic trees \citep{cock2009biopython,sokal1958statistical}.
After generating the reconstructed tree topology, we performed a second pass to adjust branch lengths so that each internal tree node sat at the mean of its estimated 95\% confidence generation bounds.
%We found that the neighbor joining (NJ) approach occasionally yielded reconstructions with impossible ``negative generation'' branches \citep{saitou1987neighbor} after knowledge bounding the absolute generation of internal nodes (i.e., MRCA's between pairs of extant organisms) was applied, so we did not use it.

\subsection{Software and Data}

% A prototype of this approach has been implemented \url{https://github.com/mmore500/dishtiny/blob/incoming/include/dish2/genome/PhyloFingerprints.hpp} and preliminarily tested \url{https://github.com/mmore500/dishtiny/blob/incoming/tests/dish2/genome/PhyloFingerprints.cpp}.

As part of this work, we published the \texttt{hstrat} Python library with a stable public-facing API intended to enable incorporation in other projects with extensive documentation and unit testing on GitHub at \url{https://github.com/mmore500/hstrat} and on PyPI.% at \url{https://pypi.org/project/hstrat/}.
In the near future, we intend to complete and publish a corresponding C++ library.

Supporting software materials can be found on GitHub at \url{https://github.com/mmore500/hereditary-stratigraph-concept}
Supporting computational notebooks are available for in-browser use via BinderHub at \url{https://hopth.ru/bk} \citep{ragan2018binder}.
Our work benefited from many pieces of open source scientific software \citep{sukumaran2010dendropy,virtanen2020scipy,hunter2007matplotlib,virtanen2020scipy,waskom2021seaborn,bostock2011d3,meurer2017sympy,smith2020treedist,smith2020treedistdata,paradis2004ape,ushey2022reticulate,wickham2022dplyr}.
The ground truth phylogenies used in this work as well as supplementary figures, tables, and text are available via the Open Science Framework at
\url{https://osf.io/4sm72/} \citep{foster2017open,moreno2022hstratconceptsupplement}.
Phylogenetic data associated with this project is stored in the Alife Community Data Standards format \citep{lalejini2019data}.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/text/body/results-and-discussion.tex <==
\section{Results and Discussion} \label{sec:results}

\input{fig/reconstruction-example.tex}

In this section, we analyze the quality of reconstructions of known phylogenetic trees using hereditary stratigraphy.
Figure \ref{fig:reconstruction-example} compares an example reconstruction from columns using tapered depth-proportional stratum retention, an example reconstruction using recency-proportional stratum retention,  and the underlying ground truth phylogeny.
Interactive in-browser visualizations comparing all reconstructed phylogenies to their corresponding ground truth are available at \url{https://hopth.ru/bi}. %TODO: replace this with anonymous link

\subsection{Reconstruction Accuracy}

Measuring tree similarity is a challenging problem, with many conflicting approaches that all provide different information \citep{smith2020information}.
Ideally, we would use a metric of reconstruction accuracy that 1) is commonly used so that there exists sufficient context to understand what constitutes a good value, 2) behaves consistently across different types of trees, and 3) behaves reasonably for the types of trees common in artificial life data.
Unfortunately, these objectives are somewhat in conflict.
The primary source of this problem is multifurcations, nodes from which more than two lineages branch at once.
In reconstructed phylogenies in biology, multifurcations are generally assumed to be the result of insufficient information.
It is thought that the real phylogeny had multiple bifurcations that occurred so close together that the reconstruction algorithm is unable to separate them.
In artificial life phylogenies, however, we have the opposite problem.
When we perfectly track a phylogeny, it is common for us to know that a multifurcation did in fact occur.
However, it is challenging for our reconstructions to properly identify multifurcations, because it requires perfectly lining up multiple divergence times.
Many of the most popular tree distance metrics interpret the difference between a multifurcation and a set of bifurcations as a dramatic change in topology.
For some use cases, this change in topology may indeed be meaningful, although research on the extent of this problem is limited.
Nevertheless, we suspect that for the majority of use cases, the tiny branch lengths between the internal nodes will make this source of error relatively minor.

To overcome this obstacle, we have measured our reconstruction accuracy using multiple metrics.
We will primarily focus on Mutual Clustering Information (as implemented in the R TreeDist package) \citep{smith2020treedist}, which is a direct measure of the quantity of information in the ground truth phylogeny that was successfully captured in the reconstruction.
It is relatively unaffected by the failure to perfectly reproduce multifurcations.
For the purposes of easy comparison to the literature, we also measured the Clustering Information Distance \citep{smith2020treedist}.

\input{fig/info_plot.tex}

Across ground truth phylogenies, we were able to reconstruct the phylogenetic topology with between 47.75\% and 85.70\% of the information contained in the original tree using a 64-bit column memory footprint, between 47.75\% and 80.36\% using a 512-bit column memory footprint, and between 51.13\% and 83.53\% using a 4096-bit column memory footprint.
While the Clustering Information Distance reached its maximum possible score (1.0) for the heavily-multifurcated EcoEA phylogeny, it agreed with the Mutual Clustering Information score for less multifurcated phylogenies, such as fitness sharing.
Using the Recency Proportional Resolution retention policy and a 4096-bit column memory footprint, we were able to reconstruct a fitness sharing phylogeny with a Clustering Information Distance of only 0.2923471 from the ground truth.
For context, that result is comparable to the distance between phylogenies reconstructed from two closely-related proteins in H3N2 flu (0.25) \citep{jones2021parallel}.
To build further intuition, we strongly encourage readers to refer to our interactive web reconstruction.
Figure \ref{fig:info_plot} summarizes error reconstructing the fitness sharing selection phylogeny in terms of the mutual clustering information metric \citep{smith2022robust}.
The phylogenies reconstructed from the EcoEA condition performed comparably, with lexicase and random selection faring somewhat worse \citep{moreno2022hstratconceptsupplement}.
In the case of random selection, we suspect that this reduced performance is the result of having many nodes that originated very close together at the end of the experiment.
As expected, we did observe overall more accurate reconstructions from columns that were allowed to occupy larger memory footprints.

\subsection{Differentia Size}

Among the surveyed ground truth phylogenies and target column footprints, we consistently found that smaller differentia were able to yield more or as accurate phylogenetic reconstructions.
The stronger performance of narrow differentia was particularly apparent in low-memory-footprint scenarios where overall phylogenetic inference power was weaker.
Overall, single-bit differentia outperformed 64-bit differentia under 20 conditions, and were indistinguishable under 6 conditions, and were worse under 4 conditions.
We used Cluster Information Distance to perform these comparisons.
Full results are available in Supplementary Section \ref{sec:differentia-size-full}.
Although narrower differentia have less distinguishing power on their own, their smaller size allows more to be packed into the memory footprint to cover more generations, which seems to help reconstruction power.
We must note that narrower differentia can pack more thoroughly into the footprint caps we imposed on column size, so their extant columns tended to have slightly more overall bits.
However, this was a small enough imbalance (in most cases $<10\%$) that we believe it is unlikely to fully account for the stronger performance of narrow-differentia configurations.

\subsection{Retention Policy}

Across the surveyed ground truth phylogenies and target column memory footprints, we found that the recency-proportional resolution stratum retention policy generally yielded better phylogenetic reconstructions.
Phylogenetic reconstruction quality was better in 28 conditions, equivalent in 13 conditions, and worse in 4 conditions.
Again, this effect was most apparent in the small-stratum-count scenarios where overall inference power was weaker.
We used Cluster Information Distance to perform these comparisons.
Full results are available in Supplementary Section \ref{sec:retention-policy-full}.
The stronger performance of recency-proportional resolution is likely due to the denser retention of recent strata under the recency-proportional metric, which help to resolve the more numerous (and therefore typically more tightly spaced) phylogenetic events in the near past \citep{zhaxybayeva2004cladogenesis}.
Recency-proportional resolution tended to be able to fit fewer strata within the prescribed memory footprints (except in cases where it could not fit within the footprint) so its stronger performance cannot be attributed to more retained bits in the end-state extant columns.


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/text/frontmatter.tex <==
\title{ Hereditary Stratigraphy: Genome Annotations to Enable Phylogenetic Inference over Distributed Populations }

\author{Matthew Andres Moreno, Emily Dolson, \and Charles Ofria \\
\mbox{}\\
Michigan State University, East Lansing, MI 48103 \\
mmore500@msu.edu}

\maketitle


==> hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/tex/text/references.tex <==
% \section*{References}

\putbib


==> hereditary-stratigraph-concept/tex/tab/_experimentcolumnsizesmacro.tex <==
% \pragmaonce
% ^adapted from https://tex.stackexchange.com/a/195173

% adapted from https://tex.stackexchange.com/a/118450
\providecommand{\experimentcolumnsizesmacro}[2]{
\def\dataname{#1}\def\fulldataname{#2}\input{tab/_experimentcolumnsizestemplate.tex}
}


==> hereditary-stratigraph-concept/tex/tab/_experimentcolumnsizestemplate.tex <==
\input{lib/dissertationonly.tex}
% \input{lib/importpath.tex}
\makeatletter
  \def\importpathx{\import@path}
\makeatother

\begin{table}[h!]

  \caption{
  Hereditary stratigraph column memory footprint outcomes for phylogenetic reconstruction experiments on the \dataname dataset.
  All treatments' stratum retention policies were parameterized to use as much of the target per-column memory footprint as possible without exceeding it.
  Treatments where the stratum retention policy could not be parameterized low enough to meet the target per-column memory footprint are highlighted in red.
  TDPR denotes the ``Tapered Depth-Proportional Resolution'' policy and RPR denotes the ``Recency-Proportional Resolution'' policy.
  }

  % adapted from https://tex.stackexchange.com/a/15708
  \StrSubstitute{\dataname}{ }{-}[\temp]
  \StrSubstitute{\temp}{A}{a}[\temp]
  \StrSubstitute{\temp}{B}{b}[\temp]
  \StrSubstitute{\temp}{C}{c}[\temp]
  \StrSubstitute{\temp}{D}{d}[\temp]
  \StrSubstitute{\temp}{E}{e}[\temp]
  \StrSubstitute{\temp}{F}{f}[\temp]
  \StrSubstitute{\temp}{G}{g}[\temp]
  \StrSubstitute{\temp}{H}{h}[\temp]
  \StrSubstitute{\temp}{I}{i}[\temp]
  \StrSubstitute{\temp}{J}{j}[\temp]
  \StrSubstitute{\temp}{K}{k}[\temp]
  \StrSubstitute{\temp}{L}{l}[\temp]
  \StrSubstitute{\temp}{M}{m}[\temp]
  \StrSubstitute{\temp}{N}{n}[\temp]
  \StrSubstitute{\temp}{O}{o}[\temp]
  \StrSubstitute{\temp}{P}{p}[\temp]
  \StrSubstitute{\temp}{Q}{q}[\temp]
  \StrSubstitute{\temp}{R}{r}[\temp]
  \StrSubstitute{\temp}{S}{s}[\temp]
  \StrSubstitute{\temp}{T}{t}[\temp]
  \StrSubstitute{\temp}{U}{u}[\temp]
  \StrSubstitute{\temp}{V}{v}[\temp]
  \StrSubstitute{\temp}{w}{w}[\temp]
  \StrSubstitute{\temp}{X}{x}[\temp]
  \StrSubstitute{\temp}{Y}{y}[\temp]
  \StrSubstitute{\temp}{Z}{z}[\temp]

  \def\labeltext{%
    {tab:experiment-column-sizes-\temp}%
  }
  \expandafter\label\labeltext

\begin{tabularx}{\columnwidth}{X | X | X | X | X | X}%
  \adjustbox{
    minipage=12em,
    rotate=90,
  }{
    \raggedright
    \bfseries
    Target Per-Column Memory Footprint (bits)
    \par
  }
  & \adjustbox{
      minipage=12em,
      rotate=90,
    }{
      \raggedright
      \bfseries
      Actual Mean Per-Column Memory Footprint (bits)
      \par
  }
  & \adjustbox{
      minipage=12em,
      rotate=90,
    }{
      \raggedright
      \bfseries
      Memory Footprint Percent Error
      \par
  }
  & \adjustbox{
      minipage=12em,
      rotate=90,
    }{
      \raggedright
      \bfseries
      Fingerprint Differentia Width (bits)
      \par
  }
  & \adjustbox{
      minipage=12em,
      rotate=90,
    }{
      \raggedright
      \bfseries
      Stratum Retention Policy
      \par
  }
  & \adjustbox{
      minipage=12em,
      rotate=90,
    }{
      \raggedright
      \bfseries
      Retention Policy Resolution Parameter
      \par
  }
  \\\hline\hline  % specify table head
  \csvreader[
    filter expr={
          test{\ifnumgreater{\thecsvinputline}{2}}
    }
  ]{\importpathx submodules/hereditary-stratigraph-concept-binder/binder/phylogenetic-inference/\fulldataname }{}% use head of csv as column names
{
  \csvcolix
  & \num[round-precision=1,round-mode=places]{\csvcolii}
  &
  \ifthenelse{
    \lengthtest{\csuse{csvcolii}pt > \csuse{csvcolix}pt}
    }{\cellcolor{red!25}}{}%

  \num[round-precision=1,round-mode=places]{
    \fpeval{ 100 * \csvcolii / \csvcolix - 100 }
  }
  & \csvcolvi
  &
  \StrDel{\csvcolvii}{a}[\temp]
  \StrDel{\temp}{b}[\temp]
  \StrDel{\temp}{c}[\temp]
  \StrDel{\temp}{d}[\temp]
  \StrDel{\temp}{e}[\temp]
  \StrDel{\temp}{f}[\temp]
  \StrDel{\temp}{g}[\temp]
  \StrDel{\temp}{h}[\temp]
  \StrDel{\temp}{i}[\temp]
  \StrDel{\temp}{j}[\temp]
  \StrDel{\temp}{k}[\temp]
  \StrDel{\temp}{l}[\temp]
  \StrDel{\temp}{m}[\temp]
  \StrDel{\temp}{n}[\temp]
  \StrDel{\temp}{o}[\temp]
  \StrDel{\temp}{p}[\temp]
  \StrDel{\temp}{q}[\temp]
  \StrDel{\temp}{r}[\temp]
  \StrDel{\temp}{s}[\temp]
  \StrDel{\temp}{t}[\temp]
  \StrDel{\temp}{u}[\temp]
  \StrDel{\temp}{v}[\temp]
  \StrDel{\temp}{w}[\temp]
  \StrDel{\temp}{x}[\temp]
  \StrDel{\temp}{y}[\temp]
  \StrDel{\temp}{z}
  & \csvcolviii
  \\
}% specify your columns here
\end{tabularx}
\end{table}


==> hereditary-stratigraph-concept/tex/tab/experiment-column-sizes-nk-ecoeaselection.tex <==
\input{tab/_experimentcolumnsizesmacro.tex}

\experimentcolumnsizesmacro{NK EcoEA Selection}{a=actual_retained_bits+source=nk_ecoeaselection_seed110_pop100_mut.01_snapshot_3000.csv}


==> hereditary-stratigraph-concept/tex/tab/experiment-column-sizes-nk-lexicaseselection.tex <==
\input{tab/_experimentcolumnsizesmacro.tex}

\experimentcolumnsizesmacro{NK Lexicase Selection}{a=actual_retained_bits+source=nk_lexicaseselection_seed110_pop165_mut.01_snapshot_500.csv}


==> hereditary-stratigraph-concept/tex/tab/experiment-column-sizes-nk-randomselection.tex <==
\input{tab/_experimentcolumnsizesmacro.tex}

\experimentcolumnsizesmacro{NK Random Selection}{a=actual_retained_bits+source=nk_randomselection_seed7_pop100_mut.01_snapshot_5000.csv}


==> hereditary-stratigraph-concept/tex/tab/experiment-column-sizes-nk-sharingselection.tex <==
\input{tab/_experimentcolumnsizesmacro.tex}

\experimentcolumnsizesmacro{NK Sharing Selection}{a=actual_retained_bits+source=nk_sharingselection_seed10_pop100_mut.01_snapshot_5000.csv}


==> hereditary-stratigraph-concept/tex/tab/experiment-column-sizes-nk-tournamentselection.tex <==
\input{tab/_experimentcolumnsizesmacro.tex}

\experimentcolumnsizesmacro{NK Tournament Selection}{a=actual_retained_bits+source=nk_tournamentselection_seed140_pop100_mut.01_snapshot_5000.csv}


==> hereditary-stratigraph-concept/tex/tab/ground-truth-phylogenies.tex <==
\begin{table}[ht]
\centering
\caption{
Evolutionary conditions of ground-truth phylogenies taken from \citep{dolson2018applying}.
} \label{tab:ground-truth-phylogenies}
\begin{tabular}{p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}}
Selection Scheme & Per-bit Mutation Rate & Number Generations & Population Size & Phylogeny Download URL \\\toprule
Eco-EA           & 0.01                  & 3000               & 100             & \url{https://osf.io/5d3be/} \\
Lexicase         & 0.01                  & 500                & 165             & \url{https://osf.io/8ycq7/} \\
Random           & 0.01                  & 5000               & 100             & \url{https://osf.io/ydxt7/} \\
Sharing          & 0.01                  & 5000               & 100             & \url{https://osf.io/cz9fk/} \\
Tournament       & 0.01                  & 5000               & 100             & \url{https://osf.io/5ubn8/}
\end{tabular}
\end{table}


==> hereditary-stratigraph-concept/tex/tab/recency-proportional-space-complexity.tex <==
\input{lib/dissertationelse.tex}
\input{lib/importpath.tex}

\begin{table}
{\dissertationelse{\fontsize{9}{10}\selectfont}{\footnotesize}
\begin{tabularx}{\columnwidth}{c | X | X | X | X}%
  \multirow{2}{*}{\makecell{\bfseries Num Gens \\ \bfseries Elapsed}}& \multicolumn{4}{m{0.6\columnwidth}}{\bfseries \centering
  Guaranteed MRCA-Recency-Proportional Resolution}\\ % specify table head
  \bfseries  & 1 & 4 & 10 & 100\\\hline\hline  % specify table head
  \csvreader[
    filter expr={
          test{\ifnumgreater{\thecsvinputline}{2}}
    }
  ]{\importpath submodules/hereditary-stratigraph-concept-binder/binder/retention-policies/a=space-complexity+policy=recency-proportional-resolution+ext=.csv}{}% use head of csv as column names
{\num[scientific-notation=true,round-precision=2,round-mode=figures]{\csvcolii} & \csvcoliii & \csvcoliv & \csvcolv & \csvcolvi\\}% specify your columns here
\end{tabularx}
}
\caption{
Number strata retained after one thousand, one million, one billion, and one trillion generations under the recency-proportional resolution stratum retention policy.
Four different policy parameterizations are shown, the first where MRCA generation can be determined between two extant columns with a guaranteed relative error of 100\%, the second 25\%, the third 10\%, and the fourth 1\%.
A column's memory footprint will be a constant factor of these retained counts based on the fingerprint differentia width chosen.
For example, if single byte differentia were used, the column's memory footprint in bits would be $8\times$ the number of strata retained.
} \label{tab:recency-proportional-space-complexity}
\end{table}


==> hereditary-stratigraph-concept/tex/tab/reconstruction-quality-results-by-differentia-bits.tex <==
\input{lib/C.tex}
\input{lib/dissertationonly.tex}
% \input{lib/importpath.tex}
\makeatletter
  \def\importpathx{\import@path}
\makeatother

\begin{singlespacing}
\dissertationonly{\fontsize{9}{10}\selectfont}
\csvreader[
  longtable=C{3cm}cccccc,
  table head=\caption{
    Comparison of phylogenetic reconstruction quality across differentia bit counts.
    Reconstruction quality measured as clustering information distance (lower is better), mutual clustering information (higher is better), and generalized Robinson-Foulds similarity (higher is better) between reconstructed phylogeny and ground truth phylogeny \citep{smith2020information, smith2020treedist}.
    RPR is recency-proportional resolution stratum retention policy and TDPR is tapered depth-proportional resolution stratum retention policy.
  }\label{tab:reconstruction-quality-results-by-differentia-bits} \\
    \toprule \thead{Tree Comparison Metric} & \thead{Selection\\ Scheme} & \thead{Stratum\\ Retention\\ Policy} & \thead{Target\\ Num\\ Column\\ Bits} & \thead{1 \\Differentia \\ Bit\\ Score} & \thead{8 \\Differentia \\ Bits\\ Score} & \thead{64 \\Differentia \\ Bits\\ Score} \\ \midrule\endfirsthead
    \caption*{\tablename{} \thetable{} (cont'd)} \\
    \toprule \thead{Tree Comparison Metric} & \thead{Selection\\ Scheme} & \thead{Stratum\\ Retention\\ Policy} & \thead{Target\\ Num\\ Column\\ Bits} & \thead{1 \\Differentia \\ Bit\\ Score} & \thead{8 \\Differentia \\ Bits\\ Score} & \thead{64 \\Differentia \\ Bits\\ Score} \\ \midrule\endhead
    \bottomrule\endfoot,
  late after line=\\,
]{\importpathx submodules/hereditary-stratigraph-concept-binder/binder/reconstruction-quality/outplots/reconstruction_quality_results_by_differentia_bits.csv}{}
{\vcell{\csvcoli} & \vcell{\csvcolii} & \vcell{\csvcoliii} & \vcell{\csvcoliv} & \vcell{\csvcolv} & \vcell{\csvcolvi} & \vcell{\csvcolvii} \\[-\rowheight]
\printcellmiddle & \printcellmiddle & \printcellmiddle & \printcellmiddle & \printcellmiddle & \printcellmiddle & \printcellmiddle \\}
\end{singlespacing}


==> hereditary-stratigraph-concept/tex/tab/reconstruction-quality-results-by-policy.tex <==
\input{lib/dissertationonly.tex}

% \input{lib/importpath.tex}
\makeatletter
  \def\importpathx{\import@path}
\makeatother

\begin{singlespacing}
\dissertationonly{\fontsize{9}{10}\selectfont}
\csvreader[
  longtable=cccccc,
  table head=\caption{
    Comparison of phylogenetic reconstruction quality between stratum retention policies.
    Reconstruction quality measured as clustering information distance (lower is better), mutual clustering information (higher is better), and generalized Robinson-Foulds similarity (higher is better) between reconstructed phylogeny and ground truth phylogeny \citep{smith2020information, smith2020treedist}.  }\label{tab:reconstruction-quality-results-by-policy} \\
    \toprule \thead{Tree Comparison Metric} & \thead{Selection\\ Scheme} & \thead{Num\\ Differentia\\ Bits} & \thead{Target\\ Num\\ Column\\ Bits} & \thead{Recency- \\Proportional \\ Resolution\\ Score} & \thead{Tapered\\ Depth-\\ Proportional\\ Resolution\\ Score} \\ \midrule\endfirsthead
    \caption*{\tablename{} \thetable{} (cont'd)} \\
    \toprule \thead{Tree Comparison Metric} & \thead{Selection\\ Scheme} & \thead{Num\\ Differentia\\ Bits} & \thead{Target\\ Num\\ Column\\ Bits} & \thead{Recency- \\Proportional \\ Resolution\\ Score} & \thead{Tapered\\ Depth-\\ Proportional\\ Resolution\\ Score} \\ \midrule\endhead
    \bottomrule\endfoot,
  late after line=\\,
]{\importpathx submodules/hereditary-stratigraph-concept-binder/binder/reconstruction-quality/outplots/reconstruction_quality_results_by_policy.csv}{}
{\csvcoli & \csvcolii & \csvcoliii & \csvcoliv & \csvcolv & \csvcolvi}
\end{singlespacing}


==> hereditary-stratigraph-concept/tex/text/abstract.tex <==
\begin{abstract}
Phylogenies provide direct accounts of the evolutionary trajectories behind evolved artifacts in genetic algorithm and artificial life systems.
Phylogenetic analyses can also enable insight into evolutionary and ecological dynamics such as selection pressure and frequency-dependent selection.
Traditionally, digital evolution systems have recorded data for phylogenetic analyses through perfect tracking where each birth event is recorded in a centralized data structure.
This approach, however, does not easily scale to distributed computing environments where evolutionary individuals may migrate between a large number of disjoint processing elements.
To provide for phylogenetic analyses in these environments, we propose an approach to enable phylogenies to be inferred via heritable genetic annotations rather than directly tracked.
We introduce a “hereditary stratigraphy” algorithm that enables efficient, accurate phylogenetic reconstruction with tunable, explicit trade-offs between annotation memory footprint and reconstruction accuracy.
In particular, we demonstrate an approach that enables estimation of the most recent common ancestor (MRCA) between two individuals with fixed relative accuracy irrespective of lineage depth while only requiring logarithmic annotation space complexity with respect to lineage depth.
This approach can estimate, for example, MRCA generation of two genomes within 10\% relative error with 95\% confidence up to a depth of a trillion generations with genome annotations smaller than a kilobyte.
We also simulate inference over known lineages, recovering up to 85.70\% of the information contained in the original tree using 64-bit annotations.
\end{abstract}


==> hereditary-stratigraph-concept/tex/text/acknowledgement.tex <==
\section*{Acknowledgment}


This research was supported in part by NSF grants DEB-1655715 and DBI-0939454 as well as by Michigan State University through the computational resources provided by the Institute for Cyber-Enabled Research.
This material is based upon work supported by the National Science Foundation Graduate Research Fellowship under Grant No. DGE-1424871.
Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the National Science Foundation.
Thank you to Santiago Rodriguez Papa for manuscript comments.


==> hereditary-stratigraph-concept/tex/text/body.tex <==
\input{text/body/introduction.tex}

\input{text/body/methods.tex}

\input{text/body/results-and-discussion.tex}

\input{text/body/conclusion.tex}


==> hereditary-stratigraph-concept/tex/text/body/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}

To our knowledge, this work provides a novel design for digital genome components that enable phylogenetic inference on asexual populations.
This provides a viable alternative to perfect phylogenetic tracking, which is complex and possibly cumbersome in distributed computing scenarios, especially with fallible nodes.
Our approach enables flexible, explicit trade-offs between space complexity and inference accuracy.
Hereditary stratigraphic columns are efficient: our approach can estimate, for example, the MRCA generation of two genomes within 10\% error with 95\% confidence up to a depth of a trillion generations with genome annotations smaller than a kilobyte.
However, they are also powerful: we were able to achieve tree reconstructions recovering up to 85.70\% of the information contained in the original tree with only a 64-bit memory footprint.

This and other methodology to enable decentralized observation and analysis of evolving systems will be essential for artificial life experiments that use distributed and best-effort computing approaches.
Such systems will be crucial to enabling advances in the field of artificial life, particularly with respect to the question of open-ended evolution \citep{ackley2011pursue,moreno2021conduit,moreno2021case}
Mork work is called for to further enable experimental analyses in distributed, best-effort systems while preserving those systems' efficiency and scalability.
As parallel and distributed computing becomes increasingly ubiquitous and begins to more widely pervade artificial life systems, hereditary stratigraphy should serve as a useful technique in this toolbox.

Important work extending and analyzing hereditary stratigraphy remains to be done.
Analyses should be performed to expound MRCA resolution guarantees of stratum retention policies when using narrow (i.e., single-bit) differentia.
Constant-size-complexity stratum retention policies that preferentially retain a denser sampling of more-recent strata should be developed and analyzed.
Extensions to sexual populations should be explored, including the possibility of annotating and tracking individual genome components instead of whole-genome individuals.
An alternate approach might be to define a preferential inheritance rule so that at each generation slot within a column, a single differentia sweeps over an entire interbreeding population.
Optimization of tree reconstruction from extant hereditary stratigraphs remains an open question, too, particularly with regard to properly handling multifurcations.
It would be particularly valuable to develop methodology to annotate inner nodes of trees reconstructed from hereditary stratigraphs with confidence levels.

The problem of designing genomes to maximize phylogenetic reconstructability raises unique questions about phylogenetic estimation.
Such a backward problem --- optimizing genomes to make analyses trivial as opposed to the usual process of optimizing analyses to genomes --- puts questions about the genetic information analyses operate on in a new light.
In particular, it would be interesting to derive upper bounds on phylogenetic inference accuracy given genome size and generations elapsed.


==> hereditary-stratigraph-concept/tex/text/body/introduction.tex <==
\section{Introduction} \label{sec:introduction}

In traditional serially-processed digital evolution experiments, phylogenetic trees can be tracked perfectly as they progress \citep{bohm2017mabe,wang2018vine,lalejini2019data} rather than reconstructed afterward, as must be done in most biological studies of evolution.
Such direct phylogenetic tracking enables experimental possibilities unique to digital evolution, such as perfect reconstruction of the sequence of phylogenetic states that led to a particular evolutionary outcome \citep{lenski2003evolutionary, dolson2020interpreting}.
In a shared-memory context, it is not difficult to maintain a complete phylogeny by ensuring that offspring retain a permanent reference to their parent (or vice versa).
As simulations progress, however, memory usage would balloon if all simulated organisms were stored permanently.
Garbage collecting extinct lineages and saving older history to disk greatly ameliorates this issue \citep{bohm2017mabe,dolson2019modes}.

If sufficient memory or disk space can be afforded to log all reproduction events, recording a perfect phylogeny in a distributed context is also not especially difficult.
Processes could maintain records of each reproduction event, storing the parent organism (and its associated process) with all generated offspring (and their destination processes).
As long organisms are uniquely identified globally, these ``dangling ends'' could be joined in postprocessing to weave a continuous global phylogeny.
Of course, for the huge population sizes made possible by distributed systems, such stitching may become a demanding task in and of itself.
Additionally, even small amounts of lost or corrupted data could fundamentally degrade tracking by disjoining large tree subsections.

However, if memory and disk space are limited, distributed phylogeny tracking becomes a more burdensome challenge.
A naive approach might employ a server model to maintain a central store of phylogenetic data.
Processes would dispatch notifications of birth and death events to the server, which would curate (and garbage collect) phylogenetic history much the same as current serial phylogenetic tracking implementations.
Unfortunately, this server model approach would present scalability challenges: burden on the server process would worsen in direct proportion to processor count.
% ELD: This is making me wonder if there's a middle ground that could be explored in the future where we could use a sort of UDP phylogeny protocol, where no confirmation occurs
This approach would also be similarly brittle to any lost or corrupted data.

A more scalable approach might record birth and death events only on the process(es) where they unfold.
However, lineages that went extinct locally could not be safely garbage collected until the extinction of their offspring's lineages on other processors could be confirmed.
Garbage collection would thus require extinction notifications to wind back across processes each lineage had traversed.
Again, this approach would also be brittle to loss or corruption of data.

% Under a best-effort model, no system of phylogeny tracking can guarantee proper garbage collection.
% For example, it would be possible for an offspring that was dispatched to a neighboring process to have failed to arrive, and both processes would need to keep going, despite the failure.
% So, extinction notifications for the lineage founded by that offspring would never be dispatched --- putting in motion a memory leak of un-garbage-collectible phylogenetic history.
% The situation becomes even more leaky when the possibility of extinction notifications themselves being lost.

In a distributed context --- especially, a distributed, best-effort context --- phylogenetic reconstruction (as opposed to tracking) could prove simpler to implement, more efficient at runtime, and more robust to data loss while providing sufficient information to address experimental questions of interest.
However, phylogenetic reconstruction from genomes with a traditional model of divergence under gradual accumulation of random mutations poses its own difficulties, including
\begin{itemize}
\item accounting for heterogeneity in evolutionary rates (i.e., the rate at which mutations accumulate due to divergent mutation rates or selection pressures) between lineages \citep{lack2010identifying},
\item performing sequence alignment \citep{casci2008lining},
\item mutational saturation \citep{hagstrom2004using},
\item appropriately selecting and applying complex reconstruction algorithms \citep{kapli2020phylogenetic}, and
\item computational intensity \citep{sarkar2010hardware}.
\end{itemize}

The computational flexibility of digital artificial life experiments provides a unique opportunity to overcome these challenges: designing heritable genome annotations specifically to ensure simple, efficient, and effective phylogenetic reconstruction.
For maximum applicability of such a solution, these annotations should be phenotypically neutral heritable instrumentation \citep{stanley2002evolving} that can be applied to any digital genome.

In this paper, we present ``hereditary stratigraphy,'' a novel heritable genome annotation system to facilitate post-hoc phylogenetic inference on asexual populations.
This system allows explicit control over trade-offs between space complexity and accuracy of phylogenetic inference.
Instead of modeling genome components diverging through a neutral mutational process, we keep a record of historical checkpoints that allow comparison of two lineages to identify the range of time in which they diverged.
Careful management of these checkpoints allows for a variety of trade-off options, including:
\begin{itemize}
  \item linear space complexity and fixed-magnitude inference error,
  \item constant space complexity and inference error linearly proportional to phylogenetic depth, and
  \item logarithmic space complexity and inference error linearly proportional to time elapsed since MRCA (which we suspect will be the most broadly useful trade-off).
\end{itemize}

In Methods we motivate and explain the hereditary stratigraphy approach.
Then, in Results and Discussion we simulate post-hoc inference on known phylogenies to assess the quality of phylogenetic reconstruction enabled by the hereditary stratigraphy method.


==> hereditary-stratigraph-concept/tex/text/body/methods.tex <==
\section{Methods} \label{sec:methods}

This section will introduce intuition for the strategy of our hereditary stratigraph approach, define the vocabulary we developed to describe aspects of this approach, overview configurable aspects of the approach, present mathematical exposition of the properties of space complexity and inference quality under particular configurations, and then recap digital experiments that demonstrate this approach in an applied setting.

\subsection{Hereditary Strata and the Hereditary Stratigraphic Column}

\input{fig/column-comparison.tex}

Our algorithm, particularly the vocabulary we developed to describe it, draws loose inspiration from the concept of geological stratigraphy, inference of natural history through analysis of successive layers of geological material \citep{steno1916prodromus}.
As an introductory intuition, suppose a body of rock being built up through regular, discrete events depositing of geological material.
Note that in such a scenario we could easily infer the age of the body of rock by counting up the number of layers present.
% Note that it is crucial to this scenario that each layer has some differentiating feature that allows it to be distinguished from layers above and below it, but also potentially from layers present in another body of rock in a distant and unrelated geographic position.
Next, imagine making a copy of the rock body in its partially-formed state and then moving it far away.
As time runs forward on these two rock bodies, independent layering processes will cause consistent disparity in the layers forming on each forwards from their point of separation.

To deduce the historical relationship of these rock bodies, we could simply align and compare their layers.
Layers from their base up through the first disparity would correspond to shared ancestry; further disparate layers would correspond to diverged ancestry.
% Interestingly, and powerfully for phylogenetic inference, we can readily distinguish a scenario where both rock bodies deposited ten layers after diverging from a scenario where one deposited eighteen layers and the other deposited two.
Figure \ref{fig:column-comparison} depicts the process of comparing columns for phylogenetic inference.

Shifting now from intuition to implementation, a fixed-length randomly-generated binary tag provides a suitable ``fingerprint'' mechanism mirroring our metaphorical ``rock layers.''
We call this ``fingerprint'' tag a \textit{differentia}.
The width of this tag controls the probability of spurious collisions between independently generated instances.
At 64 bits wide the tag effectively functions as a UID: collisions between randomly generated tags are so unlikely ($p < 5.42\times10^{-20}$) they can essentially be ignored.
At the other end of the spectrum, collision probability would be $1/256$ for a single byte and $1/2$ for a single bit.
In the case of narrow differentia, in order to set a lower bound for the MRCA generation, you would have to backtrack common strata from the last commonality until the probability of that many successive spurious collisions was enough to satisfy your desired confidence level (e.g., 95\% confidence).
Even then, there would be a possibility of the the true MRCA falling before the estimated lower bound.
Note, however, that no matter the width of the differentia the generation of the first discrepancy provides a hard upper bound on the generation of the MRCA.

In accordance with our geological analogy, we refer to the packet of data accumulated each generation as a \textit{stratum}.
This packet contains the differentia and, although not employed in this work, could hold other arbitrary user-defined data (i.e., simulation timestamp, phenotype characteristics, etc.).
Again in accordance with the geological analogy, we refer to the chronological stack of strata that accumulate over successive generations as a \textit{hereditary stratigraphic column}.

\subsection{Stratum Retention Policy}

\input{fig/deposit-process.tex}

As currently stated, strata in each column will accumulate proportionally to the length of evolutionary history simulated.
In an evolutionary run with thousands or millions of generations, this approach would soon become intractable --- particularly when columns are serialized and transmitted between distributed computing elements.
To solve this problem, we can trade off precision for compactness by strategically deleting strata from columns as time progresses.
Figure \ref{fig:deposit-process} overviews how stratum deposit and stratum elimination might progress over two generations under the hereditary stratigraphic column scheme.

Different patterns of deletion will lead to different trade-offs, both in terms of the scaling relationship of column size to generations elapsed and in terms of the arrangement of inference precision over evolutionary history (i.e., focusing precision on more recent evolutionary history versus spreading it evenly over the entire history).

We refer to the rule set used to selectively eliminate strata over time as the ``stratum retention policy.''
We explore several different retention policy designs here, and implement our software to allows for free, modular interchange of retention policies.

Our software allows specification of a policy as either a ``predicate'' or a ``generator.''
The predicate method requires a function that takes the generation of a stratum and the current number of strata deposited and returns whether that stratum should be retained at that point in time.
The generator method requires a function that takes the current number of strata deposited and yields the set of generations that should be deleted at that point in time.
Although the predicate form of a policy is useful for analyzing and proving properties of policies, the generator form is generally more efficient in practice.
We provide equivalent predicate and generator implementations for each stratum retention policy discussed here.

Strata elimination causes a stratum's position within the column data structure to no longer correspond to the generation it was deposited.
Therefore, it may seem necessary to store the generation of deposit within the stratum data structure.
However, for all deterministic retention policies a perfect mapping exists backwards from column index to recover generation deposited without storing it.
We provide this formula for each stratum retention policy surveyed here.
Finally, for each policy we provide a formula to calculate the exact number of strata retained under any parameterization after $n$ generations.

The next subsections introduce several stratum retention policies, explain the intuition behind their implementation, and elaborate their space complexity and resolution properties.
For each policy, patterns of stratum retention are illustrated in Figure \ref{fig:retention-policies}.
The formulas for number of strata retained after $n$ generations, the formulas to calculate stratum deposit generation from column index, and the retention predicate specifications of each policy are available in Supplementary Section \ref{sec:condemner-implementations}.
The generator specification of each policy is available in Supplementary Section \ref{sec:predicate-implementations}.
For tapered depth-proportional resolution and recency-proportional resolution, the accuracy of MRCA estimation can also be explored via an interactive in-browser web applet at \url{https://hopth.ru/bi}.

\input{fig/retention-policies.tex}

\subsection{Fixed Resolution Stratum Retention Policy}

The fixed resolution retention policy imposes a fixed absolute upper bound $r$ on the spacing between retained strata.
The strategy is simple: permanently retain a stratum every $r$th generation.
(For arbitrary reasons of implementation convenience, we also require each stratum to be retained during at least the generation it is deposited).
See top panel of Figure \ref{fig:retention-policies}.

This retention policy suffers from linear growth in a column's memory footprint with respect to number of generations elapsed: every $r$th generation generation a new stratum is permanently retained.
For this reason, it is likely not useful in practice except potentially in scenarios where the number of generations is small and fixed in advance.
We include it here largely for illustrative purposes as a gentle introduction to retention policies.

\subsection{Depth-Proportional Resolution Stratum Retention Policy}

The depth-proportional resolution policy ensures spacing between retained strata will be less than or equal to a proportion $1/r$ of total number of strata deposited $n$.
Achieving this limit on uncertainty requires retaining sufficient strata so that no more than $n/r$ generations elapsed between any two strata.
This policy accumulates retained strata at a fixed interval until twice as many as $r$ are at hand.
Then, every other retained stratum is purged and the cycle repeats with a new twice-as-wide interval between retained strata.
See second from top panel of Figure \ref{fig:retention-policies}.

When comparing stratigraphic columns from different generations, the resolution guarantee holds in terms of the number of generations experienced by the older of the two columns.
Because this retention policy is deterministic, for two columns with the same policy, every stratum that is held by the older column is also guaranteed to be present in the younger column (unless it hasn't yet been deposited on the younger column).
Therefore, the strata that would enable the desired resolution when comparing two columns of the same age are guaranteed to be available, even when one column has elapsed more generations.

Because the number of strata retained under this policy is bounded as $2r+1$, space complexity scales as $O(1)$ with respect to the number of strata deposited.
It follows that the MRCA generation estimate uncertainty scales as $O(n)$ with respect to the number of strata deposited.

\subsection{Tapered Depth-Proportional Resolution Stratum Retention Policy}

This policy refines the depth-proportional resolution policy to provide a more stable column memory footprint over time.
The naive depth-proportional resolution policy builds up strata until twice as many are present as needed then purges half of them all at once.
The tapered depth-proportional resolution policy functions identically to the depth-proportional policy except that it removes unnecessary strata gradually from back to front as new strata are deposited, instead of eliminating them simultaneously.
See third from top panel of Figure \ref{fig:retention-policies}.

The column footprint stability of this variation makes it easier to parameterize our experiments to ensure comparable end-state column footprints for fair comparison between retention policies, in addition to making this policy likely better suited to most use cases.
By design, this policy has the same space complexity and MRCA estimation uncertainty scaling relationships with number generations elapsed as the naive depth-proportional resolution policy.

\subsection{MRCA-Recency-Proportional Resolution Stratum Retention Policy}

\input{tab/recency-proportional-space-complexity.tex}

The MRCA-recency-proportional resolution policy ensures distance between the retained strata surrounding any generation point will be less than or equal to a user-specified proportion $1/r$ of the number of generations elapsed since that generation.

This policy can be constructed recursively.
So, to begin, let's consider setting up just the \textit{first} generation $g$ of the stratum after the root ancestor we will retain when $n$ generations have elapsed.
A simple geometric analysis reveals that providing the guaranteed resolution for the worst-case generation within the window between generation 0 and generation $g$ (i.e., generation $g-1$) requires
\begin{align*}
  g \leq \lfloor n / (r + 1) \rfloor.
\end{align*}

We now have an upper bound for the generation of the first stratum generation we must retain.
However, we must guarantee that strata at these generations are actually available for us to retain (i.e., haven't been purged out of the column at a previous time point).
We will do this by picking the generation that is the highest power of 2 less than or equal to our bound.
If we repeat this procedure as we recurse, we are guaranteed that this generation's stratum will have been preserved across all previous timepoints.

Why does this work?
Consider a sequence where all elements are spaced out by strictly nonincreasing powers of 2.
Consider the first element of the list.
All multiples this first element will be included in the list.
So, when we ratchet up $g$ to $2g$ as $n$ increases, we are guaranteed that $2g$ has been retained.
This principle generalizes recursively down the list.
This is a similar principle to the approach of strictly-doubling interval sizes used in the Depth-Proportional Resolution stratum retention policies described above.

This step of truncating to the nearest less than or equal to power of 2 affects our recursive step size is at most halved.
So, because step size is a constant fraction of remaining generations $n$ (at worst $\frac{n}{2(r+1)}$), the number of steps made (and number of strata retained) scales as $O(\log(n))$ with respect to the number of strata deposited.
Table \ref{tab:recency-proportional-space-complexity} provides exact figures for the number of strata retained under different parameterizations of the recency-proportional retention policy between one thousand and one trillion generations.

As for MRCA generation estimate uncertainty, in the worst case it scales as $O(n)$ with respect to the greater number of strata deposited.
However, with respect to estimating the generation of the MRCA for lineages diverged any fixed number of generations ago, uncertainty scales as $O(1)$.

How does space complexity scale with respect to the policy's specified resolution $r$?
Through extrapolation from OEIS sequences A063787 and A056791 via guess and check \citep{sloane2021a063787,sloane2021a056791}, we posited the exact number of strata retained after $n$ generations as

\begin{align*}
  \mathrm{HammingWeight}(n)
  + \sum_1^r \lfloor \log_2( \lfloor n / r \rfloor ) \rfloor
  + 1.
\end{align*}

This expression has been unit tested extensively to ensure perfect reliability.
Approximating and applying logarithmic properties, this policy's space complexity can be calculated within a constant factor as

\begin{align*}
\log(n) + \log\Big(\frac{n^r}{r!}\Big).
\end{align*}

To analyze the relationship between space complexity and resolution $r$, we will examine the ratio of space complexities induced when scaling resolution $r$ up by a constant factor $f > 1$.
Evaluating this ratio as $r \to \infty$, we find that space complexity scales directly proportional to $f$,

\begin{align*}
\lim_{r \to \infty}
\frac{
  \log(n) + \log\Big(\frac{n^{fr}}{(fr)!}\Big)
}{
  \log(n) + \log\Big(\frac{n^r}{r!}\Big)
}
= f.
\end{align*}

Evaluating this ratio as $n \to \infty$, we find that this scaling relationship is never worse than directly proportional for any $r$,

\begin{align*}
\lim_{n \to \infty}
\frac{
  \log(n) + \log\Big(\frac{n^{fr}}{(fr)!}\Big)
}{
  \log(n) + \log\Big(\frac{n^r}{r!}\Big)
}
&= \frac{fr+1}{r+1}\\
&= f\frac{r + 1/f}{r + 1}\\
&\leq f.
\end{align*}


\subsection{Computational Experiments}

In order to assess the practical performance of the hereditary stratigraph approach in an applied setting, we simulated the process of stratigraph propagation over known ``ground truth'' phylogenies extracted from pre-existing digital evolution simulations \citep{hernandez2022phylogenetic}.
These simulations propagated populations of between 100 and 165 bitstrings between 500 and 5,000 synchronous generations under the NK fitness landscape model \citep{kauffman1989nk}.
In order to ensure coverage of a variety of phylogenetic conditions, we sampled a variety of selection schemes that impose profoundly different ecological regimens \citep{dolson2018ecological},
\begin{itemize}
  \item EcoEA Selection \citep{goings2012ecology},
  \item Lexicase Selection \citep{helmuth2014solving},
  \item Random Selection, and
  \item Sharing Selection \citep{goldberg1987genetic}.
  % \item Tournament Selection \citep{miller1995genetic}.
\end{itemize}

Supplementary Table \ref{tab:ground-truth-phylogenies} provides full details on the conditions each ground truth phylogeny was drawn from.
The phylogenies themselves are available with our supplementary material.

For each ground truth phylogeny, we tested combinations of three configuration parameters:
\begin{itemize}
  \item target end-state memory footprints for extant columns (64, 512, and 4096 bits),
  \item differentia width (1, 8, and 64 bits), and
  \item stratum retention policy (tapered depth-proportional resolution and recency-proportional resolution).
\end{itemize}

Stratum retention policies were parameterized so that the maximum number of strata possible were present at the end of the experiment without exceeding the target memory footprint.
If the target memory footprint is exceeded by the sparsest possible parameterization of a retention policy, then that sparsest possible parameterization was used.
Supplementary Tables \cref{tab:experiment-column-sizes-nk-ecoea-selection,tab:experiment-column-sizes-nk-lexicase-selection,tab:experiment-column-sizes-nk-random-selection,tab:experiment-column-sizes-nk-sharing-selection,tab:experiment-column-sizes-nk-tournament-selection} provide the calculated paramaterizations and memory footprints of extant columns.

\input{fig/phylogenetic-inference.tex}

In order to assess the viability of phylogenetic inference using hereditary stratigraphic columns from extant organisms, we used the end-state stratigraphs to reconstruct an estimate of the actual ground truth phylogenetic histories.
The first step to reconstructing a phylogenetic tree for the history of an extant population at the end of an experiment is to construct a distance matrix by calculating all pairwise phylogenetic distances between extant columns.
We defined phylogenetic distance between two extant columns as the sum of each extant organism's generational distance back to the generation of their MRCA, estimated as the mean of the upper and lower 95\% confidence bounds.
Figure \ref{fig:phylogenetic-inference} provides a cartoon summary of the process of calculating phylogenetic distance between two extant columns.

We then used the unweighted pair group method with arithmetic mean (UPGMA) reconstruction tool provided by the BioPython package to generate estimate phylogenetic trees \citep{cock2009biopython,sokal1958statistical}.
After generating the reconstructed tree topology, we performed a second pass to adjust branch lengths so that each internal tree node sat at the mean of its estimated 95\% confidence generation bounds.
%We found that the neighbor joining (NJ) approach occasionally yielded reconstructions with impossible ``negative generation'' branches \citep{saitou1987neighbor} after knowledge bounding the absolute generation of internal nodes (i.e., MRCA's between pairs of extant organisms) was applied, so we did not use it.

\subsection{Software and Data}

% A prototype of this approach has been implemented \url{https://github.com/mmore500/dishtiny/blob/incoming/include/dish2/genome/PhyloFingerprints.hpp} and preliminarily tested \url{https://github.com/mmore500/dishtiny/blob/incoming/tests/dish2/genome/PhyloFingerprints.cpp}.

As part of this work, we published the \texttt{hstrat} Python library with a stable public-facing API intended to enable incorporation in other projects with extensive documentation and unit testing on GitHub at \url{https://github.com/mmore500/hstrat} and on PyPI.% at \url{https://pypi.org/project/hstrat/}.
In the near future, we intend to complete and publish a corresponding C++ library.

Supporting software materials can be found on GitHub at \url{https://github.com/mmore500/hereditary-stratigraph-concept}
Supporting computational notebooks are available for in-browser use via BinderHub at \url{https://hopth.ru/bk} \citep{ragan2018binder}.
Our work benefited from many pieces of open source scientific software \citep{sukumaran2010dendropy,virtanen2020scipy,hunter2007matplotlib,virtanen2020scipy,waskom2021seaborn,bostock2011d3,meurer2017sympy,smith2020treedist,smith2020treedistdata,paradis2004ape,ushey2022reticulate,wickham2022dplyr}.
The ground truth phylogenies used in this work as well as supplementary figures, tables, and text are available via the Open Science Framework at
\url{https://osf.io/4sm72/} \citep{foster2017open,moreno2022hstratconceptsupplement}.
Phylogenetic data associated with this project is stored in the Alife Community Data Standards format \citep{lalejini2019data}.


==> hereditary-stratigraph-concept/tex/text/body/results-and-discussion.tex <==
\section{Results and Discussion} \label{sec:results}

\input{fig/reconstruction-example.tex}

In this section, we analyze the quality of reconstructions of known phylogenetic trees using hereditary stratigraphy.
Figure \ref{fig:reconstruction-example} compares an example reconstruction from columns using tapered depth-proportional stratum retention, an example reconstruction using recency-proportional stratum retention,  and the underlying ground truth phylogeny.
Interactive in-browser visualizations comparing all reconstructed phylogenies to their corresponding ground truth are available at \url{https://hopth.ru/bi}. %TODO: replace this with anonymous link

\subsection{Reconstruction Accuracy}

Measuring tree similarity is a challenging problem, with many conflicting approaches that all provide different information \citep{smith2020information}.
Ideally, we would use a metric of reconstruction accuracy that 1) is commonly used so that there exists sufficient context to understand what constitutes a good value, 2) behaves consistently across different types of trees, and 3) behaves reasonably for the types of trees common in artificial life data.
Unfortunately, these objectives are somewhat in conflict.
The primary source of this problem is multifurcations, nodes from which more than two lineages branch at once.
In reconstructed phylogenies in biology, multifurcations are generally assumed to be the result of insufficient information.
It is thought that the real phylogeny had multiple bifurcations that occurred so close together that the reconstruction algorithm is unable to separate them.
In artificial life phylogenies, however, we have the opposite problem.
When we perfectly track a phylogeny, it is common for us to know that a multifurcation did in fact occur.
However, it is challenging for our reconstructions to properly identify multifurcations, because it requires perfectly lining up multiple divergence times.
Many of the most popular tree distance metrics interpret the difference between a multifurcation and a set of bifurcations as a dramatic change in topology.
For some use cases, this change in topology may indeed be meaningful, although research on the extent of this problem is limited.
Nevertheless, we suspect that for the majority of use cases, the tiny branch lengths between the internal nodes will make this source of error relatively minor.

To overcome this obstacle, we have measured our reconstruction accuracy using multiple metrics.
We will primarily focus on Mutual Clustering Information (as implemented in the R TreeDist package) \citep{smith2020treedist}, which is a direct measure of the quantity of information in the ground truth phylogeny that was successfully captured in the reconstruction.
It is relatively unaffected by the failure to perfectly reproduce multifurcations.
For the purposes of easy comparison to the literature, we also measured the Clustering Information Distance \citep{smith2020treedist}.

\input{fig/info_plot.tex}

Across ground truth phylogenies, we were able to reconstruct the phylogenetic topology with between 47.75\% and 85.70\% of the information contained in the original tree using a 64-bit column memory footprint, between 47.75\% and 80.36\% using a 512-bit column memory footprint, and between 51.13\% and 83.53\% using a 4096-bit column memory footprint.
While the Clustering Information Distance reached its maximum possible score (1.0) for the heavily-multifurcated EcoEA phylogeny, it agreed with the Mutual Clustering Information score for less multifurcated phylogenies, such as fitness sharing.
Using the Recency Proportional Resolution retention policy and a 4096-bit column memory footprint, we were able to reconstruct a fitness sharing phylogeny with a Clustering Information Distance of only 0.2923471 from the ground truth.
For context, that result is comparable to the distance between phylogenies reconstructed from two closely-related proteins in H3N2 flu (0.25) \citep{jones2021parallel}.
To build further intuition, we strongly encourage readers to refer to our interactive web reconstruction.
Figure \ref{fig:info_plot} summarizes error reconstructing the fitness sharing selection phylogeny in terms of the mutual clustering information metric \citep{smith2022robust}.
The phylogenies reconstructed from the EcoEA condition performed comparably, with lexicase and random selection faring somewhat worse \citep{moreno2022hstratconceptsupplement}.
In the case of random selection, we suspect that this reduced performance is the result of having many nodes that originated very close together at the end of the experiment.
As expected, we did observe overall more accurate reconstructions from columns that were allowed to occupy larger memory footprints.

\subsection{Differentia Size}

Among the surveyed ground truth phylogenies and target column footprints, we consistently found that smaller differentia were able to yield more or as accurate phylogenetic reconstructions.
The stronger performance of narrow differentia was particularly apparent in low-memory-footprint scenarios where overall phylogenetic inference power was weaker.
Overall, single-bit differentia outperformed 64-bit differentia under 20 conditions, and were indistinguishable under 6 conditions, and were worse under 4 conditions.
We used Cluster Information Distance to perform these comparisons.
Full results are available in Supplementary Section \ref{sec:differentia-size-full}.
Although narrower differentia have less distinguishing power on their own, their smaller size allows more to be packed into the memory footprint to cover more generations, which seems to help reconstruction power.
We must note that narrower differentia can pack more thoroughly into the footprint caps we imposed on column size, so their extant columns tended to have slightly more overall bits.
However, this was a small enough imbalance (in most cases $<10\%$) that we believe it is unlikely to fully account for the stronger performance of narrow-differentia configurations.

\subsection{Retention Policy}

Across the surveyed ground truth phylogenies and target column memory footprints, we found that the recency-proportional resolution stratum retention policy generally yielded better phylogenetic reconstructions.
Phylogenetic reconstruction quality was better in 28 conditions, equivalent in 13 conditions, and worse in 4 conditions.
Again, this effect was most apparent in the small-stratum-count scenarios where overall inference power was weaker.
We used Cluster Information Distance to perform these comparisons.
Full results are available in Supplementary Section \ref{sec:retention-policy-full}.
The stronger performance of recency-proportional resolution is likely due to the denser retention of recent strata under the recency-proportional metric, which help to resolve the more numerous (and therefore typically more tightly spaced) phylogenetic events in the near past \citep{zhaxybayeva2004cladogenesis}.
Recency-proportional resolution tended to be able to fit fewer strata within the prescribed memory footprints (except in cases where it could not fit within the footprint) so its stronger performance cannot be attributed to more retained bits in the end-state extant columns.


==> hereditary-stratigraph-concept/tex/text/frontmatter.tex <==
\title{ Hereditary Stratigraphy: Genome Annotations to Enable Phylogenetic Inference over Distributed Populations }

\author{Matthew Andres Moreno, Emily Dolson, \and Charles Ofria \\
\mbox{}\\
Michigan State University, East Lansing, MI 48103 \\
mmore500@msu.edu}

\maketitle


==> hereditary-stratigraph-concept/tex/text/references.tex <==
% \section*{References}

\putbib


==> lib/dissertationexclude.tex <==
% \pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\providecommand{\dissertationexclude}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION
\else
#1
\fi
}


==> lib/importpath.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/17491
\makeatletter
  \def\importpath{\import@path}
\makeatother


==> lib/safepercent.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/351125
\catcode`\%=12
\newcommand\safepercent{%}
\catcode`\%=14


==> lib/safetilde.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/425957
\newcommand\safetilde{\string~}


==> text/acknowledgement.tex <==
\section*{Acknowledgment}

This material is based upon work supported by the Eric and Wendy Schmidt AI in Science Postdoctoral Fellowship, a Schmidt Futures program.


==> text/body/experimental-evaluation.tex <==
\section{Experimental Evaluation} \label{sec:experimental-evaluation}

TODO: add content from alife paper here


==> text/body/introduction/hereditary-stratigraphy.tex <==
\subsection{Hereditary Stratigraphy} \label{sec:hereditary-stratigraphy}

Digital systems excel at copying and distributing information \citep{miller2001taking}.
Provenance among digital artifacts produced through copy operations can be represented as a tree of parent-child relationships (in this case, original-copy relationships).
The structure of digital ancestry trees can answer important questions pertinent to cybersecurity, misinformation, and cultural anthropology \citep{aslan2020comprehensive,dupuis2019spread,ling2021dissecting}.
To explain how and why such ancestry analysis might be accomplished, we next contrast direct ancestry tracking with distributed ancestry tracking, outline hereditary stratigraphy methodology for distributed ancestry tracking, and review applications of distributed ancestry tracking.

\subsubsection{Direct Ancestry Tracking}

Most work on ancestry trees of digital artifacts relies on centralized lineage tracking \citep{friggeri2014rumor,cohen1987computer,dolson2023phylotrackpy}.%
\footnote{A notable exception, \cite{libennowell2008tracing} exploit a serendipitous mechanistic opportunity to reconstruct global dissemination of chain emails --- discussed further below.}
Direct approaches to tracking replicator provenance in digital systems operate on this graph structure directly, distilling it from the full set of parent-child relationships over the history of a population to yields an exact historical account.

Unfortunately, typical lineage tracking is difficult to scale.
At scale, practical limitations preclude comprehensive records of replication events, which accumulate linearly with elapsed generations \citep{dolson2023algorithms}.
So, extinct lineages must be pruned.
Detecting lineage extinctions requires either (1) collation of all replication and destruction events to a centralized data store or (2) peer-to-peer transmission of extinction notifications that unwind a lineage's (possibly many-hop) trajectory across host nodes.
Both options oblige runtime communication overhead.
To boot, the perfect-tracking paradigm is fragile to single missing relationships --- these can entirely disjoin knowledge of how large portions of phylogenetic history relate.
This fragility makes direct lineage tracking highly sensitive to data loss and dynamic network topology rearrangements, which are ubiquitous at scale \citep{cappello2014toward,ackley2011pursue}.

\subsubsection{Motivation for Decentralized Ancestry Tracking}

Under an alternate framing, biological phylogenetics almost certainly constitutes the single most extensive investigation of artifact provenance ever conducted.
Decades of phylogenetics researchers have waged a vast and sophisticated campaign to stitch together millions of lines of descent via analysis of fossil records, phenotypic traits, and --- especially --- genetic information \citep{hinchliff2015synthesis,lee2015morphological}.
The successes of biological phylogenetics resoundingly demonstrate the viability of robust phylogenetic analyses over large, long-running, and fully-distributed systems.

Inspired by systematic biology, we can consider post hoc inference from heritable data as an alternative to direct tracking.
At core, biological processes of mutation, recombination, conjugation, transformation, transduction, and gene transfer induce patterns of heritable variation that can be mined to reveal historical relationships \citep{davis1992populations}.

Indeed, in digital systems with imperfect copy processes (e.g., digital evolution), phylogenetic reconstructions can be accomplished ad hoc, i.e., directly from copy artifacts themselves \citep{moreno2021case}.
However, this approach has major drawbacks ---
(1) ad hoc reconstruction algorithms are highly dependent on representational specifics so do not readily generalize;
(2) ad hoc approaches suffer from many of the complications that plague phylogenetic analyses of biological systems such as back mutation and mutational saturation;
(3) systems without mutational dynamics (i.e., perfect copies) entirely lack information on heredity.

The challenges associated with ad hoc ancestry estimation begs the question of how to design genetic material to optimize phylogenetic reconstruction.
If sufficiently compact, such a representation could be annotated onto artifacts of interest in order to facilitate phylogenetic inference.
This scheme assigns each artifact an annotation, with parents' annotations passed down to offspring artifact copies.

The recently developed ``hereditary stratigraphy'' methodology implements this approach, providing a design for heritable annotations that facilitate universal system-invariant phylogenetic reconstruction with well-defined, tunable expectations for inference accuracy \citep{moreno2022hereditary}.

\subsubsection{Mechanisms for Decentralized Ancestry Tracking}

The core mechanism of hereditary stratigraphy is accretion, and subsequent inheritance, of a new randomized data packet each copy generation.
These stochastic fingerprints, which we call ``differentia,'' serve as a sort of checkpoint for lineage identity at a particular generation.
At future time points, extant annotations will share identical differentia for the generations they experienced shared ancestry.
So, the first mismatched fingerprint between two annotations bounds their common ancestry.

To circumvent annotation size bloat, hereditary stratigraphy prescribes a ``pruning'' process to delete differentia on the fly as generations elapse.
This pruning, however, comes at a cost to inference power.
The last generation of common ancestry between two lineages can be resolved no finer than retained checkpoint times.
In the context of hereditary stratigraphy, we refer to the procedure for down sampling as a ``stratum retention algorithm'' and the resulting patterns of retained differentia as a ``stratum retention policy.''
Stratum retention algorithms must decide how many records to discard, but also how remaining records distribute over past time.
Discussion considers tuning stratum retention trade-offs elsewhere as an instance of the more general ``stream curation'' problem --- introduced separately below in Section \ref{sec:streaming-curation} and fully presented in Section \ref{sec:annotation-algorithms}:

Procedures for ancestry tree reconstruction from a population of stratigraph annotations follow from the same principle as pairwise annotation comparison, but merit some further elaboration.
Section \ref{sec:reconstruction-algorithm} provides a trie-based algorithm for this task.

\subsubsection{Distributed Ancestry Trees in Digital Evolution}

Digital evolution refers to computational systems that combine replication, mutation, and selection to instantiate an evolutionary process.
The field sits at the intersection of evolutionary biology, viz. simulation experiments, and machine learning, viz. heuristic optimization.
Within digital evolution, complications of distributed tracking have historically restricted most phylogenetic analyses to single-process or centralized leader/follower simulations.
Need for phylogenetic methods compatible with parallel and distributed simulation motivated original development of hereditary stratigraphy \citep{moreno2022hereditary}.

Computational scale matters in digital evolution and, more broadly, artificial life \citep{ackley2014indefinitely} --- particularly with respect to open-ended evolution (OEE), the question of how (and if) closed systems can indefinitely grow in complexity, novelty, and adaptation \citep{taylor2016open}.
OEE is inexorably intertwined with computational scale, and has been implicated as meaningfully compute-constrained in at least some systems \citep{channon2019maximum}.
It is not an unreasonable possibility that orders-of-magnitude changes in computational scale of digital evolution could induce qualitative effects \citep{moreno2022engineering}, analogously to the renaissance of deep learning with the advent of GPGPU computing \citep{krizhevsky2012imagenet}.

% ELD: TODO: consider cutting this paragraph
Indeed, digital evolution work already commonly marshals substantial parallel and distributed computing  --- in some cases reaching petaflop scale \citep{gilbert2015artificial}.
Methods range from entirely independent evolutionary replicates across compute jobs \citep{dolson2017spatial, hornby2006automated}, to data-parallel fitness evaluation of single individuals over independent test cases using hardware accelerators \citep{harding2007fast_springer, langdon2019continuous}, to application of primary-subordinate/controller-responder parallelism to delegate costly fitness evaluations of single individuals \citep{cantu2001master,miikkulainen2019evolving}.

Fully decentralized, highly-distributed computation is also applied, such as island models \citep{bennett1999building,schulte2010genetic} and mesh-computing approaches \citep{ackley2018digital,moreno2021conduit}.
However, a major barrier to effective applications of the fully-distributed paradigm has been difficulty of observing system state at scale.
In the absence of a global population-level view, the course of evolution becomes much more challenging to study --- undercutting applications of large-scale evolutionary simulation systems as an experimental platform.
Among other instrumentations, including phylogenetic information can help boost observability by providing insight into the mode and tempo of evolution \citep{dolson2020interpreting}.

\subsubsection{Further Applications of Distributed Ancestry Trees}

Replication of digital artifacts pervades computing, and interest in understanding structure of copy trees extends far beyond digital evolution.
Classic examples include the branching reported on the routes through which digital misinformation and computer viruses propagate \citep{friggeri2014rumor,cohen1987computer}.
Studies in this realm have generally relied on centralized tracking, leaving
circumstances where this is not feasible largely underexplored.

Where it has been performed, decentralized copy tracking has proven quite informative.
Work by \cite{libennowell2008tracing} on chain email provides a rare example.
These researchers applied post hoc methods to estimate phylogenies of chain mail messages.
These phylogenies then served as a reference to tune agent-based models, ultimately yielding a remarkable elucidation of email user behavior and underlying social dynamics.
Interestingly, this study's reconstructions were solely enabled by a special peculiarity of the sampled messages: they were email petitions.
Thus, users would append their name to the list before forwarding it on --- a mechanism similar in broad strokes to hereditary stratigraphy.

As an aside, loose parallels between hereditary stratigraphy and visual sedimentation, a dynamic graphic representation that draws on a similar geological metaphor to visualize data streams by progressively stacking, compressing, and then fusing visualized data objects with age, also bear mention \citep{huron2013visual}.

Hereditary stratigraphic techniques enabled new possibilities to delve into hereto cloistered processes through which digital artifacts spread.
Peer-to-peer and federated social networks, which have recently enjoyed substantial upticks in popularity \citep{la2021understanding}, make a prime example.
Within social networks, the structure of share chains is key to understanding, detecting, and mitigating misinformation \citep{kucharski2016study,raponi2022fake} and predatory viral marketing (e.g., spamming and phishing attacks) \citep{guidi2018managing}.
However, existing work relies on the capacity for direct ancestry tracking afforded by monolithic platforms (e.g., Facebook, Twitter, etc.).
Hereditary stratigraphy could enable robust, semi-anonymized extraction of share chain diagnostics within decentralized social networks.

Substantial limitations on uses cases for hereditary stratigraphy should be noted, however.
Annotations predicate influence over the artifact copy process necessary to ensure generational updates.
Additionally, the methodology is susceptible to removal or spoofing of annotation data by antagonistic actors.


==> text/body/methods.tex <==
% \section{Preliminaries} \label{sec:methods}
% This section should introduce the necessary definitions, concepts, and notations that will be used throughout the paper.


==> text/body/perfect-tracking-algorithm.tex <==
\section{Perfect Tracking Algorithm} \label{sec:perfect-tracking-algorithm}

Traditionally, the problem of recording the phylogenies of replicating digital
artifacts has been solved using a ``perfect tracking'' approach where all replication
events are recorded and stored in a tree (or forest, if there are multiple roots) \citep{dolson2023phylotrackpy}.
In this section, we present results on the time and memory size complexity of perfect tracking;
these results will serve as a basis of comparison for hereditary stratigraphy's curation policy and reconstruction algorithms.

Perfect tracking algorithms are designed to augment an ongoing replication process by performing supplementary record-keeping.
As such, perfect tracking algorithms execute three separate routines: 1) initialization, 2) handling the birth of new objects, and 3) (optionally) handling the removal of existing artifact.
The initialization step happens when the founding set of replicating artifacts is introduced.
The birth handling routine executes any time an artifact is replicated.
Similarly, the removal-handling sub-algorithm gets called any time an artifact is removed from the set of currently active artifacts (i.e. the population).

Perfect tracking can be used regardless of whether each artifact has one or multiple parents (i.e., asexual vs. sexual reproduction).
Our analysis here will focus on the case where each artifact has only parent, but most of our results generalize to the multi-parent case.
The primary exception is the results presented in Section \ref{sec:perfect-tracking-pruning-space}, which will underestimate memory use in the average multi-parent case.

Perfect tracking can be done at an arbitrary level of abstraction \citep{dolson2020interpreting, dolson2023phylotrackpy}.
For example, individual replicator objects could be grouped on the basis of a particular genetic or phenotypic trait.
As in biological phylogenetics, phylogenies can be used to show relationships between individuals, species, or any other taxonomic unit.
Increasing the level of abstraction scales down memory use by a constant (but often large) factor.
Here, we will assume that the entities being tracked are the underlying replicating artifacts, as this case is the most computationally expensive.

In the following subsections, we present two different algorithms for perfect phylogenetic tracking: one which naively accumulates records for every node that ever existed and another which reclaims memory as lineages go extinct.

\subsection{Naive perfect tracking}
\label{sec:naive-perfect-tracking}

The naive perfect tracking algorithm is fairly straightforward.
It is formally desribed in Algorithm \ref{alg:perfect-tracking}.

\input{alg/perfect-tracking.tex}

\subsubsection{Time complexity}

The naive perfect tracking algorithm can be implemented in constant time (see Theorem \ref{thm:perfect-tracking-time}).

\input{thm/perfect-tracking-time.tex}


\subsubsection{Performance in parallel and distrbuted environments}
\label{sec:perfect-tracking-distrbuted}

% TODO: Matthew, double-check this
Naive perfect tracking can be easily adapted to parallel computing environments.
The only added challenge is the potential for race conditions where the phylogeny tracker is notified of a birth event involving a parent it does not yet know about.
This situation can be mitigated fairly cheaply by having a pool of ``waiting'' nodes that will be added once the appropriate parent node is added.
Bigger problems occur in distributed environments, where passing messages to a centralized data structure could become expensive \citep{moreno2022hereditary}.
Worse, many distributed environments are noisy and involve the potential for data loss.
It is unclear how a perfect tracking algorithm could recover from missing data.

\subsubsection{Size order of growth}

Naive perfect tracking has a very large size order of growth, owing to the fact that it maintains a tree containing a node for every object that ever existed (see Theorem \ref{thm:perfect-tracking-space}).

\input{thm/perfect-tracking-space.tex}

\subsection{Pruning-enabled perfect tracking}
\label{sec:naive-perfect-tracking-with-pruning}

For most substinative applications, the amount of memory used by naive perfect tracking is prohibitive.
As such, it is common to use a ``pruning''-enabled algorithm that deletes records associated with extinct lineages (see Algorithm \ref{alg:perfect-tracking-pruning}) \citep{dolson2023phylotrackpy}.
This procedure removes all parts of the phylogeny that are no longer relevant to explaining the history of currently extant objects.
Thus, like naive perfect tracking, it introduces no uncertainty into down-stream analyses.

\input{alg/perfect-tracking-pruning.tex}

\subsubsection{Time Complexity}

The pruning-enabled algorithm has amortized constant time complexity (see Theorem \ref{thm:perfect-tracking-with-pruning-time}).

\input{thm/perfect-tracking-with-pruning-time.tex}

\subsubsection{Performance in parallel and distrbuted environments}
\label{sec:perfect-tracking-pruning-distrbuted}
% TODO: Matthew, double-check this
Pruning-enabled perfect tracking has all of the same issues in parallel and distributed environments that naive perfect tracking has.
It also adds an additional cost: parallel processes must be synced up before a pruning operation can be performed.
Otherwise, the algorithm risks incorrectly pruning a lineage that it will later learn produced a new artifact.
This requirement translates to a substantial speed cost in practice. 


\subsubsection{Size order of growth}
\label{sec:perfect-tracking-pruning-space}

As with naive (i.e. unpruned) perfect tracking, the primary memory cost of this algorithm comes from maintaining the tree of records, $T$.
Thus, our analysis in this section will focus on the size of $T$.
Technically, the worst-case size order of growth of perfect tracking with pruning is the same as for naive perfect tracking (see Theorem \ref{thm:perfect-tracking-space}).
However, whereas that order of growth is also the best case for naive perfect tracking, it is a somewhat pathological case with pruning.
When using pruning, such a case would only occur when every object is copied before being removed (i.e., no lineages go extinct).
There are some legitimate reasons these cases might occur, but most of them are fairly esoteric (see Section \ref{sec:perfect-tracking-space-supp}).

% These scenarios might legitimately occur if objects are never removed or the number of objects is allowed to continuously grow, but in these cases $N$ would also be growing continuously.
% They could potentially also happen when tracking digital objects that are copied with very small amounts of stochasticity.

With pruning, the asymptotic behavior of the average case turns out to be substantially better than that of the worst case. 
Luckily, in the vast majority of applications, the average case is more practically informative than the asymptotic behavior of the worst case.
Here, we investigate the expected size of $T$ (which we will call $E(|T|)$) in the average case as the population size ($N$) and number of time points ($G$) increase.
Of course, investigating the average case requires making some assumptions about the scenarios where this algorithm may be used.
An expedient assumption to make is that objects to be replicated are selected at random from the population (i.e., drift).
This process is described by a neutral model.
While this assumption is obviously not completely true in most cases, it will turn out that $E(|T|)$ is actually smaller for most realistic cases (e.g. any evolutionary scenario with directional selection).

Conveniently, the asymptotic behavior of $E(|T|)$ as $N$ increases has been studied under a variety of random selection models \citep{berestyckiRecentProgressCoalescent2009, tellierCoalescenceMultipleBranching2014, nordborgCoalescentTheory2019}.
The relevant branch of mathematics is coalescence theory, which describes the way particles governed by random processes agglomerate over time.
There are a variety of models of random selection, all of which yield different behavior.
Neutral models that could plausibly describe a process of replicating digital artifacts experience ``coalesence'' events.
In these events, the population establishes a more-recent common ancestor as a result of old lineages dying out.
This observation implies that when we run our perfect tracking with pruning algorithm for sufficiently long periods of time, on average we should expect our tree $T$ to have a long unifurcating ``stem.''
The most recent node in this chain will be the most recent common ancestor (MRCA) of the whole extant population.
The descendants of the MRCA will form a sub-tree, which we will call $T_c$.

The expected size of $T_c$ (denoted $E(|T_c|)$ here), then, will be the dominant factor affecting $E(|T|)$.
$E(|T_c|)$ is closely related to a value commonly studied in coalescence theory literature called the expected total branch length (usually denoted $L_n$ or $T_{tot}$; we will refer to it as $L_n$).
$L_n$ assumes that the phylogeny is represented by a tree, $T'$, that contains the leaf nodes, MRCA, and any internal nodes from which multiple lineages diverge (i.e. no unifurcations).
Edges in this tree have weights that represent the amount of time between the origin of the parent and the origin of the child.
$L_n$ is the sum of these weights.
Although the asymptotic behavior of $L_n$ depends on specifics of the evolutionary process, it scales sub-linearly with respect to population size for all realistic models that have been investigated in the literature to our knowledge \citep{gnedinLcoalescentsSurvey2014} \footnote{A possible exception is spatial models, which have recieved less formal analysis but are known to exhibit slower coalescence \citep{berestyckiRecentProgressCoalescent2009}}.  
How is this possible?
Under realistic neutral models, various subsets of the population will coalesce to common ancestors much faster than the whole population does \citep{nordborgCoalescentTheory2019}.
Consequently, there are many shallow branches.
The farther back in $T_c$ you go, the fewer branches there are.
As a result, the marginal impact of increasing $N$ diminishes as $N$ increases.

What do these observations tell us about $E(|T_c|)$?
Because $T_c$ contains unifurcations, each edge in $T'$ corresponds to a chain of unifurcating nodes in $T_c$.
The length of this chain in $T_c$ will, on average, be proportional to the weight of the corresponding edge in $T'$.
Thus, the expected value of $L_n$ is almost identical to $E(|T_c|)$.
However, there is one important difference.
The reason $T'$ is able to scale sub-linearly with $N$ is that as $N$ goes to infinity the lengths of the branches to the leaf nodes (i.e. the extant population) approach zero \citep{nordborgCoalescentTheory2019, delmasAsymptoticResultsLength2008, drmotaAsymptoticResultsConcerning2007}.
In contrast, the space taken up by each of the $N$ leaf nodes in $T_c$ cannot drop below a fixed constant.
Thus, $E(|T_c|)$ is $\mathcal{O}(L_n + N)$.
Note that the time to coalescence depends entirely on the population size ($N$); the total number of generations elasped since the start of the process ($G$) does not affect the asymptotic growth rate of $E(|T_c|)$.

The precise asymptotic scaling of $L_n$ with respect to population size $N$ depends on the exact model of random replication used \citep{tellierCoalescenceMultipleBranching2014}.
Under the best-studied model, Kingman's Coalescent, it is $\mathcal{O}(log(N))$ \citep{kingmanCoalescent1982, delmasAsymptoticResultsLength2008}.
Under another reasonable model, the Bolthausen-Sznitman coalescent, it is $\mathcal{O}(\frac{N}{log(N)})$ \citep{drmotaAsymptoticResultsConcerning2007}.
% Some exotic models could also produce the star-shaped coalescent, in which all $N$ offspring descend directly from the most recent common ancestor. 
% While this scenario actually takes less memory in total, its asymptotic growth is $\mathcal{O}(N)$.
Because these growth rates are all less than $N$, $E(|T_c|)$ ends up being dominated by $N$ term. 
Thus the overall memory usage of pruning-enable perfect tracking is $\mathcal{O}(N + G)$.
Trivially, the ``stem'' part of $T$ can be pruned off when coalescence occurs, producing a bound of $\mathcal{O}(N)$.

%TODO: This could move to supplement if we need space
While $L_n$ is not the primary factor determining the memory use of this algorithm, it still has a substantial practical impact on resource usage.
Thus, it is worth briefly exploring our practical expectations of its size.
Earlier, we mentioned that in practice $T$ will usually be smaller than predicted by neutral models.
These models represent a scenario called ``neutral drift'' in evolutionary theory. 
Under drift, coalescence can be slow because it needs to happen entirely by chance.
When some members of the population are more likely to be selected than others and that selective advantage is hereitable (assuming population size $N$ is stable), we expect to see ``selective sweeps'' in which those members of the population outcompete others.
A selective sweep will usually speed up coalescence (unless it is competing with a different simultaneous selective sweep) \citep{neherGeneticDraftSelective2013}.
Thus, in general, in the presence of non-random selection, we expect $T_c$ to be much smaller than we would expect under drift.
Note, however, that the Bolthausen-Sznitman coalescent mentioned above does model scenarios with selection.

Would we ever expect $T_c$ to be larger than under drift?
Only if lineages coexist for longer than we would expect by chance.
Such a regime can theoretically occur when there is selection for stable coexistence or diversity maintenance.
However, such a regime also involves introducing non-random (balancing/stablizing) selection.
Thus, in practice, while these regimes maintain multiple deep branches, there is often frequent coalesence within those branches.
Theoretically, though, extreme pressure for diversity could cause $E(|T|)$ to scale faster than $\mathcal{O}(N)$.
Such scenarios could potentially be created via ecological interactions.

One factor that we have glossed over in this analysis is the possibility for $N$ to change over time.
For reasons that are explored further in Section \ref{sec:perfect-tracking-space-supp}, allowing $N$ to fluctuate complicates mathematical analysis but does not substantially alter our conclusions.

\subsection{Comparison between perfect tracking and hereditary stratigraphy}

In choosing between perfect tracking and hereditary stratigraphy, there are multiple factors to consider: 1) time complexity in the relevant model of computation, 2) memory use, and 3) amount of information retained.

\subsubsection{Time complexity}

In a non-distributed, serial computing environment, perfect tracking runs in constant time and is likely the better choice. 
Especially in long-running processes, this makes it faster than hereditary stratigraphy.
Hereditary stratigraphy's primary time cost comes when new artifacts are born and their parent's column is copied over.
Consequently, the exact time complexity depends on the curation policy but scales with $G$.
Note that hereditary stratigraphy incurs an additional time complexity cost due to the fact that its output generally requires post-processing before analysis.

In contrast, in parallel or distributed environments, perfect tracking suffers from the problems discussed in Sections \ref{sec:perfect-tracking-distrbuted} and \ref{sec:perfect-tracking-pruning-distrbuted}.
Thus, hereditary stratigraphy usually runs faster in these environments and is generally the better choice.
Moreover, it is robust to data loss, making it possible to use in situations where perfect tracking would break.

\subsubsection{Memory use}

As discussed in Section \ref{sec:perfect-tracking-pruning-space}, pruning-enabled perfect tracking is fairly memory efficient ($\mathcal{O}(N)$) under a wide range of practical circumstances.
However, in practice, its memory use can vary dramatically over time.
This variation is partially due to the fact that the expected distribution of coalescence times is exponential, leading to substantial variation about the mean.
It is also due to the potential for large variation in tree size caused by the ecological and evolutionary dynamics at play in a given scenario being tracked.
Anecdotally, the memory cost of perfect tracking often poses a real-world obstacle to using it at the desired resolution.

Hereditary stratigraphy's memory footprint scales with both $N$ and $G$ (with the specifics depending on the curation policy).
While this memory footprint is larger than the expected memory footprint for pruning-enabled perfect tracking, it is a guarantee. 
Hereditary stratigraphy will never use more memory than expected.
Consequently, it can be a good choice in cases where large fluctuations in memory use are not acceptable.
It can also be helpful in circumstances that inhibit coalescence and start pushing perfect tracking towards worst-case performance.

\subsubsection{Accuracy}

As its name implies, perfect tracking returns completely accurate phylogenetic data. 
There is no potential for reconstruction error to be introduced.
However, the only way to tune its memory use is to reduce the resolution of data recorded (i.e. make the taxonomic unit represented by each node more abstract).

Hereditary stratigraphy introduces imprecision that can potentially lead to inaccuracy.
At the same time, it introduces tools for precisely controlling the level of inaccuracy and its trade-off with memory and time costs.
As such, it is capable of measuring aspects of phylogeny that perfect tracking cannot practically capture. 
Hereditary stratigraphy is always tracked at the level of the individual (i.e. maximum taxonomic resolution), meaning it can capture phylogenetic events that perfect tracking would have to lump together due to memory constraints.

%TODO: Plug ALife paper if its not already in reconstruction

\subsubsection{Overall take-away}

Perfect tracking and hereditary stratigraphy are complimentary techniques that occupy different methodological niches.
In many simple cases, perfect tracking requires fewer resources and provides more accurate data.
However, hereditary stratigraphy can operate in computational environments that perfect tracking cannot.
It also enables new trade-offs to be made between data resolution, memory use, and data accuracy.
Lastly, while perfect tracking is often more memory efficient, hereditary stratigraphy can make more reliable guarantees about memory use.

% Considerations:
% - Distributed vs. not
%     - data loss
%     - have to eventually collect data into a centralized representation?
%     - have to propagate extinction notifications during experiment (unlike phylogeny collation which could hypothetically occur after the fact)
% - Accuracy
% - Memory fluctuations


==> text/body/reconstruction-algorithm.tex <==
\section{Phylogenetic Inference Algorithms} \label{sec:reconstruction-algorithm}

This section surveys methodology to reconstruct patterns of descent among hereditary stratigraphic annotations.  % TODO: pass for vocabulary consistency (annotation vs column)
Sections \ref{sec:distance-based-reconstruction} and \ref{sec:trie-based-reconstruction} present, one after the other, a naive and a more apt approach, respectively, to inferring hierarchical relatedness (i.e., phylogeny) among many hereditary stratigraphic annotations.
Phylogenetic reconstruction requires synthesis of relatedness relationships across an entire population to assemble a holistic historical account.  % TODO: put population in the glossary
To lay groundwork for this discussion, Section \ref{sec:pairwise-relatedness} first explores relatedness estimation between individual pairs of hereditary stratigraphic annotations.

\subsection{Pairwise Relatedness}
\label{sec:pairwise-relatedness}

Recall that hereditary stratigraphic annotations consist of a sequence of inherited ``checkpoint'' fingerprint differentia.
These sequences have a new randomly-generated differentia appended each generation.
Independent lineages accrue probabilistically-distinct differentia.
Relatedness estimation between annotations derives from a simple principle: mismatching differentia values at a time point indicates divergence of any two annotations' lineages.

Assuming both annotations employed the same stream curation policy algorithm, if they share identical record depth they will have retained strata from identical time points.
What if one annotation has greater record depth (i.e., more generations elapsed) than the other?
We can truncate any strata beyond the depth of the younger annotation --- we already know no common ancestry will be shared at those time points.
Due to the self-consistency requirements of stream curation, the younger annotation's curated time points will now superset those of the older annotation.
(During its excess stratum accumulation, the older annotation may have discarded some time points.)
So, we will search for the first mismatching stratum among the deeper annotation's early time points.

The possibility of spurious collisions between differentia (i.e., identical values by chance) complicates any application of binary search to identify the earliest time point with mismatched strata.
Consider lineage divergence as a boolean predicate: it evaluates false for all strata before some the threshold of true lineage divergence and then true for all strata after.
Spurious collisions introduce the possibility of false negatives into search for this predicate's satisfaction threshold.
Take $c$ as retained stratum count per annotation.
If probabilistic confidence were acceptable, sufficient differentia could be tested at each binary search step to bound the probability of misidentifying the point of divergence.
The net failure rate depends on the number of opportunities for false negative divergence detections.
In the worst case, this number of opportunities will be $\mathcal{O}(\log c)$.
However, absolute certainty in determining the earliest differentia discrepancy will require worst case $\mathcal{O}(c)$ comparison (i.e., all diffentia pairs when two annotations share no mismatching differentia).

Spurious collisions introduce false relatedness, causing a second complication: systematic overestimation of relatedness.
Expected bias can be readily calculated, as spurious collision probability stems from the number of unique differentia values.
As such, expected bias may be subtracted out to satisfy statistical analyses requiring mean-unbiased relatedness estimation.

\subsection{Distance-based Reconstruction}
\label{sec:distance-based-reconstruction}

The ease of calculating pairwise relatedness lends a straightforward option for whole-tree estimation: distance-based tree construction methods.
Such methods, like neighbor joining and UPGMA \citep{peng2007distance}, operate simply on pairwise distance estimates between taxa.
This distance-based approach was used in early work with hereditary stratigraphy \citep{moreno2022hereditary}, and is packaged within the accompanying \texttt{hstrat} library.

All-pairs comparisons necessary to prepare the distance matrix make such reconstructions at least $\mathcal{O}(c n^2)$, with $n$ as population size and $c$ as retained stratum count per annotation.
As will be shown presently, better results can be achieved by working directly with hereditary stratigraphic annotations' underlying structure.

\subsection{Trie-based Reconstruction}
\label{sec:trie-based-reconstruction}

The objective of phylogenetic reconstruction can be interpreted as production of a tree structure where leaf nodes share a common path from the root for the duration of their common ancestry.
Anatomically, hereditary stratigraphic annotations share common differentia up through the end of common ancestry.
Restated, annotations share a common prefix until the point of lineage divergence.
This observation suggests application of a trie data structure \citep{fredkin1960trie} to phylogenetic reconstruction.

As a preliminary simplification to be relaxed later, assume our population of $n$ annotations share consistent record depth.
Assuming identical retention policy algorithms, annotations will then also have consistent retained stratum count $c$.
Phylogenetic reconstruction through trie building follows as $\mathcal{O}(c n)$ \citep{mehta2018handbook}.
As an anecdotal reference for computational intensity, consider recent work using the Python-based \texttt{hstrat} library trie-building implementation \citep{moreno2023toward}.
This work achieved reconstructions over a population of 32,768 ($2^15$) synchronous $\approx 1,200$ stratum annotations within about five minutes wall time.

Two reconstruction biases should be noted.
First, because spurious differentia collisions bias toward overestimation of relatedness, as noted above in Section \ref{sec:pairwise-relatedness}, branching events in the reconstructed tree will --- on average --- be more recent than in reality.
The expected rate of spurious collision is easily predictable, so this bias can be readily modeled or corrected for.
% Another possibile approach to counteract overrelatedness bias when analyzing tree structure would be Monte Carlo sampling of tree space with sets of inner nodes ``unzipped'' as if they had arisen due to spurious collision.
Second, trie reconstruction can overrepresent polytomies (i.e., internal multifurcations).
Branches that may have unfolded as separate events but fall within the same uncertainty gap within annotations' historical records will all lump together into a single polytomy.
This bias can be counteracted by splitting polytomies into arbitrary bifurcations with zero-length edges.
% TODO talk about completely eliminating polytomies bad and different bifurcations non-equivalent?

Allowing for uneven record depth among annotations complicates trie-based reconstruction.
As described in Section \ref{sec:pairwise-relatedness}, time points retained within deeper annotations effectively subset time points within younger annotations.
So, arranging youngest-first insertion order for trie construction ensures that no insertion retroactively injects a trie node between existing nodes.
Instead, in oldest-first order, inserted annotations may encounter a trie node with a time point for which they do not have a corresponding retained stratum (i.e., having discarded it under stream curation).

This missing information is conceptually equivalent to a query string wildcard position \citep{fukuyama2016partial}.
Such wildcard queries can require evaluation of many branch paths during insertion, instead of just one.
An inserted taxon's lineage could proceed along any of the outgoing edges from the trie node preceding the wildcard.
Among possible paths, the path with the longest successive streak of strata consistent with the inserted annotation is best-evidenced.
Unfortunately, in the case of multiple wildcard positions, finding the best-evidenced path requires exploring a number of alternate paths potentially exponential with respect to maximum stratum count $c$ (i.e., maximum trie depth).
Taking the number of possible differentia values $d$ into account as the maximum branching factor, the worst case time complexity devolves to $\mathcal{O}(c d^c n)$ \citep{fukuyama2016partial}.
Calculation of the average case depends on the stream curation policy algorithm at play and the underlying phylogenetic structure being reconstructed, which introduces analytical complexity and likely varies significantly between use cases.
Fortunately, the number of wildcard sites is limited due to: 1) record depth similarity, and 2) the tendency for there to be relatively few deep branches in most phylogenies, due to coalescence \citep{nordborgCoalescentTheory2019, berestyckiRecentProgressCoalescent2009}.
These factors likely reduce time costs.
%Limitations in the number of wildcard sites due to record depth similarity and tendency for low branching factor early in underlying phylogenies likely damp time costs.
% TODO ^^^^ justify branching factor point with a cite
% ELD: Added it, and also took a stab at making the sentence more readable (old sentence commented out)
Experimental performance evaluation with annotations derived from representative phylogenies is warranted to explore the in-practice run time of wildcarding pruned-away strata.



% TODO patch in comparison to "real life" phylogenetic reconstruction somewhere?
% Althouh statistically-optimal reconstructions are generally NP-hard \citep{giribet2007efficient}, sub-quadratic heuristics are possible \citep{truszkowski2013fast}.


==> text/body/results-and-discussion.tex <==
\section{Main Results} \label{sec:results}


==> thm/curbed-recency-proportional-resolution-algo-self-consistency.tex <==
% TODO: missing proof
\begin{theorem}{Curbed Recency-Proportional Resolution Self-Consistency}
\label{thm:curbed-recency-proportional-resolution-algo-self-consistency}

\end{theorem}

\begin{proof}
\label{prf:curbed-recency-proportional-resolution-algo-self-consistency}

\end{proof}


==> thm/curbed-recency-proportional-resolution-algo-space-complexity.tex <==
\begin{theorem}{Curbed Recency-proportional Resolution Space Complexity}
\label{thm:curbed-recency-proportional-resolution-algo-space-complexity}

\end{theorem}

\begin{proof}
\label{prf:curbed-recency-proportional-resolution-algo-space-complexity}

\end{proof}


==> thm/curbed-recency-proportional-resolution-algo-uncertainty-bound.tex <==
\begin{theorem}{Curbed Recency-proportional Resolution Uncertainty Bound}
\label{thm:curbed-recency-proportional-resolution-algo-uncertainty-bound}

\end{theorem}

\begin{proof}
\label{prf:curbed-recency-proportional-resolution-algo-uncertainty-bound}

\end{proof}


==> thm/depth-proportional-resolution-algo-space-complexity.tex <==
\begin{theorem}{Depth-proportional Resolution Space Complexity}
\label{thm:depth-proportional-resolution-algo-space-complexity}

\end{theorem}

\begin{proof}
\label{prf:depth-proportional-resolution-algo-space-complexity}
\end{proof}


==> thm/depth-proportional-resolution-algo-uncertainty-bound.tex <==
\begin{theorem}{Depth-proportional Resolution Uncertainty Bound}
\label{thm:depth-proportional-resolution-algo-uncertainty-bound}

\end{theorem}

\begin{proof}
\label{prf:depth-proportional-resolution-algo-uncertainty-bound}

\end{proof}


==> thm/fixed-resolution-algo-space-complexity.tex <==
\begin{theorem}{Fixed Resolution Space Complexity}
\label{thm:fixed-resolution-algo-space-complexity}

\end{theorem}

\begin{proof}
\label{prf:fixed-resolution-algo-space-complexity}

Given a resolution $a \in \mathbb{N}$, let $f(n) := \frac{n}{a}$. Given $c, k \in \mathbb{N}$, let $P(n) := 0 \le f(n) \le cn \; \forall n \ge k.$

Take $c = a$ and $k = 1$. Then, $P(1): 0 \le \frac{1}{a} \le a,$ so $P(n)$ holds for $n = 1$.

Now, assume that $P(n)$ holds. Then,

\begin{align*}
    P(n + 1) :& \frac{n + 1}{a} &\le (n + 1)a \\
    & \frac{n}{a}  + \frac{1}{a} &\le an + a \\
    & \frac{1}{a} &\le a &&\text{(via $P(n)$)}\\
\end{align*}

And so $P(n) \implies P(n + 1).$ Given that $P(1)$ holds, we can conclude that this algorithm has an $O(n)$ space complexity.

\end{proof}


==> thm/fixed-resolution-algo-uncertainty-bound.tex <==
% TODO: missing proof
\begin{theorem}{Fixed Resolution Uncertainty Bound}
\label{thm:fixed-resolution-algo-uncertainty-bound}

\end{theorem}

\begin{proof}
\label{prf:fixed-resolution-algo-uncertainty-bound}

\end{proof}


==> thm/geom-seq-nth-root-algo-self-consistency.tex <==
% TODO: missing proof
\begin{theorem}{Geometric Sequence $n$th Root Self-Consistency}
\label{thm:geom-seq-nth-root-algo-self-consistency}

\end{theorem}

\begin{proof}
\label{prf:geom-seq-nth-root-algo-self-consistency}

\end{proof}


==> thm/geom-seq-nth-root-algo-space-complexity.tex <==
% TODO: missing proof
\begin{theorem}{Geometric Sequence $n$th Root Space Complexity}
\label{thm:geom-seq-nth-root-algo-space-complexity}
The \gls{extant record size} of the Geometric Sequence $n$th Root Policy Algorithm grows with order $\mathcal{\theta}{(k)}.$

\end{theorem}

\begin{proof}
\label{prf:geom-seq-nth-root-algo-space-complexity}



\end{proof}


==> thm/geom-seq-nth-root-algo-uncertainty-bound.tex <==
% TODO: missing proof
\begin{theorem}{Geometric Sequence $n$th Root Uncertainty Bound}
\label{thm:geom-seq-nth-root-algo-uncertainty-bound}

\end{theorem}

\begin{proof}
\label{prf:geom-seq-nth-root-algo-uncertainty-bound}

\end{proof}


==> thm/perfect-tracking-space.tex <==
\begin{theorem}{Naive Perfect Tracking Space Complexity}
\label{thm:perfect-tracking-space}
The space complexity of the naive perfect tracking algorithm is $\mathcal{\theta}(\sum_{t=0}^{G} N_t$), where $N_t$ is the number of new objects born at time $t$ and $G$ is the number of time steps.
\end{theorem}

\begin{proof}
\label{prf:perfect-tracking-space}
The birth-handling algorithm adds a node to the tree ($T$) each time it is called.
It is called once for every birth event.
No nodes are ever removed from $T$.
Therefore, the number of nodes in $T$ is the total number of nodes ever created.
\end{proof}


==> thm/perfect-tracking-time.tex <==
\begin{theorem}{Naive Perfect Tracking Time Complexity}
\label{thm:perfect-tracking-time}
The naive perfect tracking algorithm can be implemented in constant time ($\mathcal{O}(1)$) per birth event.
\end{theorem}

\begin{proof}
\label{prf:perfect-tracking-time}
For the purposes of this proof, we use the RAM model of computation. 
Initialization takes a single simple operation and only happens once. 
Thus, it is trivially constant-time.
Handling a birth event takes two simple operations.
Thus, each run of the birth-handling algorithim trivially takes constant time.
The birth-handling algorithm will run once per birth event.
Although the number of birth events is likely not constant with respect to the size of the population or the number of generations,
these birth events are not part of the tracking algorithm and would have happened regardless of whether phylogeny tracking was in place.
Consequently, adding phylogeny tracking will only increase the time complexity of a computational process to which it is added by a constant amount per birth event.
\end{proof}



==> thm/perfect-tracking-with-pruning-time.tex <==
\begin{theorem}{Pruning Time Complexity}
\label{thm:perfect-tracking-with-pruning-time}
The time complexity of pruning in perfect phylogenetic tracking is $\mathcal{O}(1)$, amortized. 
\end{theorem}

\begin{proof}
\label{prf:perfect-tracking-with-pruning-time}
The initialization and birth-handling steps of the pruning algorithm are trivially constant-time, as explained in proof \ref{prf:perfect-tracking-time} (technically the pruning algorithm adds two constant-time operations to the birth-handling step, but this fact is inconsequential).
Next, we prove that the removal-handling pruning algorithm runs in amortized constant time.
When an arbitrary taxon $t$ is removed, there are three possibilities: 1) $t$ has living descendants, 2) $t$ has no living descendants, but $t$'s parent is either alive or has other descendants that are alive, or 3) $t$ was the last living descendant of its parent.
In case 1, nothing can be removed from the phylogeny.
Case 1 takes contant time, because it only requires executing a single comparison operation.
In case 2, only $t$ can be removed from the phylogeny.
Case 2 also takes constant time, as it only requires removing a single node from the tree and doing three comparison operations.

In case 3, pruning must be done.
We recurse back up the lineage until we find a taxon, $a$, that is either alive or has living descendants. 
Let the distance between $t$ and the root of the tree be $d_t$ and the distance between $a$ and the root of the tree be $d_a$.
The pruning operation, then, takes $\mathcal{O}(d_t - d_a)$ steps. 
In the worst case, this value will be equal to the number of elapsed generations.

However, for case 3 to occur, all taxa from $t$ to $a$ (including $a$ but not including $t$) must have already been removed.
Consequently, $d_t - d_a$ case 1 removal operations must happen for every case 3 removal operation.
Thus, the amortized time to remove the sequence of taxa from $t$ to $a$ (including both $t$ and $a$) is:

\[
\frac{2(d_t - d_a) + 1}{d_t - d_a + 1}
\]

Since

\[
\lim_{d_t - d_a\to\infty} \frac{2(d_t - d_a) + 1}{d_t - d_a + 1} = 2
\],

the amortized time complexity of pruning is bounded by a constant, i.e. it is $\mathcal{O}(1)$.


\end{proof}

% TODO: missing proof
% \begin{theorem}{Average Space Complexity of Perfect Tracking with Pruning}
% \label{thm:perfect-tracking-with-pruning-space}
% Average case is best described by the upper-case-lambda coalescent, but math on that is maybe
% less well understood than Kingman coalescent. Kingman coalescent makes a number of more limiting
% assumptions, but most of them are actually fairly appropriate for most phylogeny tracking situations
% (fixed-size population, wright-fisher model). The biggest problem is that it assumes only bifurcations
% (no multi-furcations). However, a strictly bifurcating tree is the worst case for average space complexity
% (a series of non-bifurcating trees is the absolute worst case, but under random selection it would
% quickly turn into a pretty good (best?) case). So, if we can't do an exact proof based on the upper
% case lambda coalescent, we can still do worst average case proof based on the Kingman coalescent
% Oh wait, maybe bifurcations aren't the worst case? Apparently there is a paradoxical result that shows
% that the Kingman Coalescent decreases fastest???

% Okay, here's the thing - all of these different models behave in ways that populations being tracked
% might behave. The argument to make here is that for a ton of them, the size of the tree (Ln) has been
% shown to be constant, proportional to n, limited by some distribution or asymptote, etc. It may even
% be sufficient to say that they come down from infinity. We end up with a space complexity something like
% O(generations + Ln) which in the worst case could translate to something like O(generations + 2*pop_size^2),
% except I think we can actually prove it's actually something more like O(generations + pop_size + log(pop_size))
% slight risk that pop_size should be multiplied by log(pop_size)

% \end{theorem}

% \begin{proof}
% \label{prf:perfect-tracking-with-pruning-space}

% \end{proof}

==> thm/recency-proportional-resolution-algo-self-consistency.tex <==
% TODO: missing proof
\begin{theorem}{Recency-proportional Resolution Self-Consistency}
\label{thm:recency-proportional-resolution-algo-self-consistency}

\end{theorem}

\begin{proof}
\label{prf:recency-proportional-resolution-algo-self-consistency}

\end{proof}


==> thm/recency-proportional-resolution-algo-uncertainty-bound.tex <==
% TODO: missing proof
\begin{theorem}{Recency-proportional Resolution Uncertainty Bound}
\label{thm:recency-proportional-resolution-algo-uncertainty-bound}

\end{theorem}

\begin{proof}
\label{prf:recency-proportional-resolution-algo-uncertainty-bound}

\end{proof}

